Aspects of inflation and the very early universe

Until recently our knowledge of the primordial curvature perturbation was relatively modest. Ever since COBE delivered its map of data we know the scalar spectrum of primordial perturbations is approximately flat, with the power being only slightly stronger at larger scales. Most inflationary models predict an approximately scale-invariant spectrum, which therefore cannot be used as a distinctive signature. To distinguish between different inflationary microphysics we need to study higher point statistics of the primordial perturbation, which can encode non-gaussian data. In the first part of this thesis we study the bispectrum in all single-field models with a well-defined quantum field theory during a quasi-de Sitter inflationary phase. Any single-field models without ghost-like instabilities fall into this description: from canonical, to Dirac-Born-Infeld inflation and galileon inflation theories. We investigate the scale and shape- dependences of the bispectrum to next-order in the slow-roll approximation. We illustrate our results by applying them to different models and argue these corrections must be taken into account to keep the theoretical error below the observational precision set by the Planck satellite. We then explore the ability of using bispectrum shapes to distinguish between inflationary models more efficiently. We further extend the study of the bispectrum of single-field models beyond the slow-roll approximation, demanding the spectral index to be close to, but not exactly, unity. In the second part of this thesis we explore the process by which the universe is repopulated with matter particles at the end of a Dirac-Born-Infeld inflation phase. We place some mild bounds on the reheating temperature of these models. We argue that the constraints arising from the preheating analysis are complementary to those derived from the primordial perturbation.

==> app1.tex <==
\chapter{The slow-variation approximation}
\label{app:sr}



This appendix contains helpful material 
related to chapters \ref{chapter:two} and 
\ref{chapter:three}.



	\section{Propagator corrections}
	\label{appendix:propagator}
	
	At leading-order, the wavefunctions can be obtained from 
	Eq.~\eqref{eq:wavefunction} by setting all
	slow-variation parameters 
	to zero. Choosing a reference
	scale $k_\star$, this yields the standard result
	\begin{equation}
		\zeta_k(\tau)
			= \im
				\dfrac{H_{\star}}{2\sqrt{z_{\star}}}
				\dfrac{1}{(k \csstar)^{3/2}}
				(1-\im k\csstar\tau) \, e^{\im k \csstar\tau}\ \  .
		\label{eq:wavefunction_background}
	\end{equation}
	Next-order corrections to the propagator were
	discussed by Stewart \& Lyth \cite{Stewart:1993bc},
	who quoted their result in terms of special functions
	and expanded uniformly to next-order after taking a late-time limit.
	The uniform next-order expansion at a generic time was given by
	Gong \& Stewart~\cite{Gong:2001he} for canonical models,
	and by Chen~{\etal}~\cite{Chen:2006nt} in the non-canonical case.
	Their result was cast in a more convenient
	form in Ref.~\cite{Burrage:2010cu} whose argument we briefly review. 

	The next-order correction is obtained
	after systematic expansion of each quantity in 
	Eq. \eqref{eq:wavefunction} to linear order in the slow-variation parameters.
	Contributions arise from each time-dependent factor
	and from the order of the Hankel function.
	Collecting the formulae quoted in Ref.~\cite{Chen:2006nt},
	one finds
	\begin{equation}
		\left.
		\frac{\partial H^{(2)}_{\nu}(x)}{\partial\nu}
		\right|_{\nu = \frac{3}{2}}
			=
			- \dfrac{\im}{x^{3/2}} \sqrt{\dfrac{2}{\pi}}\ 
			\bigg\{
				\e{\im x} (1-\im x) \Ei(-2 \im x)
				- 2 \e{-\im x}
				- \im \dfrac{\pi}{2} \e{-\im x} (1+\im x)
			\bigg\} \ \ ,
		\label{eq:orderderiv}
	\end{equation}
	where $\Ei(x)$ is the exponential integral,
	\begin{equation}
		\Ei(x)
			=
			\int_{-\infty}^{x} \dfrac{\e{t}}{t}\, \d t
		\qquad
		\text{if $x \in \reals$}.
		\label{eq:exponential-integral}
	\end{equation} 
	This is well-defined for $x<0$.
	For $x\geq 0$
	it should  be understood as a Cauchy principal value.
	For complex argument---required by~\eqref{eq:orderderiv}---one promotes Eq.~\eqref{eq:exponential-integral}
	to a contour integral,
	taken on a path running between $t = x \in \complex$
	and $|t| \rightarrow \infty$ in the half-plane $\Re(t) < 0$.
	Using Cauchy's theorem to rotate this contour onto the
	negative real $t$-axis, one finds
	\begin{equation}
		\Ei(2\im k \cs \tau)
			=
			\lim_{\epsilon \rightarrow 0}
			\int_{-\infty(1+\im \epsilon)}^{\tau}
				\dfrac{\d\xi}{\xi} \; \e{2\im k \cs \xi} \ \ .
	\end{equation}
	The next-order correction to~\eqref{eq:wavefunction_background},
	expanded uniformly to $\Or(\varepsilon)$ in slow-variation
	parameters but including the \emph{exact} time-dependence, is therefore
	\begin{equation}
		\begin{split}
			\delta \zeta_k( \tau)
				= \mbox{} &
				\dfrac{\im H_{\star}}{2\sqrt{z_{\star}} (k \csstar)^{3/2}}
				\Bigg\{
					- \varpi_{\star} \e{-\im k \csstar \tau}
						(1+\im k \csstar \tau)
						\int_{-\infty(1+\im \epsilon)}^{\tau}
							\dfrac{\d\xi}{\xi} \;
							\e{2\im k \csstar \xi}
					\\ & \mbox{}
					+ \e{\im k \csstar \tau}
						\Big[
							\mu_{0 \star}
							+ \im \mu_{1 \star} k \csstar \tau
							+ s_{\star} k^2 \csstar^2 \tau^2
							+ \Delta N_{\star} \left(
								\varpi_{\star}
								- \im \varpi_{\star} k \csstar \tau
								- s_{\star} k^2 \csstar^2 \tau^2
							\right)
						\Big]
				\Bigg\} \ \ ,
		\end{split}
		\label{eq:varyingu}
	\end{equation}
	where
	\begin{equation}
		\mu_0 \equiv \varepsilon +v +2s +\im\dfrac{\pi}{2}\varpi
		\quad
		\textrm{and}
		\quad
		\mu_1 \equiv \varepsilon +s -\im\dfrac{\pi}{2}\varpi\ \  ,
	\end{equation}
	and quantities labelled `$\star$' are evaluated at
	the horizon-crossing time for the reference scale $k_\star$.
	We have used $\Delta N_{\star}$ to denote the number of e-folds
	which have elapsed since this time, so $\Delta N_\star =
	\ln |k_\star \csstar \tau|$.
	The limit $\epsilon \rightarrow 0$ should be understood
	after the integration has been performed
	and merely guarantees convergence
	as $\xi \rightarrow -\infty$.
	Eq.~\eqref{eq:varyingu} 
	is \textit{exact} in 
	powers of $k\tau$. 
	Although terms of high-order in $k\tau$ become increasingly
	irrelevant as $|k\tau| \rightarrow \infty$,
	all such terms make comparable contributions to a generic $n$-point
	function at the time of horizon crossing, when $|k\tau| \sim 1$,
	and must not be discarded.
	This reflects interference
	effects between the growing and decaying modes
	at horizon exit.
	

	To evaluate the cubic action~\eqref{eq:s3tau} we will require
	the time-derivative $\delta \zeta'_k$.	
	Using the identity $\mu_0+\mu_1-2\varpi_1=0$, it follows that
	\begin{equation}
		\begin{split}
			\delta \zeta_k'( \tau)
				= \mbox{} &
				\dfrac{\im H_{\star} (k \csstar)^{1/2}}
					{2\sqrt{z_{\star}}}
				\tau
				\Bigg\{
					- \varpi_{1 \star} \e{-\im k \csstar \tau}
					\int_{-\infty(1+\im\epsilon)}^{\tau}
						\dfrac{\d\xi}{\xi} \; \e{2\im k \csstar \xi}
				\\ & \hspace{1cm} \mbox{}
				+ \e{\im k \csstar \tau}
					\Big[
						s_{\star}
						- \mu_{1\star}
						+ \im s_{\star} k \csstar \tau
						+ \Delta N_{\star} \left(
							\varpi_{1\star}
							- 2s_{\star}
							- \im s_{\star} k \csstar \tau
						\right)
					\Big]
				\Bigg\} \ \ .
		\end{split}
		\label{eq:varyinguprime}
	\end{equation} 
	
	For the power spectrum to be conserved
	on super-horizon scales,
	$\delta \zeta_k \rightarrow \textrm{constant}$ and
	$\delta \zeta'_k  \rightarrow 0$ as $|k\tau| \rightarrow 0$.
	The explicitly time-dependent term $\Delta N_\star$
	apparently spoils this behaviour, but
	is compensated by a logarithmic divergence from the integral in \eqref{eq:varyinguprime}, 
	and for $\tau \rightarrow 0$ one finds
	\begin{equation}
		\int_{-\infty(1+\im\epsilon)}^{\tau}
			\dfrac{\d\xi}{\xi} \; \e{2\im k \csstar \xi}
		= \ln |2\im k \csstar \tau| + \Or( k \csstar \tau ) \ \ .
	\end{equation}
	This precisely cancels the time-dependence arising from $\Delta N_\star$.
	Note the incomplete cancellation of the logarithm, which
	leaves a residual of the form $\varpi_\star \ln 2$
	and is the origin of the $\ln 2$ term in the Stewart--Lyth constant
	$C = -2 + \ln 2 + \EulerGamma$ \cite{Stewart:1993bc,Lidsey:1995np}.
	This is similar to what happens
	to the residual $\ln k_i/k_t$ and $\ln k_t / k_\star$ terms
	after cancellation of the $\ln \tau$ logarithms in the three-point function.
	
	
	
	
	\section{Integrals involving the exponential integral function, $\Ei(z)$}
	\label{appendix:a}

	The principal obstruction to evaluation of the next-order
	corrections using standard methods is the $\Ei$-term
	in Eq. \eqref{eq:varyingu}.
	This can not be expressed directly in terms of elementary functions
	whose integrals can be computed in closed form.
	It was explained in Appendix~\ref{appendix:propagator}
	that although $\Ei(2\im k \cs \tau)$
	contains terms of higher-orders in
	$k\tau$ which become increasingly irrelevant as $|k\tau| \rightarrow 0$,
	these cannot usually be neglected when computing
	$n$-point functions.
	The integrals we require are of the form
	\cite{Burrage:2010cu}
	\begin{equation}
		I_m(k_3)
			=
			\int_{-\infty}^{\tau}
				\d\zeta	\; \zeta^m \e{\im (k_1+k_2-k_3)\cs \zeta}
				\int_{-\infty}^{\zeta}
					\dfrac{\d\xi}{\xi} \; \e{2\im k_3 \cs \xi}\ \  .
		\label{eq:iminitial}
	\end{equation}
	We are again using the convention that,
	although $I_m$ depends on all three $k_i$, only the
	asymmetric momentum is written explicitly.
	In the following discussion we specialize to $I_0$.
	Results for arbitrary $m$ 
	can be obtained similarly
	and are given in Ref.~\cite{Burrage:2010cu}.

	We introduce the dimensionless combinations
	\begin{equation}
		\vartheta_3
			=
			1
			- \dfrac{2k_3}{k_t}
		\quad
		\text{and}
		\quad
		\theta_3
			=
			\dfrac{k_3}{k_t-2k_3}
			=
			\frac{1-\vartheta_3}{2 \vartheta_3}\ \ , 
		\label{eq:theta-def}
	\end{equation}
	and perform a contour rotation
	to express $I_0$ in terms of
	$\vartheta_3$ and $\theta_3$ \cite{Burrage:2010cu}
	\begin{equation}
		I_0(k_3)
			=
			- \dfrac{\im}{\vartheta_3 k_t \cs}
				\int_{0}^{\infty}{\d u \; \e{-u}}
				\int_{\infty}^{\theta_3 u}{\dfrac{\d v}{v} \; \e{-2v}} \ \ .
		\label{eq:i02}
	\end{equation}
	The $v$-integral has a series representation
	\begin{equation}
		\int_{\infty}^{\theta_3 u}
			\dfrac{\d v}{v} \e{-2v}
		=
		\EulerGamma
		+ \ln(2\theta_3 u)
		+ \sum_{n=1}^{\infty}
			\dfrac{(-2\theta_3 u)^n}{n! n}
		\label{eq:puiseaux}
	\end{equation}
	where the sum converges uniformly for all complex $\theta_3 u$.
	The right-hand side has a singularity at $\theta_3 u = 0$,
	and the logarithm generates
	a branch cut along the negative real axis.
	The $u$-independent term $\EulerGamma$ is the Euler--Mascheroni
	constant
	$\EulerGamma \equiv \int_{\infty}^{0}{\e{-x}\ln x \, \d x}$
	and is obtained
	by expanding $\e{-2v}$ in series, integrating term-by-term,
	and matching the undetermined constant of integration
	with the left-hand side of~\eqref{eq:puiseaux}
	in the limit $u \rightarrow 0$.
It follows that \cite{Burrage:2010cu}
	\begin{equation}
		I_0(k_3)
			=
			-\dfrac{\im}{\vartheta_3 k_t \cs}
			\left[
				\ln (2\theta_3) +
				\sum_{n=1}^{\infty}
					\frac{(-2\theta_3)^n}{n}
			\right] \ \ .
		\label{eq:i03}
	\end{equation}
	This is singular when $\vartheta_3 \rightarrow 0$,
	which is the squeezed limit where
	either $k_1$ or $k_2 \rightarrow 0$.
	There is nothing unphysical about this arrangement of momenta,
	for which $\theta_3 \rightarrow \infty$,
	but $I_0(k_3)$ will be
	power-law divergent unless the bracket $[ \cdots ]$
	vanishes sufficiently rapidly in the same limit.

	The sum above is absolutely convergent if 
	$-1/2 < \Re(\theta_3) <1/2$,
	corresponding to the narrow physical region $0 < k_3 < k_t / 4$
	where $k_3$ is being squeezed.
	For $\theta_3$ satisfying this
	condition the summation can be performed explicitly,
	yielding
	$\ln (1+2\theta_3)^{-1} = \ln \vartheta_3$.
	It can be verified that $I_0(k_3)$ is analytic
	in the half-plane $\Re(\theta_3) > 0$.
	Therefore it is possible to
	analytically continue to $\theta_3 \geq 1/2$,
	allowing the behaviour as $\theta_3 \rightarrow \infty$
	and $\vartheta_3 \rightarrow 0$
	to be studied.
	We find
	\begin{equation}
		I_0(k_3)
			=
			- \frac{\im}{\vartheta_3 k_t \cs} \ln ( 1 - \vartheta_3 )
			\equiv
			- \frac{\im}{k_t \cs} J_0(k_3) \ \ .
		\label{eq:I0final}
	\end{equation}
	It is more convenient to express our final bispectra in terms of
	$J_0$ rather than $I_0$.
	In the limit $\vartheta_3 \rightarrow 0$, Eq.~\eqref{eq:I0final}
	is finite with $J_0 \rightarrow -1$.
	The $\theta_3 \rightarrow \infty$ behaviour of the sum has
	subtracted both the power-law divergence of the prefactor
	and the logarithmic divergence of $\ln (2 \theta_3)$.
	Had we truncated the $k_3  c_s\zeta$-dependence of Eq. \eqref{eq:iminitial},
	or equivalently the $\theta_3 u$-dependence of Eq. \eqref{eq:puiseaux},
	and
	we would have encountered a spurious divergence in the squeezed
	limit and a misleading prediction of a strong signal in the local
	mode. Several of our predictions, including
	recovery of Maldacena's limit
	described by Eq. \eqref{eq:fnlsvanilla},
	depend on the precise numerical value of $J_0$
	as $\theta_3 \rightarrow \infty$ and therefore constitute tests
	of this procedure.

	We can now evaluate $I_m(k_3)$ for arbitrary $m$,
	although only the cases $m \leq 2$ are required for the calculation
	presented in the main text.
	The necessary expressions are
	\begin{subequations}
		\begin{align}
			I_1(k_3)
				& =
				\dfrac{1}{(\vartheta_3 k_t \cs)^2}
				\left[
					\vartheta_3
					+ \ln(1-\vartheta_3)
				\right]
				\equiv
				\dfrac{1}{(k_t \cs)^2} J_1(k_3)
			\\
			I_2(k_3)
				& =
				\dfrac{\im}{(\vartheta_3 k_t \cs)^3}
				\left[
					\vartheta_3 (2+\vartheta_3)
					+ 2\ln(1-\vartheta_3)
				\right]
				\equiv
				\dfrac{\im}{(k_t \cs)^3} J_2(k_3) \ \ .
		\end{align}
		\label{eq:otheris}
	\end{subequations}
	In the squeezed limit when $\vartheta_3 \rightarrow 0$ one can verify
	that $J_1 \rightarrow -1/2$ and $J_2 \rightarrow -2/3$.





	\section{Useful integrals}
	\label{appendix:b}

	To simplify evaluation of the integrals 
	arising in the calculation of the bispectrum,
	we introduce a master integral,
	$\mathcal{J}$,
	for which the integrals of interest are special cases
	\cite{Burrage:2010cu}.
	We define
	\begin{equation}
		\begin{split}
			\mathcal{J}_{\star}
			=
			\im \int_{-\infty}^{\tau} \d\xi \; \e{\im k_t \csstar\xi}
			\bigg\{
				&
				\gamma_0
				+ \im \gamma_1 \csstar \xi
				+ \gamma_2 \csstar^2 \xi^2
				+ \im\gamma_3 \csstar^3 \xi^3
				+ \gamma_4 \csstar^4 \xi^4
			\\ & \mbox{}
				+ N_\star \left(
					\delta_0
					+ \im \delta_1 \csstar \xi
					+ \delta_2 \csstar^2 \xi^2
					+ \im \delta_3 \csstar^3 \xi^3
					+ \delta_4 \csstar^4 \xi^4
				\right)
			\bigg\}\ \ ,
		\end{split}
		\label{eq:masterj}
	\end{equation}
	where 
	$N_\star = \ln | k_\star \csstar \xi |$.
	Eq.~\eqref{eq:masterj} is an oscillatory integral,
	for which asymptotic techniques are well-developed,
	and which can be evaluated using repeated integration by parts.
	To evaluate the $N_\star$-dependent terms one requires the
	standard integral
	\begin{equation}
		\lim_{\tau \rightarrow 0} \int_{-\infty}^{\tau} \d\xi
		\; N_{\star} \, \e{\im k_t \csstar} 
		=
		\dfrac{\im}{k_t \csstar}
		\left(
			\EulerGamma +
			\im \dfrac{\pi}{2}
		\right) \ \ .
	\end{equation}
	We conclude
	\begin{equation}
		\begin{split}
			\mathcal{J}_\star
			=
			\frac{1}{k_t \csstar}
			\bigg\{
				&
				\gamma_0
				- \frac{\gamma_1 + \delta_1}{k_t}
				- \dfrac{2\gamma_2+3\delta_2}{k_t^2}
				+ \dfrac{6\gamma_3+11\delta_3}{k_t^3}
				+ \dfrac{24\gamma_4+50\delta_4}{k_t^4}
				\\
				& \mbox{}
				- \left(
					\EulerGamma
					+ \ln \frac{k_t}{k_\star}
					+ \im \dfrac{\pi}{2}
				\right)
				\left(
					\delta_0
					- \dfrac{\delta_1}{k_t}
					- 2 \dfrac{\delta_2}{k_t^2}
					+ 6 \dfrac{\delta_3}{k_t^3}
					+ 24\dfrac{\delta_4}{k_t^4}
				\right)
			\bigg\} \ \ .
		\end{split}
		\label{eq:masterjresult}
	\end{equation} 
	We use this result repeatedly in \S\ref{sec:3pf}
	to evaluate integrals in closed form.
	


==> app4.tex <==
\chapter{Steps beyond exact scale-invariance}
\label{app:beyond-sr}

In this appendix we include some details of the calculation described 
in chapter \ref{chapter:five}.
Some of the material is similar to that discussed 
in appendix \ref{app:sr}. Nevertheless we include it here 
for completeness, since the choice of 
time coordinates is different.




\section{Dynamics in $y$---why?}
\label{appendix:y}
In this appendix we motivate the use of the time-coordinate $y$
instead of the conformal time variable, $\tau$.
Why is this choice of space-time foliation, 
which defines a hypersurface at each $y=\textrm{constant}$, 
preferred compared to 
the more traditional conformal time? 
Were we to solve for the perturbations starting from 
Eq. \eqref{eq:quadratic action1} in $\tau$ coordinates, we would
obtain a formula for the propagator for scalar perturbations, 
$G_k$, which corresponds to 
the two-point correlator:
\begin{equation}
\langle \zeta (\vec{x},\tau) \zeta (\vec{y},\tilde{\tau}) \rangle =
G(\vec{x}, \tau; \vec{y},\tilde{\tau})
\end{equation}

We would proceed to solve the Green's function equation for the propagator, 
in Fourier space, which reads
\begin{equation}
\bigg\{
\dfrac{\d ^2}{\d \tau^2}+
\bigg(\dfrac{1}{z}\dfrac{\d z}{\d\tau}+ \dfrac{2}{a}\dfrac{\d a}{\d\tau}  \bigg)
 \dfrac{\d}{\d\tau} 
+k^2 c_s^2
\bigg\} G_k (\tau ; \tilde{\tau}) = -\dfrac{\im}{2a^2 z} \delta (\tau-\tilde{\tau})\ \ ,
\end{equation}
where $k$ is the comoving wavenumber and the Dirac delta
enforces evaluation at $\tau=\tilde{\tau}$.
Because scalar fluctuations will propagate at a phase 
velocity $c_s$ generically different from that of the light, 
one usually performs a change of variables, $z=-k c_s \tau$, so that 
the propagator is a function of the sound horizon.
To get the equation for the evolution of $G_k$ in $z$ would demand inverting
$\d z/\d \tau$, which without the premiss of working 
with perturbative $s$ becomes algebraically challenging 
when plugging into the equations of motion since 
a Taylor expansion could not be truncated.
In particular, it would be very hard to show that the propagator 
is explicitly symmetric under the interchange 
$\tau \leftrightarrow \tilde{\tau}$.

It turns out that expressing the $y$-evolution of background quantities 
allows to naturally 
accommodate a rapidly changing $c_s$, 
and therefore large $s$,
avoiding the difficulty just described.
In other words, the $y$ variable allows to sum all the powers 
in $s$. 

Moreover, writing the quadratic action for the fluctuations in 
the form \eqref{eq:quadratic action2} makes the reproduction of 
Bessel's equation more transparent, without any need for perturbative expansions. 
For these reasons, our dynamical analysis is presented in $y$-time, and 
follows the analysis of Khoury \& Piazza \cite{Khoury:2008wj}.







\section{The spectral index beyond exact scale-invariance}
\label{app:ns}
In chapter \ref{chapter:five} we use $n_s-1$ as a perturbative parameter, but 
never its explicit formula, since it is not necessary
throughout the calculation. We have surpassed the need to know this
because of the special properties of the two-point correlator of 
single-field models, in particular that it should be 
time-independent on super-horizon scales.
  Here we 
present the formula for $n_s-1$ for completeness.
In the action \eqref{eq:quadratic action2} the variable $q=a\sqrt{z c_s}$
obeys the following differential equation
\[ \dfrac{\d \ln q}{\d\ln y} =-\dfrac{1}{1-\varepsilon -s}
\bigg[1+\dfrac{w}{2} +\dfrac{s}{2} \bigg]  \, 
\bigg[1+\dfrac{\varepsilon \eta +t s}{(1-\varepsilon -s)^2} 
\bigg] \ \ , \]
which implies 
\begin{equation}
\dfrac{q''}{q} = \dfrac{1}{2y^2} \dfrac{\rho}{1-\varepsilon -s} +
\dfrac{1}{2y^2}\dfrac{1}{(1-\varepsilon -s)^2}
\bigg[
\frac{\rho^2}{2}+wx+ts+
\dfrac{\varepsilon \eta +t s}{(1-\varepsilon -s)^2}
\rho  (4-2\varepsilon -s+w )
\bigg] \ \ ,
\end{equation}
where $\rho\equiv 2+w+s$ and $x\equiv\d \ln w/\d N$ 
(which contributes at next-order only 
in the scale-invariant approximation).
We conclude that the spectral index in these theories 
satisfies
\begin{equation}
n_s-1=3-\sqrt{1+\frac{2\rho}{1-\varepsilon -s} +\frac{2}{(1-\varepsilon -s)^2}
\bigg[
\frac{\rho^2}{2}  +wx+ts+
\dfrac{\rho(\varepsilon \eta +t s)}{(1-\varepsilon -s)^2}
  (4-2\varepsilon -s+w )
\bigg]  }\ \ .
\label{eq:ns}
\end{equation}
To leading-order in the scale-invariant approximation, 
we find
\begin{equation}
n_s-1=\dfrac{-2\varepsilon -3s-w}{1-\varepsilon -s}\ \ ,
\label{eq:qsi_relation}
\end{equation}
in agreement with the result from table \ref{table:spectral-index}.
If we instead assume that $\varepsilon$ and $s$ are 
strictly constant and consider only 
$P(X,\phi)$ models, we recover the formula
deduced in Ref. \cite{Khoury:2008wj} that 
\begin{equation}
n_s-1=- \dfrac{2\varepsilon+s}{1-\varepsilon -s}\ \ , 
\end{equation}
which reproduces the exact scale-invariance relation
$s=-2\varepsilon$. In the slow-roll approximation
this reduces to
\begin{equation}
n_s-1 \simeq -2\varepsilon -s
\end{equation}
at leading-order, 
which again agrees with the results from 
table \ref{table:spectral-index}.

In the scale-invariant approximation scheme, $\delta$ is a next-order quantity 
defined by $\delta=s+2\varepsilon$, in $P(X,\phi)$ models. 
The general formula for $\delta$ in a generic Horndeski model will 
depend on the form of $w$, and therefore $x$. 
Using \eqref{eq:ns} we conclude that
\begin{equation}
n_s-1= -\dfrac{\eta+\delta}{1+\varepsilon}
-\dfrac{2}{3(1+\varepsilon)^2}
\Big\{
2 \varepsilon x+ 4 \big( \varepsilon \eta +t s \big) - \varepsilon t
\Big\}\ \ .
\end{equation}
This formula agrees with our expectation that $\delta$ is indeed 
a parameter contributing at next-order only.






\section{Next-order corrections---useful formulae}
\label{app:propagator}
When applying the Schwinger-Keldysh formalism we will summon
formulae for the corrections of the 
elementary wavefunctions for $\zeta$ at next-order in 
scale-invariance. This is 
because one should perform a uniform expansion in the slow-variation parameters
which include the interaction vertices, but also the propagator for 
scalar perturbations. In this appendix we collect some of the 
necessary formulae for this expansion.

\para{Background evolution}As explained in the main text, we wish to 
study the evolution of the background quantities in the 
time coordinate $y$.
To do so, we make a Taylor expansion around the time $y$ of 
horizon crossing of some reference scale $k_\star$ and make 
a uniform expansion for small $\eta_\star$ and $t_\star$.
Such expansion is well defined provided we restrict our analysis to a few e-folds
after horizon crossing. This ensures that $\varepsilon$ and $s$
have not varied significantly up to that point, such that 
we can treat $\eta$ and $t$ as perturbative parameters in the dynamics.
As justified in the main text, this is indeed a good approximation.

To get the $y$-evolution of the speed of sound, $c_s$, we start
by evaluating 
\begin{equation}
\dfrac{\d\ln c_s}{\d \ln(-k_\star y)}=-\dfrac{s_\star}{1-\varepsilon_\star-s_\star}
\bigg\{1+
 \dfrac{\varepsilon_\star\eta_\star+t_\star s_\star}{(1-\varepsilon_\star-s_\star)^2} 
-\bigg[\dfrac{t_\star}{1-\varepsilon_\star - s_\star}+ \dfrac{\varepsilon_\star \eta_\star
+t_\star s_\star}{(1-\varepsilon_\star-s_\star)^2}
 \bigg]
 \ln(-k_\star y) \bigg\}\ \ .
\end{equation}
To avoid cluttering the notation, we introduce
the following parameters which contribute 
at next-order only in scale-invariance:
	\begin{subequations}
		\begin{align}
			\alpha
			& = \dfrac{t }{1-\varepsilon  - s }+ \dfrac{\varepsilon  \eta
+t s}{(1-\varepsilon -s )^2}\\ 
\beta  
			& =\dfrac{\varepsilon \eta +t  s}{(1-\varepsilon -s)^2} \ \ .
		\end{align}
			\label{eq:alphabeta}
	\end{subequations}
Upon integration, we find
\begin{equation}
c_s=c_{s\star} (-k_\star y)^{-\frac{s_\star}{1-\varepsilon_\star -s_\star}}
\bigg\{1-\dfrac{s_\star}{1-\varepsilon_\star -s_\star}
\bigg[\beta_\star \ln (-k_\star y) -\dfrac{\alpha_\star}{2} \big(\ln(-k_\star y)\big)^2 \bigg]
 \bigg\}\ \ .
 \label{eq:cs}
\end{equation}
This simplifies if we write $s_\star=-2\varepsilon_\star +\delta_\star$
and work perturbatively in $\delta_\star$ [that is, assuming
$\Or(\delta_\star)=\Or(\eta_\star)=\Or(t_\star)$], as follows
\begin{equation}
c_s=c_{s\star} (-k_\star y)^{\frac{2\varepsilon_\star}{1+\varepsilon_\star}}
\bigg\{1+ \frac{2\varepsilon_\star}{1+\varepsilon_\star} 
\bigg[ 
\beta_\star +\dfrac{\delta_\star (\varepsilon_\star -1)}{2\varepsilon_\star (1+\varepsilon_\star)}
\bigg]\, \ln (-k_\star y)
-\frac{\alpha_\star \varepsilon_\star}{1+\varepsilon} \, \big(\ln (-k_\star y)\big)^2
 \bigg\}\ \ .
 \label{eq:cs2}
\end{equation}
In the limit when $\varepsilon$ and $s$ are both
strictly constant, $\alpha_\star=0=\beta_\star$, and
we reproduce the results of Ref. \cite{Khoury:2008wj}:
\[ c_s \sim (-k_\star y)^{-\frac{s_\star}{1-\varepsilon_\star -s_\star}}\ \ , \]
where we have temporarily restored the dependence in $s$ through $\delta$.
The additional contributions appearing in Eq. \eqref{eq:cs2}
are precisely the corrections to this purely power-law behaviour
and are relevant whenever $\varepsilon$ and $s$ are slowly-varying.


Proceeding similarly to get the dynamical evolution of the Hubble parameter, 
we obtain
\begin{equation}
H=H_{\star} (-k_\star y)^{\frac{\varepsilon_\star}{1-\varepsilon_\star -s_\star}}
\bigg\{1+\dfrac{\varepsilon_\star}{1-\varepsilon_\star  -s_\star}
\bigg[\beta_\star \ln (-k_\star y) -\dfrac{\alpha_\star}{2} \big(\ln(-k_\star y)\big)^2 \bigg]
 \bigg\}\ \ , 
 \label{eq:h}
\end{equation}
which in the limit of constant $\varepsilon$ and $s$ reduces to simply
\[ H \sim (-k_\star y)^{\frac{\varepsilon_\star}{1-\varepsilon_\star -s_\star}} \ \ .\]
Again, recasting this result in terms of only one non-perturbative 
parameter, we find
\begin{equation}
H=H_{\star} (-k_\star y)^{\frac{\varepsilon_\star}{1+\varepsilon_\star}}
\bigg\{1+\dfrac{\varepsilon_\star}{1+\varepsilon_\star }
\bigg[\bigg(\beta_\star +\frac{\delta_\star}{1+\varepsilon_\star} \bigg)\ln (-k_\star y) 
-\dfrac{\alpha_\star}{2} \big(\ln(-k_\star y)\big)^2 \bigg]
 \bigg\}\ \ .
 \label{eq:h2}
\end{equation}
The explicit formulae in Eqs. \eqref{eq:cs2} and \eqref{eq:h2}
are relevant when replacing in Eq. \eqref{eq:a} for the scale factor, $a(y)$.






\para{Derivatives of the elementary wavefunctions}When calculating the bispectra of Horndeski operators which are at least once
$y$-differentiated, we will require the derivatives of the 
elementary wavefunctions. We find 
\begin{equation}
\dfrac{\d }{\d y}\zeta_k^{\textrm{(background)}} =
\dfrac{\im H_\star (1+\varepsilon_\star)}{2\sqrt{z_\star}\, (k\, c_{s\star})^{3/2}}
k^2 y e^{\im ky}\ \ ,
\end{equation}
whereas the wavefunction corrections to the internal lines of the Feynman diagram obey
\begin{equation}
		\begin{split}
\dfrac{\d }{\d y} \delta \zeta_k^{\textrm{(internal)}}=
\dfrac{\im H_\star (1+\varepsilon_\star)}{2\sqrt{z_\star}\, (k c_{s\star})^{3/2}}
k^2 (-y)
\bigg\{ &
-\dfrac{n_s-1}{2}  e^{-\im ky} \int_{-\infty}^{y}\dfrac{e^{2\im k\xi}}{\xi} \d\xi\\
&+e^{\im ky}
\bigg[
\dfrac{\delta_\star}{1+\varepsilon_\star } -
\dfrac{\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2} 
+\im \dfrac{\pi}{4} (n_s-1)
+\dfrac{n_s-1}{2}\ln (-k_\star y)
\bigg]
\bigg\} \ .
		\end{split}
		\label{eq:yderivatives}
\end{equation}
To obtain these we have explicitly eliminated the non-perturbative
dependence in the variation of the speed of sound, parametrised by $s$, 
in favour of the perturbative parameter, $\delta$.


The time variation of the wavefunctions is relevant 
in correctly reproducing the time-independence
of the correlation functions for $\zeta$.











 \section{Useful integrals}
\label{app:integrals}
In this appendix we list the integrals which occur when computing the 
three-point correlators. They fall in essentially two different varieties:
integrals involving the exponential integral function 
(which first appeared in Eq. \eqref{eq:zetakinternal}) 
and those which involve power-laws and logarithmic integrand functions. We will identify master integrals 
for each of these families and analyse them separately.
This section generalises the results obtained in \S\ref{appendix:a}.



\subsection{Integrals involving the exponential integral function, $\Ei(\xi)$}
These integrals appear in the form
\begin{equation}
I_\gamma (k_3) \equiv 
\int_{-\infty}^0 {\d y}\, \bigg\{  {(-y)^\gamma}  
e^{\im (k_1+k_2-k_3) y}\, \int_{-\infty}^{y}{\dfrac{\d \xi}{\xi}\, e^{2\im k_3 \xi}} 
\label{eq:integfunctionint}
\bigg\}
\end{equation}
where we have explicitly written $I$ as a function of the 
asymmetric momentum (in this case $k_3$), 
even though it is a function of the three
momenta through $k_t$ 
(perimeter in momentum space, $k_t=k_1+k_2+k_3$).
The constant $\gamma$ need not be an integer, 
and this is where the algebra differs
from that presented in Refs. \cite{Burrage:2010cu, Burrage:2011hd}
and in appendix \ref{app:sr}. 

In what follows we consider positive, arbitrary $\gamma$.
To simplify this integral, one follows the algorithm
developed in these references: 
we apply a transformation of variables 
to convert this integral into its dimensionless 
version [defining $x=\im (k_t-2k_3)y$]. 
We then make a rotation in the complex plane
[using $w=-\im k_3 \xi$]. 
Applying Cauchy's integral theorem we arrive at 
\begin{equation}
I_\gamma (k_3)= \bigg(\dfrac{1}{\im \vartheta_3 k_t}\bigg)
\ \int_{0}^{\infty}{\d x} \ \bigg\{ x^\gamma e^{-x} \ 
\int_{\infty}^{\theta_3 x} \dfrac{\d w}{w}\, e^{-2w}\bigg\}\ \ 
\label{eq:integfunctionint2}
\end{equation}
where
\[ \theta_3 \equiv\dfrac{k_3}{k_t-2k_3} \ \ \textrm{and}\ \ \ \vartheta_3\equiv 
\dfrac{1}{k_t} (k_t-2k_3) \ \ .\]
Focusing on the inner integral in \eqref{eq:integfunctionint2},
upon integrating by parts and using the expansion series of the exponential 
function, we find it has a convergent series representation 
\begin{equation}
\int_\infty^{\theta_3 x}\dfrac{\d w}{w} \ e^{-2w}= \EulerGamma
+\ln(2\theta_3 x) +\sum_{n=1}^{+\infty}\dfrac{(-1)^n}{n!} \dfrac{(2\theta_3 x)^n}{n}\ \ .
\end{equation}
Plugging this result into Eq. \eqref{eq:integfunctionint}
gives
\begin{equation}
I_\gamma(k_3)=\bigg(\dfrac{1}{\im \vartheta_3 k_t} \bigg)^{\gamma+1}
\bigg\{
\Gamma(1+\gamma) \Big[ \EulerGamma+
\ln (2\theta_3) +\psi^{(0)}(1+\gamma)
\Big]+
\sum_{n=1}^{\infty}\dfrac{(-2\theta_3)^n (n+\gamma)!}{n\, n!}
\bigg\}\ \ ,
\label{eq:integfunctionint3}
\end{equation}
in which $\psi^{(0)}(z)$ denotes the polygamma function of order 
zero and argument $z$.\footnote{The polygamma function of order $m$, $\psi^{(m)}(z)$,
						is the $(m+1)^{\mathrm{th}}$-derivative of the
						logarithm of the gamma function, $\Gamma$.
						We will only require polygamma functions of order
						zero and one in our formulae.} 
In obtaining this result 
we assumed $\Re(\gamma)>-1$ for the first two contributions, 
whereas $\Re(\gamma)>-2$ for the last term. This is true for all
the integrals since $\gamma$ is strictly non-negative. 
Finally, we can perform the last sum 
in Eq. \eqref{eq:integfunctionint3} by observing 
that it converges for $ -1/2<\Re(\theta_3)< 1/2 \big[$.
We conclude that 
the integral \eqref{eq:integfunctionint} has a closed-form 
representation, given by
\begin{equation}
		\begin{split}
I_\gamma(k_3)=\bigg(\dfrac{1}{\im \vartheta_3 k_t} \bigg)^{\gamma+1} &
\bigg\{
\Gamma(1+\gamma) \big[
\EulerGamma +\ln(2\theta_3) +\psi^{(0)}(1+\gamma)
\big]\\
& -2\theta_3 \Gamma (2+\gamma) \ \ 
_3 F_2\Big( \{1,1,2+\gamma\}, \{2,2\}, -2\theta_3 \Big)
\bigg\}\ \ ,
\end{split}
\label{eq:final_I-gamma}
\end{equation}
where $F$ is a (convergent) 
generalised hypergeometric function, 
$\mathrm{HypergeometricPFQ}$ \cite{mABR70a}. In chapter
\ref{chapter:five}
we will use the following abbreviated notation 
\begin{equation}
I_\gamma(k_3)=\bigg(\dfrac{1}{\im \vartheta_3 k_t} \bigg)^{\gamma+1} 
\ \tilde{I}_\gamma (k_3)\ \ ,
\end{equation}
which, given that $\tilde{I}_\gamma$
is a real-valued function, 
makes the identification of the real part of the result
of the integral more transparent. Explicit results for 
positive integers $\gamma=0,1,2$ are listed in 
Eqs. \eqref{eq:I0final} and \eqref{eq:otheris}.

Eq. \eqref{eq:final_I-gamma}
generalises Eqs. \eqref{eq:I0final}
and \eqref{eq:otheris}
for non-negative, but otherwise 
arbitrary $\gamma$.
In particular, Eq. \eqref{eq:final_I-gamma}
is valid for non-integer values of $\gamma$, 
which did not arise in chapter \ref{chapter:three}.
This generalisation arises from the deviation of 
the slow-roll approximation.






\subsection{Other integrals}

The other family of integrals which 
arises in the calculation of the bispectrum is of the form
\begin{equation}
J_\gamma \equiv \int_{-\infty}^{0} \d y e^{\im k_t y} \ (-y)^\gamma 
\bigg\{
A_\star + B_\star \ln (-k_\star y)+C_\star \big(\ln (-k_\star y) \big)^2 
\bigg\}\ \ ,
\label{eq:Jintegral}
\end{equation}
where the constant coefficients $A_\star$, $B_\star$ and $C_\star$ contain, in 
general, leading and next-order contributions in the scale-invariant 
approximation. 
This integral is a generalisation of Eq. \eqref{eq:masterj}
in \S\ref{appendix:b}.
Provided $\Re(\gamma)>-1$, which is indeed the case for all the 
integrals which arise in chapter \ref{chapter:five}, 
this integral converges and gives
\begin{equation}
\begin{split}
J_\gamma= \bigg(\dfrac{1}{\im k_t}\bigg)^{1+\gamma} \, \Gamma (1+\gamma) \
\bigg\{ &
A_\star + \bigg[\ln (k_\star/k_t)-\im \frac{\pi}{2} \bigg]\, 
\bigg[B_\star + C_\star \bigg(\ln (k_\star/k_t)-\im \frac{\pi}{2}  \bigg) \bigg]+\\
& +\psi^{(0)} (1+\gamma) \bigg[
B_\star +2C_\star \bigg(\ln(k_\star/k_t)-\im \frac{\pi}{2} \bigg)
+C_\star \psi^{(0)} (1+\gamma)
\bigg]+ \\
&+ C_\star \psi^{(1)} (1+\gamma)
\bigg\} \ \ .
\label{eq:this_integral}
\end{split}
\end{equation}
Again, to simplify the notation we will refer to this integral in the form
\begin{equation}
J_\gamma \equiv \bigg(\dfrac{1}{\im k_t}\bigg)^{1+\gamma} 
\ \tilde{J}_\gamma\ \ .
\end{equation}
We note that $\tilde{J}_\gamma$ is a complex-valued function, but 
given we only require the real part of $J_\gamma$ 
we need to use Euler's function to write
\[ \bigg( \dfrac{1}{\im k_t} \bigg)^{1+\gamma} =
\bigg( \dfrac{1}{ k_t} \bigg)^{1+\gamma}  \, \bigg\{
\cos\Big[\frac{\pi}{2} (1+\gamma) \Big] -\im \sin \Big[\frac{\pi}{2} (1+\gamma) \Big]
\bigg\}
\ \ .\]
This explains the presence of trigonometric functions 
in tables \ref{table:bbfunctions1} and \ref{table:bbfunctions2}.

These integrals are the generalisation of the integrals discussed 
in appendix \ref{app:sr}.






\section{Listing variables}
\label{app:list}
In the main tables of chapter \ref{chapter:five}, 
to simplify the formulae, we have introduced a compact 
notation for combinations of momenta and slow-variation parameters. 
This is summarised in the following table.


\vspace*{2cm}

	\begin{table}[htpb]

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

	\begin{center}
		\small
		\begin{tabular}{cc}

			\toprule
		
			variable & mathematical expression \\
			\midrule
		
			\rowcolor[gray]{0.9}
				$\tilde{k}$ &
				$ -k_t +\frac{\kappa^2}{k_t}+\frac{k_1 k_2 k_3}{k_t^2} $ 
				\\[2mm]

				$\kappa^2$ &
				$k_1k_2+k_1k_3+k_2k_3 $ 
				\\[2mm]

			\rowcolor[gray]{0.9}
$\Omega_{1\star}$ &
							
				
				$1+3\tilde{E}_\star +\frac{n_s-1}{2} \ln \Big(\frac{k_1 k_2 k_3}{k_\star^3} \Big) +  \frac{2\delta_\star}{1+\varepsilon_\star}-\frac{2\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2} $   \\
				 [2mm]

				$\Omega_{2\star}$ &
				$ - \frac{\delta_\star+h_{3\star}}{1+\varepsilon_\star}+
				\frac{2\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2} $ 
				\\[2mm]

			\rowcolor[gray]{0.9}
				$\Omega_{3\star}$ &
				$
				 \Omega_{1\star}-\frac{\delta_\star}{1+\varepsilon_\star}+\frac{\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2} $   \\
				  [2mm]

			
\multirow{3}*{$f(k_1,k_2,k_3)$} &
				$  (n_s-1)\big[-k_t \ln \frac{8k_1k_2k_3}{k_t^3} +2 \big(k_1 \ln2k_1/k_t
   +k_2 \ln2k_2/k_t  +  k_3 \ln2k_3/k_t \big)$ \\

   &  $+3\tilde{k} (\EulerGamma -\ln k_\star/k_t)  
   -3\frac{k_1k_2k_3}{k_t^2} +4k_t-2\kappa^2/k_t   \big]$\\

   &
   $-3\tilde{k} \Big(\frac{\delta_\star}{1+\varepsilon_\star}-\frac{\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2} \Big) $ 

				\\   				  [2mm]

				   			\rowcolor[gray]{0.9}

					$\Xi$ &
				$  \Gamma\bigg(1+\frac{4\varepsilon_\star}{1+\varepsilon_\star} \bigg)
			  \cos\bigg[\frac{2\pi \varepsilon_\star}{1+\varepsilon_\star}\bigg] $ 
				\\
 			\bottomrule
		\end{tabular}
	\end{center}
	\caption{Collection of the abbreviated variables used in the tables
	included in chapter \ref{chapter:five}. 
	\label{table:list}}
	\end{table}	


==> app6.tex <==
\chapter{Details of the preheating stage}
\label{app6}

This appendix serves two purposes.
First, in \S\ref{appendix:canonicnorm} we  
present the dictionary between physical and 
bare quantities in a DBI theory. 
The discussion is presented in the language 
of an arbitrary non-canonical field theory for
generality.
Second, in \S\ref{appendix:Hill} we give details of
our derivation of the Floquet exponent in Hill's equation. 
This generalises what is known for Mathieu's equation.
This appendix is companion of chapter \ref{chapter:six}.






\section{Canonically normalised theory}
\label{appendix:canonicnorm}

	We start by considering a general higher-derivative Lagrangian
	of the form $P(\phi, X)$, given by Eq.~\eqref{eq:action-preheating}
	in chapter \ref{chapter:six}.
	We let $\delta\phi$ denote small excitations around the background
	field $\phi_0$. Assuming derivatives of $\phi_0$
	are negligible then we can write
	$\delta X = \delta\dot{\phi}^2 - (\partial{\delta \phi})^2$.
	To quadratic order in $\delta \phi$ but including all orders
	in other fields, the field propagates in a locally
	Minkowski region according to the action
	\begin{equation}
		S =
			\int \d^4 x \;
			\left\{
				P_0 +\dfrac{\partial P}{\partial \phi} \delta \phi
				+ \dfrac{\partial P}{\partial X} \left[
					\delta \dot{\phi}^2 - (\partial{\delta \phi})^2
				\right]
				+ \dfrac{1}{2} \dfrac{\partial^2 P}{\partial\phi^2}
					\delta\phi^2
				+ \cdots
			\right\} \ \  ,
		\label{eq:action:decay1}
	\end{equation}
	where $P_0 = P(X=0, \phi_0)$
	and `$\cdots$' denotes higher-order terms in $\delta \phi$
	and its derivatives.
	
	Eq.~\eqref{eq:action:decay1}
	will give a reliable description of scattering and
	decay processes involving inflaton particles
	provided derivatives of the background
	field are negligible over the relevant time and distance scales
	our analysis applies.
	In this limit we can neglect the curvature of space-time
	and work in a locally flat region, 
	which should be chosen to be somewhat larger
	than the interaction region.
	Eq.~\eqref{eq:action:decay1} therefore applies within this patch.
	Local scattering probabilities can be described 
	by taking the associated $S$-matrix elements. On the other hand,
	if the background field $\phi$ varies significantly
	over the timescale of the scattering event then the definition
	of asymptotic \emph{in}- and \emph{out}-states becomes more complicated,
	and the concept of well-defined particles
	with an associated S-matrix may be invalidated.%
		\footnote{For example, this may happen in models where $\phi_0$
		evolves at a constant rate, such as the ghost inflation
		proposal of Arkani-Hamed {\etal}
		\cite{ArkaniHamed:2003uy,ArkaniHamed:2003uz}.
		We do not consider these models here.}
	
	
	
	\para{Canonical normalisation}If the vacuum is locally stable on timescales comparable with
	decay processes, then $\langle \partial P/\partial \phi \rangle$ must be
	negligible when evaluated there. We must nevertheless
	retain perturbative
	excitations contained in this term, whenever fermion
	Yukawa couplings are present.
	After canonical normalisation of $\delta \phi$,
	the interaction terms in the Lagrangian arise from
	\begin{equation}
		\mathcal{L}_{\mathrm{int}} \supseteq
			\frac{P_{,\phi}}{\sqrt{2 P_{,X}}} \delta \phi
			+ \frac{1}{4} \frac{P_{,\phi\phi}}{P_{,X}} \delta \phi^2 \ \ ,
	\end{equation}
	where a comma denotes a partial derivative
	evaluated in the background.
	In a cut-off throat,
	the models we have been considering
	correspond to $P =- f^{-1} (1 - f X)^{1/2} + f^{-1} - V(\phi)$ with
	$f$ constant and $V(\phi)$ chosen to be
	Eq.~\eqref{masterequation} or~\eqref{eq:pot-sym}.
	Consider the symmetry-breaking potential~\eqref{eq:pot-sym}.
	We only wish to canonically normalize $\delta \phi$, which represents
	fluctuations around the mean field visible to local observers as
	particles.
	Therefore, one should shift to canonical normalisation
	only after expanding in powers of fluctuations
	around the background field.
	Applying this procedure implies that we should make the transformations
	\begin{equation}
		m^2 \rightarrow \mstar^2 = \frac{m^2}{2 P_{,X}}
		\quad \mbox{and} \quad
		g^2 \rightarrow \gstar^2 = \frac{g^2}{\sqrt{2 P_{,X}}}\ \  .
		\label{eq:paramshifts}
	\end{equation}
	
	\para{Measurable masses and couplings}Whatever model we consider, the predictions of the 
	preheating theory should refer to the 
	\emph{same} particles. Therefore
	our results should be written in terms of the masses and couplings
	which are measured, for example, by a local observer who can record the outcome of
	scattering events. We therefore need to abandon the comfort of bare 
	quantities, and rewrite our final formulae in terms of 
	physical quantities.
	
	For non-canonical kinetic terms, it is possible that the
	evolution of the background field causes the masses and couplings
	to change in time. In this case, it is the masses and couplings
	measured by a local observer at the time of reheating which are
	the relevant quantities.
	
	At tree-level,
	the coupling $\gstar$ of the canonically normalized field is
	the coupling which is measured by experiment,
	and the mass $\mstar$ of the canonically normalized field
	determines the position of the pole in its propagator.
	These are unambiguous, physical definitions of the interaction
	coefficient and the mass of a particle.
	It is therefore the quantities $\mstar$ and $\gstar$ which should
	be compared with the mass and coupling in a theory with canonical
	kinetic terms.
		
	If a Yukawa coupling is present than
	we should similarly rescale its coupling constant:
	\begin{equation}
		h \rightarrow \hstar = \frac{h}{\sqrt{2 P_{,X}}} .
	\end{equation}







	\section{Floquet exponents from Hill's equation}
	\label{appendix:Hill}

	In this appendix we derive the Floquet exponent associated
	with Hill's equation.\footnote{I thank Joel Weller for sharing his preheating notes, 
													which have helped me to arrive at this result.}
													
\subsection{$\theta_0 , \theta_2, \theta_4 \neq 0$}
We start with the case when $\theta_2, \theta_4 \neq 0$, and $\theta_{2n}=0$, for $n>2$ and by noting that in the edges of the resonance bands $\mu_k=0$; it turns out that for the most important instability band and for $\theta_2  ,  \theta_4  <  1$
\begin{displaymath}
\theta_0 \simeq 1 \pm \theta_2 \, \left[1\mp \dfrac{\left(\theta_4\right)^2}{6\, \theta_2} \right] \ \ .
\end{displaymath} 
For $\theta_4 ^2 /\theta_2\ll 1$, this essentially reduces to 
\begin{equation}
\theta_0 \simeq 1 \pm \theta_2 \ \ \ .
\label{eq:theta0}
\end{equation} 
This implies that, at lowest-order, $\theta_0^{1/2} \simeq 1\pm \theta_2/2$. 

Now, the instability parameter is given by \cite{McLachlan}
\begin{equation}
\sin^{2}\left[{i\mu_{k} \frac{\pi}{2}}\right]=\triangle(0) \, \sin^{2}\left[{\theta_0^{1/2}  \, \frac{\pi}{2}}\right] \ \ ,
\label{eq:mu}
\end{equation}
where 
$\triangle (0)$ is exclusively determined by $\theta_0$, $\theta_2$ and $\theta_4$  and is approximately given by
\begin{displaymath}
\triangle(0)\simeq 1+\dfrac{\pi}{4\, \theta_0^{1/2} }\, \cot{\left[\theta_0^{1/2} \, \dfrac{\pi}{2}  \right] \, \left\{ \dfrac{\theta_2\, ^2}{1-\theta_0}  +  \dfrac{\theta_4\, ^2}{4-\theta_0}      \right\}} \ \ .
\end{displaymath} 
We can show that this yields 
\begin{equation}
\triangle(0) \simeq 1\mp \left(\dfrac{\pi}{2}\right)^2\, \left[\mp \left(\dfrac{\theta_2}{2}\right)^2 +\dfrac{\theta_2}{3}\, \left(\dfrac{\theta_4}{2}  \right)^2 +\dfrac{\left(\theta_2  \right)^3}{2}     \right]  \ \ .
\label{eq:triangle0}
\end{equation} 
We thus arrive at an approximate expression for the Floquet exponent
\begin{equation}
\mu_k \simeq \sqrt{\left(\dfrac{\theta_2}{2}\right)^2 -\left(\theta_0^{1/2}  -1 \right)^2  \mp \dfrac{\theta_2}{3}\, \left(\dfrac{\theta_4}{2}  \right)^2      \mp  \dfrac{\left(\theta_2  \right)^3}{2}     } \ \ .
\end{equation} 
This expression for $\mu_k$ is valid for $\theta_2, \theta_4 \ll 1$. 



\subsection{$\theta_0 , \theta_2, \theta_6 \neq 0$}

If we now proceed and consider the case with non-vanishing $\theta_0$, $\theta_2$ and $\theta_6$,
 we observe that the instability parameter may be computed using again (\ref{eq:mu}), where now 
\begin{equation}
\Delta(0) \simeq 1+ \dfrac{\pi \cot\left[\dfrac{\pi}{2}\, \theta_0^{1/2}  \right]}{4\theta_0^{1/2}} \ \left( \dfrac{\theta_2^2}{1-\theta} +\dfrac{\theta_6^2}{9-\theta_0}  \right) \ \ .
\label{eq:defindelta}
\end{equation} 
By considering the first instability band, we take $\theta_0 \simeq 1 \pm \theta_2$, so that
\begin{equation}
\theta_0^{1/2}\simeq 1 \pm \dfrac{\theta_2}{2} \ \ , \ \ \dfrac{\theta_2^2}{1-\theta_0} = \mp \theta_2  \ \ ,\ \ \dfrac{\theta_6^2}{9-\theta_0} \simeq \mp \dfrac{\theta_6^2}{8}\, \left(1 \pm \dfrac{\theta_2}{8} \right)\ , \ \    \textrm{and} \ \ \cot\left[\dfrac{\pi}{2}\, \theta_0^{1/2} \right] \simeq \mp \dfrac{\pi}{4}\, \theta_2  \ \ .
\end{equation} 
Plugging these into (\ref{eq:defindelta}), we find that, up to lowest-order
\begin{displaymath}
\Delta (0) \simeq 1 \mp \left(\dfrac{\pi}{4}\right)^2 \ \left(\mp \theta_2^2 +\dfrac{\theta_2\theta_6^2}{8} +\dfrac{\theta_2^3}{2}  \right) \ \ .
\end{displaymath} 
Moreover, 
\[\sin\left[\dfrac{\pi}{2}\, \theta_0^{1/2} \right] \simeq 1-\dfrac{1}{2}\, \left( \dfrac{\pi}{2}\right)^2\, \left(\theta_0^{1/2}-1 \right)^2 \ \ .\]
Finally, by substituting into (\ref{eq:mu}), we obtain 
\begin{equation}
\mu_k \simeq \sqrt{\left(\dfrac{\theta_2}{2}\right)^2\mp \dfrac{\theta_2\theta_6^2}{32} \mp \left(\dfrac{\theta_2}{2}\right)^3 -\left(\theta_0^{1/2} -1 \right)^2     } \ \ .
\end{equation} 
This generalises Eq. \eqref{eq:mumathieu}
suitable to compute the Floquet exponent in Mathieu's equation.



\newpage
\thispagestyle{empty}
\newpage

==> five.tex <==


\begin{savequote}[30pc]
Real science is a revision in progress, always. \\
It proceeds in fits and starts of ignorance.
\qauthor{Stuart Firestein, in \textit{Ignorance: How It Drives Science}}
\end{savequote}





\chapter{Inflationary Signatures of Single-Field Models Beyond Slow-Roll}
\label{chapter:five}
\hrule
\vspace*{1cm}




As we have seen in the previous two chapters, 
until recently to compute the bispectrum we
started from the action for 
the comoving curvature perturbation, $\zeta$, 
for each model independently.
However, recent developments have taught us that, in single-field models 
without ghost-like instabilities, 
the cubic action for $\zeta$ can always be written in the form
	\begin{equation}
		S^{(3)} = 
		\int \d^3 x \, \d\tau \; \Big\{ 
			a \Lambda_1 \zeta'^3 +a^2 \Lambda_2 \zeta \, \zeta'^2
			+ a^2 \Lambda_3 \zeta (\partial \zeta)^2
			+ a^2 \Lambda_4 \dot{\zeta} \partial_i \zeta
				\partial^i (\partial^{-2}\, \zeta')
			+ a^2 \Lambda_5 \partial^2 \zeta
				(\partial_i \partial^{-2}\, \zeta')^2	
		\Big\} \ \ .
		\label{eq:zeta-action3}
	\end{equation}
The model-dependent imprints are encoded in each of the 
\textit{five} coefficients $\Lambda_i$ of 
the Horndeski operators.
This action will be our starting point to compute the bispectrum
in this chapter.

Many authors have focused on the study of the action 
\eqref{eq:zeta-action3} under the assumption of
slow-roll regime in which the inflationary expansion 
is quasi-de Sitter, whilst
allowing for a small variation of the sound speed of perturbations. 
In this approximation, $\varepsilon\equiv -\d \ln H/\d N$, 
$\eta\equiv \d \ln \varepsilon /\d N$
and $s\equiv \d \ln c_s/\d N $ all obey 
$\varepsilon, |\eta|, |s| \ll 1$.
Examples of such works include
Refs. \cite{Seery:2005wm, Chen:2006nt, Burrage:2010cu}, 
and the calculation introduced in chapter \ref{chapter:two}.
But, what if inflation was \textit{not} very close to de Sitter, and these parameters 
cannot be treated perturbatively?
Khoury \& Piazza \cite{Khoury:2008wj} showed that this scenario was still
compatible with a perfectly
scale-invariant spectrum of perturbations,
in fair agreement with observations \cite{Larson:2010gs}, 
provided the relation $s=-2 \varepsilon$ was satisfied 
in $P(X,\phi)$ models.\footnote{These authors have also considered 
													solutions within the ekpyrotic 
													mechanism (see Ref. \cite{Lehners:2008vx} 
													for a review, and
													also Refs. \cite{Khoury:2010gw, Baumann:2011dt}). 
													Here, however, we 
													focus on the inflationary scenario.} 
													
We know that both $\varepsilon$
and |$\eta$| must be small to allow for a successful 
period of inflation. But \textit{how small} are they required to be? 
If $\varepsilon$ is not much smaller than $1$, 
then a calculation beyond slow-roll is technically required,
especially
to fit in the current era of precision cosmology.
Previous works which have attempted to study correlations
beyond the slow-roll regime include corrections to the 
power spectrum in canonical models worked out by 
Steward \& Lyth \cite{Stewart:1993bc}; moreover,
Gong \& Stewart \cite{Gong:2001he} 
(see also Ref. \cite{Choe:2004zg}) 
used the Green's function method to obtain the propagator of scalar fluctuations
to next-next-order in slow-roll.
This terminology has been explained in \S\ref{subsec:estimatesfNL}.
This was later generalised by Wei \etal\, \cite{Wei:2004xx}  who considered models
with a varying speed of sound of perturbations.
Additionally Bartolo \etal \ \cite{Bartolo:2010im} 
calculated 
the power spectrum beyond leading-order in the context of
effective field theories of inflation \cite{Cheung:2007st, Weinberg:2008hq}.


In this chapter we will be interested in models where the spectrum is almost scale-invariant, 
so that the condition found by Khoury \& Piazza is mildly broken, and becomes
\[ s=-2\varepsilon+\delta\ \ . \]
This requires working to \textit{all} orders in $\varepsilon$ and $s$, 
but \textit{perturbatively} in $\delta$, 
 in deviations of the spectral index 
from unity, $n_s-1\ll 1$, and time variations of $\varepsilon$ and $s$. This last assumption
ensures that the conditions $\varepsilon, |s|<1$ are preserved for a sufficiently
large number of e-folds, which is a primary requisite for 
 inflation to last at least $60$ e-folds.\footnote{This work explicitly excludes models with 
								features in the potentials, which can trigger the 
								slow-roll parameters to temporarily grow 
								during inflation (see, for example, the review 
								by Chen \cite{Chen:2010xka}).
										}
In this sense, this is a calculation \textit{beyond} the
slow-roll approximation, which works as a resummation technique
applied to the non-perturbative parameters $\varepsilon$ and $s$. 
We refer to it as \textit{scale-invariant 
approximation}. 
Starting from the action \eqref{eq:zeta-action3}, the calculation 
is immediately applicable to all Horndeski models.
For this reason we will work with arbitrary 
interaction coefficients $\Lambda_i$---assignments to these coefficients
will correspond to specific models.

We organise the 
calculation in increasing powers in the hierarchy of slow-variation parameters, 
focusing on leading and next-order contributions. 
Leading-order results involve the least power of perturbative 
parameters, and correspond to results obtained assuming 
a perfectly scale-invariant spectrum of perturbations. 
Next-order corrections contain small deviations 
from this which are parametrised by $n_s-1$, and therefore involve 
terms with one extra power in 
the perturbative parameters.
This organisational scheme follows the one used throughout 
Refs. \cite{Burrage:2010cu, Burrage:2011hd, Chen:2006nt}
and the previous chapter, which nevertheless applied to the slow-roll
approximation. 
On the other hand, our calculation relies on the 
\textit{scale-invariant approximation} and generalises their results
 up to next-order in scale-invariance.







\para{Outline}This chapter is organised as follows.
In \S\ref{sec:dynamics} we obtain the dynamical behaviour
of the scale factor and the other relevant background quantities
in the scale-invariant approximation.
The dynamical behaviour is exact in $\varepsilon$ and $s$, 
and perturbative in the time variation of these parameters, $\delta$ and $n_s-1$.
In \S \ref{sec:power spectrum} we obtain the power spectrum for scalar fluctuations,
and we derive in \S\ref{sec:propagator} formulae for
 the elementary wavefunctions
from which the scalar propagator is built
to next-order in scale-invariance.


We use these results to 
compute the bispectrum of perturbations in \S\ref{sec:bispectrumh}
and comment on the differences when using 
the slow-roll approximation. 
We conclude in \S\ref{sec:conclusionsh}.
Appendix \ref{app:beyond-sr}
collects useful formulae and detailed expressions 
of recurring integrals necessary to produce closed form bispectra.
Some of these are strongly related to those
investigated in Appendix \ref{app:sr}. 
However, for completeness, 
and because (as we shall see) these integrals are performed in a different
time variable, we include them in 
Appendix \ref{app:beyond-sr} as well.


This chapter is strongly based on 
Ref. \cite{Ribeiro:2012ar}.







\section{Background evolution beyond exact scale-invariance}
\label{sec:dynamics}
We are interested in nearly scale-invariant models which fall under
the class of Horndeski theories. As argued in Ref. \cite{Khoury:2008wj}
a scale-invariant spectrum for perturbations can be accommodated 
by a background where both the Hubble parameter and the speed of sound of perturbations
vary significantly in time, 
provided they obey the \textit{exact} relation $s=-2 \varepsilon$. 

We start with an arbitrary single-field theory for a homogeneous
scalar field, on which small, inhomogeneous perturbations, $\delta \phi$, develop. 
All we require is the spectrum of perturbations to be \textit{quasi} scale-invariant.
For all inflation models involving one single clock in the universe, 
the quadratic action for the primordial
comoving perturbation, $\zeta$, can be written as 
\begin{equation}
S^{(2)}=\dfrac{1}{2}\int \d^3 x \d\tau \, a^2 \, z\,
\bigg\{ \zeta'^2 -c_s^2 \big(\partial \zeta  \big)^2\bigg\} \ \ ,
\label{eq:quadratic action1}
\end{equation}
where $z$ is required to be a well defined, differentiable function
of the background dynamics and Lagrangian parameters,
but is otherwise arbitrary.\footnote{For $P(X,\phi)$ models, $z=\varepsilon/c_s^2$
									 \cite{Burrage:2011hd},
									but the same need not be true for other models,  
									such as galileon inflation theories
									\cite{Burrage:2010cu}.
									We will come back to this point in \S\ref{sec:propagator}.
									We note that $z$ here is not the usual $z$ 
									for $k$-inflation defined in Ref. \cite{Garriga:1999vw}.}
									We have seen this action before in Eq. \eqref{eq:eom2conformaltime}.
The time evolution of $z(y)$ will be parametrised by $w\equiv \d \ln z/\d N$.
For consistency, we also work to all orders in $w$.
For an arbitrary $w$, Khoury \& Piazza's relation between $\varepsilon$
and $s$ required for scale-invariance, 
is generalised to\footnote{We refer the reader to Eq. \eqref{eq:qsi_relation}
										in appendix \ref{app:ns} for details
										on the derivation of this formula.}
\[ 3s=-2\varepsilon-w\ \ . \]		
This formula reduces to $s=-2\varepsilon$ for $P(X,\phi)$ models.											
As we discuss in Appendix \ref{appendix:y}, 
it is more convenient to study the dynamics of background 
quantities as a function of $y$, satisfying $dy=c_s d\tau$, 
rather than conformal time, 
$\tau$. 
In this new time-coordinate, the action \eqref{eq:quadratic action1} becomes
\begin{equation}
S^{(2)}=\dfrac{1}{2}\int \d^3 x \d y \, q^2\,
\bigg\{  \bigg(\dfrac{\partial \zeta}{\partial y}\bigg)^2 
-\big(\partial \zeta  \big)^2\bigg\} \ \ ,
\label{eq:quadratic action2}
\end{equation}
with $q=a\sqrt{z\,c_s}$. Introducing the canonically normalised field 
$v_k=q \zeta_k$, where the subscript $k$ specifies
the Fourier mode, and
changing variables to $v_k=A_k \sqrt{-k y}$, we find that the 
modes $A_k$ obey
a Bessel equation of the form
\begin{equation*}
A_k''+\dfrac{1}{y} A_k'+
A_k \bigg\{k^2- \bigg(\dfrac{q''}{q}+\dfrac{1}{4y^2}\bigg)   \bigg\}=0 \ ~\ .
\end{equation*}
The solution to this equation is a linear combination of Hankel functions, 
$ H^{(1)}_\nu (-ky)$ and $ H^{(2)}_\nu (-ky)$, 
with order 
\begin{equation*}
\nu=\dfrac{3}{2}-\dfrac{n_s-1}{2}\ \ .
\end{equation*}
For a perfectly scale-invariant spectrum of perturbations, then $\nu_0=3/2$
and the spectral index is unity. This results in the power being 
constant in all scales. We refer the reader to Appendix \ref{app:ns} for details of
how the spectral index relates to the background quantities, 
although the precise formula will be unimportant in what follows, 
as we shall see.


Agreement with the appropriate normalization of the propagator gives the overall 
evolution of the elementary wavefunction as follows
\begin{equation}
\zeta_k=\sqrt{\dfrac{\pi}{8k}} \, \dfrac{\sqrt{-ky}}{a\sqrt{z c_s}}\ H^{(1)}_\nu (-k y)\ \ .
\label{eq:zeta_k}
\end{equation}
Finally, the power spectrum of perturbations can be obtained by
evaluating the scalar propagator at equal times 
[cf. Eq. \eqref{eq:power-spectrum-def}], yielding
\begin{equation}
\langle \zeta (\vec{k_1}) \zeta (\vec{k_2})\rangle =(2\pi)^3\, 
\delta^{(3)} (\vec{k_1}+\vec{k_2}) \dfrac{\pi}{8} 
\dfrac{(-y)}{a^2(y) \, z(y) \, c_s(y)} \, \left|H^{(1)}_\nu (-ky)  \right|^2\ \ .
\label{eq:2pf1}
\end{equation}
To further simplify this expression we will require the evolution of the
scale factor $a$ in $y$-coordinates. In order to do so, we 
specify the parameters in the slow-variation catalogue, 
which will allow us to perform a uniform expansion
up to next-order terms in the scale-invariant approximation.

\vspace*{0,3cm}


\para{Slow-variation catalogue}To obtain the dynamical evolution of the scale factor in a background
where 
$\varepsilon$ and $s$ are smaller than $1$ 
(but not necessarily \textit{much smaller} than $1$),
we introduce the following slow-variation parameters:
\begin{equation}
\eta \equiv \dfrac{\d\ln\varepsilon}{\d N} \ \ \textrm{and} \  \ 
t\equiv \dfrac{\d\ln s}{\d N}\ \ .
\end{equation}
We assume these parameters satisfy $|\eta|, |t|\ll 1$.
Our results rely on the scale-invariant expansion, and are 
organised in leading-order contributions, and terms contributing at next-order only.
Leading-order results are the lowest-order terms which are compatible with a perfectly scale-invariant 
power spectrum of perturbations, whereas next-order terms are corrections parametrising the deviation from 
$n_s-1=0$.
This organisational scheme is motivated by the cosmological
data that suggests that $n_s-1$ is very small, and can 
therefore
be treated perturbatively.

To determine the behaviour of the scale factor,
we start by integrating $ c_s d\tau$
to compute $y$. Working \textit{perturbatively} in $\eta$ and $t$,
but to \textit{all} orders in $\varepsilon$ and $s$, we find
\begin{equation*}
y=-\dfrac{c_s}{aH} \sum_{m=0}^{+\infty}\Big\{(\varepsilon+s)^m +
 (\varepsilon+s)^{m-1} \sum_{k=0}^m{k\big(ts +\varepsilon \eta  \big)} \Big\}\ \ .
\end{equation*}
These sums converge and give
\begin{equation}
a(y)=-\dfrac{c_s}{Hy\,(1-\varepsilon-s)}\, 
\bigg\{1+\dfrac{\varepsilon \eta +t s}{(1-\varepsilon -s)^2} \bigg\} \ \ .
\label{eq:a}
\end{equation}
This result was first obtained by Khoury \& Piazza in Ref. \cite{Khoury:2008wj}.
Using Eq. \eqref{eq:a} we can further simplify the two-point correlator
\eqref{eq:2pf1} in 
$y$-time, which becomes
\begin{equation}
\langle \zeta (\vec{k_1}) \zeta (\vec{k_2})\rangle =(2\pi)^3\, 
\delta^{(3)} (\vec{k_1}+\vec{k_2}) \dfrac{\pi}{8} 
\dfrac{H^2(y) (-y)^3  (1-\varepsilon-s)^2 }{z(y)\, c_s^3(y)} \,
\bigg\{1-2\dfrac{\varepsilon \eta +t s}{(1-\varepsilon -s)^2} \bigg\} 
 \left|H^{(1)}_\nu (-ky)  \right|^2\ \ .
\label{eq:2pf2}
\end{equation}

In a generic model, the two-point correlator will evolve in time. 
However, for a single-field model, by virtue of conservation of 
$\zeta$ on super-horizon scales
 \cite{Lyth:1984gv, Wands:2000dp}, 
it follows that the power spectrum 
will rapidly converge to its 
asymptotic value.\footnote{See Ref. \cite{Nalson:2011gc} for comments
							on the number of e-folds necessary for such 
							asymptotic behaviour to be reached
							after horizon crossing. There, the authors studied 
							a two-field inflation model, but the same conclusions
							 apply to single-field models.}
We have also seen this explicitly in \S\ref{subsec:second}.

Therefore, we can focus our calculation a few e-folds after horizon crossing
for a given scale, $k_\star$. This has become the standard approach
when calculating the asymptotic limit of the power spectrum.
This remains true even in multi-field inflation, 
where this procedure sets the appropriate 
initial conditions for evolving correlation functions
after horizon crossing, using techniques such as $\delta N$
\cite{Lyth:2005fi}, 
transport equations \cite{Mulryne:2009kh, Mulryne:2010rp}, 
or transfer matrices \cite{Wands:2002bn} (see, for example,
Refs. \cite{GrootNibbelink:2001qt, Lalak:2007vi, Peterson:2010np, 
Peterson:2010mv, Avgoustidis:2011em, Peterson:2011yt}). 
The advantages of applying this approach are twofold: 
on one hand, at this point in the evolution the elementary wavefunction
is completely characterised by the growing mode, since the decaying mode has 
become negligible; on the other hand, the power spectrum obtained in this way 
is already the asymptotic value, at late times.
Said differently, at this point of evaluation 
$\zeta$ has \textit{become classical} \cite{Lyth:1984gv, Lyth:2006qz}.

With this methodology in mind, and working perturbatively in $\eta$ and $t$
we obtain 
	\begin{subequations}
		\begin{align}
			\varepsilon 
			& \simeq \varepsilon_{\star} 
			\bigg\{1-\dfrac{\eta_\star}{1-\varepsilon_\star-s_\star} \ln(-k_\star y) \bigg\}\ \ \textrm{and}\\ 
			s 
			& \simeq s_{\star} 
			\bigg\{1-\dfrac{t_\star}{1-\varepsilon_\star-s_\star} \ln(-k_\star y) \bigg\}		
		\end{align}
					\label{eq:sr1}
	\end{subequations}
	to next-order in the scale-invariant approximation.
As before,
starred quantities are to be evaluated when some scale, $k_\star$, 
has exited the $y$-horizon, so that $k_\star y_\star=-1$. 
It is important to leave this 
scale arbitrary since this generates the scale-dependence
of the correlation functions. The appearance of the logarithmic 
term corresponds precisely to the number of 
e-folds, $N_\star$, measured in $y$-coordinates, 
which have elapsed since the scale $k_\star$
has exited the horizon.
The expansion in Eqs. \eqref{eq:sr1} is only valid up to a 
few e-folds outside the horizon, when one can trust the expansion in
Taylor series to first-order.
We note that quasi scale-invariance demands $\eta_\star=t_\star$, 
up to next-next-order corrections, which we do not keep in 
our calculation.



Given the individual dynamics of $c_s(y)$ and $H(y)$ derived in 
Eqs. \eqref{eq:cs} and \eqref{eq:h} of 
Appendix \ref{app:propagator}, we can 
replace for the evolution of the scale factor in
Eq. \eqref{eq:a}. We find:
\begin{equation}
a(y)=\dfrac{c_{s\star}(-k_\star y)^{-\frac{s_\star+\varepsilon_\star}{1-\varepsilon_\star-s_\star}}}{H_\star (1-\varepsilon_\star-s_\star) (-y)} 
\bigg\{ 
1+\beta_\star
-\bigg[ \dfrac{\beta_\star}{1-\varepsilon_\star - s_\star}\bigg] \ln(-k_\star y)+
\bigg[\dfrac{\alpha_\star (\varepsilon_\star +s_\star)}{2(1-\varepsilon_\star -s_\star)}\bigg]\big(\ln(-k_\star y)\big)^2 
\bigg\} \ \ ,
\label{eq:scale_factor}
\end{equation}
where the next-order parameters $\alpha$ and $\beta$
are defined in Eqs. \eqref{eq:alphabeta}.\footnote{$\alpha$ and $\beta$ here are not to be confused
										with the parameters refereed to by the same letters in the previous chapters.}
Despite its complicated structure, Eq. \eqref{eq:scale_factor} 
correctly reproduces the results 
of chapter \ref{chapter:two} and Ref. \cite{Khoury:2008wj} 
when we take the limit of \textit{exact} scale-invariance, 
for which $\eta_\star=t_\star=0$, resulting in 
vanishing $\alpha_\star$ and $\beta_\star$ [cf. Eqs. \eqref{eq:alphabeta}].
The extra terms in between brackets in 
Eq. \eqref{eq:scale_factor} are precisely
the corrections to a pure, dominant power-law evolution.



\subsection{The scalar power spectrum}
\label{sec:power spectrum}

The power spectrum $P(k)$  defined by
\begin{equation}
\langle \zeta (\vec{k_1}) \zeta (\vec{k_2})\rangle =(2\pi)^3\, 
\delta^{(3)} (\vec{k_1}+\vec{k_2})  P(k)
\end{equation}
where $k=|\vec{k}|=|\vec{k}_1|=|\vec{k}_2|$,
will in general depend on time. Taking the super-horizon limit, $|ky|\rightarrow 0$,
we find that the dominant contribution arising from the Hankel function
in Eq. \eqref{eq:2pf2} is given by
\begin{equation*}
\left|H^{(1)}_\nu (-k y)   \right|^2 \longrightarrow -\dfrac{2}{\pi k^3 y^3} 
\Big\{1+ (n_s-1) \big[-2+\EulerGamma +\ln(-2 k y)\big] \Big\} \ \ .
\end{equation*}
Whatever $y$-evolution the remaining terms in Eq. \eqref{eq:2pf2} have
in \textit{this} limit, 
they should precisely cancel the $y$-dependence of the Hankel function.
This is a requirement imposed by conservation of $\zeta$ on super-horizon
scales in single-field models.
This allows us to readily write the power spectrum as
\begin{equation}
P(k)= \dfrac{H_\star^2\, (1-\varepsilon_\star -s_\star)^2}{4\, z_\star \, (k\, c_{s\star})^3}
\Big\{1+2E_\star + (n_s-1) \ln(k/k_\star) \Big\}\ \ ,
\label{eq:powerspectrumr}
\end{equation}
where we have defined 
\begin{equation}
E_\star=-\beta_\star +
\dfrac{n_s-1}{2} \,\big\{-2+\EulerGamma +\ln 2 \big\}\ \ .
\end{equation}
This is the power spectrum for a nearly scale-invariant Horndeski 
theory. To recover the perfectly scale-invariant formula
obtained by Khoury \& Piazza \cite{Khoury:2008wj},
we simply set $E_\star$ and $n_s-1$ to zero, since 
these enter the power spectrum as next-order corrections in scale-invariance.
Whilst being time-independent, 
Eq. \eqref{eq:powerspectrumr} correctly reproduces the 
expected logarithmic scale-dependence in the 
limit when the slow-roll regime applies, 
in which $\varepsilon$ and $s$ are slow-roll parameters
[cf. Eq. \eqref{eq:powerspectrum}].
Indeed, we can check that defining the dimensionless version of the power 
spectrum using the usual rule $\mathcal{P}=k^3 P(k)/2\pi^2$, Eq. \eqref{eq:powerspectrumr}
gives\begin{equation*}
n_s-1 =\dfrac{\d \ln \mathcal{P}}{\d \ln k}\ \ .
\end{equation*}
Again, the explicit expression for $n_s-1$ will not be required 
in any stage of the calculation, but we refer the reader 
to Appendix \ref{app:ns} where its formula is derived. 
It suffices to treat it as an arbitrary next-order
quantity.





\subsection{Obtaining next-order corrections to the wavefunctions, $\zeta_k$}
\label{sec:propagator}
Our ultimate interest lies in obtaining the bispectrum of perturbations 
starting from the
action \eqref{eq:zeta-action3}. 
We will rely on the scale-invariant approximation introduced in this chapter. 
Since we will keep corrections up to next-order, 
we also require corrections 
to the elementary wavefunctions up to the same order, 
for consistency. 
We have already explained them in detail in \S\ref{eq:sources}, 
but we enumerate them here for completeness. 

%\vspace*{0,3cm}

\para{External legs}The corrections to the external lines of the Feynman diagram
correspond to evaluating the propagator in the asymptotic regime, 
when $|ky|\rightarrow 0$.
From Eq. \eqref{eq:powerspectrumr} we can read off the 
corrections to the external legs 
\begin{equation}
 \zeta_k(y)^{\textrm{(background+external)}}= \dfrac{\im}{2}
 \dfrac{H_\star (1-\varepsilon_\star-s_\star)}{\sqrt{z_\star} (k\, c_{s\star})^{3/2}}
 \Big\{1+E_\star +\dfrac{n_s-1}{2} \ln (k/k_\star) \Big\} \ \ .
 \label{eq:external legs}
\end{equation}
As argued in \S\ref{sec:power spectrum}, the time-independence of this
is guaranteed because the primordial perturbation 
$\zeta$ is conserved on super-horizon scales in single-field models.

From this it also follows that 
whatever function is assigned to $z(y)$, it must generically behave, at
leading-order in scale-invariance, as
\begin{equation}
z(y) \sim (-k_\star y)^{\frac{2\varepsilon_\star+3s_\star}{1-\varepsilon_\star - s_\star}}\ \ .
\label{eq:z}
\end{equation}
This imposes a mild requirement on an otherwise arbitrary, but smooth 
function $z(y)$. We check that for $P(X,\phi)$ models, where 
$z=\varepsilon/c_s^2$, this behaviour is consistent with 
Eqs. \eqref{eq:sr1} and \eqref{eq:cs}, supplemented by the condition
$s_\star=-2\varepsilon_\star$ (which holds at leading-order in the 
scale-invariant 
approximation scheme).
If in a given model $z$ has a different evolution from that of Eq. \eqref{eq:z}, 
it leads to a background where $\zeta$ is evolving on super-horizon
scales, which is incompatible with the single-field inflation scenario.


%\vspace*{0,3cm}

\para{Internal legs}This correction is a result of the spectrum 
being slightly tilted. Using Eq. \eqref{eq:a}, 
we rewrite, for clarity, Eq. \eqref{eq:zeta_k}
for the elementary wavefunction
as
\begin{equation}
\zeta_k (y)=\sqrt{\dfrac{\pi}{8}} \dfrac{H(y) (-y)^{3/2} (1-\varepsilon -s)  }{\sqrt{z(y)}\, c_s^{3/2}\,(y)}
\Big\{ 1-\dfrac{\varepsilon \eta+ts}{(1-\varepsilon -s)^2}  \Big\} \,H_\nu^{(1)}(-ky) \ \ .
\label{eq:zetak2}
\end{equation}
The order of the Hankel function, $\nu$, 
differs from $3/2$ by next-order corrections proportional to $(n_s-1)$. 
To evaluate corrections to $\zeta_k$ we
start by Taylor expanding the Hankel function around order $\nu_0=3/2$.
Following Refs. \cite{Chen:2006nt, Burrage:2010cu}, we find the background
evolution of the wavefunctions is given by 
\begin{equation}
 \zeta_k (y)^{\textrm{(background)}}=
 \dfrac{\im H_\star (1-\varepsilon_\star -  s_\star)}{2\sqrt{z_\star}\, (k c_{s\star})^{3/2}}
\  (1-\im ky)\, e^{\im ky}\ \ ,
 \label{eq:backzeta}
\end{equation}
which gives the leading-order behaviour of Eq. \eqref{eq:external legs}
in the limit $|ky|\rightarrow 0$.
The next-order corrections arising from $\delta \nu=\nu-3/2=-(n_s-1)/2$ and 
the slow-variation of the background quantities in \eqref{eq:zetak2} 
organise themselves into the internal leg corrections:
\begin{equation}
		\begin{split}
\delta \zeta_k(y)^{\textrm{(internal)}}=
\dfrac{\im H_\star (1-\varepsilon_\star -s_\star)}{2\sqrt{z_\star}\, (k c_{s\star})^{3/2}}
\bigg\{ &
-e^{\im ky} (1-\im ky) 
\bigg[\beta_\star +\dfrac{n_s-1}{2}\ln(-k_\star y) \bigg]\\
&+\dfrac{n_s-1}{2} 
\bigg[
e^{-\im ky} (1+\im ky) \int_{-\infty}^{y}\dfrac{e^{2\im k \xi}}{\xi} \d \xi -2e^{\im ky} 
-\im \dfrac{\pi}{2} e^{\im ky} (1-\im ky) 
\bigg]
\bigg\} \ .
		\end{split}
		\label{eq:zetakinternal}
\end{equation}
The integral representation on the second line above corresponds to the exponential 
integral function, $\mathrm{Ei} (-ky)$, defined for real, non-zero argument
\[\mathrm{Ei} (x) = \int_{-\infty}^{x} \dfrac{e^{t}}{t}\, \d t \ \ ,  \]
which was discussed in detail in Appendix \ref{appendix:propagator}.
The time-dependence of the internal leg corrections
is fairly
intricate and we verify
that there are no divergences in Eq. \eqref{eq:zetakinternal}
when we take the limit $|ky| \rightarrow 0$. This
represents a minimal check on this result. 
Expressions for the time-derivatives of the wavefunctions can 
be found in Appendix \ref{app:propagator}.

%\vspace*{0,3cm}




\para{Corrections arising from evolving interaction vertices}The interaction coefficients $\Lambda_i$ can generically 
evolve very fast, and one expects
their time evolution to be of the form
\begin{equation}
\Lambda_i \simeq \Lambda_{i\star} (-k y)^{n} \bigg\{1+ \tilde{a} \ln (-k_\star y)
+\tilde{b} \big(\ln (-k_\star y) \big)^2 \bigg\}\ \ ,
\label{eq:fastLambda}
\end{equation}
with the power $n$ depending on the exact expression of $\Lambda_{i}$,
and $\tilde{a}$ and $\tilde{b}$ being next-order terms
in the scale-invariant approximation.
This power-law dependence needs to be taken into account 
for consistency with the scale-invariant approximation---we will study an explicit example in \S \ref{subsec:features}. 
There, we explain in detail that the behaviour in 
Eq. \eqref{eq:fastLambda} can potentially bring 
problems to the convergence of the integral
in the formula for the bispectrum. 
In particular, there might be values of $\varepsilon$
for which one is unable to perform the calculation, 
because they would lead to a time-dependent three-point function.



Mainly to simplify our results, 
we assume the interaction vertices to have a very smooth and slow 
evolution in $y$-time. To this end,
we introduce a supplementary slow-variation 
parameter
\begin{equation}
h_i \equiv \dfrac{1}{\Lambda_i H}\dfrac{\d \Lambda_i}{\d t}\ \ ,
\end{equation}
which satisfies $|h_i|\ll 1$. We expect this approximation to be valid
for all Horndeski models whenever the interaction vertices are 
slowly evolving in time. 
As described in \S \ref{subsec:features}, the methods
developed in this chapter can 
still be used to compute $n$-point correlation functions in 
models where this assumption fails.
We conclude that, if $\Lambda_i$ is slowly varying, then
each interaction vertex evolves as 
\begin{equation}
\Lambda_i \simeq \Lambda_{i\star} 
\bigg\{1-\dfrac{h_{i\star}}{1-\varepsilon_\star -s_\star} \ln (-k_\star y) \bigg\}\ \ .
\label{eq:vertex corrections}
\end{equation}
This means that for simplicity in the remainder of this chapter 
we will set $n=0$ and $\tilde{b}=0$ in Eq. \eqref{eq:fastLambda}, but 
we will show how to deal with $n \neq 0$ in one simple example
in \S\ref{subsec:features}.
This assumption concludes the presentation of the 
slow-variation catalogue, which is therefore composed by the set 
$\{n_s-1 , \delta ,\eta, t, h_i \}$.

\para{Simplifying our results}We note that a further simplification to the background 
dynamics follows from inspection of Eqs. \eqref{eq:external legs}
and \eqref{eq:zetakinternal}. The variable $w$ 
that parametrises the variation of $z$, does not appear in our formulae.
Indeed such term is only present 
implicitly since it is encapsulated in the spectral index 
$(n_s-1)$ [cf. Eq. \eqref{eq:qsi_relation}]. 
Therefore the calculation is explicitly \textit{independent} of our choice of $w.$
As a consequence, we can 
effectively reduce the relation we found between $\varepsilon$, $s$
and $w$, to one which only involves the first two variables. 
To this end, we take the relation between $\varepsilon$ and $s$ to 
be 
\[ s=-2\varepsilon+\delta \ \ ,\]
where $\delta$ is a next-order parameter in the scale-invariant approximation. We emphasize that 
this procedure in no way lacks generality: the calculation is still 
non-perturbative in both $\varepsilon$ and $s$.
The formula above generalises the regime studied in Ref. \cite{Khoury:2008wj} by considering
a nearly scale-invariant spectrum.
This also implies that $t=\eta$ at next-order in the scale-invariant approximation, 
which is in agreement with the observations in \S\ref{sec:dynamics}.

This procedure dramatically simplifies our formulae 
and reduces the slow-variation catalogue to a minimum
of parameters, which we choose to be $\{n_s-1, \delta, \eta, h_i \}$. 
At the same time, our results will be displayed in terms of 
only one non-perturbative parameter, which we choose to be $\varepsilon$.\footnote{
							Our calculation is non-perturbative in \textit{both} $\varepsilon$
							and $s$. By noting that we can 
							write $s=-2\varepsilon +\delta$, 
							we can replace the non-perturbative
							parameter $s$ by the perturbative parameter $\delta$. 
							In the remainder of the text, the dependence in 
							$s$ is absorbed by $\delta$.
				}
We note that this will imply some conceptual restructuring of our formulae.
In particular, Eq. \eqref{eq:backzeta} now contains leading 
\textit{and} next-order contributions in $\delta_\star$, which can 
now be interpreted as an extra contribution to the 
external legs 
at next-order in Eq. \eqref{eq:external legs}.

 
Eqs. \eqref{eq:external legs}, \eqref{eq:zetakinternal}, and 
\eqref{eq:vertex corrections} 
combine amongst themselves to produce the overall 
corrections required to write
the bispectrum at next-order in the scale-invariant approximation.
 They naturally combine 
to produce two separate contributions to the bispectrum:
the background contributions and next-order corrections 
arising from the vertex and external legs; and 
the next-order contributions arising from the internal legs
of the Feynman diagram. We will use this way of partitioning the bispectrum to present
our results for the bispectrum in \S\ref{subsec:bispectrumh}
by labelling the first contributions as \textit{type-$a$ bispectrum},
and the second as \textit{type-$b$ bispectrum}.
This is the same notation defined in \S \ref{subsec:type-bispectra}.




\section{Non-gaussianity in the bispectrum}
\label{sec:bispectrumh}
As we have seen in the last chapters, non-gaussian signatures encoded in the CMBR work
as a powerful discriminant between inflationary models.
We compute the bispectrum in nearly scale-invariant
theories using the same \textit{in-in} rules reviewed in \S \ref{subsec:inin}.
The study of shapes is, 
however, beyond the scope of this work, 
and we leave it to forthcoming investigation.
We illustrate our results by specifying estimates of $\fNL$ in 
some useful limits.




\subsection{Bispectrum of Horndeski theories}
\label{subsec:bispectrumh}

As argued before, it will 
be convenient to write the action for perturbations in 
$y$-coordinates. From Eq. \eqref{eq:zeta-action3} this is given by
	\begin{equation}
	\begin{aligned}
		S^{(3)} = 
		\int \d^3 x \, \d y\, a^2 \; \bigg\{ 
			&\frac{c_s^2}{a} \Lambda_1 
			\bigg(\dfrac{\partial \zeta}{\partial y}\bigg)^3 +
			 c_s\Lambda_2 \zeta\, \bigg(\dfrac{\partial \zeta}{\partial y} \bigg)^2
			+ \frac{1}{c_s} \Lambda_3 \zeta (\partial_i \zeta)^2\\
			&
			+  c_s\Lambda_4 \ \bigg(\dfrac{\partial \zeta}{\partial y}\bigg) \ \partial_i \zeta
				\partial^i \bigg(\partial^{-2}\frac{\partial \zeta}{\partial y}\bigg)
			+  c_s \Lambda_5 \partial^2 \zeta
				\bigg(\partial_i \partial^{-2}\dfrac{\partial \zeta}{\partial y}\bigg)^2	
		\bigg\} \ .
		\label{eq:zeta-action3y}
			\end{aligned}
	\end{equation}
Our calculation is organised as follows:

%\vspace*{0,3cm}

\para{Bispectrum type $a$}The leading contributions  
and the corrections arising from the slow-variation 
of the interaction vertices and external legs can be 
written in the general form
\begin{equation}
B^a =\dfrac{\Lambda_{i\star}\, H_\star^4 \, (1+\varepsilon_\star)^4 }{2^6 c_{s\star}^6 z_\star^3 \prod_i k_i^3}\, N^a (k_1)\, \bigg\{
\Re\Big(P^a(k_1) \tilde{J}_\gamma \Big)+
\Re\Big(Q^a(k_1) \tilde{J}_{\gamma+1} \Big) +T^a(k_1)
  \bigg\} \ + \ \textrm{cyclic permutations}\ \ ,
  \label{eq:Ba-chapter4}
\end{equation}
where the addition of cyclic permutations entails the symmetric exchange
of momenta $k_1 \rightarrow k_2 \rightarrow k_3$. The functions 
$N^a(k_1)$, $P^a(k_1)$, $Q^a(k_1)$ and $T^a(k_1)$ 
are listed in table \ref{table:bafunctions}.
The functions $\tilde{J}_\gamma$ are studied in 
Appendix \ref{app:integrals} and defined by

\begin{equation}
\tilde{J}_\gamma \equiv  (\im k_t)^{1+\gamma} \int_{-\infty}^{0} \d y e^{\im k_t y} \ (-y)^\gamma 
\bigg\{
A_\star + B_\star \ln (-k_\star y)+C_\star \big(\ln (-k_\star y) \big)^2 
\bigg\}\ \ .
\label{eq:Jtildeintegral}
\end{equation}
Table \ref{table:JcoefficientsBa} contains the assignments $A_\star$, $B_\star$
and $C_\star$ for the functions
$\tilde{J}_\gamma$.
We note that the coefficients 
for the operators $\zeta \zeta'^2$, 
$\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta' $, 
and $\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2$
are the same. Having done the calculation independently for 
each operator, this is a minimal check of the correctness of our results.
This happens because these operators have the same time-derivative structure, and differ
only in the arrangement of spatial-derivatives, and therefore, in the momentum 
dependence.


\vspace*{1cm}


\para{Bispectrum type $b$}Likewise, the contributions from the propagator in the 
internal lines of the Feynman diagram can be consolidated
for all operators in the form
\begin{equation}
		\begin{split}
B^b =\dfrac{\Lambda_{i\star}\, H_\star^4 \, (1+\varepsilon_\star)^4 }{2^6 c_{s\star}^6 z_\star^3 \prod_i k_i^3}\, N^b(k_1)\, \bigg\{ & (n_s-1)
\sum_i\Big[\,\Re\Big(P^b_i(k_1) \Big)\tilde{I}_\gamma (k_i) +
\Re\Big(Q^b_i(k_1)\Big) \tilde{I}_{\gamma+1}(k_i)  \Big]\\
&+\Re \Big(R^b(k_1) \,\tilde{J}_\gamma\Big)
+\Re \Big(S^b(k_1)\, \tilde{J}_{\gamma+1}\Big)
+(n_s-1)\, T^b(k_1)
  \bigg\} \  \\ & + \textrm{cyclic permutations}\ \ ,
  \label{eq:Bb}
  \end{split}
\end{equation}
where again the addition of cyclic permutations entails the symmetric exchange
of momenta $k_1 \rightarrow k_2 \rightarrow k_3$. The functions 
$N^b(k_1)$, $P^b_i(k_1)$, $Q^b_i(k_1)$, $R^b(k_1)$, $S^b(k_1)$ and 
$T^b(k_1)$ are listed in tables \ref{table:bbfunctions1}, \ref{table:bbfunctions12}
and \ref{table:bbfunctions2}.
Table \ref{table:IJcoefficientsBb} contains the assignments 
$A_\star$, $B_\star$
and $C_\star$ for the functions
$\tilde{J}_\gamma$.
The functions $\tilde{I}_\gamma (k_i)$ are defined by
\begin{equation}
\tilde{I}_\gamma (k_3) \equiv 
(\im \vartheta_3 k_t)^{\gamma+1}
\int_{-\infty}^0 {\d y}\, \bigg\{  {(-y)^\gamma}  
e^{\im (k_1+k_2-k_3) y}\, \int_{-\infty}^{y}{\dfrac{\d \xi}{\xi}\, e^{2\im k_3 \xi}} 
\label{eq:Itilde}
\bigg\}\ \ ,
\end{equation}
where $\vartheta_3=(k_t-2k_3)/k_t$. 
We refer the reader to Appendix \ref{app:integrals} 
for details on the evaluation of these functions.



\clearpage


\begin{sidewaystable}[htpb]

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	\begin{center}
		\small
		\begin{tabular}{QqQqQ}

			\toprule
			\textrm{operator}
			&
			\multicolumn{4}{c}{contributions to $B^a$}
			\\
			\cmidrule(l){2-5}
		
		 	& 
		 	\multicolumn{1}{c}{$N^a(k_1)$} &
		 	\multicolumn{1}{c}{$P^a(k_1)$} &
		 	\multicolumn{1}{c}{$Q^a(k_1)$} &
		 	\multicolumn{1}{c}{$T^a(k_1)$}
		 	\\
			\midrule

			\zeta'^3 &
			12H_{\star} (1+\varepsilon_\star) \prod_i k_i^2 
			k_\star^{ \frac{5\varepsilon_\star}{1\varepsilon_\star}} & 
			-\im \bigg(\frac{1}{\im k_t} \bigg)^{3+ \frac{5\varepsilon_\star}{1+\varepsilon_\star}}
			&
			\\[2mm]

			\cmidrule{2-5}

			\zeta \zeta'^2 & 
			4 k_2^2 k_3^2 \,k_\star^{ \frac{4\varepsilon_\star}{1+\varepsilon_\star}} &
			\im \bigg(\frac{1}{\im k_t} \bigg)^{1+ \frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			& 
			-k_1 \bigg(\frac{1}{\im k_t} \bigg)^{2+ \frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			 &
			\\[2mm]

			\cmidrule{2-5}
	\multirow{3}*{$\zeta ( \partial \zeta)^2$} &
			\frac{4 \big(\vec{k}_2 \cdot \vec{k}_3 \big)}{c_{s\star}^2} &
			 &
			&
			\Omega_{1\star} \tilde{k}
			\\

			&
			 &
			&
			 &
			+\Omega_{2\star}\bigg(-k_t +\frac{k_1k_2k_3}{k_t^2}
			\bigg)			\\

			&
			 &
			&
			 &
			- \Omega_{2\star}\bigg(\EulerGamma- \ln\frac{k_\star}{k_t} \bigg) \tilde{k}
			\\[2mm]

			\cmidrule{2-5}
			
			\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta' &
			2k_1^2 \, (\vec{k}_2 \cdot \vec{k}_3)\, k_\star^{\frac{4\varepsilon_\star}{1+\varepsilon_\star}} &
			2\im\, \bigg(\frac{1}{\im k_t}\bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}  &
		-(k_2+k_3) \bigg(\frac{1}{\im k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}} \, & \\
[2mm]
			
			\cmidrule{2-5}
			
			\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2 &	 
			4k_1^2 \, (\vec{k}_2 \cdot \vec{k}_3)\, k_\star^{\frac{4\varepsilon_\star}{1+\varepsilon_\star}} &
			\im\, \bigg(\frac{1}{\im k_t}\bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}} \, &
		-k_1\, \bigg(\frac{1}{\im k_t}\bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}  \,&		\\	
 			\bottomrule
	
		\end{tabular}
	\end{center}
	\caption{Coefficients of the functions appearing in the $B^a$ bispectrum.
			For simplicity of notation, we define the quantities
			$\tilde{k}$, $\Omega_1$ and $\Omega_2$ in table \ref{table:list}
			of Appendix \ref{app:list}.
	\label{table:bafunctions}}
	\end{sidewaystable}	





\begin{table}[htpb]

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	\begin{center}
		\small
		\begin{tabular}{QqQqQ}

			\toprule
			\textrm{operator}
			&
			\multicolumn{4}{c}{assignments to $\tilde{J}\gamma$ in $B^a$}
			\\
			\cmidrule(l){2-5}
		
		 	& 
		 	\multicolumn{1}{c}{$\gamma$} &
		 	\multicolumn{1}{c}{$A_\star$} &
		 	\multicolumn{1}{c}{$B_\star$} &
		 	\multicolumn{1}{c}{$C_\star$}
		 	\\
			\midrule

			\zeta'^3 &
			2+ \frac{5\varepsilon_\star}{1+\varepsilon_\star} & 
			\Omega_{3\star}&
			-\frac{h_{1\star}-5\beta_\star \varepsilon_\star}{1+\varepsilon_\star}
			+\frac{\delta_\star (2\varepsilon_\star -3)+\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2}
		 &
			-\frac{5}{2} \frac{\alpha_\star \varepsilon_\star}{1+\varepsilon_\star}
			\\[2mm]

			\cmidrule{2-5}

			\zeta \zeta'^2 & 
			\frac{4\varepsilon_\star}{1+\varepsilon_\star} &
			\Omega_{1\star} & 
			-\frac{h_{2\star}-4\beta_\star \varepsilon_\star}{1+\varepsilon_\star}
			+\frac{\delta_\star (\varepsilon_\star -3)+2\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2}
 &
						-2\frac{\alpha_\star \varepsilon_\star}{1+\varepsilon_\star}

			\\[2mm]
			\cmidrule{2-5}

		 	
			
			\zeta ( \partial \zeta)^2 &
			\multicolumn{4}{c}{not applicable}	\\[2mm]

			\cmidrule{2-5}
			
			\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta'  &
			\frac{4\varepsilon_\star}{1+\varepsilon_\star} &
			\Omega_{1\star} & 
			-\frac{h_{4\star}-4\beta_\star \varepsilon_\star}{1+\varepsilon_\star}
			+\frac{\delta_\star (\varepsilon_\star -3)+2\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2} &
						-2 \frac{\alpha_\star \varepsilon_\star}{1+\varepsilon_\star} \\
		[2mm]
			
			\cmidrule{2-5}
			
			\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2 &	 
			\frac{4\varepsilon_\star}{1+\varepsilon_\star} &
			\Omega_{1\star} & 
				-\frac{h_{5\star}-4\beta_\star \varepsilon_\star}{1+\varepsilon_\star}
			+\frac{\delta_\star (\varepsilon_\star -3)+2\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2}
			&
						-2 \frac{\alpha_\star \varepsilon_\star}{1+\varepsilon_\star} \\	
 			\bottomrule
	
		\end{tabular}
	\end{center}
	\caption{Coefficients of the functions $\tilde{J}_\gamma$ 
	appearing in the $B^a$ bispectrum, where
			$\Omega_{1\star}$ and $\Omega_{3\star}$
			are defined in table \ref{table:list} of Appendix \ref{app:list}.
			The functions $\tilde{J}_\gamma$
			are defined in Eq. \eqref{eq:Jtildeintegral}
			and discussed in detail in Appendix \ref{app:integrals}.
	\label{table:JcoefficientsBa}}
	\end{table}	






\clearpage






\clearpage


\begin{sidewaystable}[htpb]

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	\begin{center}
		\small
		\begin{tabular}{QqQqQq}

			\toprule
			\textrm{function}
			&
			\multicolumn{3}{c}{operator}
			\\
			\cmidrule(l){2-4}
		
		 	& 
		 	\multicolumn{1}{c}{$\zeta'^3$} &
		 	\multicolumn{1}{c}{$\zeta \zeta'^2$} &
		 	\multicolumn{1}{c}{$\zeta ( \partial \zeta)^2$} 
		 	\\
			\midrule

			N^b(k_1) &
			4H_{\star} (1+\varepsilon_\star) \prod_i k_i^2 
			k_\star^{ \frac{5\varepsilon_\star}{1+\varepsilon_\star}} & 
			4 k_2^2 k_3^2 \, k_\star^{ \frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			& \frac{2 (\vec{k}_2 \cdot \vec{k}_3)}{c_{s\star}^2}  
			\\[2mm]

			\cmidrule{2-4}

P^b_1(k_1) & 
			\frac{1}{2}\bigg(\frac{1}{ \vartheta_1 k_t} \bigg)^{3+\frac{5\varepsilon_\star}{1+\varepsilon_\star}} \cos\bigg[\frac{5\pi \varepsilon_\star}{2(1+\varepsilon_\star)} \bigg] &
			\frac{1}{2}
			 \bigg(\frac{1}{ \vartheta_1 k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}\cos\bigg[\frac{2\pi \varepsilon_\star}{1+\varepsilon_\star} \bigg]  & 
			-\frac{1}{2k_t} \big( k_1 k_2 +k_1 k_3- k_2 k_3\big)
			 
			\\[2mm]

			\cmidrule{2-4}
P^b_2(k_1)&
			\frac{1}{2}\bigg(\frac{1}{ \vartheta_2 k_t} \bigg)^{3+\frac{5\varepsilon_\star}{1+\varepsilon_\star}}\cos\bigg[\frac{5\pi \varepsilon_\star}{2(1+\varepsilon_\star)} \bigg]  &
		\frac{1}{2}
			\bigg(\frac{1}{ \vartheta_2 k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}} \cos\bigg[\frac{2\pi \varepsilon_\star}{1+\varepsilon_\star} \bigg] &
						-\frac{1}{2k_t} \big( k_1 k_2 +k_2 k_3- k_1 k_3\big)
		
			\\[2mm]

			\cmidrule{2-4}
			
P^b_3(k_1) &
			\frac{1}{2}\bigg(\frac{1}{ \vartheta_3 k_t} \bigg)^{3+\frac{5\varepsilon_\star}{1+\varepsilon_\star}} \cos\bigg[\frac{5\pi \varepsilon_\star}{2(1+\varepsilon_\star)} \bigg] &		
			\frac{1}{2}
			\bigg(\frac{1}{ \vartheta_3 k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			\cos\bigg[\frac{2\pi \varepsilon_\star}{1+\varepsilon_\star} \bigg]  &
									-\frac{1}{2k_t} \big( k_1 k_3 +k_2 k_3- k_1 k_2\big)
\\
[2mm]
			
			\cmidrule{2-4}
			
Q^b_1(k_1) &	 
			 & 		-\frac{k_1}{2}
			\bigg(\frac{1}{ \vartheta_1 k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			\cos\bigg[\frac{2\pi \varepsilon_\star}{1+\varepsilon_\star} \bigg] 
			 &
		-\frac{k_1k_2k_3}{k_t^2} \, \\	
[2mm]

			\cmidrule{2-4}
			
Q^b_2(k_1) &
			 &
			\frac{k_1}{2}
			\bigg(\frac{1}{ \vartheta_2 k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}} 
			\cos\bigg[\frac{2\pi \varepsilon_\star}{1+\varepsilon_\star} \bigg] 
			 & -\frac{k_1k_2k_3}{k_t^2} \\
[2mm]
			
			\cmidrule{2-4}
			
Q^b_3(k_1) &	 
		 &
			\frac{k_1}{2}
			\bigg(\frac{1}{ \vartheta_3 k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			\cos\bigg[\frac{2\pi \varepsilon_\star}{1+\varepsilon_\star} \bigg]  &
		-\frac{k_1k_2k_3}{k_t^2}  \\	
		[2mm]

			\cmidrule{2-4}	
 					\end{tabular}
	\end{center}
	\caption{\label{table:bbfunctions1} Coefficients of the functions 
	appearing in the $B^b$ bispectrum for the first three operators, 
	where  $\vartheta_i=\frac{1}{k_t} (k_t-2 k_i) $,
	and $\Xi$ and
   $f(k_1,k_2,k_3)$ are defined in table \ref{table:list} of Appendix \ref{app:list}.}
	
	\end{sidewaystable}	







\begin{table}[htpb]

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	\begin{center}
		\small
		\begin{tabular}{QqQqQq}

			\toprule
			\textrm{function}
			&
			\multicolumn{3}{c}{operator}
			\\
			\cmidrule(l){2-4}
		
		 	& 
		 	\multicolumn{1}{c}{$\zeta'^3$} &
		 	\multicolumn{1}{c}{$\zeta \zeta'^2$} &
		 	\multicolumn{1}{c}{$\zeta ( \partial \zeta)^2$} 
		 	\\
			\midrule


R^b(k_1) &
			3\im \bigg( \frac{1}{\im kt}\bigg)^{3+\frac{5\varepsilon_\star}{1+\varepsilon_\star}}
 & 
			\im \bigg(\frac{1}{\im k_t} \bigg)^{1+ \frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			
			& 
			\\[2mm]

			\cmidrule{2-4}

S^b(k_1) & 
			  &
			-k_1 \bigg(\frac{1}{\im k_t} \bigg)^{2+ \frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			& 
		
			\\[2mm]

			\cmidrule{2-4}
			
			
			
		T^b(k_1) &
			
			  & -\bigg(\frac{1}{k_t}\bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}} 
		\Xi
			 & f(k_1,k_2,k_3)
	
	
			\\
 			\bottomrule
 			
 					\end{tabular}
	\end{center}
	\caption{\label{table:bbfunctions12} Coefficients of the functions 
	appearing in the $B^b$ bispectrum for the first three operators,
	where $\Xi$ and
   $f(k_1,k_2,k_3)$ are defined in table \ref{table:list} of Appendix \ref{app:list}.}
	
	\end{table}	

\begin{table}[htpb]

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	\begin{center}
		\small
		\begin{tabular}{QqQ}

			\toprule
			\textrm{function}
			&
			\multicolumn{2}{c}{operator}
			\\
			\cmidrule(l){2-3}
		
		 	& 
	
		 	\multicolumn{1}{c}{$\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta'$}&
		 	\multicolumn{1}{c}{$\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2 $}
		 	\\
			\midrule

			N^b &
		 2k_1^2 (\vec{k}_2\cdot \vec{k}_3) k_\star^{\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			&
					 4k_1^2 (\vec{k}_2\cdot \vec{k}_3) k_\star^{\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			\\[2mm]

			\cmidrule{2-3}

P^b_1 & 
\bigg(\frac{1}{\vartheta_1 k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}\cos\bigg[ \frac{2\pi\varepsilon_\star}{1+\varepsilon_\star} \bigg] & 
\frac{1}{2} \bigg(\frac{1}{\vartheta_1 k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
\cos\bigg[ \frac{2\pi \varepsilon_\star}{1+\varepsilon_\star}\bigg]
			\\[2mm]

			\cmidrule{2-3}
P^b_2&
 \bigg(\frac{1}{\vartheta_2 k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}\cos\bigg[ \frac{2\pi\varepsilon_\star}{1+\varepsilon_\star} \bigg] &
\frac{1}{2} \bigg(\frac{1}{\vartheta_2 k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
\cos\bigg[ \frac{2\pi \varepsilon_\star}{1+\varepsilon_\star}\bigg]			
			\\[2mm]

			\cmidrule{2-3}
			
P^b_3 &
		 \bigg(\frac{1}{\vartheta_3 k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}\cos\bigg[ \frac{2\pi\varepsilon_\star}{1+\varepsilon_\star} \bigg]\, &
		 \frac{1}{2} \bigg(\frac{1}{\vartheta_3 k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
\cos\bigg[ \frac{2\pi \varepsilon_\star}{1+\varepsilon_\star}\bigg]
 \\
[2mm]
			
			\cmidrule{2-3}
			
Q^b_1 
		 &
		 \frac{k_2+k_3}{2} \bigg(\frac{1}{\vartheta_1 k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}\cos\bigg[ \frac{2\pi\varepsilon_\star}{1+\varepsilon_\star} \bigg]
			& 
\frac{k_1}{2} \bigg(\frac{1}{\vartheta_1 k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
\cos\bigg[ \frac{2\pi \varepsilon_\star}{1+\varepsilon_\star}\bigg]			
			\\	
[2mm]

			\cmidrule{2-3}
			
Q^b_2 &
			 

				\frac{k_3-k_2}{2}\bigg(\frac{1}{\vartheta_2 k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}\cos\bigg[ \frac{2\pi\varepsilon_\star}{1+\varepsilon_\star} \bigg] &
				- \frac{k_1}{2} \bigg(\frac{1}{\vartheta_2 k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
\cos\bigg[ \frac{2\pi \varepsilon_\star}{1+\varepsilon_\star}\bigg]	
				 \\
[2mm]
			
			\cmidrule{2-3}
			
Q^b_3 &	 
		 

			\frac{k_2-k_3}{2} \bigg(\frac{1}{\vartheta_3 k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}\cos\bigg[ \frac{2\pi\varepsilon_\star}{1+\varepsilon_\star} \bigg] &
			-\frac{k_1}{2}\bigg(\frac{1}{\vartheta_3 k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
\cos\bigg[ \frac{2\pi \varepsilon_\star}{1+\varepsilon_\star}\bigg]	
						 \\	
		[2mm]

			\cmidrule{2-3}
R^b &

		-2 \im \bigg(\frac{1}{\im k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			 &
			- \im\bigg(\frac{1}{\im k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			\\[2mm]

			\cmidrule{2-3}

S^b & 

			  (k_2+k_3) \bigg(\frac{1}{\im k_t} \bigg)^{2+\frac{4\varepsilon_\star }{1+\varepsilon_\star}}
			&
			k_1 \bigg(\frac{1}{\im k_t} \bigg)^{2+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			\\[2mm]

			\cmidrule{2-3}
			
			
			
			T^b &
			
			-2 \bigg(\frac{1}{ k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
			\Xi\,&
			 
	
			-\, \bigg(\frac{1}{k_t} \bigg)^{1+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
						\Xi	

			\\
 			\bottomrule
 			
 					\end{tabular}
	\end{center}
	\caption{Coefficients of the functions appearing in the $B^b$ bispectrum
	for the last two operators, 
	where $\vartheta_i=\frac{1}{k_t} (k_t-2 k_i) $, 
	and $\Xi$  
	is defined in table \ref{table:list} of Appendix \ref{app:list}.
	\label{table:bbfunctions2}}
	\end{table}	




\begin{table}[htpb]

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	\begin{center}
		\small
		\begin{tabular}{QqQqQ}

			\toprule
			\textrm{operator}
			&
			\multicolumn{4}{c}{assignments to $\tilde{J}\gamma$ in $B^b$}
			\\
			\cmidrule(l){2-5}
		
		 	& 
		 	\multicolumn{1}{c}{$\gamma$} &
		 	\multicolumn{1}{c}{$A_\star$} &
		 	\multicolumn{1}{c}{$B_\star$} &
		 	\multicolumn{1}{c}{$C_\star$}
		 	\\
			\midrule

			\zeta'^3 &
			2+ \frac{5\varepsilon_\star}{1+\varepsilon_\star} & 
			\frac{\delta_\star}{1+\varepsilon_\star}- \frac{\varepsilon_\star\eta_\star}{(1+\varepsilon_\star)^2}+\frac{ \im  \pi}{4} (n_s-1) &
	\frac{n_s-1}{2} &

			\\[2mm]

			\cmidrule{2-5}

			\zeta \zeta'^2 & 
			\frac{4\varepsilon_\star}{1+\varepsilon_\star} &
		-\frac{3\delta_\star}{1+\varepsilon_\star}+ \frac{3\varepsilon_\star\eta_\star}{(1+\varepsilon_\star)^2}-\frac{3\pi \im }{4} (n_s-1) & 
			-\frac{3}{2} (n_s-1)
	&

			\\[2mm]
			\cmidrule{2-5}

		 	
			
			\zeta ( \partial \zeta)^2 &
			0 &\multicolumn{3}{c}{not applicable}	\\[2mm]


			\cmidrule{2-5}
			
			\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta'  &
			\frac{4\varepsilon_\star}{1+\varepsilon_\star}&
		\frac{3\delta_\star}{1+\varepsilon_\star} -\frac{3\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2}+\frac{3\pi \im}{4 }(n_s-1)  &
			\frac{3}{2} (n_s-1) 
		 & 
					\\
		[2mm]
			
			\cmidrule{2-5}
			
			\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2 &	 
			\frac{4\varepsilon_\star}{1+\varepsilon_\star} &
				\frac{3\delta_\star}{1+\varepsilon_\star} -\frac{3\varepsilon_\star \eta_\star}{(1+\varepsilon_\star)^2}+ \frac{3\pi \im}{4 }(n_s-1)
			 & \frac{3}{2} (n_s-1)
 & 
					\\	
 			\bottomrule
	
		\end{tabular}
	\end{center}
	\caption{Coefficients of $\tilde{J}_\gamma$ appearing in the $B^b$ bispectrum.
	The functions $\tilde{J}_\gamma$
			are discussed in detail in Appendix \ref{app:integrals}.
	\label{table:IJcoefficientsBb}}
	\end{table}





\clearpage

%\vspace*{3cm}





\subsection{Features of the bispectrum of Horndeski theories}
\label{subsec:features}
These results extend those obtained assuming 
a slow-roll inflationary phase in the early universe.
We now comment on our results.
\vspace*{0,1cm}


\para{Enhancement of non-gaussinities}It is apparent from 
our formulae that the enhancement of the bispectrum can be 
very different from the one found in models  
using the slow-roll approximation. 
This strictly depends on the expressions for the coefficients $\Lambda_i$. 
As observed in Ref. \cite{Burrage:2010cu}, if the interaction vertices
in the action \eqref{eq:zeta-action3} 
do not contain enough powers in the speed of sound, 
then the overall dependence in $c_s$ could be stronger than 
that commonly associated with DBI models $\fNL \sim c_s^{-2}$.
Depending on $z$, there might exist models that  
reproduce such behaviour. To gauge whether this scenario would 
be permissible could involve applying the partial wave decomposition 
method to the Horndeski overall bispectrum shape, 
described in \S\ref{sec:shapes}. Five measurements 
would be required to fix each of the $\Lambda_i$ interactions, 
and a number of additional measurements to break the degeneracy in 
other parameters in $\Lambda_i$, such as $\varepsilon$ and $c_s$.
Ultimately this would allow us to place constraints on all the 
parameters of the theory. Only then would we be able to conclude 
whether there is enhancement of non-gaussianities in these models.

\vspace*{0,1cm}

\para{Logarithms}Our formulae contain logarithms
of momenta encoded, for example, in the master integral $J_\gamma$ 
(defined in Eq. \eqref{eq:Jintegral} of Appendix \ref{app:integrals}). 
There are two varieties of logarithms
as noted in \S \ref{sec:3pf}: those which depend on the reference scale, 
$\ln (k_\star/k_t)$, and those which 
depend on the perimeter momentum scale, $\ln (k_i/k_t)$.
The first type of logarithms are clearly of the same nature as the 
ones identified in the power spectrum \eqref{eq:powerspectrumr}: 
they encode the scale-dependence of the bispectrum.
One can choose the reference scale, $k_\star$, 
so as to minimise these logarithms; alternatively, one can use this degree 
of freedom to measure primordial non-gaussianities on different scales.
The last type of logarithms are responsible 
for the shape-dependence of the bispectrum.

\vspace*{0,2cm}


\para{Away from slow-roll}If the inflationary background is almost de Sitter, 
so that $\varepsilon \ll 1$,
it is easy to see that the power-law behaviour
$k_\star^{\alpha \frac{\varepsilon_\star}{1+\varepsilon_\star}} $
(seen in table \ref{table:bafunctions}), 
where $\alpha$ is some integer, can be written as a next-order
logarithmic
correction.  
This can be checked by taking the limit of 
very small $\varepsilon$ in the Taylor series expansion and comparing our results 
to \S\ref{subsec:type-bispectra}.
Away from the slow-roll regime, the dependence on the 
reference scale, $k_\star$, arises from power-laws
(whose Taylor expansion we cannot truncate)
in addition to logarithmic contributions. 
For comparison, let us write the formula of the bispectrum \textit{type-a} 
for one operator, say $(\partial \zeta/\partial y)^3$, 
which we shall call $B_a^{(a)}$. We find that:
\begin{equation}
\begin{split}
B^{(a)}_{a} = 
\dfrac{12 H_\star^5\, (1+\varepsilon_\star) ^5 \,\Lambda_{1\star} }{2^6 \, z_\star^3\, c_{s\star}^6  \,k_t^3\, \prod_i k_i}\bigg(\dfrac{k_\star}{k_t}\bigg)^{\frac{5\varepsilon_\star}{1+\varepsilon_\star}}\, \Gamma(\xi ) &
\bigg\{ 
\cos(\varsigma) 
 \bigg[
A_\star +  \ln\frac{k_\star}{k_t}\, 
\bigg(B_\star + C_\star\ln \frac{k_\star}{k_t} \bigg)+ C_\star \psi^{(1)} (\xi) \\
		&  \ \  \ \ \ \ \ \ \ \ \ \ \  \ \,  
		+\psi^{(0)} (\xi) \bigg(
		B_\star +2C_\star \ln\frac{k_\star}{k_t}
		+C_\star \psi^{(0)} (\xi)
		\bigg) \bigg]\\
&-
\frac{\pi}{2} \, \sin(\varsigma) 
 \bigg[
B_\star + C_\star\ln \frac{k_\star}{k_t} 
+ \ln\frac{k_\star}{k_t}\, 
+2C_\star\psi^{(0)} (\xi) \bigg] \ \bigg\}\ \ \ ,
\end{split}
\label{eq:op1}
\end{equation}
with $\xi\equiv 3+\frac{5\varepsilon_\star}{1+\varepsilon_\star}$ and
$\varsigma \equiv \frac{5\pi \varepsilon_\star}{2(1+\varepsilon_\star)}$.
This expression shows an unusual power-law dependence on the reference
scale, $k_\star$, which is absent from previous studies, 
where only the logarithmic contributions $\ln(k_\star/k_t)$
were known \cite{Burrage:2011hd}. 
By keeping the reference scale $k_\star$ arbitrary in our 
calculation, the scale-dependence of the bispectrum can be calculated. 
This will include the contribution of the power-law scaling as
$k_t^{-3-\frac{5\varepsilon_\star}{1+\varepsilon_\star}}$, 
which could receive large corrections from $\varepsilon_\star$.
In Ref. \cite{Khoury:2008wj} Khoury \& Piazza chose $k_\star=k_t$, 
which masks the power-law effect.

Considering a slow-roll expansion, by which 
we take $\varepsilon_\star$ to be a slow-roll 
parameter [treating it on equal footing as $\delta$ and $(n_s-1)$], 
Eq. \eqref{eq:op1} simplifies to
\begin{equation}
\begin{split}
B^{(a)}_{a} \simeq \dfrac{3\Lambda_{1\star}H^5_\star}{8 z_{\star}^3 c_{s\star}^6 \prod_i k_i k_t^3} \bigg\{ & 1+\frac{h_{1\star}}{2} (-3+2\EulerGamma) +\frac{3 (n_s-1)}{2} (-2+\EulerGamma)
+\frac{\delta_\star}{2} (-13+6\EulerGamma) +\frac{\varepsilon_\star}{2} (25-10\EulerGamma)\\
&+\frac{3(n_s-1)}{2} \ln \bigg(\frac{2k_1k_2k_3}{k_\star^3} \bigg)
- (h_{1\star}+3\delta_\star-5\varepsilon_\star) \ln \frac{k_\star}{k_t}
 \bigg\}\ \ ,
 \label{eq:srop1}
 \end{split}
\end{equation}
which resembles the bispectrum obtained in 
\S\ref{subsec:type-bispectra}.\footnote{To be more precise, 
			we can indeed show that our results 
			for the overall bispectrum agree (adding \textit{type a} and \textit{type b}
			bispectrum), 
			including the explicit dependence on the reference scale, $k_\star$.} 
We note that in Eq. \eqref{eq:srop1} the dependence on $k_\star$ appears 
through logarithms, and the power-law behaviour has 
explicitly disappeared from the result. As advertised, by taking
$\varepsilon$ to be a small parameter, the power-law is 
well described, at next-order in the slow-roll approximation, 
by a logarithmic contribution.
The reference scale, $k_\star$, appears
in the form of two logarithmic functions: $\ln (k_i/k_\star)$
and $\ln (k_\star/k_t)$. These species of logarithms 
were thoroughly studied in \S\ref{subsec:type-bispectra}, 
to which we refer the reader for details.
It is in this sense that our work generalises the calculations which
have been performed assuming the slow-roll approximation.

The behaviour described above shows that 
whereas the power spectrum has a universal weak logarithmic scale-dependence 
[cf. Eq. \eqref{eq:powerspectrumr}], 
the bispectrum of these theories beyond the slow-roll regime can have a
 much stronger scale-dependence. 
In principle, this could be used as a diagnostic
tool from 
CMB ($k \lesssim 0.5 h \mathrm{Mpc}^{-1}$) to cluster scales 
($k \gtrsim 0.5 h \mathrm{Mpc}^{-1}$), 
interpolating with scales probed by the galaxy bispectrum.


A number of authors have studied 
constraints on non-gaussianity arising from 
galaxy surveys \cite{Matarrese:2000iz, Bernardeau:2001qr}, 
including its relation with biasing \cite{Verde:1999ij}. 
The scale-dependence of the bispectrum was initially studied 
by Chen in an infrared model of DBI inflation \cite{Chen:2005fe}, 
and later investigated in $P(X,\phi)$ models 
(a subset of the Horndeski class) by LoVerde \etal\,\cite{LoVerde:2007ri}.
It is not the aim of this chapter to present a detailed analysis 
of the scale-dependence of the bispectrum. We rather want to offer an explicit
example of theories which inherit 
a strong scale-dependence from the background dynamics.









\subsection*{Comparison with previous results}


\para{Khoury \& Piazza}Khoury \& Piazza  \cite{Khoury:2008wj} 
calculated the bispectrum of $P(X,\phi)$ theories in an exactly scale-invariant 
background, in which $s_\star=-2\varepsilon_\star$. 
In this chapter we have extended this study in two ways:
by performing 
the calculation perturbatively away from exact scale-invariance, 
as supported by observations,
and applying it to the Horndeski class of models. 


In particular, let
us take a specific example for comparison. 
Focusing on the operator $\zeta (\partial \zeta/\partial y)^2$
and in the action studied by Khoury \& Piazza, we take 
\[ \Lambda_2 (y)= \frac{\varepsilon}{c_s^4} \big(\varepsilon -3 +3c_s^2 \big) \ \ .\]
We note that $\Lambda_2(y)$ is rapidly varying in time and 
should therefore be placed inside the integral to compute the bispectrum, 
which we denote by $B_b$:
\begin{equation}
B_{b} ^{\textrm{(leading)}}\sim \int_{-\infty}^{0} {\d y } \Lambda_2(y)\,  c_s(y)\, a^2(y)  y^2 (1-\im ky)\ \ ,
\end{equation}
where the factor $y^2$ comes from the two time-derivatives of 
the wavefunctions and the last one (between brackets) from the undifferentiated wavefunction. 
For comparison purposes, we only retain the contributions 
at leading-order in scale-invariance, which means setting all the 
next-order corrections we have carefully kept track in this chapter to zero.

Therefore, selecting only the leading-order contribution
in Eq. \eqref{eq:Ba-chapter4}, 
we find 
\begin{equation}
\begin{split}
B^{(\textrm{leading})}_{b} = 
\dfrac{H_\star^4\, (1+\varepsilon_\star) ^4 \, k_2^2 k_3^2}{16 \, c_{s\star}^4 \, \varepsilon_\star^2 \, \prod_i k_i^3 \, k_t^2} &
\bigg\{ 
3c_{s\star}^2  (k_1+k_t) +\\
&+(\varepsilon_\star -3)
\bigg(\frac{k_t}{k_\star}\bigg)^{\frac{4\varepsilon_\star}{1+\varepsilon_\star}} 
\Gamma\bigg(1-\frac{4\varepsilon_\star}{1+\varepsilon_\star}\bigg) 
\cos\bigg(\frac{2 \pi \varepsilon_\star}{1+\varepsilon_\star} \bigg) 
\big(k_1+k_t +\varepsilon_\star (k_t-3k_1) \big)
\bigg\}\\
&  +\textrm{cyclic permutations}\ \ \ ,
\label{eq:BKP2}
\end{split}
\end{equation}
where we have retained the scale-dependence through $k_\star$. 
This formula reproduces the results of Ref. \cite{Khoury:2008wj}
provided we choose the reference scale to satisfy $k_\star=k_t$.
Eq. \eqref{eq:BKP2} is the bispectrum of the operator $\zeta (\partial \zeta/\partial y)^2$
for a perfectly scale-invariant spectrum of perturbations.

Whenever comparison was possible 
our results reproduce those of Ref. \cite{Khoury:2008wj}. 


\newpage

\para{Noller \& Magueijo}Second, in Ref. \cite{Noller:2011hd} 
Noller \& Magueijo estimated 
the magnitude of the next-order corrections to the bispectrum
in the scale-invariant approximation of
$P(X,\phi)$ models. In comparison, our calculation 
extends to the larger Horndeski scalar field theories.
Their estimate focused on
a subset of next-order corrections important when $|ky|\rightarrow 0$. 

However, as we pointed out in \S\ref{subsec:power-law},
there are other contributions which 
contribute equally to the bispectrum and are 
sensitive to the dynamics around horizon crossing, 
when the approximation $|ky|\rightarrow 0$ fails. 
As we have shown, these corrections can be obtained by evaluating 
the change in 
the Hankel function of order 
$\nu=3/2-(n_s-1)/2$,
rather than at the exact scale-invariant choice, $\nu=3/2$.
If these contributions are not taken into account then
the details of the interference between growing and 
decaying modes around horizon-crossing are lost.
As we have argued in the previous chapters, these details
are very important for our results to obey Maldacena's consistency condition.

Moreover, in our calculation we have performed a uniform expansion to 
next-order corrections in the scale-invariant
approximation. In particular we used Eq. \eqref{eq:scale_factor}
for the scale factor, $a$, and Eq. \eqref{eq:cs} for $c_s$. Ref. \cite{Noller:2011hd} 
on the other hand assumed a perfectly scale-invariant background, 
on top of which perturbations would develop.
This amounts to setting $\alpha_\star=\beta_\star=0$
in our Eq. \eqref{eq:scale_factor}, 
even though their contribution is as important as terms 
linear in $(n_s-1)$---as we have previously argued,
the scalar fluctuations are sensitive
to the background dynamics, and in particular 
to the next-order corrections we have calculated in the
scale-invariant approximation.

For completeness, we will investigate
 one particular limit 
 in $P(X,\phi)$ theories (these include DBI inflation) 
 studied in Ref. \cite{Noller:2011hd},
when the speed of sound of fluctuations is small, $c_s\ll 1$. This regime
is phenomenologically interesting since it is known to be
related with large non-gaussianities \cite{Alishahiha:2004eh}, 
for which the dominant operator is $(\partial \zeta/\partial y)^3$.
To make this application more explicit we apply the notation of 
\S\ref{subsec:bispectrumh}, and also Refs. \cite{Burrage:2011hd, Chen:2006nt}), 
and take the action
\begin{equation}
S^{(3)} \supseteq \int \d ^3 x \, \d y \ 
a\Lambda_1 c_s^2 \bigg( \dfrac{\partial \zeta}{\partial y} \bigg)^3\ \ ,
\label{eq:BNM}
\end{equation}
with 
\begin{equation*}
\Lambda_1= \frac{\varepsilon}{H c_s^4} \bigg(
1-c_s^2 -2c_s^2 \frac{\lambda}{\Sigma}
\bigg)
\end{equation*}
where
\begin{equation*}
\dfrac{\lambda}{\Sigma} \equiv \dfrac{1}{6}\bigg(
\dfrac{2f_X+1}{c_s^2}-1 \bigg) \ \ .
\end{equation*}

We assume $f_X$ is constant.
In DBI models, $f_X=1-c_s^2$ 
										and therefore one sees that we cannot
										require $f_X$ to be constant given that we 
										are interested precisely in the regime when 
										$c_s$ is rapidly varying.
										However, for the purposes of making this comparison
										more transparent, we assume this is the case, 
										similarly to what was done in Refs. 
										\cite{Khoury:2008wj, Noller:2011hd, Burrage:2011hd}, 
										and implemented in \S\ref{subsec:power-law}.
										Technically, a more precise estimate would have to 
										take the time-dependence of $f_X$ into account.
										
We can see that taking the limit of small $c_s$, 
corresponds to considering
$\big|\frac{\lambda}{\Sigma} \big| \gg 1$, 
in which case the interaction vertex is well
approximated by
\begin{equation*}
\Lambda_1 (y) \simeq -\dfrac{2}{3} \dfrac{\varepsilon f_X}{H c_s^4}\ \ .
\end{equation*}
Inspection of this formula reveals that this interaction 
vertex is rapidly varying, by virtue of its time-dependence in $\varepsilon$, 
$H$ and $c_s$, of which only $\varepsilon$ is slowly varying. 

Our formulae are easily adapted to the case of rapidly varying $\Lambda_i$.
For $\Lambda_1$ we find
\begin{equation}
\begin{split}
\Lambda_1 (y) =\Lambda_{1\star} (-k_\star y)^{-\frac{9\varepsilon_\star}{1+\varepsilon_\star}}
 \bigg\{ &
 1-\frac{1}{1+\varepsilon_\star}\bigg[\eta_\star +9 \varepsilon_\star \beta_\star +\frac{\varepsilon_\star \delta_\star}{1+\varepsilon_\star} +\frac{4\varepsilon_\star \delta_\star (\varepsilon_\star -1)}{1+\varepsilon_\star} \bigg] \ln (-k_\star y) \\
 & +\frac{9}{2} \frac{\alpha_\star \varepsilon_\star}{1+\varepsilon_\star} \big(\ln (-k_\star y) \big)^2
 \bigg\}\ \ ,
 \end{split}
 \label{eq:general_Lambda}
\end{equation}
up to next-order corrections in scale-invariance.
These corrections can be absorbed into the coefficients 
$A_\star$, $B_\star$ and $C_\star$ in table \ref{table:JcoefficientsBa}. 
This generalises Eq. \eqref{eq:vertex corrections} to
rapidly varying interaction vertices. Since 
\eqref{eq:general_Lambda} adds power-law contributions to the 
integral in Eq. \eqref{eq:BNM}, 
one might worry that not all the previously allowed values of $\varepsilon$
will make the final result converge---we recall that the overall power-law
needs to decay faster than $(-y)^{-1}$
for convergence criteria to be met. 
In the event this does not happen then one is required to 
perform integration by parts an appropriate number of times
to isolate the primitively divergent contributions, in a 
completely analogous way as we have dealt with the operator $\zeta (\partial \zeta)^2$
in \S\ref{subsec:type-bispectra}. 
A convergent answer should similarly place 
constraints on the allowed values of $\varepsilon$ so that 
the correlators do not evolve in time, since this could signal 
a spurious divergence.

Nevertheless, for this operator the integral \eqref{eq:Jintegral}
is evaluated for $\gamma=2-4\varepsilon_\star/(1+\varepsilon_\star)$ and is therefore
 always convergent,
since the condition $\Re \big(\varepsilon_\star/(1+\varepsilon_\star) \big)<3/4$
is satisfied for all the range of $0<\varepsilon_\star<1$.
The calculation is carried out as described in 
\S\ref{subsec:bispectrumh}.
Using the definition of $\fNL$ \eqref{eq:deffnl},
we find that at leading-order in scale-invariance
\begin{equation}
\fNL^{\textrm{(leading,\  equilateral)}} = \dfrac{5 f_X}{c_{s\star}^2} \dfrac{\prod_i k_i^2}{\sum_i k_i^3}
\bigg(\frac{k_\star}{k_t} \bigg)^{\frac{3-\varepsilon_\star}{1+\varepsilon_\star}}
k_\star^{-3} (1+\varepsilon_\star)\, \Gamma (\Upsilon )\, \cos \bigg(\dfrac{\pi (1-\varepsilon_\star)}{1+\varepsilon_\star} \bigg) \ \ ,
\label{eq:nmleading}
\end{equation}
 where $\Upsilon=\frac{3-\varepsilon_\star}{1+\varepsilon_\star}$ is 
 a non-negative constant.
$\fNL$ can change sign if $\varepsilon_\star >1/3$, when the argument 
of the trigonometric function changes from the first 
to the second quadrant.
This would be important since WMAP constraints predict 
predominantly positive values for $\fNL^{\textrm{(equilateral)}}$, 
whereas the original DBI model, under the slow-roll approximation, 
gives negative $\fNL^{\textrm{(equilateral)}}$.

Including the next-order corrections, the result becomes substantially more
complicated and in an attempt to 
simplify it as much as possible, we 
evaluate $\fNL$ in the equilateral limit
and when $k_\star=k$.
We organise the correction to the leading-order
non-gaussianity, $\delta \fNL$, in terms 
proportional to the various slow-variation parameters, as follows:
\begin{equation}
\delta \fNL^{\textrm{(equilateral)}} = (n_s-1) \fNL^{n_s-1} +
\delta \, \fNL^{\delta} +
\eta  \fNL^{\eta}\ \ ,
\label{eq:deltafNL1}
\end{equation}
with
	\begin{subequations}
		\begin{align}
			\fNL^{n_s-1}
			& =  \dfrac{5 f_X k^{2+\frac{4}{1+\varepsilon_\star}}}{2 c_{s\star}^2 (1+\varepsilon_\star)^2} \, 
			\bigg\{
			3^{-\frac{3-\varepsilon_\star}{1+\varepsilon_\star}} \cos \bigg(\frac{2\pi}{1+\varepsilon_\star}\bigg) k^{-\frac{2(3+\varepsilon_\star)}{1+\varepsilon_\star}}
			(1+\varepsilon_\star)^3\, \Gamma(\Upsilon)\ \mathcal{H} _{\varpi} \nonumber
			\\
			& \hspace*{2,8cm}- (1+\varepsilon_\star)^3\, 3^{\frac{4\varepsilon_\star}{1+\varepsilon_\star}}\,
k^{-\frac{2(3+\varepsilon_\star)}{1+\varepsilon_\star}}	 \Gamma(\Upsilon)
\cos \bigg(\frac{2\pi}{1+\varepsilon_\star} \bigg)  \bigg(2+2\EulerGamma +\ln \frac{27}{2} \bigg) \nonumber		\\
& \hspace*{2,8cm}
		-(1+\varepsilon_\star)^3 k^{-6+\frac{4\varepsilon_\star}{1+\varepsilon_\star}}
		\sin \bigg(\frac{2\pi \varepsilon_\star}{1+\varepsilon_\star } \bigg)
	\mathcal{J} \bigg\}\ \ ,
			\\ \nonumber	\\
\fNL^{\delta}
	&=	-\dfrac{5 \times 3^{-\frac{4}{1+\varepsilon_\star}}}{2 c_{s\star}^2 (1+\varepsilon_\star)}
	\, f_X \Gamma (\Upsilon)	
	\bigg\{
	\cos \bigg( \frac{\pi}{2}\Upsilon\bigg) \pi \big(3+\varepsilon_\star (-5+4\varepsilon_\star)\big) \nonumber\\
	&\hspace*{4cm} 
	+\sin \bigg(\frac{\pi}{2}\Upsilon \bigg) \bigg[
	2\Big[1+\varepsilon_\star +\ln3 \Big(-3+\varepsilon_\star (5-4\varepsilon_\star)\Big) \Big]
	\nonumber \\
	& \hspace*{6.3cm}
	+2 (3+\varepsilon_\star (-5+4\varepsilon_\star)) \psi^{(0)} (\Upsilon)
	\bigg]
	\bigg\}  \ \ , \ \ \textrm{and} \\ \nonumber \\
	\fNL^{\eta}
	& = \dfrac{5\times 3^{-\frac{4\varepsilon_\star}{1+\varepsilon_\star}}k^{2+\frac{4}{1+\varepsilon_\star}}}{2\,c_{s\star}^2 (1+\varepsilon_\star)^2} \, f_X  \Gamma(\Upsilon) 
	\bigg\{
	\cos \bigg(\frac{\pi \varpi}{2}\bigg)  k^{-\frac{2(3+\varepsilon_\star)}{1+\varepsilon_\star}}
	 \bigg[-2\varepsilon_\star (1+\varepsilon_\star)
	+\ln 3 \big(2+2\varepsilon_\star (1+2\ln 3)\big) 
	\nonumber\\
	& \hspace*{6cm} -\big(2(1+\varepsilon_\star)+ 8 \varepsilon_\star \ln 3
	 -4\varepsilon_\star \psi^{(0)} (\Upsilon) \big)\psi^{(0)} (\Upsilon)
	 +4\varepsilon_\star \psi^{(1)} (\Upsilon)\bigg] \nonumber\\
& \hspace*{4.5cm} -8\, \cos \bigg(\frac{\pi \varpi}{2}\bigg)\, k^{-3-\frac{3-\varepsilon_\star}{1+\varepsilon_\star}}	
\varepsilon_\star (1+\varepsilon_\star ) 
	\nonumber  \\
	& \hspace*{4.5cm}
	+\frac{1}{2}\sin  \bigg(\frac{\pi \varpi}{2}\bigg) k^{-\frac{2(3+\varepsilon_\star)}{1+\varepsilon_\star}}\bigg[
	\pi +4\varepsilon_\star \pi -8\varepsilon_\star \pi \psi^{(0)} (\Upsilon)
	\bigg]
	\bigg\}\  .
		\end{align}
		\label{eq:deltafNL2}
	\end{subequations}
\noindent where $\varpi\equiv  2 (1-\varepsilon_\star)/(1+\varepsilon_\star)$. 
We note the dependence on the power-law in $k$, 
expected whenever the slow-roll approximation 
breaks down.
The polygamma functions of order zero, $\psi^{(0)}$, 
were introduced in Eq. \eqref{eq:integfunctionint3}
in Appendix \ref{app:integrals}. 
$\mathcal{H}_m$
denotes the $m^{\textrm{th}}$-harmonic number which relates to 
$\psi^{(0)}$ via $\mathcal{H}_{m-1}=\psi^{(0)} (m)+\EulerGamma$,
and $\mathcal{J}$ satisfies
\begin{equation}
\mathcal{J}=
\Gamma(\Upsilon)  \bigg[\EulerGamma +\ln 2+\psi^{(0)}(\Upsilon) \bigg]
\nonumber
-2 \Gamma \bigg(\frac{4}{1+\varepsilon_\star}\bigg) \ \ 
_3 F_2\bigg( \bigg\{1,1,\frac{4}{1+\varepsilon_\star}\bigg\}, \{2,2\}, -2 \bigg)\ \ ,
\end{equation}
using the results from Appendix \ref{app:integrals}. 
Eq. 
\eqref{eq:deltafNL1}
contains all the 
next-order contributions in the scale-invariant approximation.
Eqs. \eqref{eq:nmleading} and \eqref{eq:deltafNL1} are to be 
compared to Eq. (3.15) of Ref. \cite{Noller:2011hd}.


As argued in chapter \ref{chapter:three},
there is no reason to believe these corrections will be negligible, 
but their magnitude will depend on the values of the parameters $\varepsilon$, 
$\eta$, $\delta$, and $(n_s-1)$. We do not attempt to produce an order
of magnitude of these corrections here.
We also notice that the dependence on the scale $k$ vanishes in the 
slow-roll limit, when $\varepsilon_\star$ becomes a perturbative 
parameter, $\varepsilon \ll 1$. This observation is in line with our previous comments on the 
strong scale-dependence whenever there was an appreciable deviation 
from the slow-roll regime, and the scale-invariant approach became valid.

With this example, it becomes clear that the scale-invariant approximation
allows resummation of all powers of $\varepsilon$ and $s$ in the 
slow-roll approximation, provided the spectrum of perturbations is
nearly scale-invariant.

\vspace*{0,3cm}


\para{Burrage \etal}Finally, as previously discussed, our results extend what was obtained by 
  Burrage et al. \cite{Burrage:2011hd} (on which
  our chapters \ref{chapter:two} and \ref{chapter:three} are based),
  and also Chen \etal \ \cite{Chen:2006nt}
who treated the variation of
the speed of sound of scalar fluctuations, $s$, and the expansion rate, $\varepsilon$, 
as slowly varying in the $P(X,\phi)$ class of models. 
Taking the limit of small $\varepsilon$ and restoring $s$
in our formulae 
by setting $\delta=s+2\varepsilon$, 
we find perfect agreement between our results to next-order
in slow-roll,
including the 
logarithmic corrections previously discussed.
As emphasised before, these corrections are important
to correctly evaluate the scale-dependence
of the bispectrum.
Moreover, their motivation
is driven by data and they could contribute to our estimates 
of non-gaussianities with a precision level comparable 
to the sensitivity of \textit{Planck}'s data.
As a consequence, our results obey Maldacena's factorisation 
theorem \cite{Maldacena:2002vr, Creminelli:2004yq} in the limit
when slow-roll is a good approximation, 
which represents a non trivial consistency check 
of our calculation.
The results presented in \S\S\ref{sec:running}--\ref{sec:shapes} 
regarding the scale and shape-dependences 
of the bispectrum apply to our analysis if the 
slow-roll approximation is valid. Whenever there is significant 
breaking of the slow-roll approximation, 
we expect different results.







\section{Summary of results}
\label{sec:conclusionsh}


Whereas most studies of the bispectrum assume slow-roll
conditions, cosmological constraints still allow for a deviation from
this regime, whilst being compatible with
inflation \cite{Khoury:2008wj}. In this chapter we studied
the phenomenology of inflationary 
backgrounds where 
$\varepsilon, |s|<1$, but are treated \textit{non}-perturbatively. 
They are nevertheless combined 
to produce an almost scale-invariant spectrum 
of scalar perturbations. Under these assumptions, we have calculated 
the bispectrum for single-field Horndeski models \textit{perturbatively}
in $(n_s-1)$, but to \textit{all orders} in $\varepsilon$ and $s$.
We have found that the scale-dependence 
of the bispectrum is encapsulated not only in a logarithmic 
[cf. \S\ref{sec:3pf}], 
but in a stronger, power-law form. 
The power-law behaviour is more relevant if the breaking from
slow-roll is stronger, and the slow-roll approximation fails.


In an optimistic scenario, 
such behaviour can be used to constrain
the parameters of a given theory more
tightly, and potentially 
eliminate it from the list of sensible models against observations. 
It is quite likely that with \textit{Planck} 
the amount of information one is able to 
extract from the CMBR about the early universe will 
come to an end. It is therefore 
important to be able to retain the scale-dependence of the bispectrum
in our theoretical computations and estimations, 
so as to use results from the complementary smaller scales 
(LSS) \cite{Sefusatti:2007ih, Afshordi:2008ru, Verde:2010wp, Desjacques:2010jw}.

We have obtained the general expression 
for the bispectrum in Horndeski theories
for both constant and rapidly varying interaction coefficients, $\Lambda_i$.  
This work should be regarded as a first step towards 
estimating observables on a background that 
does not obey the slow-roll regime. 
Because these theories have a strong scale-dependence,
they are more vulnerable to data constraints arising 
from different scales. 






We leave the study of decomposing bispectrum shapes
into fundamental harmonics (basis shapes)
for future work. This 
partial-wave decomposition is very important
in distinguishing between models as discussed in Ref. \cite{Ribeiro:2011ax}
and throughout chapter \ref{chapter:four}. 
Also, it will be interesting to derive the consistency relations between the 
amplitudes of each harmonic. This could enable us to project out
models whose dynamics is beyond slow-roll, if those relations were not supported by data. 
If single field models are excluded by observations, we 
will have to embark on a multi-field
inflation exploration, where the interplay between curvature and 
isocurvature modes can be quite intricate
(see, for example, Refs. \cite{Byrnes:2010ft, Byrnes:2010xd, Seery:2012vj}) .

%
%
%\vspace*{15cm}
%
%\clearpage
%
%\newpage
%\thispagestyle{empty}
%\newpage 
%
%\clearpage 
%
%\newpage






==> four.tex <==
\begin{savequote}[30pc]
Mystery creates wonder and wonder is the basis of man's desire to understand. 
\qauthor{Albert Einstein}
\end{savequote}




\chapter{Decoding the Bispectrum of Single-Field Inflation}
\label{chapter:four}

This chapter reports a thorough investigation of the
properties of the bispectrum in single-field inflation, based on the results obtained in chapter
\ref{chapter:three}.
The main object of study will be the scale
and the shape-dependences of the bispectrum.
They offer very insightful information about the microphysics
of the early universe, and together with the amplitude $\fNL$,
they fully characterise the bispectrum as an intricate `three-dimensional'
object.
This chapter is therefore complementary to
chapter \ref{chapter:three}.




	\para{Outline}We obtain in \S\ref{sec:running} a generic formula 
	for the overall running of $\fNL$ with
	scale in single-field inflation theories. This is particularly important if we want to use 
	data collected at different scales---the ability to 
	use different sets of data makes the constraints 
	on the parameters of the theory tighter \cite{Cortes:2007ak}.
	
	In \S\ref{sec:shapes} we catalogue the Horndeski shapes appearing
	at leading and next-order in the slow-roll approximation.
We identify what appears to be 
	a `new' bispectrum shape uncorrelated with the 
	common templates used in CMB analysis. This shape can 
	show up both at leading and at next-order in the slow-roll approximation, 
	and it had appeared before in a galileon model 
	constructed by Creminelli \etal \ \cite{Creminelli:2010qf}.
	To explain the recurrent emergence of this shape
	we decompose in \S\ref{sec:modal-decomposition}  
	the 
	primordial bispectrum into fundamental harmonics. We elaborate on the consistency relations
	obtained between the amplitudes of each fundamental eigenmode, 
	and discuss their usefulness.
	We present in \S\ref{sec:summary4} a summary
	of our findings.
	
	This chapter contains material 
	discussed in Ref. \cite{Burrage:2011hd} in collaboration with Clare
	Burrage \& David Seery, and Ref. \cite{Ribeiro:2011ax} in 
collaboration with David Seery.
	

\section{Scale-dependence}
	\label{sec:running}

	As we discussed in \S\ref{sec:3pf}, we can use 
	the logarithms $\ln (k_i / k_\star)$
	and $\ln (k_t / k_\star)$ to study the scale-dependence
	of the three-point function.
	In the squeezed limit this is determined
	by Maldacena's consistency condition \eqref{eq:maldacena-condition}.
	The only scale which survives the factorisation procedure 
	is the common hard momentum
	$\khard$, and the variation of $\fNL$ with this scale is dictated by
	the variation of $(n_s - 1)$. This is typically called the
	\emph{running with scale} of the scalar spectral index \cite{Kosowsky:1995aa}.
	It follows that the running of Eq. \eqref{eq:maldacena-condition} 
	leads to a further consistency relation inherited from
	Maldacena's.\footnote{In general, a hierarchy of such
										consistency equations can be 
										generated by taking an arbitrary number
										of derivatives of both sides 
										of Eq. \eqref{eq:maldacena-condition}---this has been investigated in Ref. \cite{Cortes:2006ap}.
										However, so far only the first of such derivatives 
										has been the subject of investigation.}
	In the case of single-field canonical inflation,
	studied in \S\ref{sec:vanilla}, we were able to verify this
	explicitly.
	
	Away from the squeezed limit, deformations of
	the momentum triangle may change either its shape or scale.
	Scale dependence appears in all models, for the 
	same reason that the spectrum $\Ps$ and spectral index
	$n_s$ depend on scale
	\cite{Lyth:2005fi,Maldacena:2002vr,Seery:2005wm,Seery:2005gb,Chen:2006nt}.
	
	As the spectral index measures the running of the power spectrum
	with scale, one can similarly apply the same technique to the 
	bispectrum.
	Chen \cite{Chen:2005fe} introduced a tilt of $\fNL$, 
	denoted by $\nfNL$ and
	defined by%
		\footnote{Chen implicitly worked in the equilateral limit
		$k_i  = k$,
		for which $k_t = 3k$
		and $\d \ln k_t = \d \ln k$.
		We are defining $\nfNL$ to be the variation of
		$\fNL$ with the perimeter of an arbitrary triangular configuration
		with fixed shape.}
	\begin{equation}
		\nfNL \equiv \frac{\d \fNL}{\d \ln k_t} \ \  .
	\end{equation}
	For a fixed triangular shape, this measures changes in $\fNL$
	as the perimeter varies.
	Scale-dependence of this type
	was subsequently studied by several authors
	\cite{LoVerde:2007ri,Leblond:2008gg}.
	Observational constraints have been determined
	by Sefusatti {\etal} \cite{Sefusatti:2009xu}.
	Byrnes {\etal}
	performed a similar analysis in
	multiple-field models producing a local bispectrum
	\cite{Byrnes:2009pe,Byrnes:2010ft}.
	They
	allowed for deformations of the momentum triangle
	including a change of shape, but found
	these to be less important than rescalings of $k_t$.
	
	As we shall see in the next section, 
	shape-dependence is often substantially more
	complicated than
	scale-dependence.
	By construction, Eq.~\eqref{eq:deffnl} makes $\fNL$ dimensionless, but
	contains both powers and logarithms of the momenta $k_i$.
	The powers occur as dimensionless ratios in which $k_t$
	does not appear, but the shape-dependence remains.
	The argument of each logarithmic term is also a dimensionless ratio,
	but an extra scale becomes available:
	the reference scale $k_\star$. 
	When present, this gives rise to the scaling
	logarithms $\ln (k_i / k_\star)$ and $\ln (k_t / k_\star)$, 
	which depend on $k_t$ as well as the shape.
	In particular we observe that any $\ln k_t$ appears in 
	the form  $\ln (k_t/k_\star)$; said differently, 
	all the dependence of the triangle with scale is rescaled with 
	respect to the pivot scale, $k_\star$.
	
	It follows that a simple way to track the $k_t$-dependence of
	$\fNL$ is through the $k_\star$-logarithms:
	\begin{equation}
		\nfNL = - \frac{\d \fNL}{\d \ln k_\star}\ \  .
	\end{equation}

	For an arbitrary Horndeski model, $\nfNL$ can be written
	\begin{equation}
		\begin{split}
		\nfNL \rightarrow
		\frac{5}{24 z_\star}
		\bigg\{
			&
			g_{1\star} H_\star
			\big( h_{1\star} -\varepsilon_\star - v_\star   \big) \, f_1(k_i)
			+ g_{2\star}
			\big( h_{2\star}-v_\star \big) \, f_2(k_i)
			\\ & \mbox{}
			+ \frac{ g_{3\star}} {\csstar^2}
			\big( h_{3\star}- v_\star - 2 s_\star  \big) \, f_3(k_i)
			+ \frac{ g_{4\star}}{ \csstar^2}
			\big( h_{4\star} - v_\star \big) \, f_4(k_i)
			\\ & \mbox{}
			+ \frac{ g_{5\star}}{ \csstar^2}
			\big( h_{5\star} - v_\star \big) \, f_5(k_i)
		\bigg\}\ \ ,
		\end{split}
		\label{eq:runningfNLtable}
	\end{equation}
	where the functions $f_m(k_i)$ correspond to 
	dimensionless ratios of polynomials of $k_i$ 
	and are listed in Table \ref{table:nfNL}.

	\begin{sidewaystable}

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{3}
	\begin{center}
		\small
		\begin{tabular}{SS}

			\toprule
			f_1(k_i) &
			\frac{24k_1^2k_2^2k_3^3}{k_t^3(k_1^3+k_2^3+k_3^3)}
			\\[2mm]

			\rowcolor[gray]{0.9}
			f_2(k_i) &
			\frac{4[k_1^2k_2^2(k_1+k_2)+2k_1^2k_2^2k_3+(k_1+k_2)(k_1^2+k_1k_2+k_2^2)k_3^2+(k_1^2+k_2^2)k_3^3]}{k_t^2(k_1^3+k_2^3+k_3^3)}
	 		\\[2mm]

			f_3(k_i) &
			\frac{2(k_1^2+k_2^2+k_3^2)[k_1^3+2k_1^2(k-2+k_3)+2k_1(k_2^2+k_2k_3+k_3^2)+(k-2+k_3)(k_2^2+k_2k_3+k_3^2)]}{k_t^2(k_1^3+k_2^3+k_3^3)}
			\\[2mm]

			\rowcolor[gray]{0.9} f_4(k_i) &
			\frac{2k_1^5+3k_1^4(k_2+k_3)+(k_2-k_3)^2(k_2+k_3)(2k_2+k_3)(k_2+2k_3)+3k_1(k_2^2-k_3^2)^2-5k_1^3(k_2^2+k_3^2)-k_1^2(k_2+k_3)(5k_2^2+k_2k_3+5k_3^2)}{k_t^2(k_1^3+k_2^3+k_3^3)}
			\\[2mm]

			f_5(k_i) &
			\frac{2k_1^5+k_1^4(k_2+k_3)+k_1(k_2^2-k_3^2)^2-3k_1^3(k_2^2+k_3^2)+(k_2-k_3)^2(k_2+k_3)(2k_2^2+3k_2k_3+2k_3^2)}{k_t^2(k_1^3+k_2^3+k_3^3)}
			\\[2mm]
						
 			\bottomrule
	
		\end{tabular}
	\end{center}
	\caption{Functions $f_m(k_i)$ 
	determining the momentum dependence of the running of $\fNL$
	in Eq. \eqref{eq:runningfNLtable}.
	\label{table:nfNL}}
	\end{sidewaystable}	
	
	
	
	
	
	
	
	\para{Squeezed and equilateral limits}In the equilateral limit, we find
	\begin{equation}
		\begin{split}
		\nfNL
		\rightarrow
		- \frac{5}{81 z_\star}
		\bigg\{
			&
			g_{1\star} H
			\big( \varepsilon_\star + v_\star - h_{1\star} \big)
			+ 3 g_{2\star}
			\big( v_\star - h_{2\star} \big)
			+ \frac{51 g_{3\star}}{4 \csstar^2}
			\big( v_\star + 2 s_\star - h_{3\star} \big)
			\\ & \mbox{}
			+ \frac{12 g_{4\star}}{4 \csstar^2}
			\big( h_{4\star} - v_\star \big)
			+ \frac{12 g_{5\star}}{4 \csstar^2}
			\big( h_{5\star} - v_\star \big)
		\bigg\}\ \ .
		\end{split}
		\label{eq:nfnl-equilateral}
	\end{equation}
	The squeezed limit gives a simpler result,
	\begin{equation}
		\nfNL \rightarrow \frac{5}{24 z_\star} \bigg\{
			g_{2\star} \big( h_{2\star} - v_\star \big)
			+ \frac{3 g_{3\star}}{\csstar^2}
			\big( h_{3\star} - 2 s_{\star} - v_\star \big)
		\bigg\} \ \ .
		\label{eq:nfnl-squeezed}
	\end{equation}
	
	
	To illustrate an application of the hierarchy condition 
	deduced from Maldacena's consistency condition \eqref{eq:maldacena-condition},
	we define the running of the spectral index, $\alpha_s$, by
	\cite{Kosowsky:1995aa}
	\begin{equation}
		\alpha_s = \frac{\d (n_s - 1)}{\d \ln k} \ \ .
		\label{eq:spectral-running}
	\end{equation}
	Compatibility with Eq. \eqref{eq:maldacena-condition}
	in the squeezed limit
	requires
	\begin{equation}
		\nfNL \rightarrow - \frac{5}{12} \left. \alpha_s \right|_{\khard} \ \  .
		\label{eq:running-consistency}
	\end{equation}

For canonical single field inflation, discussed in \S\ref{sec:vanilla}, 
specializing to the equilateral limit of $\nfNL$, we find
	\begin{equation}
		\nfNL^{\textrm{(equilateral)}} \rightarrow \frac{5}{216} \eta_\star
			( 66 \varepsilon_\star + 18 \xi_\star ) \ \  .
	\end{equation}
	In the squeezed limit one obtains
	\begin{equation}
		\nfNL^{\textrm{(squeezed)}} \rightarrow \frac{5}{12} \eta_\star
			( 2 \varepsilon_\star + \xi_\star ) 
			= - \frac{5}{12} \alpha_{s \star} \ \ ,
		\label{eq:runningsvanilla}
	\end{equation}
	which describes the running of the scalar
	spectral index, $\alpha_{s\star}$,
	in agreement with Eq. \eqref{eq:maldacena-condition}.
	The consistency
	conditions~\eqref{eq:fnlsvanilla}
	and~\eqref{eq:runningsvanilla} represent a
	nontrivial check on the correctness of our calculation.
	Throughout the calculation
	we have carefully separated the conceptually \textit{different}
	scales $k_t$ and $k_\star$. Therefore
	the correct formula~\eqref{eq:runningsvanilla} is \emph{not}
	simply
	a consequence of obtaining the correct leading-order terms
	in Eq. \eqref{eq:fnlsvanilla}.
	It rather depends on a careful 
	matching between the spectral index and $\fNL$
	in this limit.
	
	As anticipated, 
	$\nfNL^{\textrm{(squeezed)}} = \Or(\varepsilon^2)$
	in non-canonical models.
	Therefore a next-next-order calculation is required
	to estimate the running of $\fNL$ in these models; this will 
	be slow-roll suppressed compared to $\fNL$ itself.
	










	\section{Shape-dependence}
	\label{sec:shapes}

In the early days of computing
next-order corrections to the power spectrum, 
pioneered by Stewart \& Lyth \cite{Stewart:1993bc}, 
the main purpose was to obtain an accurate estimate of its amplitude.
	
	
	In comparison, next-order corrections to the bispectrum
	can be relevant for at least three reasons. First, 
	they can change the
	amplitude of three-point correlations beyond 
	\textit{Planck}'s experimental sensitivity. 
	Second, as we have seen in the previous section, 
	next-order corrections allow us to investigate the 
	scale-dependence of the bispectrum.
	Third, they could potentially lead to the appearance of new
	``shapes,'' by which we mean the momentum dependence of
	$B(k_1, k_2, k_3)$ \cite{Babich:2004gb},
	defined in Eq. \eqref{eq:bispectrum-def}. In principle, all these 
	three
	effects are measurable.
	
	The plots and overlapping cosines included in this chapter 
							were produced by David Seery and originally presented 
							in Refs. \cite{Burrage:2011hd, Ribeiro:2011ax}.
	
	
	
	
	\subsection{Inner product and cosine}
	\label{subsec:inner-prod}
	How similar, or dissimilar, are two given bispectrum shapes?	
	Conservation of 3-momentum in the bispectrum
	requires that the momenta $\vect{k}_i$ form a triangle in
	momentum space.
	The bispectrum is a function on this space of triangles.
	Babich \etal~\cite{Babich:2004gb} described its
	functional form as
	the ``shape'' of the bispectrum and introduced a measure
	to distinguish \textit{qualitatively} different shapes.
	We briefly recall their method.	
	We define the shape $S_i$ as
	\begin{equation}
S_i \equiv (k_1 k_2 k_3)^2 \ B_i\ \ .
\end{equation}
One can introduce a formal ``cosine'' which may be used
	as a \textit{quantitative} measure of 
	similarity in shape between different bispectra.	
	The inner product between two bispectra is defined by 
	\begin{equation}
		B_1 \cdot B_2 \equiv \;\int\limits_{\mathclap{\text{triangles}}}
			\d k_1 \, \d k_2 \, \d k_3 \; \,
			S_1(k_1, k_2, k_3) \, S_2(k_1, k_2, k_3)\ \ ,
		\label{eq:inner-prod-def}
	\end{equation}
	where the integral is to be taken over all triangular configurations of
	momenta $\vect{k}_i$. The cosine between $B_1$ and $B_2$ is
	given by
	\begin{equation}
		\cos (B_1, B_2) \equiv \frac{B_1 \cdot B_2}
			{(B_1 \cdot B_1)^{1/2} \, (B_2 \cdot B_2)^{1/2}}\ \  .
		\label{eq:cosine-def}
	\end{equation}
	These expressions require some care.
	In certain cases the result
	may be infinite, requiring the integral to be regulated.
	This is usually the case when one of the bispectra peaks 
	in the squeezed configuration. We will comment on how to deal 
	with these cases next.
	
\vspace*{1cm}	
	
	\para{Parametrisations}One can represent each shape $S_i$ as a function of the 
	three momenta, $k_i$, subject to the $\delta$-distribution, that constrains
	only two of these to be linearly independent.
	Take $k_3$ to be the privileged scale in the triangle. 
	Then $k_1$ and $k_2$ can be rescaled with respect to 
	$k_3$, and $S_i$ can be represented in terms of $k_1/k_3$
	and $k_2/k_3$.
	This is the Babich \etal \ parametrisation \cite{Babich:2004gb}, 
	where the shape function is given by
	\begin{equation*}
		S_i \rightarrow \bigg(\dfrac{k_1}{k_3} \bigg)^2
		\bigg(\dfrac{k_2}{k_3} \bigg)^2
		B_i\bigg(\dfrac{k_1}{k_3}, \dfrac{k_2}{k_3}, 1  \bigg) \ \ .
	\end{equation*}
	
	There is another useful parametrisation
	which enhances the symmetry in surfaces of the 
	shape with equal magnitude.
	This is the parametrisation 
	proposed by Fergusson \& Shellard
	\cite{Fergusson:2008ra}, in which
	the momenta $k_i$ in the inner product \eqref{eq:inner-prod-def}
	can be parametrized geometrically in terms of the
	perimeter, $k_t$ (which becomes the privileged scale), 
	and two dimensionless ratios.	
	As a result, for scale-invariant correlators 
	only two variables, denoted $\alpha$ and $\beta$, 
	are linearly independent, and these are defined by 
	\cite{Fergusson:2008ra}
	\begin{subequations}
		\begin{align}
			\label{eq:fergusson-shellard-a}
			k_1 & = \frac{k_t}{4}\, ( 1 + \alpha + \beta ) \\
			\label{eq:fergusson-shellard-b}
			k_2 & = \frac{k_t}{4}\, ( 1 - \alpha + \beta ) \\
			\label{eq:fergusson-shellard-c}
			k_3 & = \frac{k_t}{2} \, ( 1 - \beta ) \ \ ,
		\end{align}
	\end{subequations}
	where $0 \leq \beta \leq 1$ and $\beta - 1 \leq \alpha \leq 1 - \beta$.
	The shape function is given by the combination
	\begin{equation*}
		S \rightarrow k_1^2\,  k_2^2 \, k_3^2 \ B\big(k_1 , k_2 , k_3\big)\ \  .
	\end{equation*}	
	The measure
	$\d k_1 \, \d k_2 \, \d k_3$ 
	 in the integrand of Eq. \eqref{eq:inner-prod-def}
	is proportional to
	$k_t^2 \, \d k_t \, \d \alpha \, \d \beta$.
	Therefore we can write
	\begin{equation}
		B_1 \cdot B_2 = N
		\int\limits_{\mathclap{\substack{ 0 \leq \beta \leq 1 \\
			\beta - 1 \leq \alpha \leq 1 - \beta}}}
		\d \alpha \, \d \beta \; (1 - \beta)
		(1 + \alpha + \beta)(1 - \alpha + \beta)
		\ S_1(\alpha, \beta)
		\, S_2(\alpha, \beta) \ \  ,
		\label{eq:inner-prod-well-defined}
	\end{equation}
	where $N$ is a harmless normalisation which can
	be divided out. With this understanding we
	use Eq. \eqref{eq:inner-prod-well-defined} to determine
	the cosine in Eq.~\eqref{eq:cosine-def}.
	
	
	In practice, our bispectra are not scale-invariant
	and therefore Eq. \eqref{eq:inner-prod-well-defined} does not
	strictly apply.
	However, as we have already studied in 
	\S\ref{sec:running}
	the violations of scale-invariance are small, and 
	to a good approximation 
	Eq. \eqref{eq:inner-prod-well-defined} can be used.
	
	\vspace*{1cm}	

	
	\para{Divergences}As mentioned before, the cosine defined in Eq. \eqref{eq:cosine-def} 
	requires some care.
	In particular, Eq.~\eqref{eq:inner-prod-well-defined} may be infinite.
	For example, the well-studied local bispectrum
	diverges like $(1 + \alpha + \beta)^{-2}$
	or $(1 - \alpha + \beta)^{-2}$ in the limit
	$\beta \rightarrow 0$, $\alpha \rightarrow \pm 1$,
	or like $(1-\beta)^{-2}$ in the limit $\beta \rightarrow 1$,
	$\alpha \rightarrow 0$ \cite{Babich:2004gb}.
	These correspond to the squeezed limits discussed
	in~\S\ref{sec:bispectrum}.
	Eq.~\eqref{eq:inner-prod-well-defined}
	therefore exhibits power-law divergences on the boundaries
	of the region of integration, and
	in such cases the integral must be regulated to obtain a finite
	answer. For simplicity, we adopt a sharp cutoff which requires
	$k_i / k_t > \deltamin$.
	As $\deltamin \rightarrow 0$ the cosine~\eqref{eq:cosine-def} may
	converge to a nonzero limit if $B_1 \cdot B_2$,
	$B_1 \cdot B_1$ and $B_2 \cdot B_2$ diverge at the same rate.
	
	
	For this reason,
	where divergences exist, the value assigned to $\cos (B_1, B_2)$
	is largely a matter of convention, and should be interpreted
	as an indicative number.
	Nevertheless, to resolve the practical question of
	whether two shapes can be distinguished by observation
	it should be remembered that experiments cannot measure
	arbitrarily small wavenumbers \cite{Lyth:2009zz}.
	Therefore their ability to distinguish shapes peaking in the squeezed
	limit is limited.
	In this case, to obtain accurate forecasts of
	what can be distinguished (especially today in 
	anticipation to \textit{Planck}'s results), one should restore the $k_t$-dependence
	in~\eqref{eq:inner-prod-well-defined}
	and restrict the integration to observable wavenumbers, yielding
	a manifestly finite answer
	\cite{Fergusson:2008ra,Fergusson:2009nv}.
	We do not attempt this here.



\subsubsection*{Template Shapes}
It is often useful to compare the bispectrum shapes in a given model
with certain templates.
There are essentially four main templates used in CMB analysis: 
\textsf{local}\footnote{See Komatsu \& Spergel~\cite{Komatsu:2001rj}
				and Babich {\etal}~\cite{Babich:2004gb}.}, 
\textsf{equilateral}\footnote{See Babich {\etal}~\cite{Babich:2004gb}.}, 
\textsf{orthogonal} and 
\textsf{enfolded}\footnote{See Meerburg {\etal}~\cite{Meerburg:2009ys}
				and Senatore {\etal}~\cite{Senatore:2009gt}.}.
At this point there is a potential
issue with the notation used in this thesis. 
To distinguish between the equilateral \textit{template} 
and the bispectrum shapes 
which can \textit{peak at the equilateral limit}, 
we use a different 
font for the \textsf{templates}.
A shape which peaks in the equilateral limit
need not be $100\%$ correlated with 
the \textsf{equilateral} template.

The name attributed to the templates
is usually related to the triangular 
configuration
which 
maximises the amplitude of the bispectrum, 
that is, $\fNL$. 
However, that need not be the case.
For example, the \textsf{orthogonal} shape was proposed by 
Senatore, Smith \&
Zaldarriaga \cite{Senatore:2009gt}
(also see Chen \cite{Chen:2010xka} for a review), 
and it is constructed so as to peak both in the equilateral
and flattened configurations (when two of the sides of the triangle
are equal to half the third side).


We quote on table \ref{table:cos-templates} 
the overlap cosines between the four templates
mentioned above.
The templates have variable 
overlap amongst themselves.
For example, the \textsf{local} template overlaps mildly
with the \textsf{equilateral} ($\sim 34\%$) 
template, but significantly with the
\textsf{orthogonal} ($\sim 49\%$)
and the \textsf{enfolded} ($\sim 60\%$)
templates.
The \textsf{equilateral} template is practically 
uncorrelated with the \textsf{orthogonal},
by construction, 
but overlaps roughly $51\%$ with the 
\textsf{enfolded} template. 
Finally, the \textsf{orthogonal} template
is correlated with the 
\textsf{enfolded} template
roughly $85\%$.



\vspace*{1cm}


	\begin{table}[h]
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

	\sbox{\tableA}{%
		\begin{tabular}{lTcTc}

			\toprule
			
			&
				\multicolumn{1}{c}{\textsf{local}} &
				\multicolumn{1}{c}{\textsf{equilateral}} &
				\multicolumn{1}{c}{\textsf{orthogonal}} &
				\multicolumn{1}{c}{\textsf{enfolded}}
			\\
			\cmidrule{2-5}
			
			\textsf{local} &
				1.00 &
				&
				&
			\\
			
			\textsf{equilateral} &
				0.34 &
				1.00 &
				&
			\\
			
			\textsf{orthogonal} &
				0.49 &
				0.03 &
				1.00 &
			\\
			
			\textsf{enfolded} &
				0.60 &
				0.51 &
				0.85 &
				1.00
			\\
			
			\bottomrule
		
		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}
	
	\begin{center}
		\usebox{\tableA}
	\end{center}

	\caption{\label{table:cos-templates}Overlap cosines between common
	templates, depicted in Table~\ref{table:template-plots}.}

	\end{table}


\vspace*{1cm}

In table \ref{table:template-plots} we depict 
the four templates in the two different parametrisations.

\begin{table}
	
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

    \sbox{\boxplot}{%
    	\includegraphics[scale=0.16]{Plots/Orthogonal/alpha1/Babich/3D/O}
    }
    \settowidth{\plotw}{\usebox{\boxplot}}
    \sbox{\boxplota}{%
    	\includegraphics[scale=0.14]{Plots/Orthogonal/alpha1/Babich/2D/O}
    }
    \settowidth{\plotwa}{\usebox{\boxplota}}
    
    \sbox{\tableA}{%
		\begin{tabular}{cccc}

			\toprule

			\multicolumn{2}{c}{Fergusson \& Shellard} &
			\multicolumn{2}{c}{Babich {\etal}}
			\\
			
			\cmidrule(r){1-2}
			\cmidrule(l){3-4}
			
			\multicolumn{4}{c}{\textsf{local} template}
			\\
			
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{templates/fergusson/2d/local}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.19]{templates/fergusson/3d/local}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{templates/babich/2d/local}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.19]{templates/babich/3d/local}}
			\\
			
			\midrule
			
			\multicolumn{4}{c}{\textsf{equilateral} template}
			\\
			
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{templates/fergusson/2d/equilateral}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.19]{templates/fergusson/3d/equilateral}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{templates/babich/2d/equilateral}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.19]{templates/babich/3d/equilateral}}
			\\

			\midrule
			
			\multicolumn{4}{c}{\textsf{orthogonal} template}
			\\
			
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{templates/fergusson/2d/orthogonal}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.19]{templates/fergusson/3d/orthogonal}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{templates/babich/2d/orthogonal}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.19]{templates/babich/3d/orthogonal}}
			\\
			
			\midrule
			
			\multicolumn{4}{c}{\textsf{enfolded} template}
			\\
			
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{templates/fergusson/2d/enfolded}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.19]{templates/fergusson/3d/enfolded}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{templates/babich/2d/enfolded}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.19]{templates/babich/3d/enfolded}}
			\\

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
			
	\caption{\label{table:template-plots}
	The bispectrum templates used in CMB analysis
	in the Fergusson \& Shellard \cite{Fergusson:2008ra},
	 and Babich \etal \ \cite{Babich:2004gb} parametrisations.
	 We see that the first parametrisation enhances the symmetry of the shape
	 in $\{\alpha, \beta\}$ space.}

	\end{table}

\clearpage









	\subsection{Bispectrum shapes from slow-variation parameters}
	\label{subsec:bispectrum-shapes-NO}
	In a model with arbitrary interaction vertices $g_i$, 
	the bispectrum is a linear combination
	of the shapes produced by the five operators
	in the action \eqref{eq:s3tau}:
	\begin{equation}
B=(k_1 k_2 k_3)^{-2}\ \sum_{i=1}^5 S_i\ \ ,
\end{equation}
where each operator $i$ yields a shape $S_i$.
	We will now examine in detail the shapes 
	arising at leading and next-order in the slow-variation 
	approximation.
	
\vspace*{1,5cm}	



	\para{Leading-order shapes}We quote the cosines of the shapes $S_i$,
	computed at lowest-order in the slow-roll approximation,
	with the common templates %used in
	in table~\ref{table:leading_overlaps}. We also plot
	the shapes $S_i$ in table \ref{table:shapes-leading-order}, 
	using the two different parametrisations mentioned in \S\ref{subsec:inner-prod}.
	The $\zeta'^3$, $\zeta'\partial \zeta \partial \partial^{-2} \zeta'$
	and $\partial^2 \zeta (\partial \partial^{-2} \zeta')^2$ shapes
	are largely correlated with the {\Equilateral} template.
	The $\zeta \zeta'^2$ and $\zeta (\partial \zeta)^2$
	shapes are in turn correlated with the {\Local} template.
	In most cases there is a moderate overlap with
	the {\Enfolded} template, as we would expect from the correlations 
	between the templates---see table \ref{table:cos-templates}.


\vspace*{0,5cm}

\begin{table}[h]

	\tablepreamble
		
	\sbox{\tableA}{%
		\begin{tabular}{QqQqQq}
			 	\toprule

			&
			\multicolumn{5}{c}{shapes at leading-order in slow-roll}
			\\

			\cmidrule(l){2-6}

		 	&
		 	\multicolumn{1}{c}{$S_{\zeta'^3}$} &
		 	\multicolumn{1}{c}{$S_{\zeta \zeta'^2}$} &
		 	\multicolumn{1}{c}{$S_{\zeta (\partial \zeta)^2}$} &
		 	\multicolumn{1}{c}{$S_{\zeta' \partial_i \zeta \partial^{i} (\partial^{-2}\zeta')}$} &
		 	\multicolumn{1}{c}{$S_{\partial^2 \zeta (\partial_i \partial^{-2}\zeta')^2}$} 
		 	
		 	\\

			\midrule

			\textrm{{\Local}} &

			0.42 &
			0.99 & 
			1.00 & 0.35 & 0.31
			\\

			\cmidrule{2-6}

			\textrm{{\Equilateral}} &
			0.94 	&
			 0.44 &
			0.38 & 1.00 & 0.99
			\\

		

			\cmidrule{2-6}

			\textrm{{\Orthogonal}} &
				0.29 &
			0.50 &
			0.49 & 0.02 & 0.12
			\\

		

			\cmidrule{2-6}

			\textrm{{\Enfolded}} &
			0.75 &
			0.65 &
			0.62 & 0.55 & 0.43
			\\
			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}

	\renewcommand{\arraystretch}{1}
	


	\caption{\label{table:leading_overlaps}Cosines
	between the leading-order shapes and the
	common templates.}
	
	\end{table}



	
\begin{sidewaystable}
	
	\tablepreamble

   \sbox{\boxplot}{%
   	\includegraphics[scale=0.15]{Plotsdecoding/Babich/3D/ShapeLO/Lambda1}
   }
   \settowidth{\plotw}{\usebox{\boxplot}}
   \sbox{\boxplota}{%
   	\includegraphics[scale=0.1]{Plotsdecoding/Babich/2D/ShapeLO/Lambda1}
   }
   \settowidth{\plotwa}{\usebox{\boxplota}}

   \sbox{\tableA}{%
		\begin{tabular}{ccccc}

			\toprule

			&
			\multicolumn{2}{c}{Babich {\etal}} &
			\multicolumn{2}{c}{Fergusson \& Shellard}
			\\
			
			\cmidrule(r){2-3}
			\cmidrule(l){4-5}
			
			$S_{\zeta'^3}$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Babich/2D/ShapeLO/Lambda1}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Babich/3D/ShapeLO/Lambda1}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Fergusson/2D/ShapeLO/Lambda1}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Fergusson/3D/ShapeLO/Lambda1}}
			\\

	$S_{\zeta \zeta'^2}$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Babich/2D/ShapeLO/Lambda2}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Babich/3D/ShapeLO/Lambda2}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Fergusson/2D/ShapeLO/Lambda2}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Fergusson/3D/ShapeLO/Lambda2}}
			\\
			
			$S_{\zeta (\partial \zeta)^2}$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Babich/2D/ShapeLO/Lambda3}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Babich/3D/ShapeLO/Lambda3}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Fergusson/2D/ShapeLO/Lambda3}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Fergusson/3D/ShapeLO/Lambda3}}
			\\

			$S_{ \zeta' \partial_i \zeta \partial^{i} (\partial^{-2} \zeta)}$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Babich/2D/ShapeLO/Lambda4}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Babich/3D/ShapeLO/Lambda4}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Fergusson/2D/ShapeLO/Lambda4}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Fergusson/3D/ShapeLO/Lambda4}}\\
			
			$S_{ \partial^2 \zeta (\partial_i \partial^{-2}\zeta')^2}$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Babich/2D/ShapeLO/Lambda5}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Babich/3D/ShapeLO/Lambda5}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plotsdecoding/Fergusson/2D/ShapeLO/Lambda5}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/Fergusson/3D/ShapeLO/Lambda5}}\\
			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
			
	\caption{\label{table:shapes-leading-order}Bispectrum shapes 
	at leading-order in slow-roll for the operators in the
	action~\eqref{eq:s3tau}, using the
	Babich {\etal} \cite{Babich:2004gb},
	and Fergusson-Shellard \cite{Fergusson:2008ra}
	parametrisations.}
	\end{sidewaystable}










\clearpage
	
	
	
	
	
	
	
	\para{A `new' shape emerges at leading-order}What is the overall bispectrum shape at leading-order?
Factoring out an overall normalisation,
	the shape $S$ of the bispectrum can be written
	\begin{equation}
		S \propto
		\mbox{} 
		\alpha  S_{\zeta'^3} +
		\beta   S_{\zeta \zeta'^2} + \gamma S_{\zeta (\partial\zeta)^2}+
		\delta   S_{\zeta' \partial_i \zeta \partial^i (\partial^{-2}\zeta')}+
		\omega   S_{\partial^2 \zeta (\partial_i \partial^{-2}\zeta')^2}\ \  ,
		\label{eq:start_ortho}
	\end{equation}
	where $\alpha, \beta, \gamma, \delta, \omega$ are 
	rescaled versions of the interactions $g_i$.\footnote{$\alpha$ and $\beta$ here
						should not be confused with the $\{\alpha, \beta\}$ parameters
						in the Fergusson-Shellard parametrisation.}
	In a generic model we could perhaps expect all these ratios to be
	order unity.

	
	We assume arbitrary $g_i$.
	By adjusting these coefficients it is possible to find a
	``critical surface'' in the 
	space of bispectrum shapes on which $B$ becomes orthogonal to
	the
	set $Z = \{ \text{\Equilateral}, 
	\text{\Local}, 
	\text{\Enfolded} \}$.
	The bispectrum can be then be written in the form
	\begin{equation}
		S \propto
		\big(
			\begin{array}{ccc}
				\delta & \omega 
			\end{array}
		\big) \cdot 
		\left(
			\begin{array}{c}
				S_{\delta} \\
				S_{\omega} 
			\end{array}
		\right)
		+
		\big(
			\begin{array}{ccc}
				a & b & c
			\end{array}
		\big) \cdot
		\left(
			\begin{array}{c}
				S_{\zeta'^3} \\
				S_{\zeta \zeta'^2} \\
				S_{\zeta (\partial \zeta)^2}
			\end{array}
		\right)
		\ \ ,
	\end{equation}
	where the shapes $S_\delta$ and $S_\omega$ are
	orthogonal to 
	each template in $Z$.
	The coefficients $\delta$ and $\omega$
	act as coordinates on the
	subspace of bispectra orthogonal to these templates, whereas
	$a$, $b$ and $c$ are coordinates labelling
	departures from this critical surface.
	The appropriate choice is
	\begin{subequations}
		\begin{align}
			\alpha 
			& \simeq 2.394 \delta + 2.208 \omega + a\\ 
			\beta & \simeq 0.473 \delta + 0.642 \omega + b\\
			\gamma  & \simeq -0.183 \delta - 0.248 \omega	+ c\ \ .
			\label{eq:alphabetagamma}
		\end{align}
	\end{subequations}
	
	The shapes $S_\delta$ and $S_\omega$ then satisfy
	\begin{subequations}
		\begin{align}
			S_{\delta} & \simeq
				2.394 S_{\zeta'^3}
				+ 0.473S_{\zeta \zeta'^2}
 				- 0.183 S_{\zeta (\partial \zeta)^2}
 				+ S_{\zeta' \partial_i \zeta \partial^i (\partial^{-2}\zeta')}
 			\\
 			S_{\omega} & \simeq
 				2.208 S_{\zeta'^3}
				+ 0.642 S_{\zeta \zeta'^2}
 				- 0.248 S_{\zeta (\partial \zeta)^2}
 				+ S_{\partial^2 \zeta (\partial_i \partial^{-2}\zeta')^2}
 			\ \ .
 		\end{align}
	\end{subequations}
	Although we did not require it,
	these shapes
	have negligible overlap with the
	\Orthogonal \ template.
	But they \textit{need not} be orthogonal amongst themselves. To measure
	\emph{independent} combinations from data typically requires
	a dedicated template which has negligible overlap with other
	combinations. We follow the procedure of
	Refs.~\cite{Senatore:2009gt,Chen:2010xka}.
	The inner product matrix is $C_{ij} \equiv S_i \cdot S_j$.
	It is diagonalized by an orthogonal matrix
	$\vect{P}$ whose columns are formed from the eigenvectors
	of $\vect{C}$. Setting $a = b = c =  0$ so that the bispectrum
	shape lies within the required critical surface,
	we write
	$\vect{x} = ( \begin{array}{ccc} \delta  & \omega  \end{array} )$,
	and
	$\vect{S} = ( \begin{array}{ccc} S_{\delta} & S_{\omega}
	\end{array} )^T$.
	The part of the bispectrum on the
	critical subspace can be written as
	$B^\parallel \propto \vect{q}\vect{H}$,
	where $\vect{q} \equiv \vect{x} \vect{P}$
	and $\vect{H} \equiv \vect{P}^T \vect{S}$.

	The shapes $S_{\zeta \zeta'^2}$ and $S_{\zeta (\partial \zeta)^2}$
	have {\Local}-type divergences,
	which can be subtracted out by
	taking a suitable linear combination. This leaves four
	independent terms, from which we wish to construct a linear combination
	orthogonal to the three templates. We should expect a unique solution.
	This can be extracted from $\vect{H}$, and is given by
%		\footnote{This is not to be confused 
%		with the Hubble parameter, also 
%		conventionally denoted by $H$.}
	\begin{equation}
		S_H = -0.805 S_{\delta} +  0.593 S_{\omega}\ \  .
		\label{eq:o-def}
	\end{equation}
	This procedure discards the independent linear combination
	of $S_{\zeta\zeta'^2}$ and $S_{\zeta (\partial \zeta)^2}$.
	For practical purposes, we expect
	its divergence in the squeezed limit
	to make it almost indistinguishable from the
	{\Local} template.
	We ignore it in the equations which follow,
	although in principle one should remember that it is present.
	$S_H$ is sometimes confusingly referred to in the 
	literature as ``orthogonal'' since it results from
	an \textit{orthogonalisation} procedure.
	We shall rather describe the shapes constructed this way as 
	orthogonally designed.
	
	We quote the overlap cosines between $S_H$ and 
	the templates in table \ref{table:orthogonal-cosines}.
	In table~\ref{table:ortho-approx-SH} we plot $S_H$
	in the Fergusson \& Shellard parametrisation.
	Given that this parametrisation highlights 
	the symmetry of the surface of the shape, it 
	will be very useful in what follows.
	As a function of the $k_i$
	there are multiple peaks in the critical surface, and therefore $S_H$
	is not maximised on a unique type of triangle.
	
	









	\begin{table}[h]

	\tablepreamble
	
	\sbox{\tableA}{%
		\begin{tabular}{cTcT}

			\toprule
			

				\multicolumn{1}{c}{{\Local}\tmark{a} } &
				\multicolumn{1}{c}{{\Equilateral}} &
				\multicolumn{1}{c}{{\Orthogonal}} &
				\multicolumn{1}{c}{{\Enfolded}} 
			\\
			\cmidrule{1-4}

			
				 0.02 &
				 0.00 &
				 0.00 &
				 0.00 
\\
			\bottomrule
		
		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}
	
	\begin{center}
		\usebox{\tableA}
	\end{center}
	
	\renewcommand{\arraystretch}{1.0}
	\scriptsize
	
	\sbox{\tableB}{%

	}
	
	\begin{center}
		\usebox{\tableB}
	\end{center}

	\caption{\label{table:orthogonal-cosines}Cosines 
	between the $S_H$-shape~\eqref{eq:o-def} and
	common templates.}
	\end{table}


\vspace*{0.5cm}


	\begin{table}[h]
	
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

    \sbox{\boxplot}{%
    	\includegraphics[scale=0.15]{Plotsdecoding/Orthogonal/alpha1/Babich/3D/O}
    }
    \settowidth{\plotw}{\usebox{\boxplot}}
    \sbox{\boxplota}{%
    	\includegraphics[scale=0.2]{Plotsdecoding/Orthogonal/alpha1/Babich/2D/O}
    }
    \settowidth{\plotw}{\usebox{\boxplota}}
    
    \sbox{\tableA}{%
		\begin{tabular}{cc}

			\toprule

			\multicolumn{2}{c}{$S_H$ shape }
			\\
			\midrule
			

				
			
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plotsdecoding/orthofergusson/plots-1}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.2]{Plotsdecoding/orthofergusson/plots-2}}
			\\

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
			
	\caption{\label{table:ortho-approx-SH}
	The $S_H$-shape in the Fergusson \& Shellard parametrisation.
	}

	\end{table}




	The shape $S_H$ smoothly converges to zero in the squeezed limit but
	exhibits a distinctive
	drumlin-shaped features near the corners of the triangle.	
	This shape will occur in a typical bispectrum with
	coefficients which depend on $\omega$ and $\delta$.
	We find
	\begin{equation}
		S = (0.593 \omega - 0.805\delta) S_H
		+ \left(
			\begin{array}{c}
				\alpha - 2.394 \delta - 2.208 \omega  \\
				\beta -0.473 \delta - 0.642  \omega \\
				\gamma +0.183 \delta + 0.248  \omega
			\end{array}
		\right) \cdot
		\left(
			\begin{array}{c}
				S_{\zeta'^3} \\
				S_{\zeta \zeta'^2} \\
				S_{\zeta (\partial \zeta)^2}
			\end{array}
		\right) .
		\label{eq:b-generic}
	\end{equation}
	How significant is its contribution to the overall 
	bispectrum shape?
	Since all prefactors will generically be of order unity,
	by assumption of a generic Horndeski model,
	the question reduces to the relative magnitudes of $S_H$ and
	$S_{\zeta'^3}$, $S_{\zeta \zeta'^2}$ and $S_{\zeta (\partial \zeta)^2}$. 
	We find $\| S_H \|\sim10^{-2}$,
	whereas $\| S_{\zeta'^3} \| \sim 1$.
	The precise values assigned to $\| S_{\zeta \zeta'^2} \|$
	and $\| S_{\zeta (\partial \zeta)^2} \|$
	depend on how their squeezed divergences are regulated,
	but generically we find
	$\| S_{\zeta \zeta'^2} \|$
	and $\| S_{\zeta (\partial \zeta)^2} \| \sim 10^{1}-10^{2}$.
	We conclude that $S_H$
	has an amplitude suppressed by roughly $10^3$
	to $10^{4}$ compared with
	the leading-order shapes, all of which are well-matched by the standard templates.
	For the `new' shape $S_H$ to be visible requires \emph{either}:
	\begin{enumerate}[i.]
		\item the leading-order shapes to be suppressed,
		so that $a \simeq b \simeq c \simeq 0$ to an accuracy
		of a few parts in $10^3$ to $10^4$.
		This could happen in a specific model,
		but requires fine-tuning.
		\item the overall amplitude of the bispectrum
		to be sufficiently large so that the suppressed
		$S_H$ is visible.
		Without a dedicated analysis of the signal-to-noise
		available in the $S_H$-channel for a CMB survey,
		it is not possible to know how large the bispectrum must be.
		However, it is unlikely that the signal to noise for $S_H$
		will be dramatically better than that for the {\Equilateral} template.
		Therefore, it seems reasonable to suggest that
		the leading-order operators would have to produce
		$\big|\fNL^{\mathrm{equilateral}}\big| \gtrsim 100$
		in order for the $S_H$-shape to be visible.
		This is presently under stress by experimental
		sensitivity
		\cite{Creminelli:2005hu,Creminelli:2006rz,
		Senatore:2009gt,Komatsu:2010fb}.
	\end{enumerate}
	
	We conclude that it is both 
	theoretically and observationally hard to realise $S_H$.
	There is another curious feature about this shape: 
	it is extraordinarily similar to a shape encountered by 
	Creminelli \etal \ \cite{Creminelli:2010qf}, 
	and which we plot on table \ref{table:creminelli-shape}.
		We will return to this issue in \S\ref{sec:modal-decomposition}.



	\begin{table}[h]
	
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

    \sbox{\boxplot}{%
    	\includegraphics[scale=0.1]{Plots/Creminelli/Babich/2D}
    }
    \settowidth{\plotw}{\usebox{\boxplot}}
    \sbox{\boxplota}{%
    	\includegraphics[scale=0.15]{Plots/Creminelli/Babich/3D}
    }
    \settowidth{\plotwa}{\usebox{\boxplota}}
    
    \sbox{\tableA}{%
		\begin{tabular}{cccc}

			\toprule

			\multicolumn{2}{c}{Babich {\etal}} &
			\multicolumn{2}{c}{Fergusson \& Shellard}
			\\

			\cmidrule(r){1-2}
			\cmidrule(l){3-4}
			
			\parbox[c]{\plotw}{\includegraphics[scale=0.1]{Plots/Creminelli/Babich/2D}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{Plots/Creminelli/Babich/3D}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.1]{Plots/Creminelli/Fergusson/2D}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.15]{Plots/Creminelli/Fergusson/3D}}
			\\

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
	
	\caption{\label{table:creminelli-shape}Highly orthogonally designed shape
	constructed by Creminelli {\etal}~\cite{Creminelli:2010qf}.
	}

	\end{table}


	
	
	
	
	
	
	
	
	
	\para{Enhanced leading-order shapes by a reduced sound speed}As discussed in \S\ref{subsec:horndeski},
	a $P(X,\phi)$ theory imposes strong correlations amongst the $g_i$.
	In this sense it is not as generic as an arbitrary Horndeski
	model, and we might not be able
	to finely tune the $g_i$ to produce
	a `new,' exotic bispectrum shape.
	In particular, at leading-order, $g_4$ and $g_5$ do not contribute.
	
	
	We focus on a model with small sound speed, $c_s\ll 1$,
	in which next-order corrections are most likely to be observable,
	and retain only contributions enhanced by $\cs^{-2}$.
	The remaining three operators organise themselves
	into a family of shapes
	of the form
	$S_1 + \alphalambda S_2$,
	where $S_2$ arises only from $\zeta'^3$,
	but $S_1$ is a linear combination of the shapes produced
	by $\zeta'^3$, $\zeta \zeta'^2$ and $\zeta (\partial \zeta)^2$.
	The parameter $\alphalambda$ is the enhanced
	part of $\lambda/\Sigma$, that is
	\begin{equation}
		\frac{\lambda}{\Sigma} = \frac{\alphalambda}{\cs^2}
		+ \Or(1)
		\quad
		\text{for $\cs \ll 1$} .
	\end{equation}
	In the DBI model $\alphalambda = 1/2$.
	We plot the shapes $S_1$ and $S_2$ in
	Table~\ref{table:lowest-order-shapes}.
	
	

	\begin{table}[h]
	
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

    \sbox{\boxplot}{%
    	\includegraphics[scale=0.22]{Plots/Babich/3D/ShapeLO/S1}
    }
    \settowidth{\plotw}{\usebox{\boxplot}}
    
    \sbox{\tableA}{%
		\begin{tabular}{ccc}

			\toprule

			&
			Babich {\etal} &
			Fergusson \& Shellard
			\\

			\cmidrule(r){2-2}
			\cmidrule(l){3-3}
			
			Shape 1 &
			\parbox[c]{\plotw}{\includegraphics[scale=0.22]{Plots/Babich/3D/ShapeLO/S1}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.22]{Plots/Fergusson/3D/ShapeLO/S1}}
			\\
\midrule
			Shape 2 &
			\parbox[c]{\plotw}{\includegraphics[scale=0.22]{Plots/Babich/3D/ShapeLO/S2}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.22]{Plots/Fergusson/3D/ShapeLO/S2}}
			\\

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
			
	\renewcommand{\arraystretch}{1}
	\tiny
	
	\sbox{\tableB}{%
	}
	
	\begin{center}
		\usebox{\tableB}
	\end{center}
	
	\caption{\label{table:lowest-order-shapes}Lowest-order
	bispectrum shapes
	enhanced by $\cs^{-2}$ in $P(X,\phi)$ models.}

	\end{table}	
	
	Note that although $S_1$ involves a linear combination of the
	local-shape operators $\zeta \zeta'^2$
	and $\zeta (\partial \zeta)^2$, the
	$P(X,\phi)$ Lagrangian correlates their amplitudes in such a way
	that there is no divergence in the squeezed limit. Both $S_1$
	and $S_2$
	are strongly correlated with the \Equilateral \ template.
	They are similar to the $M_1$- and $M_2$-shapes studied
	by Creminelli {\etal}
	\cite{Creminelli:2010qf}.





	\para{Next-order shapes}Even though most next-order
	shapes are largely correlated with their parent leading-order shape, 
	more shapes become available at next-order.
	Na\"{\i}vely,
	the family of enhanced bispectra is
	labelled by $\varepsilon$, $\eta$, $s$, and also $\ell$.
	In practice there is some degeneracy, because the shapes
	corresponding to these independent parameters may be strongly
	correlated.
	We will see these degeneracies emerge naturally in our analysis.
	
	The $\cs^{-2}$-enhanced next-order shape can be written
	as a linear-combination
	of shapes proportional to the $\varepsilon$,
	$\eta$, $s$ and $\ell$ parameters, modulated by $\alphalambda$,
	\begin{equation}
		S_{next-order} \sim \varepsilon S_\varepsilon
		+ \eta S_\eta
		+ s S_s
		+ \alphalambda \left(
			\varepsilon S'_\varepsilon
			+ \eta S'_\eta
			+ s S'_s
			+ \ell S'_\ell
		\right)\ \  .
		\label{eq:next-order-shape}
	\end{equation}
	Primed shapes are enhanced by a small
	sound speed since they multiply $\tilde{\alpha}$ 
	(prime here just denotes
	the $c_s^{-2}$-enhanced next-order shapes).
	We give overlap cosines between $S_i$ and $S'_i$ with
	the standard templates in Table~\ref{table:slow-roll-shapes}
	and plot them in Table~\ref{table:next-order-shapes}.
	
	\vspace*{0,5cm}
	
	\begin{table}[h]

	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

	\sbox{\tableA}{%
		\begin{tabular}{QsSsSsSs}

			\toprule

			&
			\multicolumn{1}{c}{$S_\varepsilon$} &
			\multicolumn{1}{c}{$S'_\varepsilon$} &
			\multicolumn{1}{c}{$S_\eta$} &
			\multicolumn{1}{c}{$S'_\eta$} &
			\multicolumn{1}{c}{$S_s$} &
			\multicolumn{1}{c}{$S'_s$} &
			\multicolumn{1}{c}{$S'_\ell$}
			\\

			\cmidrule{2-8}

			\multicolumn{1}{l}{local} &
				0.38\tmark{a} &
				0.50\tmark{a} &
				0.37\tmark{a} &
				0.43\tmark{a} &
				0.54\tmark{a} &
				0.39\tmark{a} &
				0.42\tmark{a}
				\\	

			\multicolumn{1}{l}{equilateral} &
				0.99 &
				0.87 &
				1.00 &
				0.93 &
				0.80 &
				0.94 &
				0.94
				\\

			\multicolumn{1}{l}{orthogonal} &
				0.084 &
				0.46 &
				0.065 &
				0.31 &
				0.52 &
				0.25 &
				0.29
				\\

			\multicolumn{1}{l}{enfolded} &
				0.60 &
				0.86 &
				0.59 &
				0.77 &
				0.87 &
				0.72 &
				0.75
				\\

			\bottomrule
		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}
	
	\begin{center}
		\usebox{\tableA}
	\end{center}
	
	\renewcommand{\arraystretch}{1.0}
	\tiny
	
	\sbox{\tableB}{%
		\begin{tabular}{l@{\hspace{1mm}}l}	
			\tmark{a} &
				\parbox[t]{\tblw}{
				The \textsf{local} template, and the operators
				$\zeta \zeta'^2$ and $\zeta (\partial \zeta)^2$, are strongly
				peaked in the ``squeezed'' limit where one momentum becomes much
				softer than the other two. For these shapes the inner product
				which defines the cosine is divergent, and must be regulated.
				The resulting cosines are almost entirely
				regulator-dependent. See the discussion
				in \S\ref{sec:shapes}.
		
				The values we quote are meaningful only for our choice
				of regulator. For the values quoted above we
				used $\deltamin = k/k_t = 10^{-3}$, where
				$\deltamin$ is defined in the main text.}
		\end{tabular}
	}
	
	\begin{center}
		\usebox{\tableB}
	\end{center}

	\caption{\label{table:slow-roll-shapes}Overlap cosines
	for the bispectrum shape proportional to each slow-variation parameter.
	Sign information has been discarded.}

	\end{table}


	

	\begin{table}
	
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

    \sbox{\boxplot}{%
    	\includegraphics[scale=0.15]{Plots/Babich/3D/ShapeNLO/epsilon}
    }
    \settowidth{\plotw}{\usebox{\boxplot}}
    \sbox{\boxplota}{%
    	\includegraphics[scale=0.1]{Plots/Babich/2D/ShapeNLO/epsilon}
    }
    \settowidth{\plotwa}{\usebox{\boxplota}}
    
    \sbox{\tableA}{%
		\begin{tabular}{ccccc}

			\toprule

			&
			\multicolumn{2}{c}{Babich {\etal}} &
			\multicolumn{2}{c}{Fergusson \& Shellard}
			\\
			
			\cmidrule(r){2-3}
			\cmidrule(l){4-5}
			
			$S_\varepsilon$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Babich/2D/ShapeNLO/epsilon}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Babich/3D/ShapeNLO/epsilon}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Fergusson/2D/ShapeNLO/epsilon}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Fergusson/3D/ShapeNLO/epsilon}}
			\\

			$S'_\varepsilon$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Babich/2D/ShapeNLO/epsilonL}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Babich/3D/ShapeNLO/epsilonL}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Fergusson/2D/ShapeNLO/epsilonL}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Fergusson/3D/ShapeNLO/epsilonL}}
			\\

			$S_\eta$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Babich/2D/ShapeNLO/eta}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Babich/3D/ShapeNLO/eta}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Fergusson/2D/ShapeNLO/eta}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Fergusson/3D/ShapeNLO/eta}}
			\\

			$S'_\eta$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Babich/2D/ShapeNLO/etaL}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Babich/3D/ShapeNLO/etaL}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Fergusson/2D/ShapeNLO/etaL}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Fergusson/3D/ShapeNLO/etaL}}
			\\

			$S_s$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Babich/2D/ShapeNLO/s}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Babich/3D/ShapeNLO/s}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Fergusson/2D/ShapeNLO/s}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Fergusson/3D/ShapeNLO/s}}
			\\

			$S'_s$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Babich/2D/ShapeNLO/sL}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Babich/3D/ShapeNLO/sL}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Fergusson/2D/ShapeNLO/sL}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Fergusson/3D/ShapeNLO/sL}}
			\\

			$S'_\ell$ &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Babich/2D/ShapeNLO/lL}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Babich/3D/ShapeNLO/lL}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Fergusson/2D/ShapeNLO/lL}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Fergusson/3D/ShapeNLO/lL}}
			\\

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
			
	\caption{\label{table:next-order-shapes}Bispectrum shapes enhanced
	by $\cs^{-2}$ at next-order in a $P(X,\phi)$ model.}

	\end{table}
	
	
	
	
	
	
\clearpage	

	Overall these shapes have strong overlaps with the
	\textsf{equilateral} template. However, two
	are quite different in appearance
	and have a slightly smaller cosine $\sim 0.85$
	with this mode:
	these are $S'_\varepsilon$ and $S_s$.
	We fix two coefficients
	in~\eqref{eq:next-order-shape} by
	choosing a linear combination
	orthogonal
	to both $S_1$ and $S_2$.
	Without loss of generality we can choose these
	to be $\eta$ and $s$. We find
	the required orthogonal combination is
		\begin{subequations}
	\begin{align}
		\eta &
		\simeq
			\frac{0.12 \alphalambda \ell
				(\alphalambda + 0.72)
				(\alphalambda + 1.82)
				-
				0.88 \varepsilon
				(\alphalambda - 9.15)
				(\alphalambda - 0.22)
				(\alphalambda + 1.82)}
				{(\alphalambda - 10.24)
				(\alphalambda - 0.23)
				(\alphalambda + 1.82)}\ \ \textrm{and}
			\vspace*{1cm}			
			\\ 
			\vspace*{1cm}			
		s &
		\simeq
			\frac{\alphalambda \ell
				(3.88 - 0.12 \alphalambda)
				- 1.12 \varepsilon (\alphalambda - 8.51)
				(\alphalambda - 0.08)}
				{(\alphalambda - 10.24)
				(\alphalambda - 0.23)} \ \ .
	\end{align}
	\end{subequations}
	It is possible this procedure is stronger than necessary.
	Both $S_1$ and $S_2$ are correlated with the \textsf{equilateral} template,
	and it may be sufficient to find a linear combination orthogonal
	to that.
	In what follows, however, we insist on orthogonality with
	$S_1$ and $S_2$.
	For certain values of $\alphalambda$ the denominator
	of both $\eta$ and $s$ may simultaneously
	vanish, making the required
	$\eta$ and $s$ very large. This implies that, near these
	values of $\alphalambda$, no shape orthogonal
	to both $S_1$ and $S_2$ can be found within the
	validity of next-order perturbation theory.
	Therefore,
	we restrict attention to those $\alphalambda$
	which allow acceptably small $\eta$ and $s$.
	
	This process leaves two linear combinations
	proportional to $\varepsilon$ and $\ell$.
	In principle these can be diagonalized, yielding a \textit{pair} of shapes
	orthogonal to each other and $\{ S_1, S_2 \}$.
	However, the $2\times 2$ matrix of inner products between
	these linear combinations is degenerate. Therefore, only \textit{one} member
	of this pair is physical and can be realised in a $P(X, \phi)$
	model. The other is not: it has zero inner product
	with the shape \eqref{eq:next-order-shape}, and is impossible to realise
	because of enforced correlations between
	coefficients.
	
	We denote the physical orthogonal combination $O$.
	It has a vanishing component proportional to $\ell$.
	This was expected, because
	the shape $S'_\ell$ is the same as $S_2$.
	For this reason, Chen {\etal}
	\cite{Chen:2006nt}
	absorbed $\ell$ into a redefined
	$\lambda/\Sigma$.
	It is indistinguishable from the lowest-order prediction
	and could never be observed separately, which is the origin
	of the degeneracy. We could have arrived at the same
	$O$ by excluding $S'_\ell$ from~\eqref{eq:next-order-shape}.
	Demanding the inner product with $S_1$ and $S_2$ to be zero
	reproduces
	the physical linear combination obtained from diagonalisation.
	
	We plot the shape of $O$ in Table~\ref{table:orthogonal-plots}.
	Again, it is very similar to the highly orthogonal shape
	constructed by
	Creminelli {\etal} \cite{Creminelli:2010qf} plotted in table
	\ref{table:orthogonal-O-cosines}.
	Its dependence
	on $\alphalambda$ is modest.
	For comparison,
	we quote the cosine between $O$ and 
	the Creminelli \etal \ shape in
	Table~\ref{table:orthogonal-cosines}.
	For varying
	$\alphalambda$
	we find a cosine in the range $0.8$ -- $0.9$,
	which indicates it would be observationally difficult
	to distinguish between these shapes.
	
	\vspace*{0,5cm}
	


	\begin{table}[h]
	
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

    \sbox{\boxplot}{%
    	\includegraphics[scale=0.15]{Plots/Orthogonal/alpha1/Babich/3D/O}
    }
    \settowidth{\plotw}{\usebox{\boxplot}}
    \sbox{\boxplota}{%
    	\includegraphics[scale=0.1]{Plots/Orthogonal/alpha1/Babich/2D/O}
    }
    \settowidth{\plotwa}{\usebox{\boxplota}}
    
    \sbox{\tableA}{%
		\begin{tabular}{cccc}

			\toprule

			\multicolumn{2}{c}{Babich {\etal}} &
			\multicolumn{2}{c}{Fergusson \& Shellard}
			\\
			
			\cmidrule(r){1-2}
			\cmidrule(l){3-4}
			
			\multicolumn{4}{c}{$\alphalambda = 10^{-3}$}
			\\
			
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Orthogonal/alpha1E-3/Babich/2D/O}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Orthogonal/alpha1E-3/Babich/3D/O}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Orthogonal/alpha1E-3/Fergusson/2D/O}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Orthogonal/alpha1E-3/Fergusson/3D/O}}
			\\
			
			\midrule
			
			\multicolumn{4}{c}{$\alphalambda = 1$}
			\\
			
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Orthogonal/alpha1/Babich/2D/O}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Orthogonal/alpha1/Babich/3D/O}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Orthogonal/alpha1/Fergusson/2D/O}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Orthogonal/alpha1/Fergusson/3D/O}}
			\\

			\midrule
			
			\multicolumn{4}{c}{$\alphalambda = 10$}
			\\
			
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Orthogonal/alpha10/Babich/2D/O}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Orthogonal/alpha10/Babich/3D/O}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.1]{Plots/Orthogonal/alpha10/Fergusson/2D/O}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.15]{Plots/Orthogonal/alpha10/Fergusson/3D/O}}
			\\

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
			
	\caption{\label{table:orthogonal-plots}
	The ``orthogonal'' shape $O$ has zero overlap
	with both the shapes $S_1$ and $S_2$.}

	\end{table}

	\vspace*{0,5cm}



	In Table~\ref{table:orthogonal-O-cosines} we also give
	the overlap cosine with the
	common templates.
	The leading-order shapes $S_1$ and $S_2$ are strongly
	correlated with the \textsf{equilateral} template, and since $O$
	is orthogonal to these by construction, it also has
	small cosines with the \textsf{equilateral} template, of order $10^{-2}$.
	There is a moderate cosine with the \textsf{local} template
	of order $\sim 0.3$ -- $0.4$.
	The precise value depends on our choice of
	$\deltamin$, but the dependence is not dramatic.
	In Table~\ref{table:orthogonal-O-cosines} we have used 
	 $\deltamin = 10^{-3}$. For $\deltamin = 10^{-5}$
	the local cosines change by roughly $25\%$, but overlaps with the
	remaining templates remain stable.
	$O$ has a cosine of order $0.36$ -- $0.40$ with the \textsf{orthogonal}
	template, and of order $0.32$ -- $0.35$ with the \textsf{enfolded}
	template.
	We conclude that $O$ it is not strongly correlated with
	any of the standard templates used in CMB analysis.



	\vspace*{1cm}

	\begin{table}[htpb]
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

	\sbox{\tableA}{%
		\begin{tabular}{cTcTcT}

			\toprule
			
			$\alphalambda$ &
				\multicolumn{1}{c}{\textsf{local}} &
				\multicolumn{1}{c}{\textsf{equilateral}} &
				\multicolumn{1}{c}{\textsf{orthogonal}} &
				\multicolumn{1}{c}{\textsf{enfolded}} &
				\multicolumn{1}{c}{Creminelli {\etal}}
			\\
			\cmidrule(r){1-1}
			\cmidrule{2-6}

			$10^{-3}$ &			
				0.35\tmark{a} &
				0.012 &
				0.36 &
				0.32 &
				0.89
			\\

			$1$ &			
				0.38\tmark{a} &
				0.012 &
				0.38 &
				0.33 &
				0.86
			\\
			
			$10$ &
				0.41\tmark{a} &
				0.011 &
				0.40 &
				0.35 &
				0.81
			\\
			
			\bottomrule
		
		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}
	
	\begin{center}
		\usebox{\tableA}
	\end{center}
	
	\renewcommand{\arraystretch}{1.0}
	\tiny
	
	\sbox{\tableB}{%
		\begin{tabular}{l@{\hspace{1mm}}l}	
			\tmark{a} & \parbox[t]{\tblw}{%
				Our choice of regulator is $\deltamin = k/k_t = 10^{-3}$, where
				$\deltamin$ was defined in
				\S\ref{sec:shapes}.}
		\end{tabular}
	}
	
	\begin{center}
		\usebox{\tableB}
	\end{center}

	\caption{\label{table:orthogonal-O-cosines}Overlap cosines
	between the orthogonal shape $O$ and
	common
	templates.}

	\end{table}






	\begin{table}[htpb]
	
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

    \sbox{\boxplot}{%
    	\includegraphics[scale=0.13]{Plotsdecoding/Orthogonal/alpha1/Babich/3D/O}
    }
    \settowidth{\plotw}{\usebox{\boxplot}}
    \sbox{\boxplota}{%
    	\includegraphics[scale=0.18]{Plotsdecoding/Orthogonal/alpha1/Babich/2D/O}
    }
    \settowidth{\plotw}{\usebox{\boxplota}}
    
    \sbox{\tableA}{%
		\begin{tabular}{cc}

			\toprule

			\multicolumn{2}{c}{Orthogonally designed bispectrum shapes }
			\\
			
			\midrule	
			
			\multicolumn{2}{c}{$S_H$ shape}\\
						

		
			
			\parbox[c]{\plotw}{\includegraphics[scale=0.13]{Plotsdecoding/orthofergusson/plots-1}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.18]{Plotsdecoding/orthofergusson/plots-2}}
			\\


			\midrule
			
			\multicolumn{2}{c}{$O$ shape}
			\\
			
				\parbox[c]{\plotw}{\includegraphics[scale=0.13]{Plotsdecoding/Orthogonal/alpha1/Fergusson/2D/O}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.18]{Plotsdecoding/Orthogonal/alpha1/Fergusson/3D/O}}
			\\
						\midrule	

			\multicolumn{2}{c}{Creminelli {\etal} orthogonal shape}
			\\
			
			\parbox[c]{\plotw}{\includegraphics[scale=0.13]{Plotsdecoding/Creminelli/Fergusson/2D}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.18]{Plotsdecoding/Creminelli/Fergusson/3D}}
			\\
		

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
			
	\caption{\label{table:ortho-approx}
	The bispectrum shapes $S_H$, $O$ and the 
	one found by Creminelli \etal \ \cite{Creminelli:2010qf}.
	}

	\end{table}



\vspace*{1cm}


For completeness and to facilitate the comparison, we include here the plots 	
of all the orthogonally designed bispectrum shapes.
	Even if they could be 
	realised in an inflationary model with 
	severe fine-tuning, they could not be used to
	support one theory over another.
	From the shapes in table \ref{table:ortho-approx}, 
	shape $O$ is the one which exhibits 
	sharper features, with a steeper drumlin base.
The remaining shapes appear to be slightly smoother.
	
	These bispectrum shapes are incredibly similar, with an overlapping cosine
	in excess of roughly $85\%$. 
This raises the question of 
	 why a linear combination of 
	dome-like shapes can always give rise to 
	a drumlin-shape, with much more structure. 
	We will investigate this in the next section.
	
	

	
	
	
	\newpage






\section{Resolving the ``drumlin'' bispectrum shape}
\label{sec:modal-decomposition}

	
	
	The plots in table \ref{table:ortho-approx} 
	make it clear that the `new,'
	orthogonally designed shape cannot be used as a 
	diagnostic tool to distinguish between models.
	However, why is this shape recurrent in the 
	orthogonalisation procedure?
	
	
	The drumlin structure increases the number of nodes/anti-nodes
	in the bispectrum.
	One can think of the orthogonalisation procedure
	as taking two
	almost pure Fourier harmonics
	and constructing an orthogonal function.
	The result will be approximately
	the next available Fourier harmonic, 
	which by construction will not correlate
	with the fundamental modes.
	This suggests that to understand the appearance of these shapes, 
	it might be helpful to decompose the bispectrum into some analogue of
	Fourier modes. The underlying triangular geometry
	is different to the flat intervals which yield Fourier harmonics,
	so the appropriate analogue will be a generalised partial wave,
	though we might refer to them as fundamental
	harmonics.
	
	
	
	
	
	
	\subsection{Harmonic decomposition}
	\label{subsec:harmonic-decomposition}
	Although partial-wave decompositions have been usefully applied to
 quantum field theory, so far
	they have not been very popular in
	inflationary correlations. Recently,
	Fergusson {\etal} \cite{Fergusson:2008ra,Fergusson:2009nv}
	introduced an eigenmode decomposition,
	and emphasised its computational efficiency.
	We largely follow their method and notation. 
	Physical conclusions must be independent of the
		basis, but the analysis may be made simpler by an
		appropriate choice.\footnote{
		For comparison with the Fergusson~{\etal}
		basis, we have repeated the analysis using
		Bessel functions \cite{Fergusson:2008ra}.
		With this choice, convergence is much slower.
		A different decomposition was used by
		Meerburg~\cite{Meerburg:2010ks}.}
		
	Fergusson {\etal} suggested
	writing each shape function in the form
	\begin{equation}
		S(k_1, k_2, k_3)
		= \sum_{n} \alpha_n \ \Rbasis{n}(k_1, k_2, k_3) \ \ ,
		\label{eq:decompositionR}
	\end{equation}
	for some coefficients $\alpha_n$
	(not to be confused with $\tilde{\alpha}$ 
	in \S\ref{subsec:bispectrum-shapes-NO}) and a set
	of dimensionless
	basis functions $\Rbasis{n}$ which are orthonormal in the
	inner product~\eqref{eq:inner-prod-def}. 
						The functions $\Rbasis{n}$
						are a subset of those constructed by				
						Fergusson~{\etal}~\cite{Fergusson:2008ra,Fergusson:2009nv}
						and labelled $\mathcal{R}_n$.
						The $\Rbasis{n}$ form a basis on a fixed slice
						at constant $k_t$,
						suitable for an approximately
						scale-invariant primordial bispectrum.
						Fergusson~{\etal}'s $\mathcal{R}_n$				
						are not scale-invariant and are orthonormal in
						a three-dimensional inner product which accounts for variation in
						$k_t$.
						Our $\Rbasis{n}$ are constructed using precisely the same
						procedure,
						but because many of the $\Rbasis{n}$ are degenerate
						purely as a function of shape (but not scale)
						they are projected out of the $\Rbasis{n}$.
						It is in this sense that
						the $\Rbasis{n}$ form a 
						subset of the $\mathcal{R}_n$. 
						
	The choice of $\Rbasis{n}$ was motivated by numerical
	considerations, as follows.
	Define a complete set of orthonormal polynomials $\qpoly{p}(x)$
	on the unit
	interval $x \in [0,1]$ with measure $w(x)$
	and introduce separable quantities $\Qbasis{p}{q}{r}$ satisfying
	\begin{equation}
		\Qbasis{p}{q}{r} =
			\qpoly{p}(2 k_1/k_t) \, \qpoly{q}(2 k_2/k_t)\, \qpoly{r}(2 k_3/k_t)
			+ \text{5 permutations}\ \ .
	\end{equation}
	Fergusson~{\etal} chose $w$ to cancel
	an unwanted growth in the bispectrum at large $k$; for all details
	and the construction of the $q_p(x)$
	we refer to the original
	literature~\cite{Fergusson:2008ra,Fergusson:2009nv}.
	One may impose a fixed normalisation for the
	$\Qbasis{p}{q}{r}$ if desired.
	They can be ordered by defining
	$\rho^2 = p^2 + q^2 + r^2$
	and sorting the $\Qbasis{p}{q}{r}$ in ascending order of $\rho$.
	
	Finally, the
	$\Rbasis{n}$ are constructed by Gram--Schmidt orthonormalisation
	of the ordered $\Qbasis{p}{q}{r}$, resulting in a linear combination
	of separable functions.
	This leads to efficiencies
	in computation,
	which was the principal motivation for
	Refs.~\cite{Fergusson:2008ra,Fergusson:2009nv}.
One can obtain the expansion coefficients $\alpha_n$
	for any bispectrum $B$
	using the inner product~\eqref{eq:inner-prod-def}
	\begin{equation}
		\alpha_n = \iprod{\Rbasis{n}}{B}\ \  .
		\label{eq:r-expansion}
	\end{equation}
	Since $\| B \|^2 = \sum_n \alpha_n^2$, then $\alpha_n^2 / \alpha_m^2$ measures
	the relative
	importance of the $m^{\mathrm{th}}$ and $n^{\mathrm{th}}$
	modes.
	
	We plot the first few $\Rbasis{n}$ in Table~\ref{table:Rbasis}.
	The $n=0$ mode is a constant. The $n=1,2$ modes are a good match for
	the overall shape of both the
	{\Equilateral} and {\Orthogonal} templates.
	Strong features in the corners of the triangle,
	characteristic of the {\Local} shape,
	appear at higher $n$.
	Generically speaking, from $n=4$ onwards there is more 
	structure in each harmonic basis.
	
	
	\clearpage
	
	
	\begin{sidewaystable}[htpb]
	
	\tablepreamble
	
	\sbox{\boxplot}{%
		\includegraphics[scale=0.125]{Plotsdecoding/R/plots-1}
	}
	\settowidth{\plotw}{\usebox{\boxplot}}
	\sbox{\boxplota}{%
		\includegraphics[scale=0.18]{Plotsdecoding/R/plots-2}
	}
	\settowidth{\plotwa}{\usebox{\boxplota}}
	
	\sbox{\tableA}{%
		\begin{tabular}{cccccc}

			\toprule

			$n=0$
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-1}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-2}} &
			$n=5$ &
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-11}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-12}}
			\\

			$n=1$ 
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-3}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-4}} &
			$n=6$ &
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-13}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-14}}
			\\

			$n=2$ 
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-5}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-6}} &
			$n=7$ &
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-15}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-16}}
			\\

			$n=3$ 
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-7}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-8}} &
			$n=8$ &
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-17}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-18}}
			\\

			$n=4$ 
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-9}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-10}} &
			$n=9$ &
			\parbox[c]{\plotw}{\includegraphics[scale=0.125]{Plotsdecoding/R/plots-19}} &
			\parbox[c]{\plotwa}{\includegraphics[scale=0.18]{Plotsdecoding/R/plots-20}}
			\\

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
			
	\caption{\label{table:Rbasis}
	Bispectrum basis shapes $\Rbasis{n}$ in 2d and 3d plots
	up to $n=9$.}

	\end{sidewaystable}

	
	
	\clearpage
	
	Any arbitrary bispectrum shape will thus be the 
	product of a linear combination of the 
	fundamental $\Rbasis{n}$ basis:
	\begin{figure}[htpb]
\begin{center}
\includegraphics[width=14cm]{modal-decomposition.jpg}
\label{fig:modal-decomposition}
\caption{An arbitrary bispectrum built as a linear
combination of fundamental harmonic 
shapes.}
\end{center}
\end{figure}
	
	
	\subsubsection{Orthogonal combinations}
	That we can expand a bispectrum shape in 
	fundamental, orthogonalised harmonics is not surprising. This is 
	\textit{always} permissible.
	For our purposes, however, the $\Rbasis{n}$ depicted in the table
	\ref{table:Rbasis} are particularly useful
	since the first three partial waves
	provide a very good description of the {\Equilateral}, {\Orthogonal}
	and {\Enfolded}
	templates.
	Indeed, these can all be obtained by shifting the {\Equilateral} shape by
	a constant \cite{Senatore:2009gt,Chen:2010xka}.
	The $\Rbasis{0}$ shape is the constant shift.
	The ``first harmonic,''
	$\Rbasis{1}$, peaks in the equilateral limit,
	whereas $\Rbasis{2}$ peaks in the \emph{flattened} configuration,
	where $\alpha = \beta = 0$ (this makes $k_i=k_j=k_k/2$).




	We quote the expansion coefficients $\alpha_n$ for the
	common templates in table~\ref{table:Rtemplates},
	obtained using Eq.~\eqref{eq:r-expansion}.
	For the reasons we have explained,
	the {\Equilateral}, {\Orthogonal} and {\Enfolded} templates
	are dominated by $\{ \Rbasis{0}, \Rbasis{1}, \Rbasis{2} \}$,
	and for higher $n$ we observe the corresponding $\alpha_n$
	decrease.
	This explains why the shapes $S_H$ in Eq.~\eqref{eq:o-def}
	and $O$ depicted in table \ref{table:orthogonal-plots} 
	have negligible overlap with the {\Orthogonal} template,
	even though this was not guaranteed by its construction.
	On the other hand,
	the {\Local} shape does not have a rapidly convergent expansion
	because its squeezed divergence requires a
	comparatively larger admixture of
	modes with $n \gg 1$.
	As a result the $\Rbasis{n}$-basis
	is particularly well-adapted for an efficient description of
	the
	higher-derivative
	self-interactions of $\zeta$,
	like those arising in DBI inflation, which typically do not generate
	such divergences.

\vspace*{0.8cm}
	
\begin{table}[h]

	\tablepreamble
		
	\sbox{\tableA}{%
		\begin{tabular}{QqQqQqQqQqQ}

			\toprule

			&
			\multicolumn{1}{c}{$\alpha_0$} &
			\multicolumn{1}{c}{$\alpha_1$} &
			\multicolumn{1}{c}{$\alpha_2$} &
			\multicolumn{1}{c}{$\alpha_3$} &
			\multicolumn{1}{c}{$\alpha_4$} &
			\multicolumn{1}{c}{$\alpha_5$} &
			\multicolumn{1}{c}{$\alpha_6$} &
			\multicolumn{1}{c}{$\alpha_7$} &
			\multicolumn{1}{c}{$\alpha_8$} &
			\multicolumn{1}{c}{$\alpha_9$}

			\\

			\cmidrule{2-11}


			\text{{\Local}} &
			-2.16 & 1.78 & 0.75 & -1.21 & 0.79 &-0.49 & 0.85 & 1.01 &-0.53  & -0.55\\

			\cmidrule{2-11}

			\text{{\Equilateral}} &
			0.52 & 0.23 & -0.16 & -0.03 & -0.01 & 0.02 & 0.00 & 0.05 & 0.02 & -0.01 \\

			\cmidrule{2-11}

			\text{\textsf{orthogonal}} &
			-0.44 & 0.68 & -0.49 & -0.10 & -0.04 & 0.07 & 0.01 & 0.13 & 0.05 & -0.03 \\

			\cmidrule{2-11}

			\text{{\Enfolded}} &
			0.48 & -0.23 & 0.16 & 0.03 & 0.01 & -0.02 & 0.00 &  -0.04  & -0.02 & 0.01\\

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}


	\caption{\label{table:Rtemplates}Expansion of common templates
	in terms of the $\Rbasis{n}$ basis.}
	
	\end{table}
	
\vspace*{0.8cm}





	
	
	
	The idea that the orthogonalisation method suppresses,
	by construction,  the coefficients of the first fundamental harmonics
	$\{ \Rbasis{0}, \Rbasis{1}, \Rbasis{2} \}$, emerges from 
	the discussion above.
	We give $\alpha_n$ for the
	various `new,' orthogonally designed shapes
	discussed in \S\ref{subsec:bispectrum-shapes-NO}
	on table~\ref{table:Rorthogonal}.
	We observe that the $\Rbasis{0}$
	shape is projected out entirely both for
	the shape of Creminelli {\etal}
	and
	the $S_H$-shape
	in Eq.~\eqref{eq:o-def}.
	The situation for the $O$ shape seems more complicated,
	as previously anticipated, and we exclude it from our analysis
	for simplicity.
	For the other two shapes,
	the $n = 1,2$ harmonics are not completely removed but their
	amplitudes are significantly damped.
	The largest individual term in each orthogonalised shape
	is a nearby higher mode---in this case,
	the $n=3$ term. (This is the next highest, although recall that
	the precise
	ordering of the $\Rbasis{n}$ is somewhat arbitrary.)
	There is an admixture of the other harmonics with smaller
	amplitudes.
	Comparison with table~\ref{table:Rbasis}
	shows
	that the large $n=3$ contribution
	is essentially responsible
	for the common appearance of drumlin features.
\newpage

\clearpage




	\begin{sidewaystable}[htpb]


	\tablepreamble
		
	\sbox{\tableA}{%
		\begin{tabular}{QqQqQqQqQqQ}

			\toprule

			&
			\multicolumn{1}{c}{$\alpha_0$} &
			\multicolumn{1}{c}{$\alpha_1$} &
			\multicolumn{1}{c}{$\alpha_2$} &
			\multicolumn{1}{c}{$\alpha_3$} &
			\multicolumn{1}{c}{$\alpha_4$} &
			\multicolumn{1}{c}{$\alpha_5$} &
			\multicolumn{1}{c}{$\alpha_6$} &
			\multicolumn{1}{c}{$\alpha_7$} &
			\multicolumn{1}{c}{$\alpha_8$} &
			\multicolumn{1}{c}{$\alpha_9$}

			\\

			\cmidrule{2-11}


			\text{$S_H$-shape} &
			0.000 & 0.006 & 0.006 & 0.010 & 0.005 & -0.002 & -0.002 & -0.005 &-0.003  & 0.002\\

			\cmidrule{2-11}

			\text{$O$-shape} &
			0.047 & -0.190 & -0.100 & -0.107 & -0.024 & 0.026 & 0.028 & 0.043 & 0.024 & -0.019 \\

			\cmidrule{2-11}

			\text{Creminelli \etal\, shape} &
			0.000 & 0.015 & 0.019 & 0.024 & 0.011 & -0.006 & -0.002 & -0.012 & -0.006 & 0.003 \\

		

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}


	\caption{\label{table:Rorthogonal}Expansion of the $S_H$-shape
	(defined at leading-order in slow-roll),
	 the $O$-shape (defined at next-order in slow-roll)
	\cite{Burrage:2011hd} and 
	the Creminelli~{\etal} shape \cite{Creminelli:2010qf}
	in terms of the $\Rbasis{n}$ basis.}
	
	\end{sidewaystable}

\clearpage



	In table~\ref{table:ortho-approx-crazy-shapes}, the right-hand columns
	give an approximation to each exact shape, built from the
	first ten $\Rbasis{n}$.
	We quote the corresponding cosines in
	table~\ref{table:cosines-approx}.
	The approximations are rather good, resulting in cosines
	in excess of 0.99.
		Given a set of trial shapes,
	which could presumably be generated by considering arbitrarily
	exotic higher-derivative operators in the Lagrangian,
	this basis
	could be constructed precisely by
	the Gram--Schmidt procedure described 
	in \S\ref{subsec:bispectrum-shapes-NO}.
	



	\begin{table}[htpb]
	
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}

    \sbox{\boxplot}{%
    	\includegraphics[scale=0.12]{Plots/Orthogonal/alpha1/Babich/3D/O}
    }
    \settowidth{\plotw}{\usebox{\boxplot}}
    \sbox{\boxplota}{%
    	\includegraphics[scale=0.14]{Plots/Orthogonal/alpha1/Babich/2D/O}
    }
    \settowidth{\plotw}{\usebox{\boxplota}}
    
    \sbox{\tableA}{%
		\begin{tabular}{ccccc}

			\toprule

			\multicolumn{2}{c}{Shapes } & \multicolumn{1}{c}{} &
			\multicolumn{2}{c}{Approximations} 
			\\
			
			\cmidrule(r){1-2}
			\cmidrule(l){4-5}	
			
			\multicolumn{5}{c}{$S_H$ shape}
			\\			

			
			
			\parbox[c]{\plotw}{\includegraphics[scale=0.12]{Plotsdecoding/orthofergusson/plots-1}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.14]{Plotsdecoding/orthofergusson/plots-2}}& &
			\parbox[c]{\plotw}{\includegraphics[scale=0.12]{Plotsdecoding/OrthoApprox/Fergusson/2D/plots-17}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.14]{Plotsdecoding/OrthoApprox/Fergusson/3D/plots-18}}
			\\
\midrule


\multicolumn{5}{c}{$O$ shape}
			\\
			
				\parbox[c]{\plotw}{\includegraphics[scale=0.12]{Plotsdecoding/Orthogonal/alpha1/Fergusson/2D/O}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.14]{Plotsdecoding/Orthogonal/alpha1/Fergusson/3D/O}}& &
			\parbox[c]{\plotw}{\includegraphics[scale=0.12]{Plotsdecoding/OrthoApprox/Fergusson/2D/plots-5}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.14]{Plotsdecoding/OrthoApprox/Fergusson/3D/plots-6}}
			\\

			\midrule
			
			\multicolumn{5}{c}{Creminelli {\etal} shape}
			\\
			
			\parbox[c]{\plotw}{\includegraphics[scale=0.12]{Plotsdecoding/Creminelli/Fergusson/2D}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.14]{Plotsdecoding/Creminelli/Fergusson/3D}}& &
			\parbox[c]{\plotw}{\includegraphics[scale=0.12]{Plotsdecoding/OrthoApprox/Fergusson/2D/plots-29}} &
			\parbox[c]{\plotw}{\includegraphics[scale=0.14]{Plotsdecoding/OrthoApprox/Fergusson/3D/plots-30}}
			\\
			
			

			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}
			
	\caption{\label{table:ortho-approx-crazy-shapes}
	Approximations to the $S_H$-shape and similar bispectra, 
	up to the first ten harmonics in the $\mathcal{R}_n$
	expansion. The coefficients $\alpha_n$ are listed
	in table~\ref{table:Rorthogonal}.
	}

	\end{table}






\begin{table}[h]

	\tablepreamble
		
	\sbox{\tableA}{%
		\begin{tabular}{QqQq}
			 	\toprule

			&
			\multicolumn{3}{c}{Approximations to orthogonal shapes}
			\\

			\cmidrule{2-4}

		 	&
		 	\multicolumn{1}{c}{\text{$S_H$ shape}} &
		 	\multicolumn{1}{c}{\text{Creminelli \etal\, shape}} &
		 	\multicolumn{1}{c}{\text{$O$ shape}} 
		 	
		 	\\

			\midrule

			\text{$S_H$ shape} &

			 0.99&
			 0.98 & 0.89
			 
			\\

			\cmidrule{2-4}

			\text{Creminelli \etal \, shape} &
			 	0.97& 0.99
			  & 0.88
			
			
			\\

		

			\cmidrule{2-4}

			\text{$O$ shape} &
				0.82  &
			0.83
			 & 1.00
			
			\\


			\bottomrule

		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
	\end{center}

	\renewcommand{\arraystretch}{1}
	
	\sbox{\tableB}{%
	}
	
	\begin{center}
		\usebox{\tableB}
	\end{center}


	\caption{\label{table:cosines-approx}Cosines between 
	$\Rbasis{n}$-approximations to the orthogonal shapes
	depicted in table~\ref{table:ortho-approx-crazy-shapes}
	and the corresponding exact shape.}
	
	\end{table}






	

	\subsection{Distinguishing microphysics}
	\label{subsec:distinguishing-microphysics}
	The discussion above implies that, instead of obtaining orthogonal
	combinations from the terms 
	in Eq. \eqref{eq:start_ortho},
	it may be possible to do just as well with the $\Rbasis{n}$
	themselves.
	
	As we concluded in the last section, the recurrent appearance of
	the drumlin-like shape
	in table~\ref{table:ortho-approx} suggests
	that the \emph{shape} of the bispectrum itself will not serve 
	as a sensitive
	discriminant of microphysics.
	Most of all, it may not be an appropriate 
	diagnostic tool compared with the unprecedented 
	sensitivity of \textit{Planck}'s data.
	A significant {\Local} mode will favour dominantly
	local interactions,
	driven by gravitational evolution---usually this is related with a strong coupling between scalar 
	field fluctuations and the gravity sector.
	On the other hand, a significant {\Equilateral} mode will favour
	strong, higher-derivative self-interactions.
	However, it seems difficult to be more precise.
	Instead of focusing on shapes, it may be
	more profitable to study relations between their
	fundamental 
	\emph{amplitudes}
	in order to distinguish amongst competing inflationary scenarios.
	
	\subsubsection{Partial-wave amplitudes}
	To proceed, we define a set of dimensionless amplitudes
	$\beta_n$ for an arbitrary bispectrum $B$,
	\begin{equation}
		\iprod{B_{k_\ast}}{\Rbasis{n}} \equiv  \beta_n \  \Ps^2(k_\ast) \ \ ,
		\label{eq:beta-hierarchy}
	\end{equation}
	where $\Ps$ is the dimensionless power spectrum
	of the primordial curvature perturbation.
	We will elaborate on the scale $k_\ast$ below.
	The $\beta_n$ are similar to the
	amplitudes $\fNL$, but they are rather defined with respect to 
	an inner product.
	
	Any predictive Lagrangian will depend on only a \textit{finite} number
	of unknown parameters. If enough $\beta_n$ can be estimated
	from data,
	then Eq.~\eqref{eq:beta-hierarchy} allows these parameters
	to be expressed in terms of measurable quantities.
	The remaining relations in Eq.~\eqref{eq:beta-hierarchy},
	when expressed in terms of these measurable quantities,
	constitute predictions of the theory.
	In the inflationary literature such relationships are typically
	known as \textit{consistency relations},
	and were introduced by Copeland {\etal}
	in 1993 \cite{Copeland:1993jj,Copeland:1993zn}.
	In the language of particle physics they are
	``observables in terms of observables''---predictions which
	are independent on the parametrisation of the theory,
	and which
	the renormalisation programme has taught us represent
	the physical (not the bare) content of any quantum field theory.
	Their power lies precisely in providing important tests of entire
	classes of models.
	These consistency relations are analogous to the ones derived
	in \S\ref{sec:tensor} on tensor modes.

	In practice, the precise $\beta_n$ depend on the definition of
	the inner product, and indeed will vary between experiments.
	To perform a satisfactory analysis, one should obtain survey-dependent
	predictions for the $\beta_n$.
	The primordial bispectrum should be propagated to the surface of
	last scattering and projected on to the sky,
	and the $\beta_n$ should be computed in the resulting
	two-dimensional inner product.
	The set of basis shapes
	should be orthogonal when measured using the experiment in question,
	and may not be directly related to the $\Rbasis{n}$.
	This will lead to numerically different $\beta_n$ for each survey.
	Conversely, one can evolve the CMB bispectrum extracted from the data
	 and the $\beta_n$
	backwards, to obtain the respective primordial objects, and then compare them
	with the theoretical estimates.
	In either case, a more precise analysis 
	than the one we attempt to produce here 
	would have to be performed.
	
	In what follows, we work
	for illustrative purposes with
	the primordial, three-dimensional
	bispectrum rather than the projected bispectrum.
	We make a number of simplifications.
	We use the inner product~\eqref{eq:inner-prod-def}
	in a scale-invariant approximation, in the 
	sense described in \S\ref{subsec:power-law}.
	In evaluating $\iprod{B}{\Rbasis{n}}$
	one must choose a reference scale, $k_\ast$, at which
	$B$ is evaluated.
	The bispectrum then contains scale-dependent logarithms of the
	form $\ln (k/k_\ast)$, as discussed in \S\ref{sec:3pf},
	making $\iprod{B}{\Rbasis{n}}$ also a function of $k_\ast$.
	The (dimensionless) power spectrum on the right-hand side of Eq.~\eqref{eq:beta-hierarchy}
	is meant to be evaluated at $k_\ast$ as well.
	Because our implementation of the inner product
	does not retain scale information, we cannot apply this prescription
	precisely. We replace such logarithms
	by $\ln (k/k_t)$, where $k_t$ is the perimeter of the triangle.
	This is likely to make an impact on $\beta_n$
	at next-order, which should therefore be considered approximate.
	However, for the purposes of illustrating the construction 
	of the coefficients $\beta_n$, these assumptions are 
	not restrictive.
	
	We apply the method described above to two different models.
	
	
	\subsubsection{Case study: DBI inflation}
	As an illustration, we consider DBI inflation governed by
	the action
	\begin{equation}
		S = \int \d^4 x \; \sqrt{-g} \bigg\{
			- \frac{1}{f(\phi)} \left[
				\sqrt{1 - f(\phi)\ X} - 1
			\right] - V(\phi)
		\bigg\} \ \  ,
		\label{eq:dbi}
	\end{equation}
	where $X = -(\partial \phi )^2$.
	We discussed this model in \S\ref{sec:dbi}.
	This is a special action in the Horndeski class, and 
	it is known to lead  
	to strong non-gaussianities
	if $\gamma \gtrsim 1$ \cite{Alishahiha:2004eh,Chen:2006nt},
	where $\gamma \equiv (1 - f \dot{\phi}^2)^{-1/2}$.
	In what follows we will be interested in the case 
	where $\gamma$ is, at least, moderate.
	The algebraically special structure of the action
	makes the coefficients of the Lagrangian operators
	stable against quantum corrections.
	
	The inflationary fluctuations in this model depend on the
	parameters
	defined in Eq. \eqref{eq:srFranche} \cite{Franche:2009gk}, 
	which we recall here
	\begin{equation}
		\varepsilon_V = \frac{1}{2} \left( \frac{V'}{V} \right)^2 \ ,
		\quad
		\eta_V = \frac{V''}{V}\  ,
		\quad
		\text{and}
		\quad
		\Delta = \sgn(\dot{\phi} f^{1/2}) \, \frac{f'}{f^{3/2}} \frac{1}{3H} \ \ ,
		\label{eq:dbi-sr}
	\end{equation}
	where primed quantities are differentiated with respect to $\phi$
	 (and not conformal time).
	Typically, these must be small.
	The bispectrum was determined to $\Or(\varepsilon, \eta, \Delta)$
	in \S\ref{sec:dbi}, to which we refer the reader for details.

	
	The Lagrangian depends on the three parameters
	in Eq.~\eqref{eq:dbi-sr} and $\gamma$.
	We will therefore require \emph{four} observables
	to fix them. A further \emph{fifth} 
	observable enables the theory
	to be tested. The presently well-measured parameters
	are only the amplitude, $\Ps$, and tilt, $n_s$,
	of the scalar power spectrum.
	There are relatively weak constraints on a few modes of the bispectrum.
	In the future, possibly with \textit{Planck}, 
	we might be able to detect the tensor amplitude
	$\Ps_t$.
	Assuming it will eventually be possible to measure
	$\beta_0$ and $\beta_1$ together with the tensor-to-scalar
	ratio, $r \equiv \Ps_t / \Ps$,
	then
	using the results of \S\ref{sec:dbi}, we find
	\begin{equation}
		\left(2.88\, \frac{\beta_1}{\beta_0} - 1\right)
			=
			1.93 (n_s - 1)
			+ 0.03 r \sqrt{-\beta_0}
			+ 2.87 \left(
				6.60 \, \frac{\beta_2}{\beta_0} + 1
			\right)  \ \ .
		\label{eq:dbi-consistency-r}
	\end{equation}
	
	One of the results from our analysis is that the
	 DBI model predicts $\beta_0 < 0$
	if the bispectrum is large enough to be observable,
	as we will explain below.
	If $r$ cannot be measured, or only with poor accuracy, then it
	will be necessary to use $\beta_3$ as a substitute. In this case,
	we find
	\begin{equation}
		\left(2.88 \frac{\beta_1}{\beta_0} - 1\right)
			=
			0.65 (n_s - 1)
			- 0.02 \left(
				6.60 \frac{\beta_2}{\beta_0} + 1
			\right)
			- 0.17 \left(
				34.98 \frac{\beta_3}{\beta_0} + 1
			\right) \ \ .
		\label{eq:dbi-consistency-beta3}
	\end{equation}
	
	In 
	Eqs.~\eqref{eq:dbi-consistency-r}--\eqref{eq:dbi-consistency-beta3}
	we must recall that observables (such as the $\beta_n$)
	may mix Lagrangian \emph{parameters}
	at lowest-order, next-order and possibly other higher-orders.
	The $\beta_n$ begin at lowest-order, whereas $(n_s - 1)$
	and $r$ begin at next-order in slow-roll.
	Indeed, we find this is the case. 
	This can be seen from inspection of 
	Eqs.~\eqref{eq:dbi-consistency-r}--\eqref{eq:dbi-consistency-beta3}: 
	the numerical coefficients multiplying 
	$(n_s-1)$ and $\beta_2/\beta_0$ differ in 
	both equations.
	
	In obtaining these equations we have assumed
	that each term in Eq. \eqref{eq:dbi-consistency-beta3} 
	is roughly of the same order of magnitude, that is
	\begin{equation}
		\left|
			2.88 \frac{\beta_1}{\beta_0} - 1
		\right|
		\sim
		\left|
			6.60 \frac{\beta_2}{\beta_0} + 1
		\right|
		\lesssim
		|n_s - 1|
		\sim
		r \ \  .
		\label{eq:hierarchy}
	\end{equation}
	Which of these two equations, \eqref{eq:dbi-consistency-r} or
	\eqref{eq:dbi-consistency-beta3},
	is more useful will depend on the relative difficulty of measuring
	$r$ and $\beta_3$.
	These expressions constitute a \emph{model-independent} test of the
	DBI framework: they hold for any
	DBI action, up to
	$\Or(\varepsilon, \eta, \Delta)$, no matter what potential or warp factor
	is chosen. They are written in terms of observables only.
	By
	showing that relations such as \eqref{eq:dbi-consistency-r} or
	\eqref{eq:dbi-consistency-beta3} are not satisfied,
	one could rule out the DBI action as the origin of the inflationary
	perturbations.
	
	Unfortunately, there is no one-to-one mapping from models
	to consistency relations such
	as~\eqref{eq:dbi-consistency-r}--\eqref{eq:dbi-consistency-beta3},
	and determining that any such equation \emph{is} satisfied
	does not provide decisive evidence in favour of a model.
	The utility of such equations lies, on the other hand, 
	with their power to rule models
	out.
	Showing that the $\beta_n$ satisfy
	a hierarchy of consistency equations derived from some
	Lagrangian would, nevertheless, be circumstantial evidence in \textit{favour} of
	that model, especially if the agreement
	persists to large $n$.
	
	As mentioned above, Eqs.~\eqref{eq:dbi-consistency-r}--\eqref{eq:dbi-consistency-beta3}
	are analogues of the ``next-order'' consistency equations
	for the tensor tilt, $n_t$ [cf. Eqs. (5.6)--(5.7) of
	Lidsey~{\etal}~\cite{Lidsey:1995np}].
	If the $\beta_n$ cannot be determined with sufficient accuracy
	to test these equations, we can obtain a simpler set of ``lowest-order''
	relations obtained by systematically neglecting next-order terms
	in the slow-roll approximation.
	This entails assuming $(n_s - 1) \simeq r \simeq 0$ in Eq. \eqref{eq:hierarchy}.
	Together with~%
	\eqref{eq:dbi-consistency-r}--\eqref{eq:dbi-consistency-beta3},
	Eq.~\eqref{eq:hierarchy} then implies
	\begin{equation}
		2.88 \frac{\beta_1}{\beta_0} \simeq
		-6.60 \frac{\beta_2}{\beta_0} \approx  1 .
		\label{eq:dbi-simple}
	\end{equation}
	Even more simply, Eq.~\eqref{eq:dbi-simple}
	requires $\beta_0$ and $\beta_1$ to have the same sign,
	and $\beta_2$ to have the opposite sign.
	By consulting the individual expressions for the $\beta_n$,
	it follows that $\beta_0$ and $\beta_1$ must be negative,
	but $\beta_2$ should be positive
	whenever $\gamma$ is moderately large.
	This more primitive test 
	of the consistency relations
	is applicable even if the $\beta_n$ cannot be
	determined accurately.
	In the present framework,
	it is a manifestation of the well-known
	result that the DBI model produces $\fNL^{\mathrm{(equilateral)}} < 0$,
	whereas WMAP data favour $\fNL^{\mathrm{(equilateral)}} \gtrsim 0$.
	For this reason, present-day observations are
	already sufficient to disfavour
	DBI inflation.
	
	We note that
	Eq.~\eqref{eq:dbi-simple},
	and similar expressions for
	$\beta_n$ with $n > 2$, express the expected
	decrease in amplitude of $\iprod{B}{\Rbasis{n}}$
	with increasing $n$.
	The decrease is not monotonic, because the spikes which appear in
	$\Rbasis{n}$ at larger $n$ cause a small enhancement.
	However, the $n = 0,1,2$ harmonics are larger than the rest,
	which is required by the analysis of \S\ref{subsec:harmonic-decomposition}.
	
	
	\subsubsection{Case study: $k$-inflation}
	For comparison, consider the power-law $k$-inflation model of
	Armend\'{a}riz-Pic\'{o}n, Darmour \& Mukhanov ~\cite{ArmendarizPicon:1999rj}, 
	which we discussed in \S\ref{sec:k-inflation}.
	The action for this model satisfies
	\begin{equation}
		S = \int \d^4 x \, \sqrt{-g} \; \frac{4}{9} \frac{4-3\gamma}{\gamma^2}
			\frac{X^2 - X}{\phi^2} \ \ .
	\end{equation}
	It admits an inflationary solution for $X=(2-\gamma)/(4-3\gamma)$ 
	provided $0 < \gamma < 2/3$, unrelated to the Lorentz factor in 
	the DBI model.
	In the
	limit $\gamma \ll 1$, and
	keeping only leading-order terms, this model predicts
	\begin{equation}
		2.61 \frac{\beta_1}{\beta_0} =
		- 4.80 \frac{\beta_2}{\beta_0} = 1 \ \  .
		\label{eq:k-simple}
	\end{equation}
	Comparison with Eq. \eqref{eq:dbi-simple}
	for the DBI consistency relations shows that it
	would be necessary to measure $\beta_0 / \beta_1$ to
	about $10\%$ in order to distinguish these models.
	A sufficiently accurate measurement of $\beta_2$
	would make the test considerably easier to apply.
	Just like for DBI, $\beta_0$ is also negative for $k$-inflation.
	
	This method is closely related to a
	trispectrum-based
	test for single-field inflation
	proposed by Smidt {\etal}~\cite{Smidt:2010ra}.
	The trispectrum contains contributions from two different
	`{\Local}' shapes, with amplitudes parametrized by $\tauNL$
	and $\gNL$
	\cite{Sasaki:2006kq,Byrnes:2006vq,Seery:2006js}.
	The $\tauNL$ contribution obeys the
	Suyama--Yamaguchi inequality $\tauNL \geq (6 \fNL^{\mathrm{local}} / 5)^2$
	\cite{Suyama:2007bg,Smith:2011if}, 
	where the equality applies to single-source models.
	Smidt~{\etal} suggested studying
	$A = \tauNL / (6 \fNL^{\mathrm{local}}/5)^2$,
	which is analogous to the ratios $\beta_n / \beta_0$
	introduced above.
	Their analysis suggested that \textit{Planck} may be able to
	measure $A$ to $\pm 1.0$ at $1\sigma$, and a future CMB satellite
	may even be able to achieve $\pm 0.3$
	with the same significance.
	An accurate measurement of $A > 1$ would be sufficient to rule out
	single-field scenarios.

	In summary, like the well-known
	standard inflationary consistency relations,
	whether relations
	such as Eqs. \eqref{eq:dbi-consistency-r}--\eqref{eq:dbi-simple}
	and Eq. \eqref{eq:k-simple}
	are useful in practice will depend
	on the accuracy with which each component can be measured.
	This depends on the signal-to-noise associated with each
	harmonic shape.
	However, the method we have described can be implemented
	with \emph{any} suitable basis; it is not restricted to the
	$\Rbasis{n}$ functions described above.
	Nevertheless, our choice of $\Rbasis{n}$ makes it transparent that
	one can think about the templates used in the CMB analysis 
	arising as the first harmonics. After applying 
	the orthogonalisation 
	procedure, a shape given by higher-order 
	harmonics emerges as a result.






\section{Summary of results}
\label{sec:summary4}
In this chapter we have explored the scale
and shape-dependences of the bispectrum in single-field inflation models.
Our main findings are summarised as follows.



	
	\subsection*{``New'' bispectrum shapes}
	Our results capture the shape-dependence of the bispectrum
	even in the squeezed limit. Therefore,
	we are able to fully determine the relationship between the
	leading and next-order shapes in the slow-roll approximation,
	discussed in \S\ref{sec:shapes}.

	Working in a $P(X, \phi)$ model, the enhanced part of the leading-order
	bispectrum is well-known to correlate with the
	equilateral template.
	Only two shapes are available,
	plotted in
	Table~\ref{table:lowest-order-shapes},
	and the bispectrum is a linear
	combination of these.
	If enough fine-tuning is allowed, one
	is able to produce a distinctive shape, 
	at leading-order, which does not correlate with 
	the typical templates used in CMB analysis.
		This shape is very similar to a `new' shape constructed by
	Creminelli {\etal} \cite{Creminelli:2010qf},
	working in an
	entirely different model---a galilean shift-invariant Lagrangian
	with at least two derivatives applied to the field.
	
	
	The next-order bispectrum is a linear combination of \emph{seven}
	different shapes, although these cannot be varied independently:
	strong correlations among their coefficients are imposed by the
	$P(X,\phi)$ Lagrangian. Many of these shapes also correlate with
	the \textsf{equilateral} mode, but two of them are different:
	in the language of \S\ref{sec:shapes}, these are
	$S'_\varepsilon$ and $S_s$.
	For typical values of $\alphalambda$
	(which is the $\cs^{-2}$-enhanced part of $\lambda / \Sigma$),
	one can obtain
	a linear combination of the next-order shapes
	orthogonal to both lowest-order shapes.
	This is the orthogonal shape $O$ in
	Table~\ref{table:orthogonal-plots}.
	
	

	We conclude that provided we are willing to tolerate 
	a large fine-tuning of the coefficients $g_i$
	(or a large overall amplitude of the primordial
	 bispectrum), 
	this `new'-shape can always be produced in 
	the bispectrum of any single-field theory.
	Therefore, the presence of this shape cannot be 
	used as a diagnostic tool to support 	a specific model.
	This suggests performing a different kind of analysis
	to the bispectrum shapes.
	





	\subsection*{Insights from the modal decomposition}
Motivated by the recurrent presence of the shape with drumlin features, 
we have turned in \S\ref{sec:modal-decomposition} 
to the modal decomposition of the CMB bispectrum,
originally proposed by Fergusson \& Shellard
\cite{Fergusson:2008ra,Fergusson:2009nv}.
The decomposition into fundamental harmonics is 
naturally designed to study correlations among the
	amplitudes of shapes which \emph{are} present
	in the primordial bispectrum.
	A given Lagrangian will typically generate fluctuations which
	depend on a finite number of parameters. If enough
	modes of the bispectrum can be determined with sufficient accuracy,
	these parameters can be written in terms of observable
	quantities. Further observations then constitute
	tests of a particular theory, and can ultimately allow us to 
	reduce the number of competing inflationary models.

	As an illustration, we have applied our method
	to DBI inflation with an arbitrary potential and warp factor.
	We compared the resulting consistency relations with the 
	ones obtained in the $k$-inflation scenario.
	With sufficiently accurate observations it may be possible
	to distinguish these models.
	Similar tests can be devised for any single-field
	inflationary model.
	
	For an arbitrary Horndeski model, 
	only \textit{five} measurements of the correlations 
	between the primordial
	bispectrum and the (first five) fundamental harmonics
	are required to know the coefficients $g_i$.
	Further measurements break the degeneracy amongst
	the dynamical quantities from which each $g_i$ is built, 
	and also allow us to test the theory against observations.
	

%\clearpage 
\newpage
\thispagestyle{empty}
\newpage
%
%\clearpage




==> seven.tex <==


\begin{savequote}[30pc]

Anyway, I think that numbers are a problem in Astronomy, sizes and numbers. 
The best thing to do is to relax and enjoy the tininess of us 
and the enormity of the rest of the universe. 
Of course, if you are feeling depressed by that, 
you can always look out the other way and 
think how big you are compared to the atoms and the parts of atoms, 
and then you are the enormous universe to those atoms. 
So you can sort of stand in the middle and enjoy everything both ways.

 
\qauthor{Richard Feynman [Fun to Imagine, chapter 5 ``Big numbers'', 1983]}
\end{savequote}





\chapter{Discussion}
\label{chapter:seven}
\hrule
\vspace*{0.5cm}

In this thesis we have discussed the early inflationary 
era driven by a single scalar field, and studied the 
preheating mechanism after a Dirac--Born--Infeld period of inflation.
We will recapitulate in \S\ref{conclusions:questions} 
the questions which motivated the writing up 
of this thesis, and in \S\ref{conclusions:summary}
we will summarise what we have learned in the process.
Finally, we present in \S\ref{conclusions:outlook}
a critical analysis of this work and 
suggest directions for further research.








\section{Questions addressed in this thesis}
\label{conclusions:questions}
To understand which microphysics describes the 
early universe is one of the greatest challenges in 
cosmology. Our only clues have been encoded in the CMBR
almost 14 billion of years ago and are at present being 
mapped with high-sensitivity in sky surveys.
This is the oldest exploration in science.

Inflation has become a popular framework which,
together with quantum mechanics,
explains how small inhomogeneities developed on
a perfectly smooth background.
A period of inflation during the early universe 
is a simple idea that ameliorates the problems with the standard cosmological model.
In this thesis we have focused on inflation where
only one scalar degree of freedom, called the inflaton $\phi$, is active. 
As a result,
the comoving perturbation $\zeta$ synthesised during inflation
in these models
is only due to the quantum fluctuations of $\phi$.


During inflation cosmological scales were pushed outside 
the particle horizon. 
An important difference between single and 
multi-field inflation models is that the 
primordial perturbation $\zeta$ does not evolve on
super-horizon scales when only adiabatic modes 
are present. This implies that studying single-field inflation models
is comparatively simpler.

The \textit{Planck} satellite will soon be delivering data that 
it has been collecting since its launch, in 2009.
The huge expectations created around \textit{Planck} 
lie in its ability to make measurements with an
unprecedented sensitivity. 
It might even exhaust the amount of information
about the early universe dynamics one is able to extract from CMB observations.
On the theory side, there has been a massive effort to 
understand the statistics of $\zeta$. 
If the signal is (even slightly) non-gaussian, 
we might be able to use it to gain access to 
the microphysical Lagrangian which governed interactions
in the early universe.

The eminent arrival of \textit{Planck}'s data poses at least two timely questions, 
which were the main motivation behind the first part of this thesis.
\begin{enumerate}[i.]
\item We need to be prepared to use \textit{Planck}'s exquisite sensitivity
to learn about inflation as much as we possibly can. 
Do we know what the error associated with the theoretical 
calculations of our models is? 
\item A significant effort has been devoted over the last decade to obtain 
the bispectrum in several classes of single-field inflation models.
Do we understand how to efficiently catalogue the single-field features
imprinted in the CMBR?
\end{enumerate}

	



As we have seen, the bispectrum of perturbations in single-field
inflation is an incredibly intricate function of the underlying 
microphysics. By learning more about its structure and 
characteristics we are 
increasing our chances to use \textit{Planck}'s data more efficiently.



We also turned our attention to single-field models 
which do not evolve under the slow-roll regime. 
In particular, we set the task of
obtaining the bispectrum signatures corresponding to models
where slow-roll was not satisfied, yet allowing
for a successful period of inflation and 
producing agreement with observation.



In part II we considered the end stage of a Dirac--Born--Infeld inflation model.
We wanted to understand how different the preheating 
mechanism would be compared to an analogous canonical model.
The details of the generation of $\zeta$ largely decouple from
the physics of preheating. Therefore, if a constraint 
arises from the preheating analysis, 
it could be used in 
conjunction with the constrains arising from the 
primordial density fluctuation.

As a result, one could 
use constraints arising 
from different, yet complementary 
sets of analysis. Ultimately, using constraints 
from the analysis of the bispectrum and preheating, 
together with 
observational data, the parameter space of these theories could become so
severely fine-tuned, that it could prove those models
highly unlikely. 





\section{Summary of the main results}
\label{conclusions:summary}
This thesis is by no means the end of the story 
for single-field inflation. We hope, however, that it has 
taken small steps towards decoding the bispectrum 
in single-field inflation models.
We list below a short summary of the main results 
reported in this thesis.


\para{A universal action for perturbations}In chapters 
\ref{chapter:two} and \ref{chapter:three} we have provided a full derivation
of the cubic action for the primordial 
perturbation in single-field models, which 
is \textit{exact} in the slow-roll approximation.
We have shown it can be written in terms of only
five \textit{Horndeski} operators, whose coefficients
are model-dependent. 

\para{Sizing the theory-error}We have computed a more precise estimate of the magnitude of 
the bispectrum in the slow-roll regime which reduces the previous 
theory-error by several tens of percent.
In DBI inflation for example, the uncertainty associated with 
previous estimates is reduced by more than 90\%.
This calculation was urgently required by the imminent arrival of 
\textit{Planck}'s data, which is expected to have a sensitivity 
far superior to the precision of our previous estimates.
In chapter \ref{chapter:three} 
we have reported an analysis of the rescaled magnitude of 
the bispectrum, $\fNL$, which is valid at 
\textit{next-order} in the slow-roll approximation.

We have applied our results to several classes of single-field models, and 
have specified $\fNL$ for some common momenta configuration.
We have concluded that the previous, leading-order results for $\fNL$,
were unexpectedly much more precise than estimated. 
However, without performing the computation
to next-order, it would not have been possible 
to specify the accuracy of the leading-order results.


\para{The universe of shapes}We started in chapter \ref{chapter:four} by giving a full
expression of the scale-dependence of the bispectrum.
The remaining of that chapter was devoted to a thorough
analysis of the shapes associated with each Horndeski operator
at leading and next-order in slow-roll.
We have rediscovered an exotic shape which had previously
appeared in a class of higher-derivative galileon theories. This shape
\textit{did not} correlate with any existing bispectrum templates in CMB analysis.
We found that this shape
can actually be constructed out of a linear combination of equilateral shapes, 
provided we are prepared to tolerate some serious fine-tuning.
The recurrence of this shape raised two fundamental problems.
First, why was this shape appearing in so many distinct microphysics
scenarios?
Second, if the presence of this shape could not be used as a diagnostic
tool, then how could we use the bispectrum shape as a discriminant
between models?

These questions motivated a modal decomposition of the bispectrum, 
which revealed that on a particularly useful basis,
the usual templates could be well described by the 
first few modes. By requiring orthogonality with the templates, 
one was in fact enhancing the subsequent higher-order modes, which 
caused the drumlin-like features in the exotic shape.
We have learned that from a harmonic decomposition of the bispectrum, one 
is able to derive consistency relations between the amplitudes of each fundamental
mode.
Relations which are \textit{observables in terms of observables} 
are particularly powerful in ruling out models, since they are 
independent of the parametrisation of the theory.
We have specified these relations for DBI and $k$-inflation scenarios.




\para{Beyond the slow-roll approximation}In chapter \ref{chapter:five} we have abandoned the requirement of
slow-roll inflation. We have rather focused on the bispectrum phenomenology
of single-field models which predict an almost scale-invariant
spectrum, whilst allowing for some breaking of the slow-roll approximation.
The results of this chapter rely on the scale-invariant approximation, 
which can be regarded as a resummation technique of the 
slow-roll analysis in the parameter space compatible with a scale-invariant two-point function.

We have found that the resulting bispectrum is
strongly scale-dependent, and correctly reproduces the 
logarithmic dependence obtained in chapter \ref{chapter:three}
taking the slow-roll limit.
We have argued that because of this string scale-dependence, 
these models are more vulnerable to data constraints arising from different
scales (CMB and LSS).


\para{Preheating after DBI inflation}In the last chapter we have studied 
the preheating stage after a period of
Dirac--Born--Infeld inflation. 
We have focused on the main differences
between the resonances in particle production
compared to similar canonical models, and
considered the non-relativistic 
regime of DBI, when preheating can occur.
We have found that preheating is perturbatively 
more efficient in these scenarios, and that it allows
for production of inflaton particles. This is a novel feature
which does not find an analogue in canonical models
where only matter preheating takes place.
We have also estimated the reheating temperature 
in these models, and found it is slightly lower than in their canonical counterparts.





\section{Outlook}
\label{conclusions:outlook}

Figure 7.1 is intended to
roughly 
summarise some important advances in theoretical cosmology
(it is not to scale). 
The lower part of the cartogram zooms in 
some significant developments regarding inflation
and the early universe over the last decade.
The round rectangular shapes have width which is proportional
to the number of scientific papers whose topic is centred on 
non-gaussianities. In the last two years, the scientific production in 
this area has been greater than that from 2000 to 2006. 
This remarkable effort in attempting to understand 
the microphysics governing the early universe cannot be ignored. 
It is likely that further investigation will follow
the tendency in the last decade, and there is indeed much to be done.



\clearpage

\begin{figure}[htpb]
\begin{center}
\includegraphics[width=23cm, angle=90]{summary2.jpg}
\label{fig:summary}
\caption{Cartogram of significant developments in 
early universe theoretical cosmology roughly over the last 100 years.}
\end{center}
\end{figure}

\clearpage

\newpage

\thispagestyle{empty}

\newpage


In chapter \ref{chapter:four} we have obtained consistency relations
between the amplitudes of each bispectrum harmonic, $\beta_n$, in two different models.
For simplicity, our analysis assumed an almost scale-invariant bispectrum
and applied to the primordial bispectrum.
For a rigorous comparison to data which is likely to be necessary
given the unprecedented sensitivity offered by \textit{Planck}, 
an improved analysis must be performed. On the one hand, 
the choice of basis should be suitable for a bispectrum which
is not perfectly scale-invariant. 
In particular the CMB bispectrum shapes should be integrated over 
some range of cosmologically relevant scales, 
and this has been neglected in our analysis.
In that case, our choice of basis is weak.
On the other hand, we inevitably need to evolve the 
primordial bispectrum we have calculated to become the 
late-time, CMB bispectrum, which is visible in the data.
Conversely, one can use \textit{Planck}'s data and evolve it backwards
to obtain the primitive bispectrum, to which our formulae apply.



In chapter \ref{chapter:five} we have obtained the bispectrum
in single-field inflation theories without invoking the slow-roll approximation.
We have observed the bispectrum exhibits 
a strong scale-dependence, but we have left the 
study of shapes for future work.
It would be extremely interesting to investigate
the correlation between the slow-roll approximation and
the bispectrum shapes. Are the shapes similar to the ones found before
and well approximated by the common templates?
What would the modal decomposition reveal?

\vspace*{0.5cm}

In this thesis we have largely ignored the progress that 
has been made on multi-field theories. In these, more 
than one scalar field is active during inflation, and isocurvature
modes are not generally suppressed as a result.
Obtaining theoretical predictions in these models
is therefore rather challenging. For example, 
the amplitude of the bispectrum $\fNL$ can vary
significantly until the modes are frozen upon
horizon re-entry (see, for example, Ref. \cite{Elliston:2011dr}).
Numerical tools such as $\delta$N  \cite{Lyth:2005fi}, 
transfer matrices \cite{Amendola:2001ni}, 
and the moment transport equations \cite{Mulryne:2009kh, Mulryne:2010rp}
have been applied to obtain the evolution of the 
correlation functions in these models.
In multi-field models it is helpful to improve our
description of the inflationary trajectory in field configuration
space, and introduce the concept of \textit{bundle} of trajectories.
This concept can help us relate
a dramatic change in the magnitude 
of $\fNL$ close to a focusing region of trajectories. 
$\fNL$ will evolve until all isocurvature modes 
have decayed and $\zeta$ has become constant---we say  
the \textit{adiabatic limit} has been reached \cite{Elliston:2011dr}.

If \textit{Planck} rules out single-field inflation, this opens up 
an opportunity to develop models which are not as simple: 
multiple fields
allow for a much richer dynamics and 
can be in agreement with 
the observational data.
In particular, most of the work on multi-field inflation under the 
slow-roll approximation so far has focused 
on models where the fields have canonical kinetic terms
(see Refs. \cite{Vernizzi:2006ve, Seery:2012vj} 
for a small sample of these works).
It is important to extend these studies to models
which contain non-canonical fields and understand the
dynamics of inflation \cite{Langlois:2008wt, Langlois:2008mn, Langlois:2008qf}. 
Also relevant is to 
study the multi-field dynamics when 
some of the slow-roll parameters become temporarily large, 
making the slow-roll approximation invalid. 
Some works have performed an analysis which is higher-order in slow-roll
\cite{Avgoustidis:2011em}.
However, it is likely that more sophisticated techniques are required 
to describe the evolution of the multi-field system over the course of 
several e-folds without imposing slow-roll (see, for example, 
Ref. \cite{Dias:2012nf}).


This journey planner can suggest some of the near-future
challenges, but 
it is hard to gauge the precise direction research will take.
It will inevitably aim at some of our most elementary 
questions. Is inflation more than just a 
good theory? Did it really happen?
If so, what is the physical microscopical Lagrangian
describing these early times?
Understanding inflation may require setting it up 
in a string theory, 
but that is a different story.
In any case, we can anticipate that with 
the arrival of \textit{Planck}'s data we will be closer 
to understanding our early universe.

\clearpage

\begin{flushright}
\noindent ``Abre essa janela! Desvia-me a cortina! \\
Eu gosto de ver as nuvens... \\
E o c\'{e}u azul sobre os horizontes.\\
Gosto de contemplar os vales e os montes! \\
E tamb\'{e}m as fontes de \'{a}gua pura e cristalina! \\
Gosto de sentir a brisa! \\
Sentir o pulsar da Natureza e tudo o que se preza!…''

\vspace*{1cm}

\textit{\noindent[``Open that window! Divert me the curtain! \\
I like to see the clouds ... \\
And the blue sky on the horizon.\\ 
I like to contemplate the valleys and the hills! \\
And also the fountains of pure crystal water!\\ 
I like to feel the breeze! \\
To feel the pulse of Nature and all that cherishes!...''] 
}

\vspace*{0,5cm}
\noindent \textit{Joaquim Henriques}, unpublished work
\end{flushright}
\newpage


==> six.tex <==


\begin{savequote}[30pc]
The only mystery in the universe\\
Is that there is a mystery of the universe.\\
Yes, this Sun that unintentionally illuminates ...\\
Everything not even brings with it the explanation\\
Of existing, nor does it have mouth with which to speak.
\qauthor{Fernando Pessoa, in \textit{Fausto}}
\end{savequote}





\chapter{Preheating at the End of Inflation}
\label{chapter:six}

\hrule
\vspace*{1cm}

In the first part of this thesis we have focused 
on the inflationary imprints on the CMBR.
In particular, we have studied the bispectrum in single-field models
both using and discarding the slow-roll approximation. 
Our calculation not only reduces the theory-error associated with 
previous estimates, but it also makes small steps towards 
developing a potentially more appropriate 
diagnostic tool that enables telling models apart.

Whatever the microphysical origin of 
 the post-inflationary universe, we know that
the universe was almost empty at the end of inflation, 
as the number density in particles was diluted away 
by the exponential expansion. 
We thus find ourselves with two conceptual problems. 
First, the inflaton is not observed today.
Therefore, some mechanism must have caused its
energy density to dissipate. 
Second, matter is abundant all around us.
After all, we are made up of particles. So, 
how was the universe repopulated after inflation?

To answer these questions, we will discuss the phenomenology  
of preheating
in a DBI model in this short chapter. 
It is certainly not intended to signify a full study
of preheating in this model. We rather want to 
briefly analyse what are the main differences between preheating
in canonical and non-canonical models.
This chapter represents a departure from our 
previous programme of investigating non-gaussian features
in the bispectrum. 
We regard it as a 
transition from the study of the early universe 
during inflation, to the standard Big Bang model.




\para{Outline}We start by giving a short review of
some relevant historical developments in the 
theory of preheating in \S\ref{sec:preheating-introduction}, and 
briefly revisit the DBI model \S\ref{sec:dbi-dynamics}.
In \S\ref{sec:preheating} we discuss a 
DBI toy model in which inflation ends as the brane 
settles to its final position in the warped background. 
We show that this model is comparable to 
chaotic inflation in a theory with canonical kinetic terms, and 
discuss the parametric resonance event. 

In \S\ref{sec:reheating} we study the stage of perturbative 
reheating and provide an estimate for the reheating temperature
in models driven by a DBI kinetic term. 
We give a summary of our findings in \S\ref{sec:summary-preheating}.
Additional material related to this chapter is
collected in Appendix \ref{app6}.




This chapter is the result of work done in collaboration with 
Nazim Bouatta, Anne-Christine Davis and David Seery, and 
published as Ref. \cite{Bouatta:2010bp}.



\section{Preheating: development of a theory}
\label{sec:preheating-introduction}
In this chapter we are interested in understanding 
how the universe could have reheated after a period of 
DBI inflation. The DBI inflation model was discussed in 
\S\ref{subsec:power-law} from the point of view of 
an effective field theory. 
There, the inflaton was a scalar field whose dynamics 
was governed by the DBI action. 
Here, we review DBI from the 
brane world perspective, but perform our calculation 
from the quantum field theory point of view.

In the proposal set forth by Tong \& Silverstein
\cite{Silverstein:2003hf}, 
and later elaborated in collaboration with Alishahiha 
 \cite{Alishahiha:2004eh},
the DBI action describes the low-energy dynamics
of a D$3$-brane moving in a warped background space-time.
D-branes naturally arise in string theory and are extended objects 
in space-time where
open strings can end---for a review of their properties see the classic textbook
by Johnson \cite{Johnson:2003gi}.
		Inflation in these models was discussed 
		by
		Chen \cite{Chen:2005ad}, 
		and
		inflation in string cosmology has been reviewed by
		McAllister \& Silverstein
		\cite{McAllister:2007bg}. 

Reheating in related brane-world models has been studied
	in Refs.~\cite{Cline:2002it, Brodie:2003qv, Dvali:2003ar,
	Frey:2005jk, Chialva:2005zy}.
	Any inflationary theory needs to be completed through
	a reheating phase, which depends
	strongly on the details of the preceding inflationary phase 
	as emphasised in Refs. \cite{Kofman:1996mv,Kaiser:1995fb}.
	In principle, no two models find the same preheating phenomenology, 
	by which the universe is repopulated with matter particles.
	Preheating is a subtle function of the underlying physics, 
	probing information which can be regarded as 
	complementary to the
	physics of the density fluctuation, studied in part I of this thesis. 
	For this reason, competing inflationary models
	exhibit important differences in their preheating analysis.
	In particular, in this chapter we shall explore 
	this process and display the main dissimilarities between
	DBI models and those with canonical kinetic terms.
	Here, the DBI model is to be regarded as representative 
	of the non-canonical class.



Many authors have contributed to the theory of particle production,
	which is now well-developed in light of many authors' efforts
	\cite{Traschen:1990sw, Kofman:1994rk, Shtanov:1994ce, Kofman:1997yn}.
		The theory of preheating has been reviewed
		by Bassett {\etal} \cite{Bassett:2005xm};
		see also Ref.~\cite{Kohri:2009ac}.
		We highlight the review 
		by Kofman, Linde \& Starobinsky \cite{Kofman:2008zz}, 
		where a comprehensive study of preheating and 
		reheating was presented.
	In \emph{perturbative reheating}, the decay rate of inflaton particles
	into other species of the matter sector
	is calculated directly from an $S$-matrix.
	The calculation of this process follows the 
	well-known \textit{in-out} quantum field theory rules
	applied to scattering processes.
	By virtue of the perturbative nature of this process, 
	reheating is not particularly efficient in 
	producing a significant number density of particles.
	
	It was later understood that 
	it was possible that an enhancement of the perturbative
	decay described above could occur. This could be understood as 
	a by-product of the accumulation of several previous
	decays, leading
	to a resonant phase of \textit{non}-equilibrium production known as
	\emph{preheating}.
	By this process, inflaton particles see their energy dumped into
	the matter sector, which one can interpret as an amplification in 
	particles occupancy
	number. This will be the central topic in this chapter.
	
	A different effect, named \emph{tachyonic
	preheating} \cite{Felder:2000hj, Felder:2001kt, Copeland:2002ku, Dufaux:2006ee}, is
	associated with the end of inflation in
	certain models, usually when a spontaneous symmetry breaking occurs.
	Unlike conventional preheating, this does not merely
	convert one species
	of particle into another, but (like any tachyonic instability)
	reflects a preference for
	converting one vacuum state into another,
	by the rapid accumulation and condensation of particles.
	This phenomenon happens, for example, 
	in hybrid inflation models, initially proposed 
	by Linde \cite{Linde:1993cn}.
	The delicate dynamics between this two-field inflation 
	model makes preheating particularly hard to investigate, 
	as documented by Lyth in Refs. \cite{Lyth:2010ch, Lyth:2010zq}.

The general theory of preheating 
 has been systematically applied
 to concrete models.
	In particular this was possible for some versions of brane inflation,
 where a careful interpretation was given
	\cite{Kachru:2003sx, Barnaby:2004gg}; see also the review 
	by Sen \cite{Sen:2004nf}.
	In these models, inflation ends when the mobile $\D{3}$-brane
	becomes close to a parallel, fixed antibrane (a $\Dbar{3}$-brane), 
	allowing
	open strings stretching between the
	$\D{3}$--$\Dbar{3}$ pair
	to form. The inflaton field in these models 
	is the distance between the two branes.
	The open string states include a tachyon mode 
	which develops for sufficiently close branes.
	This tachyonic instability is believed to induce
	fragmentation of the $\D{3}$-brane into $\D{0}$-branes
	(which pack together to form the $\D{3}$-brane).
	The $\D{0}$ fragments efficiently decay into closed string states,
	which are enumerated by the
	Kaluza--Klein (``KK'') modes of supergravity fields in the warped
	background. These KK modes subsequently decay
	into the species of
	matter and radiation which build up the standard model
	content of our universe
	\cite{Barnaby:2004gg}.
	



In this chapter we shall focus on a much less dramatic version
of post-inflationary dynamics.
	We work in a model where
	the $\D{3}$-brane comes to rest near an edge of its warped
	background, the ``tip of the throat.''
	As it settles on its resting-place it 
	undergoes coherent
	oscillations, inducing
	growing, quantum fluctuations 
	which fold and wrinkle the surface of the brane.
	
	As we mentioned before, our interest lies 
	in the \emph{qualitative} differences which
	emerge between inflation models driven by canonical
	and non-canonical kinetic terms \cite{Lachapelle:2008sy}. 
	What is the effect of the extra non-linearities 
	due to the DBI action on the preheating mechanism?
	Is the reheating temperature different? 
	Focusing on the differences between these two classes of models,
	we will mostly ignore their similarities. 
	In particular,
	we acknowledge the use of perturbation theory in either case will break down 
	when back-reaction becomes important, at which point the number density of 
	the recently produced particles needs to be taken into account \cite{Kofman:1997yn}.
	For this reason, our preheating analysis is restricted to times
	before the onset of back-reaction.






\section{DBI dynamics}
\label{sec:dbi-dynamics}
The DBI model was reviewed in 
\S\ref{subsec:power-law}, and we revisit it here
in a different perspective: that of branes.
	In Ref. \cite{Silverstein:2003hf} Silverstein \& Tong
	discussed the brane-world scenario where one or more $\D{3}$-branes
	move in a warped throat, taken to be a six-dimensional elongated
	region in a higher dimensional world-volume. This is usually the AdS throat.
	Another possibility exists: the throat can be capped off
	in the infra-red limit of the underlying 
	field theory.
	
	
	A low-energy description of a $\D{3}$-brane travelling in this
	warped throat is given by the Dirac--Born--Infeld action\footnote{See, for example,
														Refs. \cite{Gibbons:1997xz, Das:1998ei, Aharony:1999ti}
														for discussions on the DBI action.		}
	\begin{equation}
		S = \frac{1}{2} \int \d x \; \sqrt{-g} \;
		\bigg\{
			R + 2\bigg[ - \dfrac{1}{f(\phi)} \, \left[ \sqrt{1 - f(\phi) X} - 1 \right]
		- V(\phi) \bigg] \ 
		\bigg\} \ \ ,
		\label{eq:action-preheating}
	\end{equation}
	where $g_{\mu\nu}$ is the pull-back
	of the $10$-dimensional metric to the brane world-volume,
	and $R$ is the Ricci scalar constructed from $g_{\mu\nu}$.
	As usually in brane world scenarios, 
	$\phi$ acts as a collective coordinate
	measuring the radial position of the brane within the throat, and
	$V$ is the potential  
	describing
	how the brane is attracted towards the bottom of the throat.
	The warp factor, $f(\phi)$, is in general a function of the 
	radial coordinate.
	A more precise interpretation is possible:
	$f^{-1}$ measures the tension of the
	$\D{3}$-brane, redshifted by the warp factor,
	giving $f$ canonical dimension $[\mathrm{mass}]^{-4}$
	(we are using units in which $\phi$ has dimensions $[\mathrm{mass}]$).
	

	If the throat is exactly
	anti-de Sitter, the result is a static BPS state
	in which the
	potential $V(\phi)$ is quartic at lowest-order in the field,
	because conformal invariance forbids the existence of a mass term.
	If the throat is capped off, then conformal invariance is broken---a typical example is the Klebanov--Strassler throat
	\cite{Klebanov:2000hb}.
	In this case we expect a mass term to be generated
	which receives contributions from moduli stabilization and bulk
	fluxes
	\cite{Kachru:2003sx,Baumann:2006th,Baumann:2007np,Baumann:2007ah,
	Krause:2007jk,
	Baumann:2009qx,Baumann:2010sx}.
	In a general compactification, a spectrum of terms will be generated
	including a $\phi^{3/2}$ term which may lead to
	a phase of inflexion-point
	inflation.
	We assume this term is absent, or forbidden by a symmetry.
	Therefore, for small departures from the equilibrium point
	for $\phi$,
	the potential attracting the brane towards the infrared
	tip of the throat is (to lowest order) quadratic \cite{Silverstein:2003hf},
	\begin{equation}
		V(\phi) = \frac{1}{2} m^2\phi^2\ \  .
		\label{eq:pot}
	\end{equation}
	D-brane inflation with this potential is sometimes referred to
	as the ``UV model.''
	A related
	small-field, IR model due to Chen \cite{Chen:2005ad}
	takes $V = V_0 - m^2 \phi^2 / 2$
	with $V_0$ dominant---we discussed its non-gaussian
	features in \S\ref{sec:dbi}.


	As the brane approaches
	the infrared tip of the throat,
	$\phi$ tends \textit{slowly} to zero.
	In this limit $\dot{\phi}^2 \ll 1$
	and the square root can be expanded in powers of $X$,
	reproducing the action for
	a canonically normalised scalar field with potential $V$.
	If, however, the brane is moving relativistically, then $X \sim 1$
	and the square root in Eq.~\eqref{eq:action-preheating} is \textit{non-expandable}.
	Said differently, in this case we 
	are forced to retain an infinite set of
		non-renormalisable operators involving powers of
		$(\partial \phi)^2$ with pre-defined Taylor coefficients,
		but higher-order derivative operators do not arise. 
		It is the algebraically special form of the action through 
		$\sqrt{1 - f X}$ which makes DBI satisfy a non-renormalisation
		theorem \cite{Silverstein:2003hf,Leblond:2008gg,Shandera:2008ai,
		deRham:2010eu} against large renormalisations of these expansion coefficients.
		
	To measure the relative importance of the nonlinear terms
	induced by the presence of the square root in the action
	\eqref{eq:action-preheating},
	it is conventional to define the equivalent of a Lorentz factor
	for the brane, as in Eq. \eqref{eq:def-gamma-dbi}, given by
	\begin{equation}
		\gamma^{-1} \equiv \sqrt{1 - f(\phi) \,\dot{\phi}^2}\ \  .
		\label{eq:lorentz}
	\end{equation}
	This is a non-analytical function which has a branch-cut
	in the negative real axis, which
	requires $\gamma$ to be real, and therefore
	$0 \leq f \dot{\phi}^2 < 1$
	\cite{Kabat:1999yq,Silverstein:2003hf}.
	This induces a limiting speed for the motion of the $\D3$-brane
	moving along the throat;
	slow-motion corresponds to $\gamma \sim 1$, whereas
	relativistic motion of the brane gives $\gamma \gg 1$.
	
	
	In FLRW space-time, the equation of motion for the inflaton is
	\begin{equation}
		\ddot\phi
		+ 3H \frac{\dot\phi}{\gamma^2}
		- \frac{1}{f} \frac{\d \ln f}{\d\phi}
		+ \frac{3}{2}\frac{\d \ln f}{\d\phi}\dot{\phi}^2
		+ \frac{1}{\gamma^3} \left(
			\frac{1}{f} \frac{\d \ln f}{\d\phi}
			+ \dfrac{\partial V}{\partial \phi}
		\right)
		= 0\ \  .
		\label{eq:inflaton}
	\end{equation}
	In the non-relativistic limit
	$\gamma \rightarrow 1$ and for constant $f$, 
	Eq.~\eqref{eq:inflaton}
	reduces to the Klein--Gordon equation for a canonically normalised
	scalar field in a FLRW background.
	
	What is the likely value for $\gamma$?
	We revisit our discussion of \S\ref{sec:dbi}.
	There, we provided an estimate, valid at next-order in slow-roll, of the 
	bispectrum amplitude in the equilateral mode.
	For our purposes it is, however, enough to 
	consider its leading-order behaviour 
	$\fNL^{\textrm{(equilateral)}} \simeq  - 0.32 \gamma^2$ \cite{Alishahiha:2004eh} 
	[cf. Eq. \eqref{eq:dbi-fnl-eq}].
	Using WMAP 7-year data
	at $65\%$ confidence level, 
	$\fNL^{\textrm{(equilateral)}}=26 \pm 140$, 
	we estimate this requires $\gamma \lesssim 9$.
	In our calculations we assume this upper limit will continue to be eroded
	especially in anticipation of \textit{Planck}'s results.
	It might be even possible that the smallness of $\gamma$
	constrains the model to be realised in its
	non-relativistic limit.
	This is perhaps the least phenomenologically interesting
	regime for DBI. Nevertheless, we will show that preheating 
	will display some interesting features.
	Accordingly,
	we suppose that inflation is approximately of the slow-roll variety.
	In this limit,
	the evolution of $\phi$ is close to that in a canonical model,
	where the corrections are controlled by the
	deviation of $\gamma$ from unity.
	We will solve Eq.~\eqref{eq:inflaton}
	perturbatively in powers of these small deviations.
	
	In this description the brane will slowly drift towards
	the tip of the throat, where inflation ends.
	Near the tip of the throat,
	the warp factor decreases
	\cite{Klebanov:2000hb,Kecskemeti:2006cg}.
	Silverstein \& Tong \cite{Silverstein:2003hf} suggested that
	the relevant physics of the capped throat could be captured by
	taking
	\begin{equation}
		f(\phi) \equiv \dfrac{\lambda}{\left(\phi^2+\mu^2\right)^2}\ \  ,
		\label{eq:tension}
	\end{equation}
	where $\lambda$ is the dimensionless 't Hooft coupling and
	$\mu$ is the energy scale associated with the
	infrared cut-off.
	For convenience, we choose coordinates so that
	the final resting place of the brane corresponds to $\phi = 0$.
	When $\phi \ll \mu$, this becomes independent of the brane position
	$\phi$, and assumes a constant value
	\begin{equation}
		f \equiv \frac{\lambda}{\mu^4} \ \ .
		\label{eq:cutoff}
	\end{equation}

	
	We suppose $m \gg H$, which is usually true after inflation.
		This means that during one Hubble time there will occur 
	many oscillations 
	and Hubble friction terms arising in Eq.~\eqref{eq:inflaton}
	can be ignored.
	Our analysis assumes the brane will oscillate around
	this position in warped space with small amplitudes,
	contained entirely within the cut-off region where $f^{-1}$
	is approximately constant. 
	We will justify these statements below.
	
	Making these approximations and assuming
	the non-relativistic limit in which $\gamma = 1$, coherent
	oscillations of the brane
	have constant amplitude, which we shall denote by $\A$. The respective solution 
	to the equation of motion \eqref{eq:inflaton} is
	\begin{equation}
		\phi_0(t) \simeq \A \cos (mt)\ \  .
		\label{solhomogene}
	\end{equation}




Our analysis relies on the approximations described above.
	We list below some important criticisms about the approximations used, and 
	justify our approach.

	\para{Perturbative approximation}What other effects can spoil the dynamics of $\phi$
	given by Eq. \eqref{solhomogene}?
	After integrating out fluxes and other UV perturbations,
	we are left with a low-energy theory controlled by
	an effective potential for the D-brane \cite{Baumann:2009qx,Baumann:2010sx},
	of the form $V = \sum_i c_i M^{4-\Delta_i} \phi^{\Delta_i}$, where $M$ is some mass scale.
	In a generic compactification, the 
	interaction coefficients are expected to be $\Or(1)$.
	The leading term corresponds to $\Delta = 3/2$.
	Invoking some symmetry may force this term to be absent.
	The next $\Delta = 2$
	term will typically dominate higher contributions
	to the potential (which start with $\Delta=3$)
	whenever $\phi \ll M$.
	
	On the other hand, 
	the infrared cutoff scale, $\mu$, must satisfy $\mu < m$.
	Therefore, provided we take $\phi < \mu$, so that we are
	safely within a region where the warp factor is constant
	and given by Eq. \eqref{eq:cutoff}.
	We can thus expect corrections from both features in the throat geometry
	and higher-order terms in the D-brane potential to be negligible.
		
		\para{Slowly evolving background}How good is our approximation that $m \gg H$?
	In practice, Hubble drag would cause $\A$ to decrease slowly,
	roughly like $1/mt$ \cite{ArmendarizPicon:2007iv}, 
	typical of a matter dominated phase.
	This is because the pressure of the fluid associated with the 
	inflaton should be averaged out over the many oscillations the 
	brane executes around $\phi=0$.
	Take $H_f$ and $H_i$ to be two values of the Hubble parameter
	separated by $N$ oscillations. 
	It follows that
	\begin{equation}
		\frac{H_i}{H_f} \sim 1 + A \, N \, \frac{H_i}{m} \ \ ,
		\label{eq:hi}
	\end{equation}
	where $A$ is some constant of order unity.
	The corresponding oscillation amplitudes, $\A_{f}$ and  $\A_{i}$, are
	related by
	\begin{equation}
		\frac{\A_i}{\A_f} \sim 1 + A' \, N \, \frac{\A_i}{\Mp}\ \  ,
		\label{eq:Ai}
	\end{equation}
	in which $A'$ is different from $A$, but also of order unity.
	Unless $N \gg 1$,
	our assumption that $m \gg H$ is sufficient to ensure
	$H_i \simeq H_f$.
	In addition,
	Eq.~\eqref{eq:Ai} shows that $\A_i \ll \Mp$ is sufficient to ensure
	$\A_i \simeq \A_f$.
	In view of the requirement $\A \ll m$
	to ensure the
	quadratic potential is an adequate approximation, where $m$ is typically
	of order the infrared cutoff scale,
	this is amply satisfied.
	Therefore, in what follows, we will
	restrict our attention to a sufficiently large number of 
	oscillations, say $N < 10^2$,
	and neglect the time-dependence of both $H$ and $\A$.
	
	

	
	\para{Relativistic corrections to the background solution.}According to the approximations listed above, 
	corrections to the non-relativistic motion
	described by~\eqref{solhomogene}
	will be perturbative provided
	$|f \dot{\phi}_0^2 | \ll 1$. To check that our analysis
	satisfies this approximation, it is useful to
	introduce a dimensionless positive quantity, which we 
	shall denote by $\varsigma$, satisfying
	\begin{equation}
		\varsigma \equiv f m^2 \A^2\ \  .
		\label{eq:def-varsigma}
	\end{equation}
	The condition above can then be rewritten as $\varsigma  \ll 1$.
	But how small can $\varsigma$ be? 
		In order for the small
	relativistic corrections
	not to be dominated by others which we have neglected, 
	one needs to impose, for consistency, 
	$\varsigma \gtrsim
	\phi/m$ or $\mu/m$.
	We should trust our analysis for perhaps $\varsigma \sim 10^{-1}$
	to $10^{-3}$, but 
	certainly not for significantly larger or smaller $\varsigma$.

	We now evaluate the next-order $\Or(\varsigma)$ corrections to the
	leading-order solution \eqref{solhomogene}.
	The governing equation can be obtained by dropping Hubble
	friction terms in Eq.~\eqref{eq:inflaton},
	in agreement with our approximation, which gives
	\begin{equation}
		\ddot{\phi}
		+ \left(
			1 - \frac{3}{2}f\dot{\phi}^2
		\right) \frac{\d V}{\d\phi}
		\simeq 0 \ \ .
		\label{approxeq}
	\end{equation}
	One could attempt to solve Eq.~\eqref{approxeq} 
	perturbatively, 
	writing $\phi = \phi_0 + \delta \phi$ with
	$\delta \phi$ of $\Or(\varsigma)$.
	However, this procedure does not produce 
	an appropriate, self-consistent solution
	since Eq.~\eqref{approxeq} 
	also induces corrections to the fundamental 
	oscillation frequency $m$.
	
	To capture these physical effects, 
	we take another ansatz: we assume a WKB-type solution
	of the form $\phi = \A \cos \theta(t)$.
	We now need to
	solve for the phase $\theta(t)$
	to order $\Or(\varsigma)$.
	To recover Eq.~\eqref{solhomogene} in the limit when
	$\varsigma \rightarrow 0$,
	we require $\theta(t) = m t + \delta \theta(t)$.
	Replacing in Eq. \eqref{approxeq}, 
	we conclude that $\delta \theta(t)$
	must satisfy the following differential equation
	\begin{equation}
		\delta \ddot{\theta} +
		2 m\, \cot (mt) \, \delta \dot{\theta} +
		\frac{3 m^2 \varsigma}{2}\, \sin (m t) \,  \cos (m t) = 0 \ \  .
	\end{equation}
	Dropping an unwanted divergent contribution,%
		\footnote{This mode is proportional to
		$\cot mt$, which is divergent at $t=0$. We choose its coefficient
		 so that this mode is projected out by the boundary conditions,
		and therefore does not lead to an instability in the solution.}
	the background solution is
	\begin{equation}
		\varphi(t) = \A \cos \left[
			(m t) \left( 1 - \frac{3 \varsigma}{16} \right) +
			\frac{3 \varsigma}{32} \sin (2 m t)
		\right] \ \ .
		\label{eq:fullphi}
	\end{equation}
In principle, one can calculate	
	corrections to the amplitude,
	but we will ignore the time-dependence
	of $\A$ (we will see in Fig. 6.1
	this is indeed a good approximation).

	In comparison with the canonical solution, the phase
	shows a drift proportional to $\varsigma m t$.
	Although the calculation remains under perturbative control,
	this drift generates order unity
	deviations from the non-relativistic background
	after $1/\varsigma$ oscillations.
	There is also a superposed phase oscillation,
	proportional to $|\varsigma \sin 2 m t| \ll 1$,
	which always generates small corrections.
	To make the comparison with the canonical solution
	more clear, we write \eqref{eq:fullphi} as 
	\begin{equation}
		\varphi(t) =
		\A
		\left\{
			1 - \frac{3 \varsigma}{16} \sin^2 \left[(m t)
			\left( 1 - \frac{3 \varsigma}{16} \right)\right]
		\right\}
		\cos \bigg[(m t) \left( 1 - \frac{3 \varsigma}{16} \right)\bigg] \ \  ,
		\label{eq:phi}
	\end{equation}
	which is equivalent to~\eqref{eq:fullphi}
	up to $\Or(\varsigma)$.
	Eq.~\eqref{eq:phi}
	exhibits the first perturbative relativistic corrections
	to the motion of the brane:
	first, a frequency shift
	in the background motion $\phi_0$, corresponding to
	$m \mapsto m\,(1 - 3 \varsigma/16)$;
	and second, a small periodic fluctuation superposed
	over the background oscillations.
	
	
	\begin{figwindow}[0,1,\includegraphics[width=10cm]
{wkb.jpg}, {Plot of the numerical (red) and approximate (blue) 
solution of Eq. \eqref{approxeq}, and the cosine function (green).}] 
\noindent  On the left we plot the numerical solution of 
Eq. \eqref{approxeq}, which is completely overlaid by the 
blue curve, given by \eqref{eq:phi}.
In contrast, the simple trigonometric solution \eqref{solhomogene}
stops being a good approximation to the dynamics of the 
background field $\phi(t)$ soon after one oscillation.
\label{fig:wkb}
\end{figwindow} 
%\vspace*{0.5cm}
\noindent Indeed, the true solution 
is shown to drift away from the simple cosine---this is 
the effect of the \textit{phase} drift mentioned above.
The amplitude, however, is very lightly modulated over the 
coherent oscillations, and remains almost constant.




	\subsection{Coupling to matter fields}
	\label{sec:coupling}

	The reheating phase is designed to
	populate the universe with Standard Model degrees of freedom,
	whilst dissipating the energy stored in the inflaton field.
	Pauli's exclusion principle usually prevents efficient preheating
	into fermions \cite{Greene:1998nh, Greene:2000ew}, so we suppose the
	inflaton $\phi$ couples to bosonic degrees of freedom,
	which are taken to have spin zero for simplicity.
	The
	subsequent decay into fermions has also been studied in Refs.
	 \cite{Kofman:1997yn, Abbott:1982hn}.
	
	We treat the couplings between the inflaton and the matter
	modes phenomenologically, denoting the matter field by
	$\chi$ and taking it to be described by the low-energy
	effective Lagrangian
	\begin{equation}
		\mathcal{L} \supseteq 
		- \frac{1}{2} (\partial \chi)^2
		- \frac{1}{2} m_\chi^2 \chi^2
		- \frac{1}{2} g^2 \phi^2 \chi^2
		\label{masterequation} \ \ ,
	\end{equation}
	where $g$ is a dimensionless coupling
	and $m_\chi$ is a bare mass.
	Eq. \eqref{masterequation} should be regarded as a subset
	of the Lagrangian of the interacting theory.
	We do not claim that such interactions necessarily
	arise in string models, although we hope the resulting phenomenology
	will be representative of those that do.
	For our purposes, it suffices to consider the subset
	\eqref{masterequation} as a possible interaction channel
	which shall expose the features of the preheating
	stage in these models.
	The equation of motion for $\chi$ is
	\begin{equation}
		\ddot{\chi} + 3 H \dot{\chi} - \frac{1}{a^2} \nabla^2 \chi
		+ \left(
			m_\chi^2 + g^2 \phi^2
		\right) \chi = 0 \ \  ,
		\label{mattereq1}
	\end{equation}
	where $\nabla^2$ is the Laplacian operator.
	Matter production in this model is studied in \S\ref{sec:preheating}.
	
	In \S\ref{sec:sym-break}
	we will study an alternative model,
	in which the matter field $\chi$ is coupled to
	a symmetry-breaking potential of the form
	\begin{equation}
		V(\phi, \chi) = \dfrac{1}{2}m^2\left(\phi-\sigma\right)^2 
		+
		\dfrac{1}{2} g^2\phi^2\chi^2 \ \ .
		\label{eq:pot-sym}
	\end{equation}
	This causes the brane to be
	attracted to a radial position which is not the tip of the 
	throat, but rather $\phi = \sigma$.
	This can be interpreted as a toy model of compactifications in which
	the D-branes are brought to rest at a finite point in the
	warped throat.



















\section{Non-perturbative preheating in DBI inflation}
\label{sec:preheating}



	As the brane settles towards $\phi=0$,
	its coherent oscillations
	cause efficient non-perturbative particle production.
	We briefly review this process.
	
	\subsection{Brief review of parametric resonance}

	
	To perform a quantum field theory treatment of preheating
	we need to quantize both 
	the inflaton $\phi$ and the matter field $\chi$. 
	In particular, framing our discussion with respect 
	to $\chi$, we want to write the two linearly
	independent solutions of 
	\begin{equation}
		\ddot{\chi}_k + 3 H \dot{\chi}_k +
		\left(
			k^2 +m_\chi^2+ g^2 \phi^2
		\right) \chi_k = 0
		\label{fouriermode} \ \ ,
	\end{equation}
	where $k$ is the comoving wavenumber.
	We label these solutions $\chi_k$ and
	$\chi_k^{\ast}$.
	We write the Heisenberg field corresponding to $\chi$
	in Fourier space as
	\begin{equation*}
		\chi(t, \vect{x})
		=
		\int \frac{\d^3 k}{(2\pi)^3}
		\left(
			\chi_k a^\dagger_k
			+ \chi_k^{\ast} a_{-k}
		\right)
		\e{\im \vec{k} \cdot \vec{x}}  \ \ ,
	\end{equation*}
	in which we have assumed that the normalisation of
	$\big\{ \chi_k, \chi_k^{\ast} \big\}$
	has been adjusted so that
	$a_k$ and $a^\dag_k$ obey the usual creation-annihilation algebra,
	\begin{equation*}
		\big[ a_k , a^\dagger_{k'} \big] = (2\pi)^3 \delta( \vec{k} - \vec{k}' ) \ \ .
	\end{equation*}
	
	How many particles are produced with momenta $k$?
	The energy density, $\rho_k$,
	associated with $\chi$-quanta of wavenumber $k$
	satisfies $2 \rho_k = \big| \dot{\chi}_k \big|^2
	+ \omega_k^2 \big| \chi_k \big|^2$  ,
	where $\omega_k^2 = k^2 + g^2 \phi^2$.
	Subtracting the zero-point energy, the occupancy number is well
	approximated by
	\begin{equation}
		n_k \simeq \frac{E_k}{\omega_k}
		= \frac{\omega_k}{2} \bigg\{
			\frac{\big| \dot{\chi}_k^{\mathrm{cl}} \big|^2}{\omega_k^2} +
			\big| \chi_k^{\mathrm{cl}} \big|^2
		\bigg\} - \frac{1}{2} \ \ .
		\label{eq:occupy}
	\end{equation}
	We conclude that
	whenever $|\chi_k|$ or
	$|\dot{\chi}_k|$ are large, the
	occupation numbers will grow.
	In particular, if $\chi_k$ experiences exponential growth, 
	then
	Eq.~\eqref{eq:occupy} shows we can expect
	$n_k$ to attain macroscopic values very rapidly.
	Eq. \eqref{eq:occupy} therefore describes 
	the phenomenon of preheating, discussed
	in \S\ref{sec:preheating-introduction}, and which we will investigate in 
	detail in \S\ref{sec:matter}.
	
	To determine when $\chi_k$ grows, it is often useful to
	translate the mode equation for $\chi_k$
	into a version of Mathieu's equation or its generalisations.
	This is because Mathieu's equation admits solutions
	which fall under instability bands (in some 
	region of the parameter space), which signal exponentially growing 
	modes when applied to preheating---particle production 
	becomes copious.
	The standard Mathieu's equation is of the form
	\cite{McLachlan,Arscott}
	\begin{equation}
		\frac{\d^2 \chi_k}{\d z^2}
		+ (A_k - 2q \cos 2z) \chi_k = 0 \ \ ,
		\label{mathieu}
	\end{equation}
	where $z$ is a dimensionless time
	to be defined below.
	In the following sections
	we give explicit model-dependent expressions for $A_k$ and $q$
	applicable to both inflaton and matter fluctuations.
	
	For certain combinations of these parameters
	the solutions exhibit exponential growth.
	If $q \gtrsim A_k$, the effective mass of the scalar field
	in question can become temporarily zero, 
	which induces a copious production of $\chi$-quanta.
	This regime is referred to as
	\emph{broad resonance}, because there is a width of momenta 
	which are favoured to experience this instability \cite{Mukhanov:2005sc}. 
	
	In the opposite regime, $q \ll A_k$, and the effective mass never vanishes.
	Instability bands are still present, but the combinations 
	of parameters $A_k$ and $q$ are such that
	the exponential growth occurs only in
	narrow bands of momentum space.
	For this reason this scenario is known as \emph{narrow resonance}.
	These bands are centred on momenta for which
	$A_k = \ell^2$, where $\ell \in \mathbb{N}$,
	corresponding to values of $k$ for which
	$|A_k - \ell^2| \lesssim q^\ell$ \cite{Kofman:1997yn}.
	If $|q| \ll 1$ then at large $\ell$
	these bands become increasingly narrow.
We will now study the solutions to Mathieu's equation
\eqref{mathieu}
when $\chi_k$ are both inflaton and matter field modes.


	\subsection{Inflaton production}
	\label{sec:inf-prod}
	

	First, consider the inflaton mode  with momentum $k$.
	We set $\phi$ equal to its background value,
	which we denote by $\varphi$,
	determined up to first-order relativistic corrections by~\eqref{eq:phi}.
	At the onset of oscillations we assume
	that the matter field, $\chi$, is in its vacuum state, and so $\chi = 0$.
	
	Until the accumulation of $\chi$-quanta
	causes the background $\chi$ field to grow,
	the inflaton fluctuations 
	$\delta\phi_k$ evolve according to the Klein-Gordon equation.
	To linear order in $\varsigma$, this is
	\begin{equation}
		\delta \ddot{\phi}_k - 3 \,\frac{f m^2 \varphi \dot{\varphi}}{\gamma}
		\delta \dot{\phi}_k + \left(
			\frac{m^2}{\gamma^3} + k^2
		\right) \delta \phi_k = 0 \ \ .
		\label{eq:infk}
	\end{equation}
	We expand this equation uniformly to leading-order in the perturbative parameter 
	$f \dot{\varphi}^2$
	and perform a change of variables 
	so that $\delta \phi_k = \xi y_k$, which can eliminate the friction term
	in Eq. \eqref{eq:infk}. In particular,
	 we choose $\xi$ to satisfy
	\begin{equation*}
		\frac{\d \ln \xi}{\d t} = \frac{3}{2} \, f m^2 \varphi
			\dot{\varphi} \ \ .
	\end{equation*}
	The solution to this differential equation is
	\begin{equation}
		\xi = \xi_0 \exp \left\{
			\frac{3}{2} f m^2 \left[ \varphi^2(t) - \varphi^2(t_0) \right]
		\right\} \ \ ,
	\label{eq:xisolution}
	\end{equation}
	where we have chosen $\xi = \xi_0$ at $t = t_0$.
	This produces a friction, or ``braking'' effect, which
	could be interpreted as a perturbative
	manifestation of the D-cceleration mechanism
	\cite{Silverstein:2003hf}.
	It is a novel effect in the DBI model, with no analogue
	in canonical scenarios. 
	Accordingly, the braking disappears
	in the limit $\varsigma \rightarrow 0$.
	
	The remaining time-dependence
	is carried by $y_k$, which satisfies a Mathieu equation with $A_k$
	and $q$ determined, to leading-order in $\varsigma$ defined 
	by \eqref{eq:def-varsigma}, by
	\begin{equation}
		A_k = \left(1 + \frac{k^2}{m^2} \right)
			\left(1 + \frac{3 \varsigma}{8} \right)
			- \frac{3 \varsigma}{4}
		\quad \mbox{and} \quad
		q = \frac{3 \varsigma}{8}\ \  .
		\label{eq:A-and-q}
	\end{equation}
	The dimensionless time $z$, used to write Eq.~\eqref{mathieu}, satisfies
	$z = m t ( 1 - 3 \varsigma / 16 )$, which corresponds to a rescaled frequency 
	$m \mapsto m ( 1 - 3 \varsigma / 16 ) $.
	Inspection of Eq. \eqref{eq:A-and-q} reveals
	$q \ll A_k$, giving resonance only in narrow bands.
	The $\ell = 1$ band is centred at momentum $k_1$, given by
	\begin{equation}
		k_1 = \frac{m}{2} \sqrt{\frac{3 \varsigma }{2}}\ \  .
	\end{equation}
	Modes with momentum $k=k_1$ will experience 
	exponential growth.
	
	From Floquet's theory it follows that
	each mode evolves as $\exp (\mu_k z)$.
	In the $\ell = 1$ band, also called the first band,
	the Floquet exponent $\mu_k$ has positive real solutions
	which signal
	exponential growth \cite{McLachlan}
	\begin{equation}
		\mu_k^2 \simeq \left(
			\frac{q}{2}
		\right)^2 -
		\left( A_k^{1/2} - 1 \right)^2 \ \  .
	\label{eq:mumathieu}
	\end{equation}
	This exponent is maximal for the central value $k = k_1$
	and decreases for larger or smaller $k$,
	forming a band of narrow width $\Delta_1$,
	\begin{equation}
		\Delta_1 = \frac{m \sqrt{3 \varsigma }}{2}
		\frac{\sqrt{2} - 1}{\sqrt{2}} \ \  .
	\end{equation}
	At the centre of the band, the Floquet exponent
	takes the value $\mu_1$
	\begin{equation}
		\mu_1 = \max_{\ell = 1 \; \mathrm{band}}\  \mu_k
		= \frac{3 \varsigma }{16}\ \  .
	\end{equation}
	
	So far, our formulae depend on the mass,
	$m$, and coupling, $g$, which appear in the Lagrangian.
	However, these \textit{bare} quantities only parametrise the theory.
	To make a meaningful comparison between DBI and the
	class of canonical models, we must express our answer in
	terms of a \textit{measurable} mass and coupling, corresponding to 
	\textit{physical} quantities. We denote these
	by $\mstar$ and $\gstar$, to distinguish them from
	the Lagrangian parameters. In the DBI theory the Lagrangian parameters
	have no direct physical significance, whereas in the case of canonical
	kinetic terms they coincide with the measurable mass
	and coupling at tree-level.
	The relations $\mstar(m)$ and
	$\gstar(g)$ are derived in Appendix~\ref{appendix:canonicnorm}.
	
	Collecting
	Eqs.~\eqref{eq:xisolution} and~\eqref{eq:mumathieu},
	and expressing the answer in terms of the physical $\mstar$ and $\gstar$,
	we find that
	the
	inflaton modes grow as
	\begin{equation}
		\delta \phi_k \sim
		\exp\left\{
			\dfrac{3\varsigma}{8} \cos
			\left[
				2 \mstar t \left(1-\dfrac{7\varsigma}{16} \right)
			\right]
			+ \dfrac{3\varsigma }{16} \mstar t
		\right\}  \ \ .
		\label{eq:resultinflaton}
	\end{equation}
	The undetermined normalisation absorbs
	$\xi_0$ in Eq. \eqref{eq:xisolution}.
	We see that at early times, the DBI friction and the resonant growth have competing effects.
	After a few oscillations, however, the cosine which represents the
	friction effect becomes negligible
	in comparison with the resonant term, and inflaton particle production thrives.

	\subsection{Matter particle production}
	\label{sec:matter}

	Ultimately, we are interested in studying the 
	production of matter particles. 
	Consider the interaction potential in the Lagrangian density \eqref{masterequation}.
	As a result of these interactions the
	$\chi$-mode receives an effective mass
	of order $k^2 + g^2 \phi^2$.
	As in \S\ref{sec:inf-prod} we assume that preheating begins
	in the vacuum $\chi = 0$, which is a good approximation until
	the $\chi$-quanta are in such number density
	that they back-react on the zero mode.
	In this vacuum, small fluctuations
	grow governed by a generalised Hill's equation 
	\begin{equation}
	\dfrac{\d^2	\delta \chi_k}{\d z^2} +
		\left(
			\theta_0 + 2 \theta_2 \cos 2z + 2 \theta_4 \cos 4z
		\right) \delta \chi_k = 0 \ \ ,
	\end{equation}
	where the parameters $\theta_0$, $\theta_2$ and $\theta_4$ obey
	\begin{equation}
		{
		\renewcommand{\arraystretch}{2}
		\begin{array}{lll}
			\theta_0 & = & \displaystyle
			\frac{k^2}{m^2} \left( 1 + \frac{3 \varsigma}{8} \right)
			+ \frac{g^2 \A^2}{2m^2} \left( 1 + \frac{9\varsigma}{32} \right)\ \ , \\
			\theta_2 & = & \displaystyle
			\frac{g^2 \A^2}{4m^2} \left( 1 + \frac{3 \varsigma}{8} \right) \ \ , \ \ \textrm{and}\\
			\theta_4 & = & \displaystyle
			\frac{3}{128} \frac{\A^2}{m^2} \varsigma g^2 \ \ ,
		\end{array}
		}
	\end{equation}
	and $z = mt(1 - 3 \varsigma / 16 )$.
	The solutions of Hill's equation grow and decay with characteristic
	Floquet exponent $\mu_k$ in a way entirely analogous to
	the solutions of Mathieu's equation.
	The exponentially growing solutions also organize themselves into
	bands, defined by integers $\ell$.
	
	According to Floquet's theory, one can
	estimate $\mu_k$ for the $\ell = 1$ band
	\begin{equation}
		\mu_k^2 \simeq
		\left( \frac{\theta_2}{2} \right)^2
		- \left( \theta_0^{1/2} - 1 \right)^2
		\mp \frac{\theta_2}{3} \left( \frac{\theta_4}{2} \right)^2
		\mp \frac{\theta_2^3}{2}\ \  .
	\end{equation}
	We believe this expression has not previously appeared in the
	preheating literature, and we provide the reader with a full
	derivation in Appendix~\ref{appendix:Hill}.
	In the region where our approximations are valid,
	$\A \ll m$.
	Therefore, the terms involving $\theta_4^2$ and $\theta_2^3$
	are negligible, and
	\begin{equation}
		\mu_k^2 \simeq \left( \frac{\theta_2}{2} \right)^2 -
			\left( \theta_0^{1/2} - 1 \right)^2 \ \ .
	\end{equation}
	The centre of the $\ell = 1$ band lies at $k = k_1$, where
	\begin{equation}
		k_1^2 = m^2\, \bigg( 1-\frac{3 \varsigma}{8} \bigg) 
		- \frac{g^2 \A^2}{2} \, \bigg(
		1-\frac{3\varsigma}{2}
		\bigg)  \ \  ,
		\label{eq:kone-a}
	\end{equation}
	for which $\theta_0(k_1) = 1$.
	Collecting terms,
	it follows that the unstable matter modes grow at a rate
	determined by
	\begin{equation}
		\delta \chi_k \sim
		\exp\left\{ 
			\left. \mu_k \right|_{max} \mstar t
			\left(1- \dfrac{3\varsigma}{16} \right)
		\right\}
		\sim 
		\exp\left\{
			\dfrac{1}{8} \left(\dfrac{\gstar\mathcal{A}}{\mstar}\right)^2
			\mstar t
			\left( 1+ \dfrac{3\varsigma}{16} \right)
		\right\} \ \ .
	\end{equation}
	This displays a slight (perturbative) enhancement compared to the equivalent
	canonical model.



	\subsection{Preheating with a symmetry breaking term}
	\label{sec:sym-break}

	Now consider the symmetry-breaking potential
	given in Eq.~\eqref{eq:pot-sym}.
	In this case, it is more convenient to redefine $\phi$ so that it
	describes excitations around the true vacuum at $\phi = \sigma$.
	Writing $\phi \rightarrow \phi+\sigma$, the
	interaction potential can be written 
		\begin{equation}
		V(\phi, \chi) = \dfrac{1}{2}m^2\phi^2
		+
		\dfrac{1}{2}g^2\phi^2\chi^2
		+
		g^2\sigma \phi \chi^2
		+
		\dfrac{1}{2}g^2\sigma^2\chi^2 \ \  .
		\label{eq:potentialbreaking}
	\end{equation}
	Around this minimum, $\phi$
	acquires an effective mass
	$m_{\mathrm{eff}}^2\left(\chi\right)=m^2+g^2\chi^2$.

	Making the same assumption as before that preheating begins
	while $\chi \approx  0$,
	the inflaton modes will behave
	as in Eq.~\eqref{eq:resultinflaton}
	until the growth of $\chi_k$ occupation numbers
	causes the $\chi$ zero-mode to grow.
	Until that time,
	$\chi$ modes with momentum $k$ obey the equation of motion
	\begin{equation}
		\delta \ddot{\chi}_k
		+
		\left(
			k^2
			+ g^2\phi^2
			+ 2g^2\sigma\phi
			+ g^2\sigma^2
		\right)
		\delta \chi_k = 0 \ \ .
	\end{equation}
	
	
	We will suppose the brane executes oscillations around $\phi = \sigma$
	with an amplitude much smaller than the symmetry breaking scale, 
	$\A \ll \sigma$, so that it has reasonably settled at its final position.
	Assuming that $\sigma \ll m/g$,
	and again neglecting any bare mass for $\chi$,
	fluctuations in the matter field will be controlled by
	Hill's equation,
	\begin{equation}
		\dfrac{\d^2 \delta \chi_k}{\d z^2}
		+ \left(
			\theta_0
			+ 2 \theta_2 \cos 2z
			+ 2 \theta_6 \cos 6z
		\right) \, \delta \chi_k
		\approx 0 \ \  ,
		\label{eq:hill-six}
	\end{equation}
	in which $2z=mt (1- 3 \varsigma / 16)$ and the parameters
	$\theta_0$, $\theta_2$ and $\theta_4$ obey
	\begin{equation}
		{
		\renewcommand{\arraystretch}{2}
		\begin{array}{lll}
			\theta_0 & = &
				\dfrac{4}{m^2}\left(k^2+ g^2\sigma^2\right)
				\left(1+\dfrac{3 \varsigma  }{8} \right) \ , \\
			\theta_2 & \simeq &
				4 \dfrac{g\sigma}{m} \dfrac{g\mathcal{A}}{m}
				\left(1+\dfrac{21\varsigma }{64} \right) \ ,\ \ \textrm{and} \\
			\theta_6 & \simeq &
				\dfrac{3\varsigma }{16} \dfrac{g\sigma}{m}
				\dfrac{g\mathcal{A}}{m} \ \  .
		\end{array}
		}
	\end{equation}
	
	To determine the growth of each $\chi$-mode we require an
	estimate of Floquet's exponent associated with Eq.~\eqref{eq:hill-six},
	which is again derived in Appendix~\ref{appendix:Hill}.
	For the $\ell = 1$ band, it is given by
	\begin{equation}
		\mu_k \simeq
			\sqrt{\left(\dfrac{\theta_2}{2}\right)^2\mp
				\dfrac{\theta_2\theta_6^2}{32} \mp
				\left(\dfrac{\theta_2}{2}\right)^3
			- \left(\theta_0^{1/2} -1 \right)^2} \ \  .
		\label{eq:floquet-six}
	\end{equation}
	As above, the terms involving $\theta_6^2$ and $\theta_2^3$
	can be neglected. The result is equivalent to a Mathieu's equation
	with coefficients $A_k$ and $q$ satisfying
	\begin{equation}
		A_k = \dfrac{4}{m^2}\left(k^2+ g^2\sigma^2\right)
			\left(1+\dfrac{3\varsigma}{8} \right)
		\quad \mbox{and} \quad
		q = \theta_2 \simeq 4 \dfrac{g\sigma}{m} \dfrac{g\mathcal{A}}{m}
			\left(1+\dfrac{21\varsigma}{64} \right) \ll A_k \ \  .
		\label{eq:mathieu3}
	\end{equation}
	Since $q$ is much smaller than $A_k$, we expect resonance to be
	of the narrow-type, if it occurs at all.
	The first instability band
	occurs when $A_k = 1$
	and is centred at momentum $k = k_1$, where
	\begin{equation}
		k_1 \simeq \dfrac{m}{2} \left(1- \dfrac{3\varsigma}{16} \right) \ \ ,
		\label{eq:kone-b}
	\end{equation}
	which is shifted
	by $\Or(\varsigma)$ in comparison with the canonical case.
	
	Eqs.~\eqref{eq:kone-a} and~\eqref{eq:kone-b} show that the
	$\ell = 1$ resonance injects energy into a narrow band of
	modes with momenta $k \sim m$.
	Kofman, Linde \& Starobinksy
	interpreted the narrowness of this
	resonance as a decay process in which a single inflaton particle
	of mass $\sim m$ decays continuously into two
	$\chi$-particles with opposite momenta
	of magnitude
	$\sim k_1$ \cite{Kofman:1996mv}.
 	Our results are 
 	in agreement with their interpretation.
 	
	The width of the resonant band satisfies
	\begin{equation}
		\Delta k_1 \simeq
		2m \dfrac{g\sigma}{m} \dfrac{g\mathcal{A}}{m}
		\left( 1+ \dfrac{9\varsigma}{64}\right)\ \  .
	\end{equation}
	Using the appropriate limit of Eq.~\eqref{eq:floquet-six} to estimate
	$\mu_k$,
	or applying Eq. \eqref{eq:mumathieu},
	we conclude that there is a perturbative enhancement of preheating
	efficiency owing to the relativistic DBI correction.
	Near the centre of the $\ell = 1$ band, the $\chi$-modes
	grow as
	\begin{equation}
		\delta \chi_k \sim
			\exp\left\{\left.\mu_k\right|_{\mathrm{max}} z \right\}
		\sim
			\exp\left\{\dfrac{\gstar\sigma}{\mstar}
			\dfrac{\gstar\mathcal{A}}{\mstar} \mstar t
			\left(1+ \dfrac{9\varsigma}{64} \right)\right\}\ \  ,
	\end{equation}
	in which the growth rate is augmented with respect to
	the non-relativistic or canonical cases by
	an $\Or(\varsigma)$ term.
	This agrees with our expectation that any change in
	the preheating process would have to be perturbative in
	$\varsigma$, by assumption.




	\subsection{Efficiency of narrow-resonance preheating}

	How efficient is the preheating mechanism described above?
	The resonances we have discussed are of narrow-type, and
	therefore occupation numbers grow only for a very limited range of
	momenta. This process is much less efficient than broad resonance,
	where a larger range of momenta experience growing occupation
	numbers. 
	
	Nevertheless, the rate of growth is exponential within the
	unstable bands, and therefore
	preheating by narrow resonance may
	still lead to an acceptably rapid conversion of inflaton modes
	into matter species. After some oscillations, gravitational redshift
	will cause
	modes of fixed comoving wavenumber
	to drift slowly through each unstable band, from ultraviolet
	to infrared. It follows that
	significant particle production will occur only when modes
	remain within an unstable band for sufficiently long
	and particle production is not diluted by the universe's expansion \cite{Kofman:1997yn}.
	If wavenumbers move through the unstable bands too rapidly,
	then little stimulated emission occurs, and the resonance
	is washed out by the expansion of the universe.
	In this situation preheating is inefficient in repopulating the 
	universe.

	The arguments of Floquet's theory show that in each resonant band,
	the inflaton and matter fluctuations of wavenumber $k$
	grow like $\exp ({\mu_k z})$.
	Let us focus on the broadest instability band,
	which corresponds to $\ell = 1$
	and which will generally dominate the particle production.
	This band has width $\sim q$, so each wavenumber remains within
	the unstable band for a time of order $q/H$.
	The resonance will be stable against Hubble expansion if
	$\left(\mu_k z/ \Delta t\right) q / H \gtrsim 1$.
	It follows that preheating will \textit{efficiently} drain energy from the
	inflaton provided
	\begin{equation*}
		\sqrt{\dfrac{2H}{\mstar}} \lesssim \dfrac{3\sigma}{8}\ \  .
	\end{equation*}
	For the matter field, preheating will operate
	in the cases $\sigma = 0$ and $\sigma \neq 0$ whenever
	\begin{equation*}
		\sqrt{\dfrac{2H}{\mstar}} \lesssim
			\dfrac{1}{4} \left( \dfrac{\gstar \mathcal{A}}{\mstar} \right)^2
			\left( 1 + \dfrac{13\sigma}{32} \right)
	\end{equation*}
	or
	\begin{equation*}
		\sqrt{\dfrac{H}{\mstar}} \lesssim 
			2\left( \dfrac{\gstar \sigma}{\mstar}\right)
			\left( \dfrac{\gstar \mathcal{A}}{\mstar}\right)
			\left( 1+\dfrac{23\sigma}{64}\right) \ \ ,
	\end{equation*}
	apply, respectively.
	In the absence of knowledge of these parameters, we assume these
	conditions are verified.



















\section{Perturbative reheating in DBI inflation}
\label{sec:reheating}


	The preheating process described and studied above
	is non-relativistic in nature and generates 
	copious production of particles. 
	While it occurs, it is still possible for
	perturbative processes to happen, by which
	the inflaton decays into matter species \cite{Albrecht:1982mp}.
	Indeed, these processes are necessary to thermalise the
	post-inflationary universe and bring reheating to an end.
	Ultimately they should take over the preheating era
	once this has become inefficient against Hubble expansion.

	In the theories we have been considering,
	such decays are allowed by the symmetry-breaking potential
	studied in \S\ref{sec:sym-break},
	where there is an effective trilinear interaction $g^2 \sigma \phi \chi^2$
	 which permits the decay $\phi \rightarrow \chi \chi$.
	The simple potential~\eqref{masterequation}
	allows only for two-body scattering.
	However, in the presence of an oscillating
	background field we can
	take the decay rate to be similar to that produced by
	the $g^2 \sigma \phi \chi$ interaction with $\sigma \sim \A$.
	
	If the inflaton couples directly to the fermionic sector, then
	perturbative production can proceed via Yukawa interactions
	described by $h \phi \bar{\psi} \psi$, with $\psi$ denoting the Dirac fermion
	and $\bar{\psi} = \im \psi^\dag \gamma^0$ its adjoint.
	In this case it is important to suppose that any interactions in which the
	inflaton participates are not sufficient to spoil the
	possibility of successful inflation.
	
	In this section we will continue to assume that the inflaton mass
	is much larger than the bare mass of $\chi$, or the mass of any
	fermionic species where such couplings exist.
	Under these conditions, the tree-level decay rates
	for $\phi \rightarrow \chi \chi$ and $\phi \rightarrow \bar{\psi} \psi$
	can be calculated straightforwardly.
	The necessary expressions were given in Kofman, Linde
	and Starobinsky's review
		\footnote{Modifications to these rates and cross-sections
		to incorporate physical quantities
		in the DBI model are derived in
		Appendix~\ref{appendix:canonicnorm}.}
	\cite{Kofman:1997yn}
	\begin{equation}
		\Gamma(\phi\to\chi\chi)
			= \frac{\gstar^4\sigma^2}{8\pi \mstar}
		 \quad \mbox{and} \quad
		\Gamma(\phi\to\bar\psi\psi)
			= \frac{\hstar^2 m}{8\pi} \ \ ,
		\label{eq:candecay}
	\end{equation}
	where $h_\star$ is the measured Yukawa coupling, determined by
	matching Eq.~\eqref{eq:candecay} to observation.
	
	Can perturbative decays compete
	with preheating?
	In one oscillation, we can estimate that perturbative decays populate the $\chi$ field
	occupation numbers 
	at a rate $\Gamma/\mstar$. In the same time interval preheating
	increases the population at a rate $\mu_k$.
	We conclude that perturbative decays dominate preheating when
	\begin{equation}
		\Gamma \gtrsim \mstar \mu_k\ \  .
		\label{eq:reheating}
	\end{equation}
	
	Let us suppose Eq. \eqref{eq:reheating} applies.
	These processes are comparatively slow
	and it is reasonable to assume that the decay products thermalise.
	This results in a transition to a radiation dominated universe 
	and we can estimate the \textit{reheating temperature}, $T_R$, to be
	 \cite{Kofman:1997yn}
	\begin{equation}
		T_R \simeq 0.2 \sqrt{\Gamma M_P} \ \  ,
	\end{equation}
	where $\Gamma$ is the rate of the dominant decay channel. 

	Let us briefly recapitulate the r\^{o}le of perturbative processes in
	canonical inflation.
	Inflaton decays $\phi \rightarrow \chi \chi$
	can become the dominant channel for inflaton decay
	only in the case of symmetry breaking, 
	for which $\sigma \neq 0$, as illustrated in the 
	interactions \eqref{eq:pot-sym}
	\cite{Kofman:1997yn}.
	These decays begin to dominate when the amplitude of inflaton
	oscillations has dropped to
	$\mathcal{A} \sim \gstar^2 \sigma / 8\pi$.
	If we suppose that the curvature perturbation synthesized during
	the inflationary phase, denoted $\zeta$,
	was dominated by fluctuations in
	the inflaton, then we must demand $m \sim 10^{-5} \Mp$
	enforced by agreement with observations. 
	This, however, need not be the case.
	For example, if $\zeta$ receives a dominant contribution
	from other sources, a wider range of masses $m$ can be tolerated.
	Supposing further that the interaction coupling $\gstar$ 
	is typically
	$\gstar \sim 10^{-1}$, we find the reheating temperature is of order
	the symmetry breaking scale
	\begin{equation}
		T_R \sim  \sigma \ \  .
	\end{equation}

	If, on the other hand, the dominant decay is into fermions, then
	the Yukawa coupling must satisfy
	\begin{equation}
		\hstar^2 \gtrsim 18\pi \left( \dfrac{\gstar\mathcal{A}}{\mstar} \right)
			\left( \dfrac{\gstar \sigma}{\mstar} \right)\ \  .
	\end{equation}
	Suitable values for the inflaton mass
	$\mstar$ and couplings $\{ \gstar, \hstar \}$
	can be found so that this condition applies, but these choices
	are fundamentally model-dependent.
	As an example, if we assume
	$\hstar \sim 10^{-1}$ and $\mstar \sim 10^{-5} M_P$, we find the universe
	reheats at a temperature
	\begin{equation}
		T_R \simeq 1.3 \times 10^{-5} M_P
		\simeq 3.12 \times 10^{13} \; \mathrm{GeV}\ \  .
	\end{equation}





	\subsection{Estimates of reheating temperatures}
	This analysis can be applied to the
	production mechanisms of
	\S\S\ref{sec:inf-prod}--\ref{sec:sym-break}.
	Let us work
	with the symmetry-breaking potential, $\sigma \neq 0$.
	Assuming a typical coupling $\gstar \sim 1$,
	Eq.~\eqref{eq:reheating} implies that the
	$\phi \rightarrow \chi\chi$ decay dominates resonant production
	when the amplitude satisfies
	\begin{equation}
		\mathcal{A} \lesssim 4\times 10^{-4} \sigma
		\left(1-\dfrac	{25\sigma}{64}  \right)\ \ .
		\label{eq:decay1}
	\end{equation}
	The resulting reheating temperature receives relativistic
	corrections in comparison with
	the temperature achieved using canonical kinetic terms. 
	In particular, we find
	\begin{equation}
		T_R \simeq 0.13 \sigma \, \left(1-\dfrac{\sigma}{8}  \right)\ \  .
	\end{equation} 
	Alternatively, decays into fermions will become predominant
	($\phi \rightarrow \psi \bar{\psi}$)
	if the associated Yukawa coupling is sufficiently large.
	To be more precise the threshold is
	\begin{equation}
		\hstar^2 \gtrsim 8\pi\, \left(\dfrac{\gstar \sigma}{\mstar} \right)
		\left(\dfrac{\gstar\mathcal{A}}{\mstar} \right)
		\left( 1+\dfrac{57\sigma}{64} \right) \ \  .
		\label{eq:decay2}
	\end{equation}
	This is compatible with the conditions
	$g\mathcal{A}/m \ll g\sigma/m \ll 1$. In this case and for a
	representative value of the coupling, say $\hstar \sim 0.1$, 
	we find that
	\begin{equation}
		T_R \simeq  3.12 \times 10^{13}
			\left(1-\dfrac{3\sigma}{8} \right) \; \mathrm{GeV} \ \  .
	\end{equation} 

The estimates above should not be regarded as rigid predictions
following a period of DBI inflation. Rather they are meant to be indicative
of the differences with respect to an analogous reheating process
after a period of canonical inflation.


\section{Summary of results}
\label{sec:summary-preheating}
In this short chapter, 
we have studied mechanisms by which the universe can be repopulated
	with matter species following an era of D-brane inflation.
	We work in the limit where the motion of the brane is, at most,
	perturbatively relativistic. This approximation
	explores the least phenomenologically interesting regime of DBI inflation, but might 
	be ultimately required by
	observation if $\fNL^{\textrm{(equilateral)}}$ is small.
	In our analysis, we assume the amplitude of oscillations
	of the D-brane as it settles towards the minimum of the potential
	is significantly smaller than
	whatever infrared scale caps the throat.
	The amplitude and phase of these oscillations are
	slightly modified in comparison with a scenario where 
	inflation is driven by a 
	canonically normalised scalar field.

	We encounter some novel, though perturbative 
	effects, which we list below.	
	\begin{enumerate}[i.]
		\item 
	In the perturbatively-relativistic
	limit of DBI inflation, non-linearities arising from the
	action cause a weak resonance
	which reaches an $\Or(1)$ effect only after
	$\sim 1/\varsigma$ oscillations. This occurs both for 
	inflaton and matter particles. In contrast, 
	in canonical inflation, only matter preheating
	is possible.
	Excessive production of inflaton particles is
	problematic,
	but since preheating typically concludes after $\lesssim 10$
	oscillations this weak resonance is unlikely to be fatal for the
	DBI model. In the ultra-relativistic limit where $\gamma \gg 1$,
	the potential becomes unimportant and 
	resonance is dynamically suppressed.
	This disappointing conclusion 
	has been confirmed in Ref. \cite{Karouby:2011xs}.
	
	\item We identify an additional `DBI friction' term in the equation
	of motion for the inflaton fluctuations, 
	which competes within the first oscillations with the preheating
	effect. 
	\item 
	We have estimated the
	final reheating temperature in these models and found
	these are typically smaller
	than in the equivalent theory with canonical kinetic terms. 
	This may be beneficial in concrete models,
	where lower reheating temperatures can allow problems associated
	with overclosure of the universe by gravitinos to be ameliorated.
	The most stringent constraint on DBI models comes from observations
	of the microwave background bispectrum, which presently require
	$\gamma \lesssim 9$. If our results are representative,
	and the reheating temperature falls as $\gamma$ increases,
	a constraint on $\gamma$ may also emerge from demanding
	agreement with the Big Bang nucleosynthesis era, which requires
	$T_{\mathrm{RH}} \gtrsim \mbox{MeV}$.
	\end{enumerate}

==> three.tex <==


\begin{savequote}[30pc]
God does not care about our mathematical difficulties. He integrates empirically.
\qauthor{Albert Einstein}
\end{savequote}





\chapter{Microphysics in Non-Gaussianity}
\label{chapter:three}
\hrule
\vspace*{1cm}
	In the previous chapter we revisited the computation 
	of the two-point correlator and 
	briefly reviewed the ``in-in'' formalism 
	for correlation functions.
	We
	have initiated the 
	calculation of
	the bispectrum of 
	single-field inflation theories 
	and have argued that 
	the cubic action for perturbations
	is simplest written in terms of five bulk operators, 
	given in Eq. \eqref{eq:zeta-action3-chapter2end}.
	The calculation we are about to describe applies 
	to \emph{any} single-field inflation model 
	where the equations of motion are at most second-order
	in derivatives of the field.
	For the purposes of understanding the implications of our results, however, 
	we will specify the coefficients $\Lambda_i$ to certain models of interest.
	
	
	
\para{Outline}In this chapter we report a calculation of the 
	next-order corrections to the bispectrum.
	We break up the next-order bispectrum
	in its magnitude, $\fNL$, 
	and its shape and scale-dependences.
	In this chapter we shall focus on its magnitude, whereas 
	 \S\S\ref{sec:running}--\ref{sec:shapes} of chapter 
	 \ref{chapter:four} will be devoted to the scale and shape-dependences of 
	 the bispectrum.
	

	Applications of our results to 
	a collection of models are displayed in
	\S\S\ref{sec:vanilla}--\ref{sec:noncanonical}.
	\S\ref{sec:vanilla} focuses on canonical single-field
	inflation models with an arbitrary potential, whilst 
	\S\ref{sec:noncanonical} explores models which can imprint
	a significant non-gaussian signature because of their non-canonical 
	structure---of these we focus on DBI inflation
	and $k$-inflation.
	In~\S\ref{sec:dbi} we discuss an important consequence of 
	obtaining next-order corrections for 
	 $\fNL$ in generalised DBI inflation model.
	 Through such corrections we gain access to 
	 compactification data, such as the
	shape of the potential and the warp factor, for the first time.
	Not only does this calculation decrease the theory error
	associated with previous estimates of the bispectrum, 
	but it also allows access to important information encoded in the CMB
	which can reveal data inaccessible by other means.
		
	
	In~\S\ref{sec:tensor} we turn to the set of observables 
	related to tensor fluctuations. Primordial gravitational 
	waves are a generic prediction of inflationary models.
	We 
	 briefly review the next-order
	computation of the power spectrum for tensor fluctuations: we compute
	the tensor-to-scalar ratio, $r$,
	and the scaling of the tensor perturbations through 
	the tensor spectral index, $n_t$.
	
	
	Finally, we summarise our findings
	in~\S\ref{sec:conclusions}.
	Appendix \ref{app:sr} supports the findings of this chapter.
	In \ref{appendix:propagator} we give details of the derivation
	of the next-order corrections to the scalar propagator.
	We collect in 
	Appendices~\ref{appendix:a}--\ref{appendix:b}
	mathematical details
	of certain integrals needed for presenting the next-order bispectrum
	in closed form. This appendix extends what had been originally obtained 
	by Chen \etal \ in Ref.~\cite{Chen:2006nt}.



This chapter is based on work done in collaboration with 
Clare Burrage and David Seery, published in Ref. \cite{Burrage:2011hd}.






	\section{The bispectrum beyond lowest-order}
	\label{sec:bispectrum}

	We define the bispectrum, $B$, in terms of the three-point function\footnote{This 
														definition may differ from 
														other notations in the literature, 
														such as that in Ref. \cite{Chen:2006nt},
														by numerical factors of $2\pi$.}
	\begin{equation}
		\langle
			\zeta(\vec{k}_1) \zeta(\vec{k}_2) \zeta(\vec{k}_3)
		\rangle
		=
		(2\pi)^3 \delta(\vec{k}_1+\vec{k}_2+\vec{k}_3) B({k}_1, {k}_2, {k}_3) \ \ .
		\label{eq:bispectrum-def}
	\end{equation}
	It turns out to be useful to define the
	\textit{reduced bispectrum}, $\fNL$, which satisfies
	\cite{Komatsu:2001rj,Lyth:2005fi}
	\begin{equation}
		\fNL \equiv \dfrac{5}{6}
		\dfrac{B({k}_1, {k}_2, {k}_3)}{P(k_1)P(k_2) + P(k_1) P(k_3) +
		P(k_2) P(k_3)} \ \  .
		\label{eq:deffnl}
	\end{equation}
	Observational constraints are typically quoted in terms of
	$\fNL$ evaluated in certain bispectrum \textit{templates} often used
	in CMB analysis to compare the measured bispectrum
	with the bispectrum predicted by the theory.
	We discuss them in \S\ref{subsec:inner-prod}.
	Each template can be thought of as being related to a specific triangular configuration, 
	although this need not be the case.
	Current constraints on $\fNL$ in the simplest inflationary models
	have been discussed by Senatore {\etal} in Ref. \cite{Senatore:2009gt}.
	Tighter constraints are expected to be placed in the upcoming year 
	using \emph{Planck}'s data.
	
	
	
	\subsection{Sources of next-order corrections}
	\label{eq:sources}
	We are now in a position to compute the three-point function
	of Eq. \eqref{eq:shiftaction}
	to next-order in the slow-roll approximation.
	As we discussed in \S\ref{subsec:boundaryterms}, the
	boundary action and $\delta S^{(2)} / \delta \zeta$ contributions
	can be discarded by construction of the \emph{in-in}
	formalism and because the propagators are evaluated on-shell. 
	
	
	
	Next-order terms arise in the bulk operators
	from a variety of sources.
	First, 
	the coefficients of each interaction vertex in Eq. \eqref{eq:shiftaction}
	contain an admixture of leading and next-order contributions
	in the slow-roll approximation.
	This allowed us to anticipate an estimate of the 
	next-order contributions to three-point correlator 
	in \S \ref{subsec:estimatesfNL}.
	Second, the leading-order part of each vertex is 
	a (slowly) time-dependent
	quantity which must be expanded around a reference time
	or scale, as in
	Eq. \eqref{eq:time-dependence}, producing next-order terms.
	Third, there are next-order corrections to the propagator,
	obtained by expanding
	Eqs. \eqref{eq:propagator}--\eqref{eq:wavefunction}
	around the reference time.
	Propagator corrections appear on both the external
	and internal legs of the diagram.
	The external legs corrections correspond 
	to the propagator arising at late times, 
	when we take $|\tau| \rightarrow 0$; the internal 
	legs corrections arise from the expansion of the order of 
	the Hankel functions in Eq \eqref{eq:wavefunction}.
	
	It may be useful to identify these corrections in the 
	Feynman diagram as follows
	\begin{figure}[htpb]
\begin{center}
\includegraphics[width=6cm]{corrections_diagram.jpg}
\label{fig:corrections_diagram}
\caption{Sources of next-order corrections in slow-roll in the tree-level Feynman diagram.}
\end{center}
\end{figure}
	
	
	
	
	
	
	
	\subsection{Reference time, factorisation scale}
	\label{subsec:refscale}
	To proceed, we must choose a reference point
	$\tau_\star$ around which to expand
	time-dependent quantities.
	Such reference point is arbitrary by construction, 
	but some choices might be more useful than others.
	Take an arbitrary correlation function of fields $\zeta(\vec{k}_i)$
	(not necessarily a three-point correlator).
	Whatever our choice of $\tau_\star$, the
	result~\eqref{eq:powerspectrum} for the power spectrum shows that
	we must expect logarithms of the form $\ln (k_i/k_\star)$
	which compensate for the difference in time of horizon crossing between
	the mode $k_i$ and the reference scale $k_\star$.
	To obtain a reliable answer we should attempt to minimise
	these logarithms.
	
	

	What typical values do 
	the logarithmic terms have?
	Consider an arbitrary three or higher order correlator.
	If all fields participating in the correlation function carry
	momenta of
	approximately common magnitude $k_i \sim k$---described as the
	``equilateral limit''---the logarithm will
	be small when $k_\star \sim k$.
	The logarithmic term
	will, in general, be less or of order unity, 
	and it will multiply a slow-variation parameter, or 
	a linear combination of these.
	In this case, na\"{\i}ve perturbation theory is not spoiled
	by the appearance of large logarithms.
	
	In the opposite limit,
	one or more fields have ``soft'' momenta of order
	$\ksoft$ which are much smaller than
	the remaining ``hard'' momenta of order $\khard$, 
	$\ksoft \ll \khard$.
	When $\ksoft/\khard \rightarrow 0$ it will not be possible
	to find a choice of $k_\star$ which keeps
	\textit{all} logarithms small; while we might be able 
	to minimise one of these, say $\ln (\ksoft/k_\star)$, 
	the hierarchy between $\ksoft$ and $\khard$ modes makes
	$\ln (\khard/k_\star)$ inevitably very large.
	Said differently, a reference scale appropriate for small scale physics
	will produce sizeable corrections to large scale physics
	and the calculation passes outside the validity of
	ordinary perturbation theory. At this point one requires a 
	resummation technique to deal with large logarithmic terms. 
	We have encountered
	the problem
	of large logarithms which led to the
	renormalisation
	group formalism of Gell-Mann \& Low
	\cite{GellMann:1954fq}.
	
	In the study of inflationary correlation functions, configurations
	mixing hard and soft momenta with $\ksoft \ll \khard$ are
	referred to as ``squeezed.''
	For this configuration
	of momenta, the 
	bispectrum for canonical inflation reaches its 
	maximum magnitude
	\cite{Maldacena:2002vr}.
	Given the analogy with ordinary
	processes in quantum chromodynamics (QCD) \cite{Collins:2011zzd}, 
	one could study the behaviour of a correlation
	function as its momenta are squeezed
	by setting up an appropriate renormalisation group analysis
	\cite{Seery:2009hs}.
	But this is more complicated
	than necessary.
	
	Maldacena argued that, as the momentum carried by one operator
	becomes soft, the three-point function factorises
	into the two-point correlation
	between the remaining hard operators
	on a background created by the soft operator
	\cite{Maldacena:2002vr}. 
	Because of the $\delta$-distribution in the bispectrum \eqref{eq:bispectrum-def}, 
	the two hard operators are described by the same 
	energy scale.
$\fNL$ arises naturally as the appropriate observable quantity
since the bispectrum factorises into two copies of 
the power spectrum multiplied by $n_s-1$
 (as we shall see in \S\ref{subsec:fnl}).
	Factorization of this kind is typical in the infrared dynamics
	of gauge theories such as QCD, where it plays an important r\^{o}le
	in extracting observational predictions.
	The various factorisation theorems for QCD correlation functions
	have been
	comprehensively reviewed by Collins,
	Soper \& Sterman \cite{Collins:1989gx}.%
	
		The concept of factorisation is not new in cosmology.
		Indeed, the separate universe method can be thought of
		as a factorisation
		theorem for time-dependent logarithms
		$\sim \ln | k \cs \tau |$.
		The $\delta N$ rules which translate
		correlation functions of the field perturbations, $\delta \phi$,
		into correlation functions of $\zeta$ are an important special case, 
		and they allow for the summation of large logarithms.
		In this sense, factorisation is as important in extracting
		observable quantities for inflation as it is for QCD.
	Maldacena's argument was later generalised by
	Creminelli \& Zaldarriaga \cite{Creminelli:2004yq}.
	The factorisation property can be illustrated by an explicit decomposition
	of the field into hard and soft modes---see Refs. 
	\cite{Ganc:2010ff,RenauxPetel:2010ty}.
	
	Because the squeezed limit can be described by Maldacena's
	technique,
	the outcome of this discussion is that the reference scale
	should usually be chosen
	to minimise the logarithms when all momenta are
	comparable.
	In the remainder of this chapter we quote results for arbitrary
	$k_\star$ for full generality,
	but frequently adopt the symmetric choice
	$k_\star = k_1 + k_2 + k_3$ when citing numerical results.%
		\footnote{In the gauge theory language discussed above,
		the scale $k_\star$ can be thought of as the factorisation
		scale. Operators carrying momentum $k \ll k_\star$
		should not be included as part of the hard subprocess,
		but factorised into the background.}
	Having done so, we will be formally unable
	to describe the squeezed limit.
	Nevertheless, 
	we will be able to verify the correctness of our calculation
	at the onset of factorisation in
	appropriate circumstances---a property usually referred to as
	Maldacena's \emph{consistency relation}.\footnote{See Renaux-Petel \cite{RenauxPetel:2010ty} 
											for a recent discussion of
											Maldacena's condition applied to 
											$P(X,\phi)$ models.}




	\subsection{Horndeski operators}%
	\label{subsec:horndeski}
	In chapter \ref{chapter:two} we obtained 
	the cubic action \eqref{eq:zeta-action3_chapter2}
	for the comoving curvature perturbation
	\begin{equation}
		\begin{split}
			S^{(3)}
			=
			\int \d^3 x \, \d \tau \; a^2
			\bigg\{
				\frac{g_1}{a} \zeta'^3
				+ g_2 \zeta \zeta'^2
				+ g_3 \zeta (\partial \zeta)^2
				+ g_4 \zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta'
				+ g_5 \partial^2 \zeta
					(\partial_j \partial^{-2} \zeta')
					(\partial_j \partial^{-2} \zeta')
			\bigg\} .
		\end{split}
		\label{eq:s3tau}
	\end{equation}
	In a $P(X,\phi)$ model
	the interaction vertices are
	\begin{equation}
		\begin{aligned}
		g_1 &
		=
		\dfrac{\varepsilon}{H \cs^4}
			\left(
				1-\cs^2-2 \dfrac{\lambdaP \cs^2}{\SigmaP}
			\right)\ \ ,
		&
		g_2 &
		=
		\dfrac{\varepsilon}{\cs^4}
			\left[
				-3(1-\cs^2)+\varepsilon-\eta
			\right] \ \ ,
		&
		&
		\\
		g_3 &
		=
		\dfrac{\varepsilon}{\cs^2}
			\left[
				(1-\cs^2) +\varepsilon+ \eta -2s
			\right] \ \ ,
		&
		g_4 &
		=
		\dfrac{\varepsilon^2}{2 \cs^4}(\varepsilon-4) \ \ ,
		&
		g_5
		&
		=
		\dfrac{\varepsilon^3}{4 \cs^4} \ \ ,
		\end{aligned}
		%\quad\Bigg\}
		\label{eq:gi}
	\end{equation}
	but our calculation will apply for arbitrary 
	coefficients $g_i$.
	Therefore, unless explicitly written otherwise, 
	the results that follow hold for any Horndeski theory.
	
	Although $\zeta$ is dimensionless by construction, 
	it is helpful to think about it as a field of
	engineering dimension $[\text{mass}]$,
	obtained after division by the Hubble rate $H$.
	In this counting scheme, the $\zeta'^3$ operator is dimension-6, whereas
	the remaining four operators are dimension-5.
	At low energies one would na\"{\i}vely expect
	the dimension-6 operator to be irrelevant in comparison to those
	of dimension-5.
	Nevertheless, the dimension-5 operators are suppressed by the scale $H$
	making all contributions equally relevant in the action \eqref{eq:s3tau}.
	This manifests itself as an extra power
	of $H$ in the denominator of $g_1$, which 
	will appear in our results.
	Estimates of the magnitude of next-order corrections
	described in \S\ref{subsec:estimatesfNL} are based on the interactions 
	\eqref{eq:gi}---we will discuss this in more detail
	in \S\ref{sec:noncanonical}.
	

	As we discussed in \S\ref{eq:sources}, 
	the vertex factors $g_i$ are time-dependent background
	quantities.
	We can therefore introduce slow-variation parameters 
	$h_i$ which measure their
	rate of change per e-fold,
	\begin{equation}
		h_i \equiv \dfrac{\dot{g}_i}{H g_i} \ \ ;
	\end{equation}
	we take these to be $\Or(\varepsilon)$ in the slow-variation approximation, that is, 
	$|h_i|\ll 1$.






	\section{Three-point correlations}
	\label{sec:3pf}

	We use these conventions to compute the bispectra at next-order in slow-roll
	for each operator in the action \eqref{eq:s3tau}.
	The resulting three-point functions
	are intricate objects of momenta, and when quoting their magnitudes
	it is often helpful to adopt an organizing principle.
	We divide the possible contributions into two natural
	classes.
In the first class, labelled `$a$,' we collect
\begin{enumerate}[i.]
\item  the leading-order bispectrum,
\item 	effects arising
	from corrections to the wavefunctions associated with external
	lines, and
\item  effects arising from the time variation of the vertices.
\end{enumerate}
	In the second class, labelled `$b$,' we focus on
	internal legs corrections to the Feynman diagrams.
	These classes are qualitatively different in character because
	wavefunctions associated with the internal lines
	are integrated over time.
	

	
	\para{Large logarithms, infrared singularities}In our answers, we expect
	at least three species of large logarithms to appear, disrupting 
	ordinary perturbation theory. We carefully track the contribution from 
	each species. The most familiar types, already encountered
	in the two-point function, measure time- and
	scale-dependences. A third type of large logarithm
	is associated with the far infrared limit
	$\ksoft / \khard \rightarrow 0$
	discussed in \S\ref{sec:bispectrum}---this is Maldacena's ``squeezed'' limit, in which the behaviour of the
	three-point function obeys a factorisation principle.
	We will show that the various large logarithms
	arrange themselves in such a way that they can be absorbed into the
	scale-dependence of background quantities.
	
	Time-dependent logarithms appear
	after expanding background quantities near a fixed reference
	scale, as in Eq. \eqref{eq:time-dependence},
	where at conformal time $\tau$ the number of elapsed 
	e-folds counts
	$N_\star = \ln | k_\star \cs \tau |$.
	In \S\ref{subsec:second} we explained
	that the correlation functions of $\zeta$ are expected to become
	time-independent far outside the horizon.
	Therefore there cannot be any time-dependence
	in our final result.
	
	
	How do the $\ln |\tau|$ terms
	disappear from the answer?
	Some $N_\star$-type
	logarithms cancel amongst themselves,
	but others cancel with time-dependent logarithms
	arising from wavefunction corrections associated with internal lines.
	The internal lines\footnote{This is explained in detail in \S 
							\ref{appendix:propagator}.} are only aware of
	the intrinsic geometrical scale $k_t \equiv k_1 + k_2 + k_3$
	and cannot depend on the
	arbitrary reference scale $k_\star$---this results in a residue of the form $\ln (k_t/k_\star)$.
	These are scaling logarithms
	describing variation of the three-point function
	with the geometrical scale $k_t$.
	They appeared before in the power spectrum \eqref{eq:powerspectrum}, 
	and they are easily distinguishable from other species of logarithms
	for they contain $k_\star$.
	Scale logarithms can also occur in the form $\ln (k_i / k_\star)$.
		
	The
	third logarithm species takes the form $\ln (k_i / k_t)$
	and first emerges in the three-point function;
	this is related to the hierarchy of momentum scales we discussed 
	in \S\ref{subsec:refscale}.
	Each side of the triangle must scale linearly with
	the perimeter, so
	despite appearances
	these have no dependence on $k_t$---they are unaffected by rigid
	rescalings of the momentum triangle.
	To better understand this,
one can write $k_i$ in terms of the perimeter, 
$k_t$, and two additional coordinates, describing the angular
dependence. This implies that $\ln(k_i/k_t)$ is effectively only
a function of the angular coordinates, and it is therefore responsible 
for the shape-dependence of the bispectrum.
	The `pure' shape logarithms become large in the squeezed
	limit $k_i / k_t \rightarrow 0$.

We will discuss the appearance of these logarithmic species
in detail next.



\subsection{The bispectra}
\label{subsec:type-bispectra}
	\para{$a$-type bispectrum}Collecting the $a$-type contributions to the bispectrum, we find
	it can be written as follows
	\begin{equation}
		\begin{split}
		B^{a} = \mbox{} &
			\frac{H_{\star}^4}{2^4 \csstar^6}
			\frac{g_{i\star}}{\zterm_\star^3}
			\frac{T^{a}(k_1)}{k_t^2\prod_i{k_i^3}}
			\bigg\{
				-\varpi_{\star} U^{a}(k_1)
					\ln\frac{k_1k_2k_3}{k_\star^3}
				\\
				& \hspace{3.2cm} \mbox{}
					+ 2V^{a}(k_1)\varepsilon_{\star}\ln\frac{k_t}{k_\star}
					+ W^{a}(k_1) h_{i\star}\ln\frac{k_t}{k_\star}
				\\
				& \hspace{3.2cm} \mbox{}
				+ X^{a}(k_1) (1 + 3E_{\star})
				+ 2Y^{a}(k_1)\varepsilon_{\star}
				+ Z^{a}(k_1) h_{i\star}	
			\bigg\}
		\\
		& \mbox{} + \text{cyclic permutations} \ \ .
		\end{split}
		\label{eq:Ba}
	\end{equation}
	The coefficients $T^{a}(k_1)$, $U^{a}(k_1)$, $V^{a}(k_1)$,
	$W^{a}(k_1)$, $X^{a}(k_1)$, $Y^{a}(k_1)$, and $Z^{a}(k_1)$ are
	functions of all three momenta $k_i$
	and are symmetric under the exchange $k_2 \leftrightarrow k_3$.
	We adopt the convention, used through the remainder of this thesis,
	of writing only the asymmetric momentum explicitly.
	The notation `cyclic permutations' denotes
	addition of the preceding term under
	cyclic permutations of the $k_i$, that is, 
	$k_1 \rightarrow k_2 \rightarrow k_3$.
	The result is symmetric under interchange of any two momenta
	by construction.	

	We give explicit expressions for the coefficient of these functions in
	Table~\ref{table:Blead}. The quantity
	$E$ is a linear combination of slow-variation parameters,
	$E = \varpi (2- \EulerGamma -\ln 2) - \varepsilon - s$,
	and it has
	also appeared in the power
	spectrum~\eqref{eq:powerspectrum}.
	The term in $X^a(k_1)$ includes the
	entire leading-order
	bispectrum.

	\begin{table}[htp]

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	\begin{center}
		\small
		\begin{tabular}{QqQqQq}

			\toprule
			
			&
			\multicolumn{5}{c}{operator}
			\\
			\cmidrule(l){2-6}
		
		 	& 
		 	\multicolumn{1}{c}{$\zeta'^3$} &
		 	\multicolumn{1}{c}{$\zeta \zeta'^2$} &
		 	\multicolumn{1}{c}{$\zeta ( \partial \zeta)^2$} &
		 	\multicolumn{1}{c}{$\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta'$} &
		 	\multicolumn{1}{c}{$\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2$}
		 	\\
			\midrule

			T^{a}(k_1) &
			6H_{\star}\frac{k_1^2k_2^2k_3^2}{k_t} &
			k_2^2k_3^2(k_1+k_t) & 
			\frac{k_t}{\csstar^4}(\vec{k}_2 \cdot \vec{k}_3) &  
			\frac{k_1^2}{2}(\vec{k}_2 \cdot \vec{k}_3) &
			\begin{array}{l}
				k_1^2(\vec{k}_2 \cdot \vec{k}_3) \\
				\; \mbox{} \times (k_1 + k_t)
			\end{array}
			\\[2mm]

			\cmidrule{2-6}

			U^{a}(k_1) & 
			1 &
			1 & 
			\csstar^2\left(K^2 - k_t^2 + \frac{k_1 k_2 k_3}{k_t} \right)	& 
			3k_t-k_1 &  
			1
			\\[2mm]

			\cmidrule{2-6}

			V^{a}(k_1) &
			1 &
			1 &
			\begin{array}{l}
				\displaystyle -\csstar^2
				\bigg(
					k_t^2-K^2-\frac{k_1k_2k_3}{k_t}
				\bigg)
			\end{array} &
			3k_t-k_1 &
			1
			\\[2mm]

			\cmidrule{2-6}
			
			W^{a}(k_1) &
			1 &
			1 &
			3\csstar^2\left(K^2 - k_t^2 + \frac{k_1 k_2 k_3}{k_t} \right) &
			3k_t-k_1 &
			1
			\\[2mm]
			
			\cmidrule{2-6}
			
			X^{a}(k_1) &	 
			1 &
			1 & 
			\csstar^2\left(K^2 - k_t^2 + \frac{k_1 k_2 k_3}{k_t} \right) &
			3k_t-k_1 &
			1
			\\[2mm]
 
			\cmidrule{2-6}

			Y^{a}(k_1) &
			\EulerGamma -\frac{1}{2} &
			\EulerGamma + \frac{k_t}{k_1+k_t} &
			\begin{array}{l}
				\displaystyle \csstar^2\bigg[
					K^2 \\
				\displaystyle \; \mbox{} -\EulerGamma
				\bigg(
					k_t^2-K^2-\frac{k_1k_2k_3}{k_t}
				\bigg)
				\bigg]
			\end{array} &
			\begin{array}{l}
				\displaystyle (3k_t-k_1)\EulerGamma \\
				\displaystyle \; \mbox{} + 2k_t
			\end{array}&
			\EulerGamma + \frac{k_t}{k_1+k_t}
			\\[2mm]

			\cmidrule{2-6}

			Z^{a}(k_1) &
			\EulerGamma-\frac{3}{2} &
			\EulerGamma - \frac{k_1}{k_1+k_t} &
			\begin{array}{l}
				\displaystyle 3\csstar^2\bigg[
					\EulerGamma K^2 \\
				\displaystyle \; \mbox{} +
				(1-\EulerGamma)
				\bigg(
					k_t^2-\frac{k_1k_2k_3}{k_t}
				\bigg)
				\bigg]
			\end{array} &
			\begin{array}{l}
				\displaystyle (3k_t-k_1) \EulerGamma \\
				\displaystyle \; \mbox{} + k_1 - k_t
			\end{array}
			&
			\EulerGamma - \frac{k_1}{k_1+k_t}
			\\[2mm]
			
 			\bottomrule
	
		\end{tabular}
	\end{center}
	\caption{Coefficients of the leading-order bispectrum,
			where $K^2 \equiv k_1k_2+k_1k_3+k_2k_3$.
	\label{table:Blead}}
	\end{table}	

\newpage

	\para{$b$-type bispectrum}The $b$-type bispectrum must be added to the
	$a$-type terms.
	It contributes at next-order \textit{only}
	and can be written as
	\begin{equation}
		\begin{split}
			B^{b} = \mbox{} &
				\frac{H_{\star}^4}{2^4 \csstar^6}
				\frac{g_{i\star}}{\zterm_\star^3}
				\frac{T^{b}(k_1)}{k_t^2\prod_i{k_i^3}}	
				\bigg\{
					\varpi_{\star}
					\sum^3_{i=1}
						\left(
							k_t U^{b}(k_i)J_0(k_i)
							+ V^{b}_i(k_1)J_1(k_i)
							+ k_t^2 W^{b}(k_i) \ln \frac{2k_i}{k_\star}
						\right)
					\\
					& \hspace{3.2cm} \mbox{}
					+ \varpi_{\star}
						\left(
							X^{b} J_2(k_1)
							+ Y^{b} k_t^3 \ln\frac{k_t}{k_\star}
						\right)
					+ Z^{b}
					+ \csstar k_t^2 \Re\left( \mathcal{J}_\star \right)
				\bigg\}
				\\
				& \mbox{} + \text{cyclic permutations}\ \  .
		\end{split}
		\label{eq:Bbchapter3}
	\end{equation}
	The same convention applies to the arguments of
	the coefficient functions
	$T^{b}(k_1)$, $U^{b}(k_i)$, $V^{b}_i(k_1)$, $W^{b}(k_i)$, $X^{b}$,
	$Y^{b}$ and $Z^{b}$; explicit expressions 
	are provided in Table~\ref{table:Bsub}.
	As before, `cyclic permutations' entails addition of the 
	preceding term under cyclic permutations of the $k_{i}$.
	
	We observe that the type-$b$ bispectrum 
	\eqref{eq:Bbchapter3} depends on three logarithmic functions $J_i$
	(which are \emph{not} Bessel functions)
	defined by
	\begin{subequations}
		\begin{align}
			\vartheta_i \, J_0(k_i) & =
				\ln \frac{2k_i}{k_t}\ \  , \\
			\vartheta_i^2 \, J_1(k_i) & =
				\vartheta_i + \ln \frac{2k_i}{k_t}\ \  , \\
			\vartheta_i^3 \, J_2(k_i) & =
				\vartheta_i (2+\vartheta_i) + 2\ln \frac{2k_i}{k_t}\ \  ,
		\end{align}
		\label{eq:clare-integrals}
	\end{subequations}
	where $\vartheta_i =1-2k_i/k_t$.
	These exhaust the `pure' shape logarithms of the form $\ln (k_i / k_t)$,
	discussed above.
	It transpires from Eqs. \eqref{eq:clare-integrals}
	that there is an obvious logarithmic divergence in the squeezed limit
	$k_i \rightarrow 0$, which we will show to be responsible for
	factorisation of the correlation function.
	There is potentially
	a power-law divergence in the limit
	$k_t \rightarrow 2 k_i$. This is \emph{also} a squeezed limit, in which
	the $i^{\mathrm{th}}$ side stays fixed while $k_j\rightarrow 0$. 
	In this limit $\vartheta_i \rightarrow 0$,
	making
	the $J_i$ na\"{\i}vely divergent.
	If present, such power-law divergences would be puzzling.
	However, it can be checked that, in combination
	with the logarithm, each $J_i$ is finite.
	This infrared-safe behaviour relies on
	a resummation procedure reached by 
	analytic continuation---see Appendix~\ref{appendix:a} for more details.

	The function $\mathcal{J}_\star$ in Eq. \eqref{eq:Bbchapter3} 
	satisfies
	\begin{equation}
		\begin{split}
			\mathcal{J}_\star
			=
			\frac{1}{k_t \csstar}
			\bigg\{
				&
				\gamma_0
				- \frac{\gamma_1 + \delta_1}{k_t}
				- \dfrac{2\gamma_2+3\delta_2}{k_t^2}
				+ \dfrac{6\gamma_3+11\delta_3}{k_t^3}
				+ \dfrac{24\gamma_4+50\delta_4}{k_t^4}
				\\
				& \mbox{}
				- \left(
					\EulerGamma
					+ \ln \frac{k_t}{k_\star}
					+ \im \dfrac{\pi}{2}
				\right)
				\left(
					\delta_0
					- \dfrac{\delta_1}{k_t}
					- 2\, \dfrac{\delta_2}{k_t^2}
					+ 6 \, \dfrac{\delta_3}{k_t^3}
					+ 24\, \dfrac{\delta_4}{k_t^4}
				\right)
			\bigg\} \ \ .
		\end{split}
	\end{equation}
	This function
	is discussed in Appendix \ref{appendix:b}.
	The coefficients $\gamma_0$, $\ldots$, $\gamma_3$,
	and
	$\delta_0$, $\ldots$, $\delta_3$
	depend on the operator under consideration, and
	they are quoted in Table~\ref{table:Jgamma}.

	\begin{table}[htp]

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	\begin{center}
		\small
		\begin{tabular}{QqQqQq}

			\toprule
			
			&
			\multicolumn{5}{c}{operator}
			\\
			\cmidrule(l){2-6}
		
		 	& 
		 	\multicolumn{1}{c}{$\zeta'^3$} &
		 	\multicolumn{1}{c}{$\zeta \zeta'^2$} &
		 	\multicolumn{1}{c}{$\zeta ( \partial \zeta)^2$} &
		 	\multicolumn{1}{c}{$\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta'$} &
		 	\multicolumn{1}{c}{$\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2$}
		 	\\
			\midrule

			T^{b}(k_1)	& 
			-\frac{3}{2}H_{\star}\csstar^2k_1^2k_2^2k_3^2 &
			k_1^2 & 
			\frac{1}{\csstar^2}(\vec{k}_2 \cdot \vec{k}_3) & 
			k_1^2(\vec{k}_2 \cdot \vec{k}_3) &  
			k_1^2(\vec{k}_2 \cdot \vec{k}_3)
	  		\\[2mm]

			\cmidrule{2-6}

			U^{b}(k_i) &
			&
			-1 & 
			2k_ik_t-2k_i^2 -K^2& 
			\csstar k_t & 
			\csstar k_t
	 		\\[2mm]

			\cmidrule{2-6}

			V^{b}_1(k_1) &
			&
			k_1 & 
			k_1k_2k_3 & 
			-\frac{1}{2}(k_2+k_3) & 
			k_1
		 	\\[2mm]

			\cmidrule{2-6}

			V^{b}_2(k_1) &
			&
			-k_1 & 
			k_1k_2k_3 & 
			\frac{1}{2}(k_2-k_3) & 
			-k_1
			\\[2mm]

			\cmidrule{2-6}

			V^{b}_3(k_2) & 
			&
			-k_1 & 
			k_1k_2k_3 &  
			\frac{1}{2}(k_3-k_2) & 
			-k_1
		 	\\[2mm]
	  
	  		\cmidrule{2-6}
			
			W^{b}(k_i) &
			&
			&
			k_t-2k_i & 
			& 
			\\[2mm]
	  
			\cmidrule{2-6}

  			X^{b} & 
			\frac{1}{\csstar^2 k_t} & 
  			& 
  			&	
  			&
			\\[2mm]

			\cmidrule{2-6}
			
			Y^{(b)} &
			&
			&
			2 & 
			& 
			\\[2mm]

			\cmidrule{2-6}

			Z^{b} &
			&
			&
			k_t^3[2\varpi_{1\star}-3\Re(\mu_{0\star})
				+3\gamma_E\varpi_{1\star}] & 
			& 
			\\[2mm]
						
 			\bottomrule
	
		\end{tabular}
	\end{center}
	\caption{Coefficients of the subleading corrections to the bispectrum,
			 where $K^2 \equiv k_1k_2+k_1k_3+k_2k_3$.
	\label{table:Bsub}}
	\end{table}	



	\begin{table}

	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	\begin{center}
		\small
		\begin{tabular}{QqQqQq}

			\toprule
			
			&
			\multicolumn{5}{c}{operator}
			\\
			\cmidrule(l){2-6}
		
		 	& 
		 	\multicolumn{1}{c}{$\zeta'^3$} &
		 	\multicolumn{1}{c}{$\zeta \zeta'^2$} &
		 	\multicolumn{1}{c}{$\zeta ( \partial \zeta)^2$} &
		 	\multicolumn{1}{c}{$\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta'$} &
		 	\multicolumn{1}{c}{$\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2$} \\
			\midrule

			\gamma_0 &
			&
			\mu_{0\star}+2s_{\star} -2\mu_{1\star} & 
			\begin{array}{l}
				\displaystyle s_{\star}k_1^2+k_1 \mu_{1\star} (k_2+k_3) \\
				\displaystyle \; \mbox{} -\mu_{0\star}k_2 k_3
			\end{array} &
			\mu_{0\star}+2s_{\star} -2\mu_{1\star} & 
			\mu_{0\star}+2s_{\star} -2\mu_{1\star}
			\\[2mm]

			\cmidrule{2-6}

			\gamma_1 & 
			& 
			\begin{array}{l}
				\displaystyle 3k_1\mu_{1\star} +k_t s_{\star} \\
				\displaystyle \; \mbox{} - 3k_1 s_{\star}
			\end{array} &
			\begin{array}{l}
				\displaystyle -s_{\star} k_{1}^2 (k_2+k_3) \\
				\displaystyle \; \mbox{} - \mu_{1\star}k_1 k_2 k_3
			\end{array} &
			\begin{array}{l}
				\displaystyle k_t s_{\star}-3k_2 s_{\star} \\
				\displaystyle \; \mbox{} +3 \mu_{1\star} k_2
			\end{array} & 
			\begin{array}{l}
				\displaystyle k_t s_{\star}-3k_1 s_{\star} \\
				\displaystyle \; \mbox{} +3 \mu_{1\star} k_1
			\end{array}
			\\[2mm]

			\cmidrule{2-6}

			\gamma_2 & 
			\frac{s_{\star}-\mu_{1 \star}}{\csstar^2} &
			k_1 k_t s_{\star} &	
			-s_{\star} k_1^2 k_2 k_3 & 
			k_2 k_t s_{\star} &	
			k_1 k_t s_{\star} 
			\\[2mm]

			\cmidrule{2-6}

			\gamma_3 &	
			k_1 \frac{s_{\star}}{\csstar^2} &
			&	 
			& 
			& 
			
			\\[2mm]

			\cmidrule{2-6}

			\delta_0 & 
			& 
			3\varpi_{1\star}-4s_{\star} & 
			-s_{\star} k_1^2-K^2\varpi_{1\star} &	
			3\varpi_{1\star}-4s_{\star} & 
			3\varpi_{1\star}-4s_{\star}
			\\[2mm]
	
			\cmidrule{2-6}

			\delta_1 &
			&
			\begin{array}{l}
				\displaystyle -k_t s_{\star} +5k_1 s_{\star} \\
				\displaystyle \; \mbox{} -3k_1 \varpi_{1\star}
			\end{array} &
			\begin{array}{l}
				\displaystyle s_{\star} k_1^2(k_2+k_3) \\
				\displaystyle \; \mbox{} +\varpi_{1\star} k_1k_2k_3 
			\end{array} & 
			\begin{array}{l}
				\displaystyle -k_t s_{\star} +5k_2 s_{\star} \\
				\displaystyle \; \mbox{} -3k_2 \varpi_{1\star}
			\end{array} & 
			\begin{array}{l}
				\displaystyle -k_t s_{\star} +5k_1 s_{\star} \\
				\displaystyle \; \mbox{} -3k_1 \varpi_{1\star}
			\end{array}
			\\[2mm]

			\cmidrule{2-6}

			\delta_2 & 
			\frac{\varpi_{1\star}-2s_{ \star}}{\csstar^2} & 
			-s_{\star} k_1 k_t	&  
			s_{\star} k_1^2 k_2k_3 &	 
			-k_2 k_t s_{\star} & 
			-k_1 k_t s_{\star} 
			\\[2mm]

			\cmidrule{2-6}

			\delta_3 & 
			-k_1 \frac{s_{\star}}{\csstar^2} &		 
			& 
			&	  
			& 
			
			\\

 			\bottomrule
	
		\end{tabular}
	\end{center}
	\caption{Coefficients appearing in the function $\mathcal{J}$
	for each operators. Note that the $\gamma_i$ contain complex numbers. The 
	imaginary part is cancelled on addition of the $+$ and $-$
	Feynman diagrams, and
	only the real part of these coefficients contribute.
	In an intermediate step for the
	three-point function of
	$\zeta (\partial \zeta)^2$,
	the cancellation of power-law divergences
	in $\tau$
	(required by Weinberg's theorem \cite{Weinberg:2005vy})
	depends on a real contribution generated
	from the product of two imaginary terms.
	\label{table:Jgamma}}
	\end{table}	
	
	
	\newpage
	
	
	
	
	\para{Comments on the calculation}The operators $\zeta \zeta'^2$,
	$\zeta' \partial_j \zeta \partial^{-2} \partial_j \zeta$
	and $\partial^2 \zeta (\partial^{-2} \partial_j \zeta')^2$
	are all dimension-5, and
	differ only in the arrangement of spatial gradients.
	For arbitrary shapes their three-point functions will not coincide,
	but for equilateral triangles the arrangement of gradients
	is irrelevant
	and the resulting $\fNL$ should agree.
	This can be confirmed upon inspection of the 
	respective coefficients quoted in tables
	\ref{table:Blead}, \ref{table:Bsub}, and \ref{table:Jgamma}.
	This represents a minimal check of our expressions.
	We will carry out further checks in
	\S\S\ref{sec:vanilla}--\ref{sec:noncanonical}
	and 	\S\ref{sec:running}
	using Maldacena's consistency condition.	
	
	
	Bispectra $a$ and $b$ are computed using the same
\textit{in-in} formalism rules briefly reviewed in 
\S\ref{subsec:inin}. 
The third Horndeski operator, $\zeta (\partial \zeta)^2$, 
presents an additional degree of complexity compared to the others.\footnote{This difficulty 
																	will also appear in 
																	chapter \ref{chapter:five}.} 
We briefly mention the technicalities of this calculation here. 

Starting from action \eqref{eq:s3tau}, we note this operator is undifferentiated, 
making the integral, at least, power-law divergent. 
This is because there will be insufficient powers of conformal time $\tau$, 
to counteract those in denominator from
 $a(\tau)$ in the integrand. As a result 
the integrand behaves, at leading-order, 
as $a^2\sim 1/\tau^2$.
At the same time, next-order corrections will add 
logarithmic terms to the integrand.
This 
has serious repercussions in the final result because it can
potentially lead to spurious 
power-law and logarithmic divergences in $\tau$ when one takes the 
limit $|\tau|\rightarrow 0$---these are \textit{dangerous interactions}, as 
named by Weinberg \cite{Weinberg:2005vy}. 

In order to ensure that 
the real part of the correlation function converges in the asymptotic limit, 
one needs to carefully isolate the primitively divergent contributions:
either power-laws like $|\tau|^{-\alpha}$, with $\alpha>0$, or logarithmic
terms $\ln (-\tau)$. 
This is done by integrating all divergent integrals by parts an
appropriate number of times. 
Only two situations occur as a result:
\begin{enumerate}[i.]
\item the isolated divergent terms contribute with a purely 
imaginary part to the correlation function. In this case, this divergence
becomes irrelevant since the total correlation function is given 
by the sum of two path integrals which are complex conjugates;
\item the isolated divergent contributions
are real and contribute to the final answer. 
When we sum type $a$ and type $b$ bispectra, however, we verify that these divergent 
contributions precisely
cancel out
amongst themselves and the final result is
finite.
\end{enumerate}
It is crucial to take these two possibilities into account 
to obtain a correct result:
first, to ensure that the correlation functions do not diverge 
in their asymptotic limit (at late times); 
and second, to guarantee that the calculation 
contains all the necessary convergent contributions to the overall 
bispectrum. This is particularly important when checking whether 
our results are consistent with Maldacena's factorisation theorem
\cite{Maldacena:2002vr, Creminelli:2004yq}.

	\para{Next-order corrections}A subset of next-order corrections to the bispectrum 
	were calculated by Chen {\etal}
	\cite{Chen:2006nt}.
	Our calculations are different in two aspects.
	First, Chen {\etal} worked to fixed order in slow-roll quantities,
	keeping terms of $\Or(\varepsilon)$ only. In a model where $\cs \ll 1$
	they reproduce the next-order corrections.
	However, in a model where $\cs \sim 1$ the leading terms are
	themselves $\Or(\varepsilon)$
	and the formulae of Chen {\etal} reduce to these
	leading contributions.
	In our calculation, we work \textit{uniformly to next-order} rather than
	at fixed order in powers of $\varepsilon$.
	When $\cs \ll 1$ our next-order corrections are $\Or(\varepsilon)$,
	and we have verified that they agree with those computed in
	Ref.~\cite{Chen:2006nt}.
	When $\cs \sim 1$ the next-order corrections are $\Or(\varepsilon^2)$.
	These were not included in the formulae quoted in Ref.~\cite{Chen:2006nt}.

	Second, we retain a floating reference scale $k_\star$,
	chosen to be $k_\star = k_t$ in Ref.~\cite{Chen:2006nt}.
	Retaining this scale allows us to extract the scale- and
	shape-dependences of
	$\fNL$---see 
	\S\S\ref{sec:running}--\ref{sec:shapes}. 





	\subsection{Formulae for $\fNL$}
	\label{subsec:fnl}

	The individual bispectra, with their detailed shape-dependence,
	are the principal observable objects containing a wealth of 
	information about the microphysics during inflation.
	However, for simple model comparisons it is helpful and quite popular to have
	an explicit expression for the nonlinearity parameter $\fNL$
	defined in Eq.~\eqref{eq:deffnl}. 
	Accounting for scale-dependent logarithms present in the power
	spectrum \eqref{eq:powerspectrum}, one finds
	\begin{equation}
		\fNL
		=
		\dfrac{5}{6}
		\left(
			\dfrac{4 z_{\star} \csstar^3}{H_{\star}^2}
		\right)^2
		\frac{B(k_1, k_2, k_3) \prod_i k_i^3}
			{\sum_i k_i^3
			\Big\{
				1
				+ 4E_{\star}
				- 2\varpi_{1\star}
				\ln \big(
					k_i^{-1} k_t^{-2} \prod_j k_j
				\big)
			\Big\}} \ \ 
		.
		\label{eq:fnl-logarithms}
	\end{equation} 
	This expression is to be expanded uniformly to
	$\Or(\varepsilon)$ in slow-variation parameters.
	It is therefore valid up to next-order corrections 
	in the slow-variation approximation.
	
	There is
	another reason to study $\fNL$, which is related 
	to Maldacena's factorisation rule.
	We have explained that
	large logarithms of the form
	$\ln (k_i / k_\star)$ or $\ln (k_i / k_t)$
	are to be expected
	in the squeezed limit $k_i \rightarrow 0$,
	describing variation of the bispectrum with shape.
	The power spectrum $P(k)$ contains similar large logarithms.
	Since copies of the power spectrum must
	be factored out to obtain $\fNL$, one may anticipate it to be
	more regular in the squeezed limit.
	Indeed, a more precise statement is possible.
	Partitioning the momenta into a single soft mode of order $\ksoft$
	and two hard modes both of order $\khard$,
	Maldacena's consistency condition requires
	\cite{Maldacena:2002vr}
	\begin{equation}
		\fNL \longrightarrow - \frac{5}{12} ( n_s - 1 )|_{\khard}\ \ ,
		\label{eq:maldacena-condition}
	\end{equation}
	as $\ksoft \rightarrow 0$,
	where the right-hand side is to be evaluated at horizon
	exit for the mode $\khard$. It is clear from Eq. 
\eqref{eq:maldacena-condition}
	that,
in this limit, two and three-point correlators talk to each other.
	Both sides of Eq.~\eqref{eq:maldacena-condition} are finite
	and independent of any logarithms associated with the
	squeezed limit;
	this factorisation procedure 
	absorbs all the power-law and logarithmic divergences.
	
	
	For each operator $i$, we write the corresponding $\fNL$
	as ${\fNL}_i$
	and quote it in the form
	\begin{equation}
		{\fNL}_i = \left. \fNL \right|_{i0} \big\{
			1
			+ \kappa_{h|i} h_{i\star}
			+ \kappa_{v|i} v_{\star}
			+ \kappa_{s|i} s_{\star}
			+ \kappa_{\varepsilon|i} \varepsilon_{\star}
		\big\} \ \  .
		\label{eq:next-order-fnl}
	\end{equation}
	In Tables~\ref{table:fNLequilateral}
	and~\ref{table:fNLsqueezed}
	we give explicit expressions for the coefficient functions
	$\left. \fNL \right|_{i0}$
	and $\kappa_i$
	specialised for equilateral%
		\footnote{The quoted quantity is $\fNL(k,k,k)$, which is
		\textit{not} the same as $\fNL^{\mathrm{(equilateral)}}$ for which constraints
		are typically given
		\cite{Senatore:2009gt,Komatsu:2010fb}.
		To obtain $\fNL^{\mathrm{(equilateral)}}$, one should
		take an appropriately normalised inner product
		(see~\S\ref{sec:shapes} for a simple example)
		between the full next-order
		bispectrum shape and the equilateral template
		\cite{Creminelli:2005hu,Creminelli:2006rz}.
		\label{footnote:equilateral}}
	and squeezed triangular configurations.
 	Table~\ref{table:fNLsqueezed} confirms
 	that $\fNL$ in Eq. \eqref{eq:next-order-fnl} 
 	is finite in the squeezed limit,
 	as required.
 	
 	In the next sections we explore our calculation
 	of the bispectrum. We start by applying our 
 	results to popular single-field models.
 
 
	\begin{sidewaystable}
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	
	\sbox{\tableA}{%
		\begin{tabular}{QqQqQq}
		   	\toprule

			&
			\multicolumn{5}{c}{operator}
			\\

			\cmidrule(l){2-6}

		 	& 
		 	\multicolumn{1}{c}{$\zeta'^3$} &
		 	\multicolumn{1}{c}{$\zeta \zeta'^2$} &
		 	\multicolumn{1}{c}{$\zeta ( \partial \zeta)^2$} &		 	\multicolumn{1}{c}{$\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta'$} &
		 	\multicolumn{1}{c}{$\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2$}
		 	\\

			\midrule

			\left. \fNL \right|_{i0} &

			\frac{5}{81} \frac{g_{1\star} H_\star}{\zterm_\star} &
			\frac{10}{27} \frac{g_{2\star}}{\zterm_\star} & 
			\frac{85}{108} \frac{g_{3\star}}{\zterm_\star \csstar^2} & 			-\frac{5}{27} \frac{g_{4\star}}{\zterm_\star} &
			\frac{10}{27} \frac{g_{5\star}}{\zterm_\star}
			\\[2mm]

			\cmidrule{2-6}

			\multirow{2}*{$\kappa_{h|i}$} &
			\EulerGamma - \frac{3}{2} + \ln \frac{3k}{k_\star} &
			\EulerGamma - \frac{1}{4} + \ln \frac{3k}{k_\star} &
			\EulerGamma - \frac{26}{17} + \ln \frac{3k}{k_\star} &
			\EulerGamma - \frac{1}{4} + \ln \frac{3k}{k_\star} &
			\EulerGamma - \frac{1}{4} + \ln \frac{3k}{k_\star}
			\\

			&
			-0.922784\tmark{a} &
			0.327216\tmark{a} &
			-0.952196\tmark{a} &
			0.327216\tmark{a} &
			0.327216\tmark{a}
			\\

			\cmidrule{2-6}

			\multirow{2}*{$\kappa_{v|i}$} &
			-\EulerGamma - \frac{29}{2} + 78\omega - \ln \frac{2k}{k_\star} &
			-\EulerGamma - \frac{1}{4} + 6\omega - \ln \frac{2k}{k_\star} &
			-\EulerGamma + \frac{22}{17} + \frac{30}{17}\omega
				- \ln \frac{2k}{k_\star} &
			-\EulerGamma - \frac{1}{4} + 6\omega - \ln \frac{2k}{k_\star} &
			-\EulerGamma - \frac{1}{4} + 6\omega - \ln \frac{2k}{k_\star}
			\\

			&
			1.14139\tmark{a} &
			0.794645\tmark{a} &
			1.48013\tmark{a} &
			0.794645\tmark{a} &
			0.794645\tmark{a}
			\\

 			\cmidrule{2-6}

			\multirow{2}*{$\kappa_{s|i}$} &
			-49 + 240 \omega &
			-\frac{3}{2} + 24 \omega &
			-2\EulerGamma + \frac{40}{17} + \frac{124}{17}\omega -
				2\ln\frac{2k}{k_\star} &
			-\frac{3}{2} + 24 \omega &
			-\frac{3}{2} + 24 \omega
			\\

			&
			-0.344187\tmark{a} &
			3.36558\tmark{a} &
			3.4882\tmark{a} &
			3.36558\tmark{a} &
			3.36558\tmark{a}
			\\

			\cmidrule{2-6}

			\multirow{2}*{$\kappa_{\varepsilon|i}$} &
			-\EulerGamma - \frac{63}{2} + 158 \omega - \ln \frac{2k}{k_\star} &
			-1 + 16 \omega &
			-\frac{8}{17} + \frac{128}{17} \omega &
			-1 + 16 \omega &
			-1 + 16 \omega
			\\

			&
			0.359993\tmark{a} &
			2.24372\tmark{a} &
			1.05587\tmark{a} &
			2.24372\tmark{a} &
			2.24372\tmark{a}
			\\

 			\bottomrule

 		\end{tabular}
 	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
 	\end{center}

	\renewcommand{\arraystretch}{1}
	
	\sbox{\tableB}{%
		\begin{tabular}{l@{\hspace{1mm}}l}
			\tmark{a} & \parbox[t]{\tblw}{%
				Evaluated at the conventional reference scale
				$k_\star = k_t$ for a quantitative result.}
		\end{tabular}
	}
	
	\begin{center}
		\usebox{\tableB}
	\end{center}

 	\caption{\label{table:fNLequilateral}Equilateral limit of $\fNL$ at
 			 leading and next-order in the slow-roll approximation.
 			 The numerical constant $\omega$ satisfies
 			 $\omega = \frac{1}{2} \ln \frac{3}{2} = \coth^{-1} 5$.}
 	
 	\end{sidewaystable}

	\begin{table}
	\small
	\heavyrulewidth=.08em
	\lightrulewidth=.05em
	\cmidrulewidth=.03em
	\belowrulesep=.65ex
	\belowbottomsep=0pt
	\aboverulesep=.4ex
	\abovetopsep=0pt
	\cmidrulesep=\doublerulesep
	\cmidrulekern=.5em
	\defaultaddspace=.5em
	\renewcommand{\arraystretch}{1.6}
	
	\sbox{\tableA}{%
		\begin{tabular}{QqQqQq}
		   	\toprule

			&
			\multicolumn{5}{c}{operator}
			\\

			\cmidrule(l){2-6}

		 	& 
		 	\multicolumn{1}{c}{$\zeta'^3$} &
		 	\multicolumn{1}{c}{$\zeta \zeta'^2$} &
		 	\multicolumn{1}{c}{$\zeta ( \partial \zeta)^2$} &
		 	\multicolumn{1}{c}{$\zeta' \partial_j \zeta \partial_j \partial^{-2} \zeta'$} &
		 	\multicolumn{1}{c}{$\partial^2 \zeta (\partial_j \partial^{-2} \zeta')^2$}
		 	\\

			\midrule

			\left. \fNL \right|_{i0} &
			&
			\frac{5}{24} \frac{g_{1\star}}{\zterm_\star} & 
			\frac{5}{8} \frac{g_{2\star}}{\zterm_\star \csstar^2} & 
			&
			\\[2mm]

			\cmidrule{2-6}

			\multirow{2}*{$\kappa_{h|i}$} &
			&
			\EulerGamma + \ln \frac{2k}{k_\star} &
			\EulerGamma - \frac{4}{3} + \ln \frac{2k}{k_\star} &
			&
			\\

			&
			&
			0.577216\tmark{a} &
			-0.756118\tmark{a} &
			&
			\\

			\cmidrule{2-6}

			\multirow{2}*{$\kappa_{v|i}$} &
			&
			-\EulerGamma + 1 - \ln \frac{2k}{k_\star} &
			-\EulerGamma + \frac{5}{3} - \ln \frac{2k}{k_\star} &
			&
			\\

			&
			&
			0.422784\tmark{a} &
			1.08945\tmark{a} &
			&
			\\

 			\cmidrule{2-6}

			\multirow{2}*{$\kappa_{s|i}$} &
			&
			3 &
			-2\EulerGamma + \frac{11}{3} - 2\ln\frac{2k}{k_\star} &
			&
			\\

			&
			&
			&
			2.51224\tmark{a} &
			&
			\\

			\cmidrule{2-6}

			\multirow{2}*{$\kappa_{\varepsilon|i}$} &
			&
			2 &
			\frac{2}{3} &
			&
			\\
			
			&
			&
			&
			0.666667 &
			&
			\\

 			\bottomrule

 		\end{tabular}
	}
	\settowidth{\tblw}{\usebox{\tableA}}
	\addtolength{\tblw}{-1em}

	\begin{center}
		\usebox{\tableA}
 	\end{center}

	\renewcommand{\arraystretch}{1}
	
	\sbox{\tableB}{%
		\begin{tabular}{l@{\hspace{1mm}}l}
			\tmark{a} & \parbox[t]{\tblw}{Evaluated at the reference scale
				$k_\star = 2 \khard$ for a quantitative result, where $\khard$ is the common
				hard momentum.}
		\end{tabular}
	}
	
	\begin{center}
		\usebox{\tableB}
	\end{center}

 	\caption{\label{table:fNLsqueezed}$\fNL$ in the squeezed limit at
 			 leading and next-order in the slow-roll approximation.}
 	
 	\end{table}






	\section{Canonical single-field inflation}
	\label{sec:vanilla}

	The simplest model of inflation is that of a single, canonical scalar field
		dominating the inflation era.
	Maldacena showed that
	the fluctuations in this model are almost
	Gaussian,
	with $\fNL$ being unobservably small \cite{Maldacena:2002vr}.
	In a canonical model, scalar field fluctuations propagate 
	at the speed of light, $\cs = 1$.
	
	
	
	
	\para{Nonlinearity parameter}To calculate $\fNL$ we need to know the expressions for the 
	 flow parameters
	$h_i$, which measure the time-dependence
	in $g_i$ of Eq. \eqref{eq:gi}.
	These are
	\begin{equation}
		\begin{aligned}
		h_1 &
		=
		0 \ \ ,
		&
		\hspace*{1cm} h_2 &
		=
		\frac{\eta\, ( 2 \varepsilon - \eta - \xi )}{\varepsilon - \eta}\ \ ,
		&
		&
		\\
		h_3 &
		=
		\frac{\eta \, ( 2 \varepsilon + \eta + \xi )}{\varepsilon + \eta}\ \ ,
		 \hspace*{1cm}&
		h_4  &
		=
		\frac{\eta \, ( 8 - \varepsilon )}{4}\ \ , \hspace*{1cm}
		&
		\hspace*{1cm} h_5
		&
		=
		3\eta\ \  .
		\end{aligned}
		\label{eq:h_i}
	\end{equation}
	In this model
	the time-dependence of $z$ is described by $v=\eta$.
	Collecting contributions from
	Table~\ref{table:fNLequilateral},
	we find the equilateral limit of $\fNL$, 
	which we shall denote by 
	$\fNL^{\textrm{(equilateral)}}$, is 
	\begin{equation}
		\begin{split}
			\fNL^{\textrm{(equilateral)}} \rightarrow
			\frac{5}{36} \bigg\{
				11 \varepsilon_\star
				+ 3 \eta_\star
				&
				+ \frac{35 \varepsilon_\star^2}{216} \bigg(
					768 \omega - 54
				\bigg)
				+ \frac{35 \eta_\star \xi_\star}{36} \bigg(
					3 \EulerGamma 
					- 8
					+ 3 \ln \frac{3k}{k_\star}
				\bigg)
				\\ & \mbox{}
				+ \frac{35 \varepsilon_\star \eta_\star}{36} \bigg(
					11 \EulerGamma
					- 14
					+ 64 \omega
					+ 11 \ln \frac{3k}{k_\star}
				\bigg)
			\bigg\} \ \ ,
		\end{split}
		\label{eq:fnlevanilla}
	\end{equation}
	where we have used the numerical constant $\omega = \coth^{-1} 5$,
	and $k$ is the common momentum scale,
	$k_i = k$.
	Likewise,
	the squeezed limit may be recovered from Table~\ref{table:fNLsqueezed}.
	We find
	\begin{equation}
		\begin{split}
			\fNL^{\textrm{(squeezed)}}
			\rightarrow
			\frac{5}{12} \bigg\{
				2 \varepsilon_\star
				+ \eta_\star
				+ 2 \varepsilon_\star^2
				+ \eta_\star \xi_\star \bigg(
					\EulerGamma
					- 2
					+ \ln \frac{2 k}{k_\star}
				\bigg)
				+ \varepsilon_\star \eta_\star \bigg(
					2 \EulerGamma
					- 1
					+ 2 \ln \frac{2 k}{k_\star}
				\bigg)
			\bigg\} \ \ ,
		\end{split}
		\label{eq:fnlsvanilla}
	\end{equation}
	where $k$ is now the scale of the hard
	momenta, $\khard$.
	In \S\ref{subsec:fnl} 
	we emphasized that $\fNL$ should
	be finite in this limit, containing
	no large logarithms, because these factorise into
	the power spectrum and are subtracted upon division.
	The surviving logarithms [the $\ln (2k / k_\star)$
	terms in Eq. \eqref{eq:fnlsvanilla}]	
	track the
	dependence of $\fNL$ on the hard scale, and will be studied below.
	Using Eq. \eqref{eq:maldacena-condition} and comparing with
	the spectral indices quoted in
	Table~\ref{table:spectral-index},
	it is easy to check that our formula correctly reproduces
	Maldacena's limit.

	
	
	
	
	\section{Non-canonical single-field inflation}
	\label{sec:noncanonical}
		
	For the non-canonical action~\eqref{eq:startingaction},
	the $h_i$ can be written as
	\begin{equation}
		\begin{aligned}
			h_1 &
			= \varepsilon + \eta - 2s +
				\frac{\frac{2\lambda}{\Sigma}
					(\eta - 2 \varepsilon - 2 s - \ell) - \frac{2}{\cs^2} s}
					{\frac{1-\cs^2}{\cs^2} - \frac{2\lambda}{\Sigma}}\ \ , 
			& \hspace*{1cm}
			h_2 &
			=
			\eta - 4s +
				\frac{\eta ( \varepsilon - \xi ) + 6 \cs^2 s}
					{\eta - \varepsilon - 3 ( 1 - \cs^2 )}\ \ ,
						\vspace*{0,5cm}
			\\
			\vspace*{0,5cm}
			h_3 &
			=
			\eta - 2s +
				\frac{\eta ( \varepsilon + \xi ) - 2s ( t - \cs^2 )}
					{\varepsilon + \eta - 2s + ( 1 - \cs^2 )}\ \ ,
			& \hspace*{1cm}
			h_4 &
			=
			2 \eta - 4s -
				\frac{\eta \varepsilon}{4 - \varepsilon}\ \ ,
			\\
			h_5 &
			=
			3 \eta - 4 s \ \ ,
		\end{aligned}
		\label{eq:general-hi}
	\end{equation}
	where we have defined $\xi \equiv \dot{\eta} / H \eta$, 
	$\ell \equiv  \dot{\lambda} / H \lambda$ \cite{Chen:2006nt}, 
 and
	$t \equiv \dot{s} / H s$.
	
	In the canonical case, it was possible to verify Maldacena's
	consistency condition to next-order.
	In the non-canonical case this is not possible without a next-next-order
	calculation, because
	for $\cs \neq 1$ the leading contribution to $\fNL$ is first-order
	in the slow-variation expansion. Therefore our calculation of subleading
	corrections produces a result valid to $\Or(\varepsilon)$, which is
	short of the $\Or(\varepsilon^2)$ accuracy required to verify the
	consistency condition at next-order.
	Chen {\etal} gave the subleading corrections in terms
	of undetermined integrals \cite{Chen:2006nt}. Expanding these
	asymptotically,
	they argued that the consistency relation would be satisfied
	at lowest-order.
	More recently, Renaux-Petel \cite{RenauxPetel:2010ty}
	gave an equivalent demonstration. Here, we have knowledge of the
	full bispectrum to subleading order. Using Eq. \eqref{eq:general-hi},
	it can be verified that in the squeezed limit,
	and expanding around a reference scale $k_\star$,
	\begin{equation}
		\fNL^{\textrm{(squeezed)}} \rightarrow \frac{5}{12} \left(
			2 \varepsilon_\star + \eta_\star + s_\star
		\right) \ \ .
	\end{equation}
	One may check that this agrees with
	Eq.~\eqref{eq:maldacena-condition} and Table~\ref{table:spectral-index}.
	
	
	
	\subsection{Asymptotically power-law models}
	\label{subsec:power-law}
	
	Power-law inflationary models were introduced by
	Lucchin \& Matarrese \cite{Lucchin:1984yf,Lucchin:1985wy}, who
	studied potentials producing an expansion history of the
	form $a(t) \propto t^{1/p}$, 
	where $p<1$ is a constant.
This describes an inflating solution.	
Exact solutions can be found in the canonical case,
	upon which the next-order calculation was based 
	\cite{Lidsey:1995np}.
	
	In this section we study two examples which
	are asymptotically described by non-canonical power-law
	inflation at late times.
	The first is Dirac--Born--Infeld (DBI) inflation,
	which produces a scale-invariant power spectrum
	of perturbations 
	at leading-order. Departures from scale-invariance
	appear at next-order in the slow-roll approximation.
	This special property implies that we can compare our results
	to a formula of Khoury \& Piazza
	which was obtained without invoking the
	slow-roll approximation, but where
	a scale-invariant spectrum was imposed \cite{Khoury:2008wj}.
		Here we expand the discussion initiated 
	in \S\ref{subsec:beyond-simple-inflation}.
	Our second example is $k$-inflation, for which the power
	spectrum is not scale-invariant at lowest-order,
	and to which Khoury \& Piazza's result does not apply.

	\subsubsection{Dirac--Born--Infeld inflation}
	\label{sec:dbi}
	The DBI action is a low-energy effective theory
	which
	describes a D3-brane moving in warped space.
	It was
	proposed as a model of inflation by Silverstein \& Tong
	\cite{Silverstein:2003hf}, and subsequently developed 
	with Alishahiha \cite{Alishahiha:2004eh}.
	The action is of the form~\eqref{eq:startingaction},
	with $P(X, \phi)$ satisfying
	\begin{equation}
 		P(X, \phi)
 		=
 		-\dfrac{1}{f(\phi)}
 		\left\{
 			\sqrt{1-f(\phi) \ X} -1
 		\right\}
 		-
 		V(\phi)\ \ ,
		\label{eq:dbiaction}
	\end{equation} 
	where $f$ is an arbitrary function of $\phi$
	known as the warp factor,
	and $V(\phi)$ is the potential arising from couplings between
	the brane and other degrees of freedom.
	The DBI Lagrangian is non-analytical but algebraically special
	\cite{Lidsey:2006ia,deRham:2010eu,Leblond:2008gg}.
	It enjoys a number of remarkable properties, including
	a form of non-renormalisation theorem
	\cite{Shmakova:1999ai,DeGiovanni:1999hr,Tseytlin:1999dj};
	its invariance under a higher-dimensional boost
	makes DBI one rare example of a 
	radiatively stable higher-derivative model against quantum corrections.
	
	In principle in the DBI action non-minimal curvature couplings
	can be present, of the form $R\phi^2$,
	which spoil inflation
	\cite{Easson:2009kk}.
	This gives a form of the $\eta$-problem,
	and
	we assume such terms to be negligible.


	It is conventional to define a
	Lorentz factor as follows
	\begin{equation}
		\gamma
		\equiv
		(1-f \dot{\phi}^2)^{-1/2}\ \  .
		\label{eq:def-gamma-dbi}
	\end{equation}
	When $\gamma \sim 1$ the motion of the brane in the warped throat 
	is nonrelativistic.
	When $\gamma \gg 1$, the brane is moving close to the speed limit.
	The Lorentz factor is related to the speed of sound of perturbations by
	$\cs = \gamma^{-1}$.
	In the limit $\gamma \gg 1$, the scalar fluctuations around
	background solutions of the action \eqref{eq:dbiaction}
	propagate at small sound speed, which is related to
	large non-gaussianities.
	The square root in Eq. \eqref{eq:dbiaction} must be real,
	imposing a dynamical speed limit for $\phi$.
	
		Eq.~\eqref{eq:dbiaction}
	makes $2\lambda / \Sigma = (1-\cs^2)/\cs^2$,
	which requires $g_1 \rightarrow 0$ but
	causes the denominator of $h_1$ given in Eq. \eqref{eq:general-hi}
	to diverge.
	Only the finite combination $g_1 h_1$ appears in the physical, 
	observable quantity $\fNL$,
	and it can indeed be checked that $g_1 h_1 \rightarrow 0$ as required.
	
	
	
	\para{``Traditional'' DBI inflation scenario}Silverstein \& Tong \cite{Silverstein:2003hf} obtained
	attractor solutions supported by \eqref{eq:dbiaction}
	and specific forms of the potential and warping, which 
	were described at late times by power-law inflation.
	In this limit,
	the slow-variation parameters $\varepsilon$ and $s$ are
	constant, with $\eta = \xi = t = 0$, but $\ell$ does not vanish.
	Variation of the sound speed gives $s = - 2\varepsilon$, making
	$\varpi = 0$ and yielding 
	scale-invariant fluctuations at
	leading-order in slow-roll [cf. Eq. \eqref{eq:rge}] \cite{Khoury:2008wj}.
	In the equilateral limit,%
		\footnote{Recall that the equilateral limit is
		$\fNL(k,k,k)$, and not the quantity constrained by
		experiment.}
	we find 
	\begin{equation}
		\fNL^{\textrm{(equilateral)}} \rightarrow
		- \frac{35}{108} \big( \gamma^2_\star - 1\big) \left\{
			1 - \frac{\gamma_\star^2}{\gamma_\star^2-1} \,
			( 3 - 4 \EulerGamma )\, \varepsilon
			+ \Or\big(\gamma_\star^{-2}\big)
		\right\}\ \  .
		\label{eq:dbi-fnl-eq}
	\end{equation}
	In \S\ref{sec:evolution_NGs} we have estimated the
	relative uncertainty in
	$\fNL$ to be $\sim 14 \varepsilon$,
	working in the limit $\gamma \gg 1$, based on
	$\Or(\varepsilon)$ terms from the vertices \eqref{eq:gi} only.
	Eq.~\eqref{eq:dbi-fnl-eq} shows that,
	because of an apparently fortuitous cancellation,
	this large contribution is almost
	completely subtracted, leaving a small fractional
	correction of only $\sim 0.69 \varepsilon$.
	
	In the squeezed limit we find
	\begin{equation}
		\fNL^{\textrm{(squeezed)}} \rightarrow
		\frac{10 \gamma^2_\star}{3} \varepsilon^2
		\left\{
			4 \EulerGamma
			- 5
			+ 4 \ln \frac{4k}{k_\star}
		\right\} \ \ 
		.
	\end{equation}
	which is $\Or(\varepsilon^2)$, as predicted by 
	Maldacena's condition~\eqref{eq:maldacena-condition}
	and the property $\varpi = 0$
	\cite{Alishahiha:2004eh}.
	
	\para{Comparison with previous results}Khoury \& Piazza estimated
	the bispectrum in
	a power-law inflationary model
	satisfying exact scale-invariance, $\varpi = 0$,
	without invoking an expansion in slow-variation parameters
	\cite{Khoury:2008wj}. 
	They quoted their
	results in terms of a quantity $f_X$
	which replaces $\lambda$, as follows
	\begin{equation}
		\lambda \equiv \frac{\Sigma}{6} \left(
			\frac{2 f_X +1}{\cs^2} - 1
		\right) \ \ .
	\end{equation}
	For the DBI model, $f_X = 1 - \cs^2$.
	They assumed constant $f_X$, making their
	result valid to all orders in $\varepsilon$
	but only lowest-order in the time dependence of $f_X$.
	Working in the
	equilateral limit
	for arbitrary but constant $f_X$,
	we find
	\begin{equation}
		\begin{split}
			\fNL^{\textrm{(equilateral)}} \rightarrow
			&
			- \frac{5}{972 \csstar^2} \Big\{
				55 ( 1 - \csstar^2 ) + 8 f_{X}
			\Big\}
			\\ & \mbox{}
			 +
			 \frac{5 \varepsilon}{972 \csstar^2}
			 \left\{
			 	149
			 	- 8 \csstar^2
			 	- 220 \EulerGamma
			 	- 220 \ln \frac{3k}{k_\star}
			 	+ f_X \left(
			 		40
			 		- 32 \EulerGamma
			 		- 32 \ln \frac{3k}{k_\star}
			 	\right)
			 \right\}\ \  .
		\end{split}
		\label{eq:khoury-piazza}
	\end{equation}
	Adopting the evaluation point $k_\star = 3k$, this precisely
	reproduces Khoury \& Piazza's Eq. (8.4) \cite{Khoury:2008wj}
	when expanded to first-order in $\varepsilon$.
	Although Eq. \eqref{eq:khoury-piazza}
	does not rigorously apply to DBI, where
	$\cs$ and thus $f_{X}$ are changing,
	it can be checked that effects due to the time-dependence
	of $f_X$ do not appear at next-order.
	Indeed, Eq.~\eqref{eq:khoury-piazza} yields Eq. \eqref{eq:dbi-fnl-eq}
	when $f_X = 1 - \gamma^{-2}$.
	
	
	
	
	
	
	\para{Generalized DBI inflation}The analysis above was restricted to the
	asymptotic power-law regime first
	obtained by Silverstein \& Tong \cite{Silverstein:2003hf}, 
	but this is not required.
	Using an arbitrary potential $V(\phi)$ in the action \eqref{eq:dbiaction}
	one can in principle construct a generic quasi-de Sitter 
	background. Many of their properties, including the attractor behaviour,
	were studied by Franche {\etal} 
	in Ref. \cite{Franche:2009gk}.
	
	
	How can we learn about the shape of the potential
	from observables such as $\fNL$? We will show that through the 
	next-order terms in $\fNL$ we will be able 
	to estimate
	corrections arising from the shape of $V(\phi)$ or $f(\phi)$.
	Analogous effects have been computed for galileon
	inflation~\cite{Burrage:2010cu}, but
	our computation enables us to determine them in
	the DBI scenario for the first time.	
	This is particularly relevant since the motivation behind DBI lies in 
	brane inflation scenarios, and we can now gain access to 
	compactification data which was previously hard, 
	or even impossible to obtain by other means.
	
	For $\gamma \gg 1$ the non-canonical structure suppresses the
	background dependence
	on details of the potential.
	But small fluctuations around the background
	cannot be shielded from these details,
	which induce three-body interactions
	whether or not they are relevant
	for supporting the quasi-de Sitter epoch.
	These interactions generate relatively unsuppressed
	contributions to the three-point function.
	
	We adapt the notation of Franche {\etal} \cite{Franche:2009gk},
	who defined
	quantities measuring the shape of the potential $V(\phi)$ and the warping
	$f(\phi)$%
		\footnote{The factor $\sgn\big( \dot{\phi} f^{1/2} \big)$ was not
		used by Franche {\etal} \cite{Franche:2009gk}, but is necessary
		here because the relativistic background solution
		requires $f X = 1 + \Or(\gamma^{-2})$
		up to corrections suppressed by
		$\Or(\varepsilon)$, which are higher-order than those we retain.
		Depending on the direction of motion,
		this yields $\dot{\phi} = \pm f^{-1/2} + \Or(\gamma^{-2})$.
		The choice of sign is important in obtaining the correct mapping between $\varepsilon$ and
		$\varepsilonSR$, and others.}
	\begin{equation}
		\varepsilonSR
			\equiv \frac{1}{2} \left( \frac{V'}{V} \right)^2 \ ,
		\quad
		\etaSR
			\equiv \frac{V''}{V} \ ,
		\quad
		\text{and}
		\quad
		\Delta
			\equiv \sgn(\dot{\phi}f^{1/2} ) \,
			\frac{f'}{f^{3/2}} \frac{1}{3H}\ \  .
			\label{eq:srFranche}
	\end{equation}
	The same branch of $f^{1/2}$ should be chosen in computing
	$f^{3/2}$ and $\sgn( \dot{\phi} f^{1/2} )$.
	Note that these shape parameters do \emph{not} coincide with
	the `global' slow-variation parameters
	$\varepsilon$ and $\eta$ defined in Eq. \eqref{eq:slowvariation}.
	Franche {\etal} argued that $\Delta \ll 1$ was required
	to obtain attractor solutions, which
	we will assume to be satisfied in what follows.
	In addition,
	we work in the equilateral limit
	and take $\gamma \gg 1$, which is the regime of principal
	interest for observationally large $\fNL$.
	With these assumptions we find
	\begin{equation}
		\varepsilon
			\rightarrow \frac{\varepsilonSR}{\gamma} \ ,
		\quad
		\eta \rightarrow 3\, \frac{\varepsilonSR}{\gamma}
			- \frac{\etaSR}{\gamma}
			- \frac{3}{2}\, \Delta \  ,
		\quad
		\text{and}
		\quad
		s \rightarrow - \frac{\varepsilonSR}{\gamma}
			+ \frac{\etaSR}{\gamma}
			- \frac{3}{2} \,\Delta \ \  .
		\label{eq:franche-shape-parameters}
	\end{equation}
	The leading-order term of Eq. \eqref{eq:dbi-fnl-eq}
	is unchanged,
	but the subleading terms are dominated by
	shape-dependent corrections, as follows:
	\begin{equation}
		\begin{split}
			\fNL^{\textrm{(equilateral)}} \rightarrow - \frac{35\gamma_\star^2}{108}
				\Bigg\{
					1
					& \mbox{}
					+ \frac{3 \Delta_\star}{14}
					\bigg(
						31
						+ 14 \EulerGamma
						- 228 \omega
						+ 14 \ln \frac{2k}{k_\star}
					\bigg)
					+ \frac{\etaSRstar}{7 \gamma_\star}
					\bigg(
						3
						- 14 \EulerGamma
						- 14 \ln \frac{3k}{k_\star}
					\bigg)
					\\ & \mbox{}
					- \frac{2 \varepsilonSRstar}{7 \gamma_\star}
					\bigg(
						43
						- 7 \EulerGamma
						- 256 \omega
						- 7 \ln \frac{3k}{k_\star}
					\bigg)
					+ \Or(\gamma_\star^{-2})
				\Bigg\} \ \  .
		\end{split}
	\end{equation}
	These subleading terms
	are more important than those present in Eq. \eqref{eq:dbi-fnl-eq},
	which began at relative order $\gamma_{\star}^{-2}$
	and are therefore strongly suppressed for $\gamma \gg 1$.
	Moreover, upon inspection of Eq. \eqref{eq:franche-shape-parameters}, 
	inflation can occur even for relatively large values of
	$\varepsilonSR$ and $\etaSR$,
	roughly whenever $\varepsilonSR / \gamma < 1$---hence these corrections need \textit{not} be extremely small.
	
	For large $\big|\fNL^{\textrm{(equilateral)}}\big|$,
	we estimate the relative correction to the 
	leading-order $\fNL^{\textrm{(equilateral)}}$ to be
	\begin{equation}
		\frac{\Delta \fNL^{\textrm{(equilateral)}}}{\fNL^{\textrm{(equilateral)}}}
		\simeq
		- 2.75  \Delta_\star
		+
		\frac{2.10 \varepsilonSRstar - 0.41 \etaSRstar}
		{\big|\fNL^{\textrm{(equilateral)}}\big|^{1/2}}\ \  .
		\label{eq:dbi-shape-corrections}
	\end{equation}
	For negative equilateral $\fNL$,
	current constraints roughly require
	$|\fNL|^{1/2} \lesssim 12$ \cite{Komatsu:2010fb}.
	Therefore, these corrections can be rather important unless
	the potential is tuned to be flat,
	although some cancellation occurs because $\varepsilonSR$
	and $\etaSR$ enter with opposite signs.
	
	To obtain an estimate, we suppose 
	for simplicity that $\Delta_\star$ is negligible.
	Taking the extreme $95\%$-confidence value $\fNL = -151$
	\cite{Komatsu:2010fb}, and
	$\varepsilonSR \simeq |\etaSR| \sim 1$ 
	for a ``generic'' potential,
	the correction is of order $14\%$ if $\etaSR > 0$
	and $20\%$ if $\etaSR < 0$.
	To reduce these shifts
	we might be prepared to assume $\varepsilonSR \simeq |\etaSR| \sim 0.1$, 
	which suppresses the correction to the percent level.
	Nevertheless, the corrections grow with decreasing $|\fNL|$.
	Keeping the generic estimate $\varepsilonSR \simeq |\etaSR| \sim 1$,
	and using
	$|\fNL| \approx  50$,\footnote{For these values $\gamma \approx 10$ and
								the approximation $\gamma \gg 1$ used to
								derive Eq. \eqref{eq:dbi-shape-corrections}
								is at the limit of its applicability.}
	we find the corrections to be of order
	$24\%$ for $\etaSR > 0$
	and $36\%$ for $\etaSR < 0$.\footnote{In producing these estimates we are discarding constraints arising from the normalisation of the power spectrum.}
	These are significant and cannot be ignored.
	
	Although Franche {\etal} argued that $\Delta_\star$ must be small
	to obtain attractor behaviour, it need not be entirely negligible.
	In such cases it introduces a dependence on the shape of the
	warp factor in addition to the shape of the potential.
	This may be positive or negative.
	If the $\Delta_\star$ and $\varepsilon_\star$ terms add
	constructively, the next-order correction can become rather large.
	This, however, will be very model-dependent.
	
	\para{Infrared model}The 
	DBI scenario can be
	realized in several ways. The original ``ultraviolet'' model
	is now disfavoured by microscopic considerations
	\cite{Baumann:2006cd,Lidsey:2006ia}.
	Chen introduced
	an alternative ``infrared'' implementation 
	\cite{Chen:2004gc,Chen:2005ad,Chen:2005fe}
	which
	evades these constraints and remains compatible with
	observation
	\cite{Bean:2007eh, Bean:2007hc, Peiris:2007gz, Alabidi:2008ej}.
	In this infrared version of DBI inflation, 
	the warp factor
	$f(\phi)$ is that of an AdS throat $\lambda/\phi^4$, 
	where $\lambda$ is a dimensionless
	parameter.
	The potential is given by 
	\[ V(\phi) = V_0 - \beta^2 H^2 \phi^2 / 2 \ \ ,  \]
	in which the mass is expressed
	as a fraction $\beta^{1/2}$ of the Hubble scale.
	The constant term $V_0$ dominates, making
	$\varepsilon$ negligible, but 
	the remaining slow-variation parameters need not be small.
	It is convenient to express our results in terms of the number
	e-folds to the end of inflation, $N_e$, which satisfies
	$\gamma \simeq \beta N_e/3$.
	Background quantities evaluated at this time carry a subscript
	`$e$.'
	
	Evaluating Eq. \eqref{eq:franche-shape-parameters}
	for these choices of $V$ and $f$,
	we obtain
	\begin{equation}
\eta_e \simeq 3/N_e \ \ \textrm{and} \ \ s_e \simeq 1/N_e \ \ .
\end{equation}
	The infrared model is an example where $\Delta_e \sim 1/N_e$ is not
	negligibly small.
	Using Eq. \eqref{eq:dbi-shape-corrections}, we find
	\begin{equation}
		\frac{\Delta \fNL}{\fNL}
		\simeq
		- \frac{1}{7 N_e} \left\{
			65
			+ 14 \EulerGamma
			- 484 \omega
			+ 14 \ln \frac{2k}{k_\star}
		\right\}
		\simeq
		\frac{4.39}{N_e} \ \ ,
	\end{equation}
	where we have chosen $k_\star = 3k$ in the final step. Adopting the
	best-fit value $N_e \approx  38$ suggested by
	Bean {\etal}~\cite{Bean:2007eh}, we find 
	the fractional correction is of
	order $12\%$.
	This relatively small correction is a consequence of the
	negligible value of $\varepsilon$ in this model.
	Keeping $N_e \approx  38$
	and using the maximum likelihood value $\beta = 1.77$
	quoted by Bean {\etal}, we find $\Delta \fNL \approx  -19$.
	The corresponding shift is from
	$\fNL \approx -163$ without next-order corrections to
	$\fNL \approx -182$ with next-order corrections included.
	This can be measured by \textit{Planck}.


	We conclude that next-order corrections not only need to 
	be taken into account to keep the theory-error below 
	\textit{Planck}'s sensitivity, but they can also reveal important details 
	about the potential and warping in DBI inflation scenarios.
	
	
	
	
	
	

	\subsubsection{$k$-inflation}
	\label{sec:k-inflation}
	
	Another model that admits power-law solutions 
	was proposed by Armend\'{a}riz-Pic\'{o}n, Damour
	\& Mukhanov
	\cite{ArmendarizPicon:1999rj}, and is known
	as $k$-inflation.
	The action is
	\begin{equation}
		P(X, \phi) = \frac{4}{9} \ \frac{4 - 3 \gamma}{\gamma^2}
		\	\frac{X^2 -X}{\phi^2}\ \  ,
		\label{eq:k-inflation-power-law}
	\end{equation}
	where $\gamma$ is some constant, no longer related to the speed
	of sound by the formula $\cs = \gamma^{-1}$ which applied for DBI.
	Unlike the DBI Lagrangian,
	Eq.~\eqref{eq:k-inflation-power-law} is not radiatively
	stable and its microscopic motivation is uncertain. 
	Nevertheless,
	non-gaussian properties
	of the inflationary fluctuations in this toy model
	were studied by Chen {\etal}\ \cite{Chen:2006nt}.
	
	There exists a solution of the action \eqref{eq:k-inflation-power-law}
	with
	\begin{equation}
		X = \frac{2 - \gamma}{4 - 3 \gamma} \ \ ,
	\end{equation}
	making $\varepsilon = 3 \gamma / 2$ and
	$\cs$ constant. Therefore this model has
	$\eta=s = 0$, but non-vanishing $\varepsilon$, and is thus not
	scale-invariant.
	Inflation occurs in the regime for which $0 < \gamma < 2/3$.
	This already requires a relatively tight 
	constraint on the allowed values for $\gamma$.
	The leading-order contribution to $\fNL$ is of order
	$1/\gamma$, making the next-order term of order unity.
	A next-next-order calculation would be required to accurately
	estimate the term of order $\gamma$.
	
	In the equilateral limit,
	Chen {\etal} \cite{Chen:2006nt} quoted the leading-order result
\[\fNL^{\textrm{(equilateral)}} \simeq - 170 / 81 \, \gamma \ \ . \]
	Proceeding as in \S\ref{sec:evolution_NGs} by 
	focusing 
	on the interaction vertices $g_i$ given in Eq. \eqref{eq:gi}, 
	one can estimate the
	fractional
	theoretical uncertainty in this prediction
	to be $\sim 9 \gamma$, or roughly $\pm 20$.
	This is comparable to
	\emph{Planck}'s error bar, and is likely to exceed the error bar
	achieved by a subsequent CMB satellite.
	Still working in the equilateral limit, we find
	\begin{equation}
		\fNL^{\textrm{(equilateral)}} \rightarrow - \frac{170}{81 \gamma} \left\{
			1 - \frac{\gamma}{34} \left( 61 - 192 \ln \frac{3}{2} \right)
			+ \Or(\gamma^2)
		\right\} \ \ .
		\label{eq:k-inflation-fnl-equilateral}
	\end{equation}
	Like for DBI inflation, a fortuitous cancellation brings the
	fractional correction down from our initial estimate
	$\sim 9 \gamma$ to $\sim 0.5 \gamma$ with all the next-order 
	corrections taken into account.
	It was not necessary to choose a reference scale $k_\star$ in order
	to evaluate Eq. \eqref{eq:k-inflation-fnl-equilateral};
	in $k$-inflation,
	$\fNL$ is scale-invariant even though
	the power spectrum is not.
	
	
	

	\para{Comparison with previous results}Because $\varpi \neq 0$ in this model, the analysis of
	Khoury \& Piazza does not apply.
	In another paper, however, Noller \& Magueijo presented a generalisation
	which was intended to be valid for
	constant, but otherwise arbitrary
	$\varepsilon$ and $s$, and small $\varpi$ 
	\cite{Noller:2011hd}.
	Their analysis also assumes constant $f_X$, 
	which is not a good approximation 
	in the regime of rapidly varying speed of sound.
	For comparison, 
	we set the reference scale to be $k_\star = 3k$
	and
	work in the equilateral limit for arbitrary constant
	$f_X$. One finds
	\begin{equation}
		\begin{split}
			\fNL^{\textrm{(equilateral)}} \rightarrow
				& - \frac{5}{972 \csstar^2}
				\Big\{
					55 (1 - \csstar^2) + 8 f_{X}
				\Big\}
				\\ & \mbox{}
				+ \frac{5\varepsilon}{972 \csstar^2}
				\left\{
					177
					+ 120 \csstar^2
					- 1024 \omega ( 1 - \csstar^2 )
					+ f_X \big(
						264
						- 1280 \omega
					\big)
				\right\}
				\\ & \mbox{}
				+ \frac{5 s}{486 \csstar^2}
				\left\{
					7
					+ 55 \EulerGamma
					+ 32 \csstar^2
					- 256 \omega ( 1 - \csstar^2 )
					+ f_X \big(
						56
						+ 8 \EulerGamma
						- 320 \omega
					\big)
				\right\}\ \  .
		\end{split}
		\label{eq:noller-magueijo}
	\end{equation}
	For $s = - 2\varepsilon$, both Eq. \eqref{eq:noller-magueijo} and
	Noller \& Magueijo's formula (A.15)
	reduce to Eq. \eqref{eq:khoury-piazza}.
	
	For $s \neq - 2\varepsilon$, Eq.~\eqref{eq:noller-magueijo}
	disagrees with Noller \& Magueijo's result.
	This occurs
	partially because they
	approximate the propagator \eqref{eq:power-spectrum-def} 
	using the elementary wavefunction~\eqref{eq:wavefunction}
	in the super-horizon limit
	$|k \cs \tau| \ll 1$; in this limit
	details of
	the interference between growing and decaying modes
	around the time of horizon exit
	are lost.
	For example,
	their approximation discards
	the $\Ei$-contributions of Eq.
	\eqref{eq:orderderiv}
	although these
	are $\Or(\varpi)$
	and as large as other contributions which are retained.
	But were these terms kept, the
	super-horizon limit $|k \cs \tau| \ll 1$ could not be used to
	estimate them.
	Infrared safety of the $J_i$ integrals in Eqs. \eqref{eq:clare-integrals}
	is spoiled if truncated at any finite order,
	causing incorrect divergences
	in the squeezed limit $\vartheta_i \rightarrow 0$ and
	a spurious contribution to the bispectrum with a local shape.
	As we explain in Appendices~\ref{appendix:propagator}
	and~\ref{appendix:a},
	it appears that---as a point of principle---if $\varpi \neq 0$
	corrections are kept, then the shape of
	the bispectrum can be accurately determined
	only if the \textit{full time-dependence}
	of each wavefunction around the time of horizon exit is retained.
	
	Another reason for the discrepancy with our results 
	lies in the dynamics assumed for the scale factor. Even though
	Ref. \cite{Noller:2011hd} assumed small deviations from 
	a perfectly scale-invariant spectrum
	of perturbations, 
	their analysis used a scale-invariant
	evolution for the scale factor. As a result, their 
	calculation dismisses contributions to the background dynamics as relevant as
	others kept in the evolution of the wavefunctions.




	\section{Tensor modes}
	\label{sec:tensor}
	We conclude our report on slow-roll 
	corrections by studying the implications to 
	tensor modes.
	Inflation has inevitably produced tensor fluctuations to
	accompany the scalar fluctuation $\zeta$.
	Detecting the B-mode polarisation signal produced by
	these fluctuations is a major aim of the \emph{Planck}
	satellite and future CMB experiments \cite{Baumann:2008aj}.
	If measured,
	this signal will provide important constraints on the energy
	scale of inflation. Above all, it will be a strong indication
	that an inflationary period took place in the early universe.



	In certain models the tensor sector provides sufficient observables
	to allow one or more quantities, such as $\fNL$,
	to be written in terms of other observables.
These \textit{consistency relations} were introduced by Copeland {\etal}
	\cite{Copeland:1993jj,Copeland:1993zn}, and are completely decoupled 
	of the way we choose to parametrise the theory.
	To be used effectively with the next-order results
	obtained in this chapter,
	we will require next-order predictions for the tensor modes.
	These were first obtained by Stewart \& Lyth
	\cite{Stewart:1993bc},
	and are unchanged by the non-canonical action~\eqref{eq:startingaction}
	for the scalar field.

	
	The tensor fluctuation is a propagating spin-2 mode which belongs
	to $h_{ij}$ of the ADM metric \eqref{eq:adm}. We write
\[ h_{ij} = a^2 \, \e{2\zeta}\,  (\e{\gamma})_{ij}\ \ , \]	
	where $\tr \gamma_{ij} = 0$.
	At quadratic order, the action for tensor fluctuations is
	\cite{Grishchuk:1974ny}
	\begin{equation}
		S_g^{(2)}
		=
		\frac{1}{8}
		\int \d^3x \, \d\tau \; a^2 \bigg\{
			\gamma'_{ij} \gamma'_{ij} 
			- \partial_k \gamma_{ij} \partial_k \gamma_{ij}
		\bigg\} \ \  .
	\end{equation}
	As described in \S\ref{subsec:fluctuations}, the tensor perturbations 
	decouple, at quadratic order, from the scalar modes.
	There are two polarisations, traditionally denoted `$+$' and `$\times$,'
	making $\gamma_{ij}$ transverse,
	$\partial_i \gamma_{ij} = 0$.
	Introducing a reference scale $k_\star$ as in \S \ref{subsec:second} and
	adding both polarisations,
	the resulting dimensionless spectrum can be written
	\cite{Stewart:1993bc}
	\begin{equation}
		\Pstensor
		=
		\frac{2H_{\star}^2}{\pi^2}
		\left\{
			1
			+ 2\varepsilon_{\star} \left(
				1
				- \EulerGamma
				- \ln\frac{2k}{k_{\star}}
			\right)
		\right\}\ \  .
	\end{equation}
	This result is equal to the sum of
	two copies of the power
	spectrum for a massless scalar field with $\cs = 1$, and
	so $\mathcal{P}_g$ is also conserved on super-horizon scales (there is no residual 
	time-dependence in the answer).
	Including next-order corrections and for arbitrary $k_\star$, 
	the scale-dependence of $\Pstensor$
	is measured by the tilt $n_t$,
	\begin{equation}
		\ntstar
		\equiv
		\dfrac{\d \ln \Pstensor}{\d \ln k}
		=
		-2 \varepsilon_{\star} \left\{
			1
			+ \varepsilon_{\star}
			- \eta_{\star} \left(
				1-\EulerGamma - \ln \frac{2k}{k_\star}
			\right)
		\right\} \ \ .
		\label{eq:nt}
	\end{equation}
	It is conventional to measure the amplitude of tensor
	fluctuations relative to $\zeta$.
	One defines the tensor-to-scalar ratio, $r$, by the rule
	\cite{Copeland:1993zn}
	\begin{equation}
		r
		\equiv
		\dfrac{\Pstensor}{\Ps}\ \  , 
	\end{equation}
	where $\Ps$ is the dimensionless version of the 
	scalar power spectrum
	\eqref{eq:powerspectrum}. We find
	\begin{equation}
		r_\star
		\simeq
		16 \varepsilon_{\star} \csstar \left\{
			1
			- 2 \eta_\star
			+ ( s_\star + \eta_\star )
			\left( \EulerGamma + \ln \frac{2k}{k_\star}
			\right)
		\right\} \ \ .
	\end{equation}
	
	
	In canonical models, $r$ can be written purely in terms of observable
	quantities. In the non-canonical case this is not automatically
	possible without the addition of new observables.
	In general,
	\begin{equation}
		r_\star \simeq  - 8 \ntstar \csstar
			\left\{
				1
				- \varepsilon_\star
				- \eta_\star
				+ s_\star \left(
					\EulerGamma + \ln \frac{2k}{k_\star}
				\right)
			\right\} \ \ .
		\label{eq:next-order-consistency}
	\end{equation}
	One may use the lowest-order result for $\nt$ to eliminate $\varepsilon$.
	To eliminate $\eta$ would require the scalar spectral index,
	$n_s$.
	It is possible to use $\fNL$ to rewrite $\cs$ in the prefactor
	\cite{Lidsey:2006ia},
	but in doing so one introduces dependence on the parameter $\ell$.
	Therefore at least two extra observables would be required to eliminate the
	dependence on $s$ and $\ell$.
	If these depend on $t$, $\xi$ or similar parameters, then further
	observables could be required.
	
	
	We conclude that at next-order in slow-roll, for a general
	$P(X,\phi)$ Lagrangian, the observables $\{ r, n_s, n_t, \fNL \}$ do not
	form a closed set.
	As we shall see in 
	\S\ref{subsec:distinguishing-microphysics}, 
	the consistency relations derived after modal decomposition of
	the bispectrum are able to circumvent this degeneracy, provided
	a sufficient number of observables (with comparable accuracy) is
	available.
	
	
	
	
	
	
	\section{Main results}
	\label{sec:conclusions}
	This chapter is one of the main backbones of this thesis, which
	we attempt to summarise here.
	In the (very) near future, we expect key cosmological observables
	to be determined to high-precision.
	In particular, \emph{Planck} 
	is expected to deliver data in less than one year's time, and
	may determine the
	scalar spectral index $n_s$ to an accuracy of roughly one part in
	$10^3$ \cite{Colombo:2008ta}.
	The level of precision reached by the present 
	CMB experiments can only be
	exploited effectively if our theoretical
	predictions keep pace.
	In this chapter we have focused on three essential 
	questions:
	\begin{enumerate}[i.]
\item 	How accurate are the theoretical estimates of 
	the bispectrum?
\item How can we reduce the theory-error
of our estimates to be in line with the
sensitivity set by \textit{Planck}? 
\item How can we efficiently explore \textit{Planck}'s data 
on the primordial bispectrum, and 
therefore learn more about the microphysics of the early universe?
\end{enumerate}
The first two questions, and partly the last one, have been addressed in this chapter.
The last question will be explored in detail in chapter \ref{chapter:four}.

	Almost twenty years ago,
	Stewart \& Lyth \cite{Stewart:1993bc}
	obtained analytic formulae
	for the two-point function
	accurate to next-order in
	the slow-roll parameter $\varepsilon \equiv - \dot{H}/H^2$.
	Subsequent observational developments have restricted attention
	to a region of the parameters space where $\varepsilon \ll 1$ is
	a good approximation,
	making the leading-order prediction
	for the power spectrum an accurate
	match for experiment.
	There is no reason to believe the same will remain true
	 for three-
	and higher $n$-point correlations,
	which will be experimentally probed with \textit{Planck}.
	
	The results of \S\ref{sec:noncanonical} show that
	next-order corrections to $\fNL$ in the equilateral mode
	may be comparable to
	\emph{Planck}'s observational precision.
	For a future CMB satellite it is actually conceivable
	that the data will
	be more precise than a leading-order estimate.
	In this chapter we have reported a next-order calculation of the
	bispectrum in the slow-roll approximation applicable to all
	single-field inflationary models:
	those belonging to the Horndeski class, 
	which includes models described by a Lagrangian of the form
	$P(X, \phi)$, where $X = (\partial \phi)^{2}$.
	Our calculation has so far focused on the
	magnitude of the bispectrum, $\fNL$,
	and in many models it provides a much more precise estimate
	than the lowest-order result.
	
	Our major results can be categorised into two groups, as follows.
	
	
	
	
	\subsection*{Accuracy and precision}
	Except in special cases where exact results are possible,\footnote{Amongst such exceptions are 
																the results of Khoury \& Piazza for constant $f_X$
																discussed in \S\ref{sec:noncanonical}, 
																and the calculation
																described in chapter \ref{chapter:five}.}
	predictions for observable quantities
	have so far been presented with a theory-error
	encapsulating uncertainty due to small
	contributions which had not been calculated.
	For inflationary observables the typical scale of the theory-error
	is set by the accuracy of the slow-variation approximation,
	where the dimensionless quantities $\varepsilon \equiv - \dot{H} / H^2$,
	$\eta \equiv \dot{\varepsilon} / H \varepsilon$,
	$s \equiv \csdot / H \cs$ (and others)
	are taken to be small.
	These are the assumptions of the
	slow-roll approximation, on which the
	results of this chapter are based.
	To obtain numerical estimates, we have 
	applied our results to some models.

	\para{Power-law DBI inflation and $k$-inflation}In \S\ref{sec:evolution_NGs} and
	\S\S\ref{sec:dbi}--\ref{sec:k-inflation}
	we estimated the \emph{precision}
	which could be ascribed to the leading-order formula
	for $\fNL$ in the
	absence of a complete calculation of next-order effects.
	Using the next-order contributions from the vertices
	$g_i$ in Eqs. \eqref{eq:gi}, 
	which can be obtained without detailed calculation,
	we estimated the fractional uncertainty to be of order 
	$14\varepsilon$ (or as large as $70\%$)
	for DBI and $9\gamma$ (or as large as 6\%) 
	for $k$-inflation.
	The prospect of such large uncertainties, also pointed out by Adshead \etal \ \cite{Adshead:2011jq}, 
	demands carrying out the
	full computation of all next-order terms in the slow-roll approximation.
	
	In DBI and
	$k$-inflation scenarios, we find the terms omitted from these
	estimates generate large cancellations,
	in each case
	reducing the next-order contribution by
	roughly $95\%$.
	This is similar to what was observed by
	Gong \& Stewart in their calculation of
	next-next-order corrections to the power spectrum
	\cite{Gong:2001he}.
	Having done this calculation,
	it seems reasonable to infer that %next-order
	the contributions
	from $g_i$ systematically overpredict the next-order
	terms. But this could not have been anticipated
	without a calculation of all next-order effects.
	Therefore,
	for power-law DBI and $k$-inflation models we conclude that
	the leading-order calculation is unexpectedly accurate.
	


	\para{Generalised DBI inflation}The situation is different
	for a generalised DBI model with arbitrary potential $V(\phi)$
	and warp factor $f(\phi)$. The largest next-order corrections measure a qualitatively new
	effect, not included in the power-law solution, arising from the
	shape of $V$ and $f$.
	The fractional shift was quoted in Eq. \eqref{eq:dbi-shape-corrections}
	and can be large, because the DBI action supports inflation
	even on relatively steep potentials, for which 
	$\varepsilon_V$ and $\eta_V$ may not be very small.
	Indeed, if one were to tune the potential to be flat, 
	say $\varepsilonSR \sim |\etaSR| \lesssim 10^{-2}$,
	then
	much of the motivation
	for a higher-derivative model would have been lost.
	Even for rather large values of $|\fNL|$, the correction can be
	several tens of percent for an ``untuned'' potential with
	$\varepsilonSR \sim |\etaSR| \sim 1$ (maintaining $\varepsilon$ and 
	$\eta$ small).
	For slightly
	smaller values of $|\fNL|$, the correction is increasingly significant,
	perhaps growing to $\sim 35\%$.
	The formulae quoted in \S\ref{sec:dbi} assume $\gamma \gg 1$
	and would require modification for very small $\fNL$
	where $\Or(\gamma^{-1})$ corrections need not be negligible.
	If desired, these can be obtained from our full formulae
	tabulated in \S\ref{sec:bispectrum}.

\para{Infrared DBI inflation}In the infrared DBI scenario
	proposed by Chen~\cite{Chen:2004gc,Chen:2005ad,Chen:2005fe},
	we
	find the correction to be
	$\sim 12\%$ for parameter values currently favoured by observation,
	which translates to
	reasonably large shifts in $\fNL$.
	For the maximum-likelihood parameter values suggested by
	the analysis of Bean {\etal} \cite{Bean:2007hc}, 
	we find that next-order corrections
	increase the
	magnitude of $\fNL$ by a shift $|\Delta \fNL| \simeq 19$.
	This is a little smaller than the error bar which \emph{Planck}
	is expected to achieve, but nevertheless of comparable
	magnitude.
	We conclude that a next-order calculation will be adequate for
	\emph{Planck}, but if the model is not subsequently ruled out,
	a next-next-order calculation may be desirable for a
	\emph{CMBPol}-
	or \emph{CoRE}-type satellite.

	

	\subsection*{Technical results}
	Our calculation includes a number of more technical results, 
	listed below.
		
	\para{Treatment of boundary terms}In \S\ref{sec:third-order-action} we gave a systematic treatment
	of boundary terms in the third-order action for $\zeta$.
	Although these terms were properly accounted for in previous
	results~\cite{Maldacena:2002vr,Seery:2005wm,Chen:2006nt},
	these calculations used a field redefinition which was not
	\emph{guaranteed}
	to remove all terms in the boundary action.
	
	Our calculation has also shown how the cubic action 
	could be written in terms of a minimal 
	number of \textit{five} Horndeski operators, 
	given in Eq. \eqref{eq:s3tau}.
	
	\para{Pure shape logarithms}The subleading correction to the propagator contains
	an exponential integral
	contribution 
	whose time-dependence cannot be described by
	elementary functions
	\cite{Gong:2001he,Chen:2006nt,Burrage:2010cu}.
	This term contributes at the level of the 
	internal legs of the Feynman diagram.
	We argue that it must be handled carefully to avoid unphysical
	infrared divergences
	in the squeezed limit, where one momentum goes to zero.
	In Appendix~\ref{appendix:a} we describe how this
	contribution yields
	the $J_i$ functions given in Eqs.~\eqref{eq:clare-integrals}.
	These are
	obtained using resummation and analytic continuation techniques
	introduced in Ref.~\cite{Burrage:2010cu}.
	
	The possibility of spurious divergences in the squeezed limit
	shows that, as a matter of principle,
	one should be cautious when determining the shape of the bispectrum
	generated by
	an approximation to the elementary wavefunctions.
	Obtaining the quantitatively correct
	\emph{momentum} behaviour requires all
	details of the interference in
	\emph{time} between growing and decaying modes
	near horizon exit.
	The possibility of such interference effects,
	absent in classical mechanics,
	is a typical feature of
	quantum mechanical processes.
	This interference correctly resolves
	the unwanted divergences in the infrared limit
	$k_j \rightarrow 0$ with $j \neq i$,
as discussed in
    detail in
	Appendices~\ref{appendix:propagator} and~\ref{appendix:a}.
	
	
	\para{Comparison with known results}We have verified Maldacena's consistency
	condition~\eqref{eq:maldacena-condition} to next-order
	in canonical models
	by doing an explicit calculation of the full bispectrum. This agrees with a recent
	calculation by Renaux-Petel \cite{RenauxPetel:2010ty}.
This matching depends carefully on keeping track of the 
scale and shape logarithms available in the next-order terms in slow-roll. 	
	
	In the case of power-law inflation with a scale-invariant spectrum
	of scalar perturbations, $\varpi = 0$,
	and constant $\varepsilon$ and $s$, we reproduce a known result
	derived by Khoury \& Piazza
	\cite{Khoury:2008wj}.
	A subset of our corrections was computed by Chen {\etal}
	\cite{Chen:2006nt}. Up to first-order terms in
	powers of slow-roll
	quantities---where our results can be
	compared---we find exact agreement.
	


\newpage
\thispagestyle{empty}
\newpage


